Audio System One Model: Typed Probabilistic Perception of Emotion in Speech

Speech applications ask many questions about the same voice: which emotion a listener perceives, how aroused the speaker sounds, whether they sound frustrated. Classifiers answer fast, over one fixed label set; audio language models (ALMs) take any question in text, but answer by generation, one pass per question, with poorly calibrated probabilities. We present ASOM (Audio System One Model), a System One model for speech: choice, score and yes/no questions written at request time are answered in one pass, without generation, each with a probability distribution. Frozen speech and text encoders feed a 6.2M-parameter reader with no per-class parameters, trained on listener vote distributions. On MSP-Podcast, ASOM matches a classifier on the same features and data, leads the best of 6 zero-shot ALMs by 0.072 and an ALM fine-tuned on the same data by 0.026, and answers 20 questions in 13.1 ms, 17-41 times faster than the ALMs. It also answers reworded, reduced and new label sets, scales and gender, and on 21 unseen corpora in 13 languages it leads the best zero-shot ALM by 0.138 where the words carry no emotion; where they do, the ALMs mostly read.

==> generated/numbers.tex <==
% generated by tools/paper/analyze.py: do not edit
\makeatletter
\newcommand{\res}[1]{\@ifundefined{res@#1}{\textbf{??\detokenize{#1}}}{\csname res@#1\endcsname}}
\expandafter\def\csname res@abl.bkt.df1\endcsname{-0.000}
\expandafter\def\csname res@abl.bkt.df1ci\endcsname{[-0.006, +0.003]}
\expandafter\def\csname res@abl.bkt.dheld\endcsname{+0.004}
\expandafter\def\csname res@abl.bkt.dheldci\endcsname{[+0.002, +0.006]}
\expandafter\def\csname res@abl.bkt.dll\endcsname{+0.004}
\expandafter\def\csname res@abl.bkt.dllci\endcsname{[+0.002, +0.006]}
\expandafter\def\csname res@abl.bkt.dzs\endcsname{-0.009}
\expandafter\def\csname res@abl.bkt.dzsci\endcsname{[-0.013, -0.003]}
\expandafter\def\csname res@abl.bkt.f1\endcsname{0.382}
\expandafter\def\csname res@abl.bkt.zs\endcsname{0.433}
\expandafter\def\csname res@abl.bkt.zsctrl\endcsname{0.442}
\expandafter\def\csname res@abl.clapobj.df1\endcsname{-0.053}
\expandafter\def\csname res@abl.clapobj.df1ci\endcsname{[-0.061, -0.044]}
\expandafter\def\csname res@abl.clapobj.dheld\endcsname{+0.366}
\expandafter\def\csname res@abl.clapobj.dheldci\endcsname{[+0.295, +0.446]}
\expandafter\def\csname res@abl.clapobj.dll\endcsname{+0.369}
\expandafter\def\csname res@abl.clapobj.dllci\endcsname{[+0.291, +0.460]}
\expandafter\def\csname res@abl.clapobj.dzs\endcsname{+0.067}
\expandafter\def\csname res@abl.clapobj.dzsci\endcsname{[+0.057, +0.074]}
\expandafter\def\csname res@abl.clapobj.f1\endcsname{0.332}
\expandafter\def\csname res@abl.clapobj.zs\endcsname{0.507}
\expandafter\def\csname res@abl.clapobj.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.control.f1\endcsname{0.382}
\expandafter\def\csname res@abl.datasetv1.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.datasetv1.df1ci\endcsname{[-0.007, +0.000]}
\expandafter\def\csname res@abl.datasetv1.dheld\endcsname{-0.002}
\expandafter\def\csname res@abl.datasetv1.dheldci\endcsname{[-0.004, -0.000]}
\expandafter\def\csname res@abl.datasetv1.dll\endcsname{-0.001}
\expandafter\def\csname res@abl.datasetv1.dllci\endcsname{[-0.002, +0.001]}
\expandafter\def\csname res@abl.datasetv1.dzs\endcsname{-0.078}
\expandafter\def\csname res@abl.datasetv1.dzsci\endcsname{[-0.087, -0.068]}
\expandafter\def\csname res@abl.datasetv1.f1\endcsname{0.382}
\expandafter\def\csname res@abl.datasetv1.zs\endcsname{0.362}
\expandafter\def\csname res@abl.datasetv1.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.datasetv2.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.datasetv2.df1ci\endcsname{[-0.008, +0.002]}
\expandafter\def\csname res@abl.datasetv2.dheld\endcsname{+0.007}
\expandafter\def\csname res@abl.datasetv2.dheldci\endcsname{[-0.000, +0.015]}
\expandafter\def\csname res@abl.datasetv2.dll\endcsname{+0.005}
\expandafter\def\csname res@abl.datasetv2.dllci\endcsname{[+0.002, +0.008]}
\expandafter\def\csname res@abl.datasetv2.dzs\endcsname{-0.018}
\expandafter\def\csname res@abl.datasetv2.dzsci\endcsname{[-0.032, -0.007]}
\expandafter\def\csname res@abl.datasetv2.f1\endcsname{0.382}
\expandafter\def\csname res@abl.datasetv2.zs\endcsname{0.422}
\expandafter\def\csname res@abl.datasetv2.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.datasetv2acted.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.datasetv2acted.df1ci\endcsname{[-0.007, +0.002]}
\expandafter\def\csname res@abl.datasetv2acted.dheld\endcsname{+0.002}
\expandafter\def\csname res@abl.datasetv2acted.dheldci\endcsname{[+0.000, +0.004]}
\expandafter\def\csname res@abl.datasetv2acted.dll\endcsname{+0.001}
\expandafter\def\csname res@abl.datasetv2acted.dllci\endcsname{[-0.002, +0.003]}
\expandafter\def\csname res@abl.datasetv2acted.dzs\endcsname{+0.029}
\expandafter\def\csname res@abl.datasetv2acted.dzsci\endcsname{[+0.014, +0.040]}
\expandafter\def\csname res@abl.datasetv2acted.f1\endcsname{0.382}
\expandafter\def\csname res@abl.datasetv2acted.zs\endcsname{0.469}
\expandafter\def\csname res@abl.datasetv2acted.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.distill.df1\endcsname{+0.000}
\expandafter\def\csname res@abl.distill.df1ci\endcsname{[-0.005, +0.005]}
\expandafter\def\csname res@abl.distill.dheld\endcsname{+0.024}
\expandafter\def\csname res@abl.distill.dheldci\endcsname{[+0.018, +0.031]}
\expandafter\def\csname res@abl.distill.dll\endcsname{+0.019}
\expandafter\def\csname res@abl.distill.dllci\endcsname{[+0.015, +0.022]}
\expandafter\def\csname res@abl.distill.dzs\endcsname{+0.019}
\expandafter\def\csname res@abl.distill.dzsci\endcsname{[+0.013, +0.024]}
\expandafter\def\csname res@abl.distill.f1\endcsname{0.385}
\expandafter\def\csname res@abl.distill.zs\endcsname{0.459}
\expandafter\def\csname res@abl.distill.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.diversity.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.diversity.df1ci\endcsname{[-0.008, +0.002]}
\expandafter\def\csname res@abl.diversity.dheld\endcsname{+0.078}
\expandafter\def\csname res@abl.diversity.dheldci\endcsname{[+0.050, +0.102]}
\expandafter\def\csname res@abl.diversity.dll\endcsname{+0.000}
\expandafter\def\csname res@abl.diversity.dllci\endcsname{[-0.002, +0.003]}
\expandafter\def\csname res@abl.diversity.dzs\endcsname{+0.011}
\expandafter\def\csname res@abl.diversity.dzsci\endcsname{[+0.006, +0.015]}
\expandafter\def\csname res@abl.diversity.f1\endcsname{0.382}
\expandafter\def\csname res@abl.diversity.zs\endcsname{0.451}
\expandafter\def\csname res@abl.diversity.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.drop16.df1\endcsname{-0.002}
\expandafter\def\csname res@abl.drop16.df1ci\endcsname{[-0.007, +0.002]}
\expandafter\def\csname res@abl.drop16.dheld\endcsname{+0.001}
\expandafter\def\csname res@abl.drop16.dheldci\endcsname{[-0.000, +0.002]}
\expandafter\def\csname res@abl.drop16.dll\endcsname{+0.002}
\expandafter\def\csname res@abl.drop16.dllci\endcsname{[+0.001, +0.004]}
\expandafter\def\csname res@abl.drop16.dzs\endcsname{+0.008}
\expandafter\def\csname res@abl.drop16.dzsci\endcsname{[+0.003, +0.013]}
\expandafter\def\csname res@abl.drop16.f1\endcsname{0.382}
\expandafter\def\csname res@abl.drop16.zs\endcsname{0.449}
\expandafter\def\csname res@abl.drop16.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.drop24.df1\endcsname{-0.005}
\expandafter\def\csname res@abl.drop24.df1ci\endcsname{[-0.012, -0.000]}
\expandafter\def\csname res@abl.drop24.dheld\endcsname{+0.004}
\expandafter\def\csname res@abl.drop24.dheldci\endcsname{[+0.001, +0.006]}
\expandafter\def\csname res@abl.drop24.dll\endcsname{+0.005}
\expandafter\def\csname res@abl.drop24.dllci\endcsname{[+0.002, +0.008]}
\expandafter\def\csname res@abl.drop24.dzs\endcsname{+0.004}
\expandafter\def\csname res@abl.drop24.dzsci\endcsname{[-0.000, +0.010]}
\expandafter\def\csname res@abl.drop24.f1\endcsname{0.380}
\expandafter\def\csname res@abl.drop24.zs\endcsname{0.444}
\expandafter\def\csname res@abl.drop24.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.drop8.df1\endcsname{+0.002}
\expandafter\def\csname res@abl.drop8.df1ci\endcsname{[-0.002, +0.007]}
\expandafter\def\csname res@abl.drop8.dheld\endcsname{-0.002}
\expandafter\def\csname res@abl.drop8.dheldci\endcsname{[-0.004, -0.001]}
\expandafter\def\csname res@abl.drop8.dll\endcsname{-0.001}
\expandafter\def\csname res@abl.drop8.dllci\endcsname{[-0.003, +0.001]}
\expandafter\def\csname res@abl.drop8.dzs\endcsname{+0.005}
\expandafter\def\csname res@abl.drop8.dzsci\endcsname{[+0.000, +0.010]}
\expandafter\def\csname res@abl.drop8.f1\endcsname{0.387}
\expandafter\def\csname res@abl.drop8.zs\endcsname{0.445}
\expandafter\def\csname res@abl.drop8.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.dyn.df1\endcsname{-0.007}
\expandafter\def\csname res@abl.dyn.df1ci\endcsname{[-0.015, -0.002]}
\expandafter\def\csname res@abl.dyn.dheld\endcsname{+0.012}
\expandafter\def\csname res@abl.dyn.dheldci\endcsname{[+0.010, +0.015]}
\expandafter\def\csname res@abl.dyn.dll\endcsname{+0.013}
\expandafter\def\csname res@abl.dyn.dllci\endcsname{[+0.009, +0.016]}
\expandafter\def\csname res@abl.dyn.dzs\endcsname{-0.047}
\expandafter\def\csname res@abl.dyn.dzsci\endcsname{[-0.055, -0.038]}
\expandafter\def\csname res@abl.dyn.f1\endcsname{0.378}
\expandafter\def\csname res@abl.dyn.zs\endcsname{0.394}
\expandafter\def\csname res@abl.dyn.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.fixedmlp.df1\endcsname{-0.018}
\expandafter\def\csname res@abl.fixedmlp.df1ci\endcsname{[-0.024, -0.013]}
\expandafter\def\csname res@abl.fixedmlp.dll\endcsname{+0.001}
\expandafter\def\csname res@abl.fixedmlp.dllci\endcsname{[-0.004, +0.007]}
\expandafter\def\csname res@abl.fixedmlp.f1\endcsname{0.361}
\expandafter\def\csname res@abl.fixedtable.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.fixedtable.df1ci\endcsname{[-0.005, +0.002]}
\expandafter\def\csname res@abl.fixedtable.dll\endcsname{-0.004}
\expandafter\def\csname res@abl.fixedtable.dllci\endcsname{[-0.006, -0.003]}
\expandafter\def\csname res@abl.fixedtable.dzs\endcsname{-0.017}
\expandafter\def\csname res@abl.fixedtable.dzsci\endcsname{[-0.021, -0.013]}
\expandafter\def\csname res@abl.fixedtable.f1\endcsname{0.379}
\expandafter\def\csname res@abl.fixedtable.zs\endcsname{0.417}
\expandafter\def\csname res@abl.fixedtable.zsctrl\endcsname{0.433}
\expandafter\def\csname res@abl.genderverified.df1\endcsname{-0.001}
\expandafter\def\csname res@abl.genderverified.df1ci\endcsname{[-0.005, +0.004]}
\expandafter\def\csname res@abl.genderverified.dheld\endcsname{-0.000}
\expandafter\def\csname res@abl.genderverified.dheldci\endcsname{[-0.004, +0.003]}
\expandafter\def\csname res@abl.genderverified.dll\endcsname{+0.000}
\expandafter\def\csname res@abl.genderverified.dllci\endcsname{[-0.003, +0.003]}
\expandafter\def\csname res@abl.genderverified.dzs\endcsname{+0.007}
\expandafter\def\csname res@abl.genderverified.dzsci\endcsname{[+0.002, +0.013]}
\expandafter\def\csname res@abl.genderverified.f1\endcsname{0.382}
\expandafter\def\csname res@abl.genderverified.zs\endcsname{0.434}
\expandafter\def\csname res@abl.genderverified.zsctrl\endcsname{0.426}
\expandafter\def\csname res@abl.lasttoken.df1\endcsname{+0.001}
\expandafter\def\csname res@abl.lasttoken.df1ci\endcsname{[-0.003, +0.005]}
\expandafter\def\csname res@abl.lasttoken.dheld\endcsname{+0.025}
\expandafter\def\csname res@abl.lasttoken.dheldci\endcsname{[+0.017, +0.034]}
\expandafter\def\csname res@abl.lasttoken.dll\endcsname{-0.000}
\expandafter\def\csname res@abl.lasttoken.dllci\endcsname{[-0.002, +0.001]}
\expandafter\def\csname res@abl.lasttoken.dzs\endcsname{+0.003}
\expandafter\def\csname res@abl.lasttoken.dzsci\endcsname{[-0.000, +0.006]}
\expandafter\def\csname res@abl.lasttoken.f1\endcsname{0.379}
\expandafter\def\csname res@abl.lasttoken.zs\endcsname{0.357}
\expandafter\def\csname res@abl.lasttoken.zsctrl\endcsname{0.354}
\expandafter\def\csname res@abl.old_all33.df1\endcsname{+0.003}
\expandafter\def\csname res@abl.old_all33.df1ci\endcsname{[-0.002, +0.008]}
\expandafter\def\csname res@abl.old_all33.dll\endcsname{-0.002}
\expandafter\def\csname res@abl.old_all33.dllci\endcsname{[-0.004, -0.001]}
\expandafter\def\csname res@abl.old_all33.f1\endcsname{0.382}
\expandafter\def\csname res@abl.old_clapobj.df1\endcsname{-0.050}
\expandafter\def\csname res@abl.old_clapobj.df1ci\endcsname{[-0.059, -0.042]}
\expandafter\def\csname res@abl.old_clapobj.dheld\endcsname{+0.368}
\expandafter\def\csname res@abl.old_clapobj.dheldci\endcsname{[+0.297, +0.449]}
\expandafter\def\csname res@abl.old_clapobj.dll\endcsname{+0.370}
\expandafter\def\csname res@abl.old_clapobj.dllci\endcsname{[+0.290, +0.462]}
\expandafter\def\csname res@abl.old_clapobj.dzs\endcsname{+0.061}
\expandafter\def\csname res@abl.old_clapobj.dzsci\endcsname{[+0.052, +0.068]}
\expandafter\def\csname res@abl.old_clapobj.f1\endcsname{0.332}
\expandafter\def\csname res@abl.old_clapobj.zs\endcsname{0.507}
\expandafter\def\csname res@abl.old_clapobj.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.old_datasetv1.df1\endcsname{-0.001}
\expandafter\def\csname res@abl.old_datasetv1.df1ci\endcsname{[-0.004, +0.005]}
\expandafter\def\csname res@abl.old_datasetv1.dheld\endcsname{-0.007}
\expandafter\def\csname res@abl.old_datasetv1.dheldci\endcsname{[-0.013, -0.001]}
\expandafter\def\csname res@abl.old_datasetv1.dll\endcsname{-0.002}
\expandafter\def\csname res@abl.old_datasetv1.dllci\endcsname{[-0.005, -0.000]}
\expandafter\def\csname res@abl.old_datasetv1.dzs\endcsname{-0.071}
\expandafter\def\csname res@abl.old_datasetv1.dzsci\endcsname{[-0.079, -0.062]}
\expandafter\def\csname res@abl.old_datasetv1.f1\endcsname{0.378}
\expandafter\def\csname res@abl.old_datasetv1.zs\endcsname{0.354}
\expandafter\def\csname res@abl.old_datasetv1.zsctrl\endcsname{0.425}
\expandafter\def\csname res@abl.old_datasetv2.df1\endcsname{-0.001}
\expandafter\def\csname res@abl.old_datasetv2.df1ci\endcsname{[-0.006, +0.002]}
\expandafter\def\csname res@abl.old_datasetv2.dheld\endcsname{+0.011}
\expandafter\def\csname res@abl.old_datasetv2.dheldci\endcsname{[+0.004, +0.017]}
\expandafter\def\csname res@abl.old_datasetv2.dll\endcsname{+0.006}
\expandafter\def\csname res@abl.old_datasetv2.dllci\endcsname{[+0.004, +0.007]}
\expandafter\def\csname res@abl.old_datasetv2.dzs\endcsname{-0.016}
\expandafter\def\csname res@abl.old_datasetv2.dzsci\endcsname{[-0.029, -0.005]}
\expandafter\def\csname res@abl.old_datasetv2.f1\endcsname{0.382}
\expandafter\def\csname res@abl.old_datasetv2.zs\endcsname{0.427}
\expandafter\def\csname res@abl.old_datasetv2.zsctrl\endcsname{0.443}
\expandafter\def\csname res@abl.old_datasetv2acted.df1\endcsname{+0.000}
\expandafter\def\csname res@abl.old_datasetv2acted.df1ci\endcsname{[-0.003, +0.003]}
\expandafter\def\csname res@abl.old_datasetv2acted.dheld\endcsname{+0.003}
\expandafter\def\csname res@abl.old_datasetv2acted.dheldci\endcsname{[+0.001, +0.005]}
\expandafter\def\csname res@abl.old_datasetv2acted.dll\endcsname{+0.002}
\expandafter\def\csname res@abl.old_datasetv2acted.dllci\endcsname{[+0.001, +0.003]}
\expandafter\def\csname res@abl.old_datasetv2acted.dzs\endcsname{+0.028}
\expandafter\def\csname res@abl.old_datasetv2acted.dzsci\endcsname{[+0.015, +0.039]}
\expandafter\def\csname res@abl.old_datasetv2acted.f1\endcsname{0.383}
\expandafter\def\csname res@abl.old_datasetv2acted.zs\endcsname{0.472}
\expandafter\def\csname res@abl.old_datasetv2acted.zsctrl\endcsname{0.444}
\expandafter\def\csname res@abl.old_datasetv2noasvp.df1\endcsname{+0.000}
\expandafter\def\csname res@abl.old_datasetv2noasvp.df1ci\endcsname{[-0.003, +0.004]}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dheld\endcsname{+0.006}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dheldci\endcsname{[+0.002, +0.011]}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dll\endcsname{+0.004}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dllci\endcsname{[+0.002, +0.005]}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dzs\endcsname{+0.017}
\expandafter\def\csname res@abl.old_datasetv2noasvp.dzsci\endcsname{[+0.005, +0.027]}
\expandafter\def\csname res@abl.old_datasetv2noasvp.f1\endcsname{0.383}
\expandafter\def\csname res@abl.old_datasetv2noasvp.zs\endcsname{0.461}
\expandafter\def\csname res@abl.old_datasetv2noasvp.zsctrl\endcsname{0.444}
\expandafter\def\csname res@abl.old_distill.df1\endcsname{+0.002}
\expandafter\def\csname res@abl.old_distill.df1ci\endcsname{[-0.004, +0.007]}
\expandafter\def\csname res@abl.old_distill.dheld\endcsname{+0.032}
\expandafter\def\csname res@abl.old_distill.dheldci\endcsname{[+0.022, +0.043]}
\expandafter\def\csname res@abl.old_distill.dll\endcsname{+0.020}
\expandafter\def\csname res@abl.old_distill.dllci\endcsname{[+0.015, +0.026]}
\expandafter\def\csname res@abl.old_distill.dzs\endcsname{+0.006}
\expandafter\def\csname res@abl.old_distill.dzsci\endcsname{[+0.001, +0.011]}
\expandafter\def\csname res@abl.old_distill.f1\endcsname{0.385}
\expandafter\def\csname res@abl.old_distill.zs\endcsname{0.452}
\expandafter\def\csname res@abl.old_distill.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.old_diversity.df1\endcsname{-0.004}
\expandafter\def\csname res@abl.old_diversity.df1ci\endcsname{[-0.008, +0.000]}
\expandafter\def\csname res@abl.old_diversity.dheld\endcsname{+0.057}
\expandafter\def\csname res@abl.old_diversity.dheldci\endcsname{[+0.031, +0.080]}
\expandafter\def\csname res@abl.old_diversity.dll\endcsname{-0.000}
\expandafter\def\csname res@abl.old_diversity.dllci\endcsname{[-0.002, +0.002]}
\expandafter\def\csname res@abl.old_diversity.dzs\endcsname{-0.000}
\expandafter\def\csname res@abl.old_diversity.dzsci\endcsname{[-0.006, +0.004]}
\expandafter\def\csname res@abl.old_diversity.f1\endcsname{0.379}
\expandafter\def\csname res@abl.old_diversity.zs\endcsname{0.445}
\expandafter\def\csname res@abl.old_diversity.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.old_multiquery.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.old_multiquery.df1ci\endcsname{[-0.007, -0.000]}
\expandafter\def\csname res@abl.old_multiquery.dheld\endcsname{+0.009}
\expandafter\def\csname res@abl.old_multiquery.dheldci\endcsname{[+0.008, +0.011]}
\expandafter\def\csname res@abl.old_multiquery.dll\endcsname{+0.004}
\expandafter\def\csname res@abl.old_multiquery.dllci\endcsname{[+0.003, +0.006]}
\expandafter\def\csname res@abl.old_multiquery.dzs\endcsname{-0.019}
\expandafter\def\csname res@abl.old_multiquery.dzsci\endcsname{[-0.023, -0.015]}
\expandafter\def\csname res@abl.old_multiquery.f1\endcsname{0.379}
\expandafter\def\csname res@abl.old_multiquery.zs\endcsname{0.425}
\expandafter\def\csname res@abl.old_multiquery.zsctrl\endcsname{0.444}
\expandafter\def\csname res@abl.old_segments.df1\endcsname{-0.019}
\expandafter\def\csname res@abl.old_segments.df1ci\endcsname{[-0.025, -0.012]}
\expandafter\def\csname res@abl.old_segments.dheld\endcsname{+0.008}
\expandafter\def\csname res@abl.old_segments.dheldci\endcsname{[+0.002, +0.014]}
\expandafter\def\csname res@abl.old_segments.dll\endcsname{+0.009}
\expandafter\def\csname res@abl.old_segments.dllci\endcsname{[+0.003, +0.015]}
\expandafter\def\csname res@abl.old_segments.dzs\endcsname{-0.002}
\expandafter\def\csname res@abl.old_segments.dzsci\endcsname{[-0.009, +0.004]}
\expandafter\def\csname res@abl.old_segments.f1\endcsname{0.364}
\expandafter\def\csname res@abl.old_segments.zs\endcsname{0.443}
\expandafter\def\csname res@abl.old_segments.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.old_tall29.df1\endcsname{-0.000}
\expandafter\def\csname res@abl.old_tall29.df1ci\endcsname{[-0.005, +0.004]}
\expandafter\def\csname res@abl.old_tall29.dll\endcsname{+0.002}
\expandafter\def\csname res@abl.old_tall29.dllci\endcsname{[-0.001, +0.004]}
\expandafter\def\csname res@abl.old_tall29.f1\endcsname{0.379}
\expandafter\def\csname res@abl.old_w24.df1\endcsname{-0.051}
\expandafter\def\csname res@abl.old_w24.df1ci\endcsname{[-0.060, -0.044]}
\expandafter\def\csname res@abl.old_w24.dheld\endcsname{+0.071}
\expandafter\def\csname res@abl.old_w24.dheldci\endcsname{[+0.055, +0.089]}
\expandafter\def\csname res@abl.old_w24.dll\endcsname{+0.059}
\expandafter\def\csname res@abl.old_w24.dllci\endcsname{[+0.047, +0.072]}
\expandafter\def\csname res@abl.old_w24.dzs\endcsname{-0.025}
\expandafter\def\csname res@abl.old_w24.dzsci\endcsname{[-0.035, -0.017]}
\expandafter\def\csname res@abl.old_w24.f1\endcsname{0.330}
\expandafter\def\csname res@abl.old_w24.zs\endcsname{0.421}
\expandafter\def\csname res@abl.old_w24.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.old_w32only.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.old_w32only.df1ci\endcsname{[-0.010, +0.001]}
\expandafter\def\csname res@abl.old_w32only.dheld\endcsname{+0.002}
\expandafter\def\csname res@abl.old_w32only.dheldci\endcsname{[-0.002, +0.007]}
\expandafter\def\csname res@abl.old_w32only.dll\endcsname{+0.002}
\expandafter\def\csname res@abl.old_w32only.dllci\endcsname{[-0.002, +0.007]}
\expandafter\def\csname res@abl.old_w32only.dzs\endcsname{-0.012}
\expandafter\def\csname res@abl.old_w32only.dzsci\endcsname{[-0.017, -0.006]}
\expandafter\def\csname res@abl.old_w32only.f1\endcsname{0.380}
\expandafter\def\csname res@abl.old_w32only.zs\endcsname{0.431}
\expandafter\def\csname res@abl.old_w32only.zsctrl\endcsname{0.443}
\expandafter\def\csname res@abl.omniaudio.df1\endcsname{-0.021}
\expandafter\def\csname res@abl.omniaudio.df1ci\endcsname{[-0.029, -0.013]}
\expandafter\def\csname res@abl.omniaudio.dll\endcsname{+0.028}
\expandafter\def\csname res@abl.omniaudio.dllci\endcsname{[+0.024, +0.034]}
\expandafter\def\csname res@abl.omniaudio.f1\endcsname{0.346}
\expandafter\def\csname res@abl.q1.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.q1.df1ci\endcsname{[-0.006, +0.001]}
\expandafter\def\csname res@abl.q1.dheld\endcsname{-0.000}
\expandafter\def\csname res@abl.q1.dheldci\endcsname{[-0.001, +0.001]}
\expandafter\def\csname res@abl.q1.dll\endcsname{+0.000}
\expandafter\def\csname res@abl.q1.dllci\endcsname{[-0.001, +0.002]}
\expandafter\def\csname res@abl.q1.dzs\endcsname{+0.003}
\expandafter\def\csname res@abl.q1.dzsci\endcsname{[-0.000, +0.007]}
\expandafter\def\csname res@abl.q1.f1\endcsname{0.382}
\expandafter\def\csname res@abl.q1.zs\endcsname{0.444}
\expandafter\def\csname res@abl.q1.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.q4.df1\endcsname{-0.000}
\expandafter\def\csname res@abl.q4.df1ci\endcsname{[-0.003, +0.002]}
\expandafter\def\csname res@abl.q4.dheld\endcsname{-0.002}
\expandafter\def\csname res@abl.q4.dheldci\endcsname{[-0.005, +0.001]}
\expandafter\def\csname res@abl.q4.dll\endcsname{-0.001}
\expandafter\def\csname res@abl.q4.dllci\endcsname{[-0.002, -0.000]}
\expandafter\def\csname res@abl.q4.dzs\endcsname{+0.002}
\expandafter\def\csname res@abl.q4.dzsci\endcsname{[-0.000, +0.005]}
\expandafter\def\csname res@abl.q4.f1\endcsname{0.382}
\expandafter\def\csname res@abl.q4.zs\endcsname{0.444}
\expandafter\def\csname res@abl.q4.zsctrl\endcsname{0.442}
\expandafter\def\csname res@abl.seg128.df1\endcsname{-0.000}
\expandafter\def\csname res@abl.seg128.df1ci\endcsname{[-0.005, +0.004]}
\expandafter\def\csname res@abl.seg128.dheld\endcsname{-0.000}
\expandafter\def\csname res@abl.seg128.dheldci\endcsname{[-0.001, +0.001]}
\expandafter\def\csname res@abl.seg128.dll\endcsname{-0.000}
\expandafter\def\csname res@abl.seg128.dllci\endcsname{[-0.001, +0.001]}
\expandafter\def\csname res@abl.seg128.dzs\endcsname{+0.001}
\expandafter\def\csname res@abl.seg128.dzsci\endcsname{[-0.004, +0.006]}
\expandafter\def\csname res@abl.seg128.f1\endcsname{0.384}
\expandafter\def\csname res@abl.seg128.zs\endcsname{0.441}
\expandafter\def\csname res@abl.seg128.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.seg16.df1\endcsname{-0.005}
\expandafter\def\csname res@abl.seg16.df1ci\endcsname{[-0.010, -0.000]}
\expandafter\def\csname res@abl.seg16.dheld\endcsname{+0.004}
\expandafter\def\csname res@abl.seg16.dheldci\endcsname{[+0.002, +0.006]}
\expandafter\def\csname res@abl.seg16.dll\endcsname{+0.004}
\expandafter\def\csname res@abl.seg16.dllci\endcsname{[+0.002, +0.006]}
\expandafter\def\csname res@abl.seg16.dzs\endcsname{-0.007}
\expandafter\def\csname res@abl.seg16.dzsci\endcsname{[-0.011, -0.002]}
\expandafter\def\csname res@abl.seg16.f1\endcsname{0.380}
\expandafter\def\csname res@abl.seg16.zs\endcsname{0.433}
\expandafter\def\csname res@abl.seg16.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.seg32.df1\endcsname{-0.003}
\expandafter\def\csname res@abl.seg32.df1ci\endcsname{[-0.007, +0.001]}
\expandafter\def\csname res@abl.seg32.dheld\endcsname{+0.002}
\expandafter\def\csname res@abl.seg32.dheldci\endcsname{[+0.001, +0.004]}
\expandafter\def\csname res@abl.seg32.dll\endcsname{+0.003}
\expandafter\def\csname res@abl.seg32.dllci\endcsname{[+0.001, +0.004]}
\expandafter\def\csname res@abl.seg32.dzs\endcsname{+0.001}
\expandafter\def\csname res@abl.seg32.dzsci\endcsname{[-0.004, +0.005]}
\expandafter\def\csname res@abl.seg32.f1\endcsname{0.382}
\expandafter\def\csname res@abl.seg32.zs\endcsname{0.441}
\expandafter\def\csname res@abl.seg32.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.seg8.df1\endcsname{-0.005}
\expandafter\def\csname res@abl.seg8.df1ci\endcsname{[-0.012, -0.000]}
\expandafter\def\csname res@abl.seg8.dheld\endcsname{+0.004}
\expandafter\def\csname res@abl.seg8.dheldci\endcsname{[+0.001, +0.007]}
\expandafter\def\csname res@abl.seg8.dll\endcsname{+0.004}
\expandafter\def\csname res@abl.seg8.dllci\endcsname{[+0.001, +0.007]}
\expandafter\def\csname res@abl.seg8.dzs\endcsname{-0.019}
\expandafter\def\csname res@abl.seg8.dzsci\endcsname{[-0.023, -0.014]}
\expandafter\def\csname res@abl.seg8.f1\endcsname{0.379}
\expandafter\def\csname res@abl.seg8.zs\endcsname{0.421}
\expandafter\def\csname res@abl.seg8.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.segments.df1\endcsname{-0.022}
\expandafter\def\csname res@abl.segments.df1ci\endcsname{[-0.028, -0.016]}
\expandafter\def\csname res@abl.segments.dheld\endcsname{+0.011}
\expandafter\def\csname res@abl.segments.dheldci\endcsname{[+0.007, +0.016]}
\expandafter\def\csname res@abl.segments.dll\endcsname{+0.011}
\expandafter\def\csname res@abl.segments.dllci\endcsname{[+0.007, +0.015]}
\expandafter\def\csname res@abl.segments.dzs\endcsname{+0.002}
\expandafter\def\csname res@abl.segments.dzsci\endcsname{[-0.006, +0.010]}
\expandafter\def\csname res@abl.segments.f1\endcsname{0.363}
\expandafter\def\csname res@abl.segments.zs\endcsname{0.442}
\expandafter\def\csname res@abl.segments.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.t14.df1\endcsname{+0.005}
\expandafter\def\csname res@abl.t14.df1ci\endcsname{[+0.000, +0.009]}
\expandafter\def\csname res@abl.t14.dheld\endcsname{+0.008}
\expandafter\def\csname res@abl.t14.dheldci\endcsname{[+0.003, +0.012]}
\expandafter\def\csname res@abl.t14.dll\endcsname{+0.002}
\expandafter\def\csname res@abl.t14.dllci\endcsname{[-0.000, +0.004]}
\expandafter\def\csname res@abl.t14.dzs\endcsname{-0.020}
\expandafter\def\csname res@abl.t14.dzsci\endcsname{[-0.026, -0.015]}
\expandafter\def\csname res@abl.t14.f1\endcsname{0.385}
\expandafter\def\csname res@abl.t14.zs\endcsname{0.426}
\expandafter\def\csname res@abl.t14.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.t7.df1\endcsname{+0.005}
\expandafter\def\csname res@abl.t7.df1ci\endcsname{[-0.002, +0.009]}
\expandafter\def\csname res@abl.t7.dheld\endcsname{+0.030}
\expandafter\def\csname res@abl.t7.dheldci\endcsname{[+0.021, +0.038]}
\expandafter\def\csname res@abl.t7.dll\endcsname{+0.005}
\expandafter\def\csname res@abl.t7.dllci\endcsname{[+0.000, +0.011]}
\expandafter\def\csname res@abl.t7.dzs\endcsname{-0.028}
\expandafter\def\csname res@abl.t7.dzsci\endcsname{[-0.033, -0.023]}
\expandafter\def\csname res@abl.t7.f1\endcsname{0.385}
\expandafter\def\csname res@abl.t7.zs\endcsname{0.418}
\expandafter\def\csname res@abl.t7.zsctrl\endcsname{0.446}
\expandafter\def\csname res@abl.v2noasvp.df1\endcsname{+0.000}
\expandafter\def\csname res@abl.v2noasvp.df1ci\endcsname{[-0.003, +0.004]}
\expandafter\def\csname res@abl.v2noasvp.dheld\endcsname{-0.002}
\expandafter\def\csname res@abl.v2noasvp.dheldci\endcsname{[-0.005, +0.000]}
\expandafter\def\csname res@abl.v2noasvp.dll\endcsname{-0.000}
\expandafter\def\csname res@abl.v2noasvp.dllci\endcsname{[-0.003, +0.002]}
\expandafter\def\csname res@abl.v2noasvp.dzs\endcsname{+0.036}
\expandafter\def\csname res@abl.v2noasvp.dzsci\endcsname{[+0.029, +0.043]}
\expandafter\def\csname res@abl.v2noasvp.f1\endcsname{0.382}
\expandafter\def\csname res@abl.v2noasvp.zs\endcsname{0.463}
\expandafter\def\csname res@abl.v2noasvp.zsctrl\endcsname{0.427}
\expandafter\def\csname res@abl.v2noemonet.df1\endcsname{-0.002}
\expandafter\def\csname res@abl.v2noemonet.df1ci\endcsname{[-0.006, +0.003]}
\expandafter\def\csname res@abl.v2noemonet.dheld\endcsname{+0.001}
\expandafter\def\csname res@abl.v2noemonet.dheldci\endcsname{[-0.004, +0.005]}
\expandafter\def\csname res@abl.v2noemonet.dll\endcsname{+0.001}
\expandafter\def\csname res@abl.v2noemonet.dllci\endcsname{[-0.002, +0.005]}
\expandafter\def\csname res@abl.v2noemonet.dzs\endcsname{+0.005}
\expandafter\def\csname res@abl.v2noemonet.dzsci\endcsname{[-0.000, +0.011]}
\expandafter\def\csname res@abl.v2noemonet.f1\endcsname{0.381}
\expandafter\def\csname res@abl.v2noemonet.zs\endcsname{0.432}
\expandafter\def\csname res@abl.v2noemonet.zsctrl\endcsname{0.426}
\expandafter\def\csname res@abl.v2repeat1.df1\endcsname{-0.002}
\expandafter\def\csname res@abl.v2repeat1.df1ci\endcsname{[-0.006, +0.004]}
\expandafter\def\csname res@abl.v2repeat1.dheld\endcsname{-0.003}
\expandafter\def\csname res@abl.v2repeat1.dheldci\endcsname{[-0.007, -0.000]}
\expandafter\def\csname res@abl.v2repeat1.dll\endcsname{-0.001}
\expandafter\def\csname res@abl.v2repeat1.dllci\endcsname{[-0.004, +0.002]}
\expandafter\def\csname res@abl.v2repeat1.dzs\endcsname{+0.001}
\expandafter\def\csname res@abl.v2repeat1.dzsci\endcsname{[-0.005, +0.007]}
\expandafter\def\csname res@abl.v2repeat1.f1\endcsname{0.381}
\expandafter\def\csname res@abl.v2repeat1.zs\endcsname{0.427}
\expandafter\def\csname res@abl.v2repeat1.zsctrl\endcsname{0.426}
\expandafter\def\csname res@abl.v2speech.df1\endcsname{+0.001}
\expandafter\def\csname res@abl.v2speech.df1ci\endcsname{[-0.002, +0.005]}
\expandafter\def\csname res@abl.v2speech.dheld\endcsname{-0.007}
\expandafter\def\csname res@abl.v2speech.dheldci\endcsname{[-0.011, -0.002]}
\expandafter\def\csname res@abl.v2speech.dll\endcsname{-0.003}
\expandafter\def\csname res@abl.v2speech.dllci\endcsname{[-0.005, -0.001]}
\expandafter\def\csname res@abl.v2speech.dzs\endcsname{+0.047}
\expandafter\def\csname res@abl.v2speech.dzsci\endcsname{[+0.039, +0.054]}
\expandafter\def\csname res@abl.v2speech.f1\endcsname{0.383}
\expandafter\def\csname res@abl.v2speech.zs\endcsname{0.474}
\expandafter\def\csname res@abl.v2speech.zsctrl\endcsname{0.427}
\expandafter\def\csname res@abl.w24.df1\endcsname{-0.056}
\expandafter\def\csname res@abl.w24.df1ci\endcsname{[-0.066, -0.049]}
\expandafter\def\csname res@abl.w24.dheld\endcsname{+0.061}
\expandafter\def\csname res@abl.w24.dheldci\endcsname{[+0.047, +0.075]}
\expandafter\def\csname res@abl.w24.dll\endcsname{+0.063}
\expandafter\def\csname res@abl.w24.dllci\endcsname{[+0.051, +0.075]}
\expandafter\def\csname res@abl.w24.dzs\endcsname{-0.011}
\expandafter\def\csname res@abl.w24.dzsci\endcsname{[-0.020, -0.002]}
\expandafter\def\csname res@abl.w24.f1\endcsname{0.328}
\expandafter\def\csname res@abl.w24.zs\endcsname{0.429}
\expandafter\def\csname res@abl.w24.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.w2432.df1\endcsname{-0.000}
\expandafter\def\csname res@abl.w2432.df1ci\endcsname{[-0.007, +0.005]}
\expandafter\def\csname res@abl.w2432.dheld\endcsname{+0.000}
\expandafter\def\csname res@abl.w2432.dheldci\endcsname{[-0.002, +0.002]}
\expandafter\def\csname res@abl.w2432.dll\endcsname{+0.001}
\expandafter\def\csname res@abl.w2432.dllci\endcsname{[-0.001, +0.003]}
\expandafter\def\csname res@abl.w2432.dzs\endcsname{-0.004}
\expandafter\def\csname res@abl.w2432.dzsci\endcsname{[-0.011, +0.001]}
\expandafter\def\csname res@abl.w2432.f1\endcsname{0.384}
\expandafter\def\csname res@abl.w2432.zs\endcsname{0.436}
\expandafter\def\csname res@abl.w2432.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.w32.df1\endcsname{-0.002}
\expandafter\def\csname res@abl.w32.df1ci\endcsname{[-0.009, +0.004]}
\expandafter\def\csname res@abl.w32.dheld\endcsname{+0.001}
\expandafter\def\csname res@abl.w32.dheldci\endcsname{[-0.005, +0.006]}
\expandafter\def\csname res@abl.w32.dll\endcsname{+0.003}
\expandafter\def\csname res@abl.w32.dllci\endcsname{[-0.002, +0.007]}
\expandafter\def\csname res@abl.w32.dzs\endcsname{-0.012}
\expandafter\def\csname res@abl.w32.dzsci\endcsname{[-0.018, -0.006]}
\expandafter\def\csname res@abl.w32.f1\endcsname{0.383}
\expandafter\def\csname res@abl.w32.zs\endcsname{0.428}
\expandafter\def\csname res@abl.w32.zsctrl\endcsname{0.440}
\expandafter\def\csname res@abl.wavlm.df1\endcsname{-0.021}
\expandafter\def\csname res@abl.wavlm.df1ci\endcsname{[-0.029, -0.014]}
\expandafter\def\csname res@abl.wavlm.dll\endcsname{+0.024}
\expandafter\def\csname res@abl.wavlm.dllci\endcsname{[+0.020, +0.027]}
\expandafter\def\csname res@abl.wavlm.f1\endcsname{0.345}
\expandafter\def\csname res@af3.subset.delta\endcsname{-0.223}
\expandafter\def\csname res@af3.subset.deltaci\endcsname{[-0.251, -0.199]}
\expandafter\def\csname res@af3.subset.deltaoff\endcsname{-0.230}
\expandafter\def\csname res@af3.subset.deltaoffci\endcsname{[-0.267, -0.199]}
\expandafter\def\csname res@af3.subset.ece\endcsname{0.203}
\expandafter\def\csname res@af3.subset.ecev\endcsname{0.247}
\expandafter\def\csname res@af3.subset.ecevoracle\endcsname{0.034}
\expandafter\def\csname res@af3.subset.f1\endcsname{0.160}
\expandafter\def\csname res@af3.subset.f1ci\endcsname{[0.145, 0.177]}
\expandafter\def\csname res@af3.subset.f1off\endcsname{0.164}
\expandafter\def\csname res@af3.subset.f1offci\endcsname{[0.145, 0.186]}
\expandafter\def\csname res@af3.subset.gap\endcsname{0.223}
\expandafter\def\csname res@af3.subset.gapci\endcsname{[0.199, 0.251]}
\expandafter\def\csname res@af3.subset.ll\endcsname{2.306}
\expandafter\def\csname res@af3.subset.lloracle\endcsname{1.932}
\expandafter\def\csname res@af3.subset.toracle\endcsname{2.90}
\expandafter\def\csname res@af3_cc.subset.delta\endcsname{-0.238}
\expandafter\def\csname res@af3_cc.subset.deltaci\endcsname{[-0.267, -0.215]}
\expandafter\def\csname res@af3_cc.subset.deltaoff\endcsname{-0.240}
\expandafter\def\csname res@af3_cc.subset.deltaoffci\endcsname{[-0.277, -0.210]}
\expandafter\def\csname res@af3_cc.subset.ece\endcsname{0.223}
\expandafter\def\csname res@af3_cc.subset.ecev\endcsname{0.226}
\expandafter\def\csname res@af3_cc.subset.ecevoracle\endcsname{0.016}
\expandafter\def\csname res@af3_cc.subset.f1\endcsname{0.145}
\expandafter\def\csname res@af3_cc.subset.f1ci\endcsname{[0.130, 0.159]}
\expandafter\def\csname res@af3_cc.subset.f1off\endcsname{0.154}
\expandafter\def\csname res@af3_cc.subset.f1offci\endcsname{[0.138, 0.168]}
\expandafter\def\csname res@af3_cc.subset.gap\endcsname{0.238}
\expandafter\def\csname res@af3_cc.subset.gapci\endcsname{[0.215, 0.267]}
\expandafter\def\csname res@af3_cc.subset.ll\endcsname{2.476}
\expandafter\def\csname res@af3_cc.subset.lloracle\endcsname{2.047}
\expandafter\def\csname res@af3_cc.subset.toracle\endcsname{5.11}
\expandafter\def\csname res@alms.full.count\endcsname{1}
\expandafter\def\csname res@alms.full.llmin\endcsname{2.257}
\expandafter\def\csname res@alms.full.lloraclemin\endcsname{1.878}
\expandafter\def\csname res@alms.full.lloraclemin.name\endcsname{Qwen2.5-Omni-3B}
\expandafter\def\csname res@alms.subset.count\endcsname{6}
\expandafter\def\csname res@alms.subset.llmin\endcsname{2.097}
\expandafter\def\csname res@alms.subset.lloraclemin\endcsname{1.751}
\expandafter\def\csname res@alms.subset.lloraclemin.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@arch.wclip.b16\endcsname{0.12}
\expandafter\def\csname res@arch.wclip.b24\endcsname{0.05}
\expandafter\def\csname res@arch.wclip.b32\endcsname{0.62}
\expandafter\def\csname res@arch.wclip.b8\endcsname{0.21}
\expandafter\def\csname res@arch.wseg.b16\endcsname{0.10}
\expandafter\def\csname res@arch.wseg.b24\endcsname{0.15}
\expandafter\def\csname res@arch.wseg.b32\endcsname{0.63}
\expandafter\def\csname res@arch.wseg.b8\endcsname{0.12}
\expandafter\def\csname res@asom.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom.full.ece\endcsname{0.054}
\expandafter\def\csname res@asom.full.ecev\endcsname{0.042}
\expandafter\def\csname res@asom.full.ecevoracle\endcsname{0.003}
\expandafter\def\csname res@asom.full.f1\endcsname{0.382}
\expandafter\def\csname res@asom.full.f1ci\endcsname{[0.355, 0.405]}
\expandafter\def\csname res@asom.full.f1off\endcsname{0.401}
\expandafter\def\csname res@asom.full.f1offci\endcsname{[0.369, 0.431]}
\expandafter\def\csname res@asom.full.ll\endcsname{1.506}
\expandafter\def\csname res@asom.full.lloracle\endcsname{1.500}
\expandafter\def\csname res@asom.full.toracle\endcsname{1.13}
\expandafter\def\csname res@asom.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@asom.subset.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom.subset.ece\endcsname{0.061}
\expandafter\def\csname res@asom.subset.ecev\endcsname{0.040}
\expandafter\def\csname res@asom.subset.ecevoracle\endcsname{0.017}
\expandafter\def\csname res@asom.subset.f1\endcsname{0.383}
\expandafter\def\csname res@asom.subset.f1ci\endcsname{[0.353, 0.412]}
\expandafter\def\csname res@asom.subset.f1off\endcsname{0.394}
\expandafter\def\csname res@asom.subset.f1offci\endcsname{[0.359, 0.430]}
\expandafter\def\csname res@asom.subset.ll\endcsname{1.507}
\expandafter\def\csname res@asom.subset.lloracle\endcsname{1.500}
\expandafter\def\csname res@asom.subset.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_30s.full.ccc.arousal\endcsname{0.62}
\expandafter\def\csname res@asom_30s.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom_30s.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_30s.full.delta\endcsname{+0.000}
\expandafter\def\csname res@asom_30s.full.deltaci\endcsname{[-0.003, +0.006]}
\expandafter\def\csname res@asom_30s.full.deltaoff\endcsname{-0.001}
\expandafter\def\csname res@asom_30s.full.deltaoffci\endcsname{[-0.005, +0.004]}
\expandafter\def\csname res@asom_30s.full.ece\endcsname{0.055}
\expandafter\def\csname res@asom_30s.full.ecev\endcsname{0.041}
\expandafter\def\csname res@asom_30s.full.ecevoracle\endcsname{0.004}
\expandafter\def\csname res@asom_30s.full.f1\endcsname{0.382}
\expandafter\def\csname res@asom_30s.full.f1ci\endcsname{[0.353, 0.409]}
\expandafter\def\csname res@asom_30s.full.f1off\endcsname{0.400}
\expandafter\def\csname res@asom_30s.full.f1offci\endcsname{[0.366, 0.431]}
\expandafter\def\csname res@asom_30s.full.gap\endcsname{-0.000}
\expandafter\def\csname res@asom_30s.full.gapci\endcsname{[-0.006, 0.003]}
\expandafter\def\csname res@asom_30s.full.ll\endcsname{1.502}
\expandafter\def\csname res@asom_30s.full.lloracle\endcsname{1.496}
\expandafter\def\csname res@asom_30s.full.toracle\endcsname{1.12}
\expandafter\def\csname res@asom_30s.subset.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_30s.subset.ccc.dominance\endcsname{0.52}
\expandafter\def\csname res@asom_30s.subset.ccc.valence\endcsname{0.72}
\expandafter\def\csname res@asom_30s.subset.delta\endcsname{-0.005}
\expandafter\def\csname res@asom_30s.subset.deltaci\endcsname{[-0.017, +0.010]}
\expandafter\def\csname res@asom_30s.subset.deltaoff\endcsname{-0.002}
\expandafter\def\csname res@asom_30s.subset.deltaoffci\endcsname{[-0.015, +0.016]}
\expandafter\def\csname res@asom_30s.subset.ece\endcsname{0.058}
\expandafter\def\csname res@asom_30s.subset.ecev\endcsname{0.039}
\expandafter\def\csname res@asom_30s.subset.ecevoracle\endcsname{0.010}
\expandafter\def\csname res@asom_30s.subset.f1\endcsname{0.378}
\expandafter\def\csname res@asom_30s.subset.f1ci\endcsname{[0.341, 0.413]}
\expandafter\def\csname res@asom_30s.subset.f1off\endcsname{0.392}
\expandafter\def\csname res@asom_30s.subset.f1offci\endcsname{[0.347, 0.435]}
\expandafter\def\csname res@asom_30s.subset.gap\endcsname{0.005}
\expandafter\def\csname res@asom_30s.subset.gapci\endcsname{[-0.010, 0.017]}
\expandafter\def\csname res@asom_30s.subset.ll\endcsname{1.503}
\expandafter\def\csname res@asom_30s.subset.lloracle\endcsname{1.497}
\expandafter\def\csname res@asom_30s.subset.toracle\endcsname{1.12}
\expandafter\def\csname res@asom_cc.subset.delta\endcsname{-0.120}
\expandafter\def\csname res@asom_cc.subset.deltaci\endcsname{[-0.142, -0.101]}
\expandafter\def\csname res@asom_cc.subset.deltaoff\endcsname{-0.131}
\expandafter\def\csname res@asom_cc.subset.deltaoffci\endcsname{[-0.162, -0.105]}
\expandafter\def\csname res@asom_cc.subset.ece\endcsname{0.073}
\expandafter\def\csname res@asom_cc.subset.ecev\endcsname{0.123}
\expandafter\def\csname res@asom_cc.subset.ecevoracle\endcsname{0.088}
\expandafter\def\csname res@asom_cc.subset.f1\endcsname{0.263}
\expandafter\def\csname res@asom_cc.subset.f1ci\endcsname{[0.242, 0.285]}
\expandafter\def\csname res@asom_cc.subset.f1off\endcsname{0.263}
\expandafter\def\csname res@asom_cc.subset.f1offci\endcsname{[0.242, 0.285]}
\expandafter\def\csname res@asom_cc.subset.gap\endcsname{0.120}
\expandafter\def\csname res@asom_cc.subset.gapci\endcsname{[0.101, 0.142]}
\expandafter\def\csname res@asom_cc.subset.ll\endcsname{2.179}
\expandafter\def\csname res@asom_cc.subset.lloracle\endcsname{1.964}
\expandafter\def\csname res@asom_cc.subset.toracle\endcsname{2.56}
\expandafter\def\csname res@asom_clip.full.ccc.arousal\endcsname{0.65}
\expandafter\def\csname res@asom_clip.full.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom_clip.full.ccc.valence\endcsname{0.72}
\expandafter\def\csname res@asom_clip.full.delta\endcsname{-0.050}
\expandafter\def\csname res@asom_clip.full.deltaci\endcsname{[-0.059, -0.039]}
\expandafter\def\csname res@asom_clip.full.deltaoff\endcsname{-0.056}
\expandafter\def\csname res@asom_clip.full.deltaoffci\endcsname{[-0.065, -0.047]}
\expandafter\def\csname res@asom_clip.full.ece\endcsname{0.038}
\expandafter\def\csname res@asom_clip.full.ecev\endcsname{0.088}
\expandafter\def\csname res@asom_clip.full.ecevoracle\endcsname{0.037}
\expandafter\def\csname res@asom_clip.full.f1\endcsname{0.332}
\expandafter\def\csname res@asom_clip.full.f1ci\endcsname{[0.301, 0.361]}
\expandafter\def\csname res@asom_clip.full.f1off\endcsname{0.345}
\expandafter\def\csname res@asom_clip.full.f1offci\endcsname{[0.311, 0.376]}
\expandafter\def\csname res@asom_clip.full.gap\endcsname{0.050}
\expandafter\def\csname res@asom_clip.full.gapci\endcsname{[0.039, 0.059]}
\expandafter\def\csname res@asom_clip.full.ll\endcsname{1.870}
\expandafter\def\csname res@asom_clip.full.lloracle\endcsname{1.793}
\expandafter\def\csname res@asom_clip.full.toracle\endcsname{1.61}
\expandafter\def\csname res@asom_clip.subset.ccc.arousal\endcsname{0.66}
\expandafter\def\csname res@asom_clip.subset.ccc.dominance\endcsname{0.54}
\expandafter\def\csname res@asom_clip.subset.ccc.valence\endcsname{0.72}
\expandafter\def\csname res@asom_clip.subset.delta\endcsname{-0.052}
\expandafter\def\csname res@asom_clip.subset.deltaci\endcsname{[-0.068, -0.032]}
\expandafter\def\csname res@asom_clip.subset.deltaoff\endcsname{-0.048}
\expandafter\def\csname res@asom_clip.subset.deltaoffci\endcsname{[-0.067, -0.025]}
\expandafter\def\csname res@asom_clip.subset.ece\endcsname{0.047}
\expandafter\def\csname res@asom_clip.subset.ecev\endcsname{0.086}
\expandafter\def\csname res@asom_clip.subset.ecevoracle\endcsname{0.043}
\expandafter\def\csname res@asom_clip.subset.f1\endcsname{0.331}
\expandafter\def\csname res@asom_clip.subset.f1ci\endcsname{[0.298, 0.361]}
\expandafter\def\csname res@asom_clip.subset.f1off\endcsname{0.346}
\expandafter\def\csname res@asom_clip.subset.f1offci\endcsname{[0.309, 0.382]}
\expandafter\def\csname res@asom_clip.subset.gap\endcsname{0.052}
\expandafter\def\csname res@asom_clip.subset.gapci\endcsname{[0.032, 0.068]}
\expandafter\def\csname res@asom_clip.subset.ll\endcsname{1.876}
\expandafter\def\csname res@asom_clip.subset.lloracle\endcsname{1.799}
\expandafter\def\csname res@asom_clip.subset.toracle\endcsname{1.61}
\expandafter\def\csname res@asom_em.subset.delta\endcsname{-0.150}
\expandafter\def\csname res@asom_em.subset.deltaci\endcsname{[-0.172, -0.130]}
\expandafter\def\csname res@asom_em.subset.deltaoff\endcsname{-0.139}
\expandafter\def\csname res@asom_em.subset.deltaoffci\endcsname{[-0.162, -0.117]}
\expandafter\def\csname res@asom_em.subset.ece\endcsname{0.156}
\expandafter\def\csname res@asom_em.subset.ecev\endcsname{0.236}
\expandafter\def\csname res@asom_em.subset.ecevoracle\endcsname{0.194}
\expandafter\def\csname res@asom_em.subset.f1\endcsname{0.233}
\expandafter\def\csname res@asom_em.subset.f1ci\endcsname{[0.217, 0.249]}
\expandafter\def\csname res@asom_em.subset.f1off\endcsname{0.255}
\expandafter\def\csname res@asom_em.subset.f1offci\endcsname{[0.232, 0.277]}
\expandafter\def\csname res@asom_em.subset.gap\endcsname{0.150}
\expandafter\def\csname res@asom_em.subset.gapci\endcsname{[0.130, 0.172]}
\expandafter\def\csname res@asom_em.subset.ll\endcsname{7.651}
\expandafter\def\csname res@asom_em.subset.lloracle\endcsname{1.818}
\expandafter\def\csname res@asom_em.subset.toracle\endcsname{15.67}
\expandafter\def\csname res@asom_text.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_text.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom_text.full.ccc.valence\endcsname{0.72}
\expandafter\def\csname res@asom_text.full.delta\endcsname{+0.012}
\expandafter\def\csname res@asom_text.full.deltaci\endcsname{[+0.007, +0.020]}
\expandafter\def\csname res@asom_text.full.deltaoff\endcsname{+0.012}
\expandafter\def\csname res@asom_text.full.deltaoffci\endcsname{[+0.006, +0.021]}
\expandafter\def\csname res@asom_text.full.ece\endcsname{0.068}
\expandafter\def\csname res@asom_text.full.ecev\endcsname{0.026}
\expandafter\def\csname res@asom_text.full.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@asom_text.full.f1\endcsname{0.394}
\expandafter\def\csname res@asom_text.full.f1ci\endcsname{[0.364, 0.421]}
\expandafter\def\csname res@asom_text.full.f1off\endcsname{0.414}
\expandafter\def\csname res@asom_text.full.f1offci\endcsname{[0.378, 0.447]}
\expandafter\def\csname res@asom_text.full.gap\endcsname{-0.012}
\expandafter\def\csname res@asom_text.full.gapci\endcsname{[-0.020, -0.007]}
\expandafter\def\csname res@asom_text.full.ll\endcsname{1.472}
\expandafter\def\csname res@asom_text.full.lloracle\endcsname{1.471}
\expandafter\def\csname res@asom_text.full.toracle\endcsname{1.05}
\expandafter\def\csname res@asom_text.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@asom_text.subset.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom_text.subset.ccc.valence\endcsname{0.72}
\expandafter\def\csname res@asom_text.subset.delta\endcsname{+0.019}
\expandafter\def\csname res@asom_text.subset.deltaci\endcsname{[+0.003, +0.043]}
\expandafter\def\csname res@asom_text.subset.deltaoff\endcsname{+0.023}
\expandafter\def\csname res@asom_text.subset.deltaoffci\endcsname{[-0.000, +0.058]}
\expandafter\def\csname res@asom_text.subset.ece\endcsname{0.056}
\expandafter\def\csname res@asom_text.subset.ecev\endcsname{0.031}
\expandafter\def\csname res@asom_text.subset.ecevoracle\endcsname{0.015}
\expandafter\def\csname res@asom_text.subset.f1\endcsname{0.402}
\expandafter\def\csname res@asom_text.subset.f1ci\endcsname{[0.365, 0.440]}
\expandafter\def\csname res@asom_text.subset.f1off\endcsname{0.417}
\expandafter\def\csname res@asom_text.subset.f1offci\endcsname{[0.367, 0.469]}
\expandafter\def\csname res@asom_text.subset.gap\endcsname{-0.019}
\expandafter\def\csname res@asom_text.subset.gapci\endcsname{[-0.043, -0.003]}
\expandafter\def\csname res@asom_text.subset.ll\endcsname{1.473}
\expandafter\def\csname res@asom_text.subset.lloracle\endcsname{1.471}
\expandafter\def\csname res@asom_text.subset.toracle\endcsname{1.05}
\expandafter\def\csname res@asom_u.subset.delta\endcsname{-0.030}
\expandafter\def\csname res@asom_u.subset.deltaci\endcsname{[-0.045, -0.019]}
\expandafter\def\csname res@asom_u.subset.deltaoff\endcsname{-0.022}
\expandafter\def\csname res@asom_u.subset.deltaoffci\endcsname{[-0.036, -0.009]}
\expandafter\def\csname res@asom_u.subset.ece\endcsname{0.087}
\expandafter\def\csname res@asom_u.subset.ecev\endcsname{0.021}
\expandafter\def\csname res@asom_u.subset.ecevoracle\endcsname{0.013}
\expandafter\def\csname res@asom_u.subset.f1\endcsname{0.353}
\expandafter\def\csname res@asom_u.subset.f1ci\endcsname{[0.327, 0.379]}
\expandafter\def\csname res@asom_u.subset.f1off\endcsname{0.372}
\expandafter\def\csname res@asom_u.subset.f1offci\endcsname{[0.339, 0.406]}
\expandafter\def\csname res@asom_u.subset.gap\endcsname{0.030}
\expandafter\def\csname res@asom_u.subset.gapci\endcsname{[0.019, 0.045]}
\expandafter\def\csname res@asom_u.subset.ll\endcsname{1.532}
\expandafter\def\csname res@asom_u.subset.lloracle\endcsname{1.532}
\expandafter\def\csname res@asom_u.subset.toracle\endcsname{1.04}
\expandafter\def\csname res@asom_v2.full.ccc.arousal\endcsname{0.62}
\expandafter\def\csname res@asom_v2.full.ccc.dominance\endcsname{0.50}
\expandafter\def\csname res@asom_v2.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2.full.delta\endcsname{+0.000}
\expandafter\def\csname res@asom_v2.full.deltaci\endcsname{[-0.004, +0.005]}
\expandafter\def\csname res@asom_v2.full.deltaoff\endcsname{-0.001}
\expandafter\def\csname res@asom_v2.full.deltaoffci\endcsname{[-0.005, +0.005]}
\expandafter\def\csname res@asom_v2.full.ece\endcsname{0.052}
\expandafter\def\csname res@asom_v2.full.ecev\endcsname{0.043}
\expandafter\def\csname res@asom_v2.full.ecevoracle\endcsname{0.004}
\expandafter\def\csname res@asom_v2.full.f1\endcsname{0.382}
\expandafter\def\csname res@asom_v2.full.f1ci\endcsname{[0.355, 0.407]}
\expandafter\def\csname res@asom_v2.full.f1off\endcsname{0.401}
\expandafter\def\csname res@asom_v2.full.f1offci\endcsname{[0.368, 0.431]}
\expandafter\def\csname res@asom_v2.full.gap\endcsname{-0.000}
\expandafter\def\csname res@asom_v2.full.gapci\endcsname{[-0.005, 0.004]}
\expandafter\def\csname res@asom_v2.full.ll\endcsname{1.506}
\expandafter\def\csname res@asom_v2.full.lloracle\endcsname{1.500}
\expandafter\def\csname res@asom_v2.full.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@asom_v2.subset.ccc.dominance\endcsname{0.52}
\expandafter\def\csname res@asom_v2.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2.subset.delta\endcsname{-0.011}
\expandafter\def\csname res@asom_v2.subset.deltaci\endcsname{[-0.020, -0.001]}
\expandafter\def\csname res@asom_v2.subset.deltaoff\endcsname{-0.005}
\expandafter\def\csname res@asom_v2.subset.deltaoffci\endcsname{[-0.016, +0.009]}
\expandafter\def\csname res@asom_v2.subset.ece\endcsname{0.058}
\expandafter\def\csname res@asom_v2.subset.ecev\endcsname{0.041}
\expandafter\def\csname res@asom_v2.subset.ecevoracle\endcsname{0.006}
\expandafter\def\csname res@asom_v2.subset.f1\endcsname{0.372}
\expandafter\def\csname res@asom_v2.subset.f1ci\endcsname{[0.342, 0.402]}
\expandafter\def\csname res@asom_v2.subset.f1off\endcsname{0.389}
\expandafter\def\csname res@asom_v2.subset.f1offci\endcsname{[0.349, 0.427]}
\expandafter\def\csname res@asom_v2.subset.gap\endcsname{0.011}
\expandafter\def\csname res@asom_v2.subset.gapci\endcsname{[0.001, 0.020]}
\expandafter\def\csname res@asom_v2.subset.ll\endcsname{1.507}
\expandafter\def\csname res@asom_v2.subset.lloracle\endcsname{1.500}
\expandafter\def\csname res@asom_v2.subset.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2_u.subset.delta\endcsname{-0.020}
\expandafter\def\csname res@asom_v2_u.subset.deltaci\endcsname{[-0.034, -0.006]}
\expandafter\def\csname res@asom_v2_u.subset.deltaoff\endcsname{-0.007}
\expandafter\def\csname res@asom_v2_u.subset.deltaoffci\endcsname{[-0.024, +0.014]}
\expandafter\def\csname res@asom_v2_u.subset.ece\endcsname{0.083}
\expandafter\def\csname res@asom_v2_u.subset.ecev\endcsname{0.026}
\expandafter\def\csname res@asom_v2_u.subset.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@asom_v2_u.subset.f1\endcsname{0.363}
\expandafter\def\csname res@asom_v2_u.subset.f1ci\endcsname{[0.333, 0.392]}
\expandafter\def\csname res@asom_v2_u.subset.f1off\endcsname{0.387}
\expandafter\def\csname res@asom_v2_u.subset.f1offci\endcsname{[0.343, 0.430]}
\expandafter\def\csname res@asom_v2_u.subset.gap\endcsname{0.020}
\expandafter\def\csname res@asom_v2_u.subset.gapci\endcsname{[0.006, 0.034]}
\expandafter\def\csname res@asom_v2_u.subset.ll\endcsname{1.530}
\expandafter\def\csname res@asom_v2_u.subset.lloracle\endcsname{1.528}
\expandafter\def\csname res@asom_v2_u.subset.toracle\endcsname{1.06}
\expandafter\def\csname res@asom_v2_vg.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_v2_vg.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom_v2_vg.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2_vg.full.delta\endcsname{-0.000}
\expandafter\def\csname res@asom_v2_vg.full.deltaci\endcsname{[-0.005, +0.007]}
\expandafter\def\csname res@asom_v2_vg.full.deltaoff\endcsname{-0.001}
\expandafter\def\csname res@asom_v2_vg.full.deltaoffci\endcsname{[-0.005, +0.006]}
\expandafter\def\csname res@asom_v2_vg.full.ece\endcsname{0.053}
\expandafter\def\csname res@asom_v2_vg.full.ecev\endcsname{0.042}
\expandafter\def\csname res@asom_v2_vg.full.ecevoracle\endcsname{0.004}
\expandafter\def\csname res@asom_v2_vg.full.f1\endcsname{0.382}
\expandafter\def\csname res@asom_v2_vg.full.f1ci\endcsname{[0.353, 0.408]}
\expandafter\def\csname res@asom_v2_vg.full.f1off\endcsname{0.401}
\expandafter\def\csname res@asom_v2_vg.full.f1offci\endcsname{[0.367, 0.433]}
\expandafter\def\csname res@asom_v2_vg.full.gap\endcsname{0.000}
\expandafter\def\csname res@asom_v2_vg.full.gapci\endcsname{[-0.007, 0.005]}
\expandafter\def\csname res@asom_v2_vg.full.ll\endcsname{1.505}
\expandafter\def\csname res@asom_v2_vg.full.lloracle\endcsname{1.498}
\expandafter\def\csname res@asom_v2_vg.full.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2_vg.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@asom_v2_vg.subset.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom_v2_vg.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2_vg.subset.delta\endcsname{+0.006}
\expandafter\def\csname res@asom_v2_vg.subset.deltaci\endcsname{[-0.008, +0.022]}
\expandafter\def\csname res@asom_v2_vg.subset.deltaoff\endcsname{+0.007}
\expandafter\def\csname res@asom_v2_vg.subset.deltaoffci\endcsname{[-0.009, +0.025]}
\expandafter\def\csname res@asom_v2_vg.subset.ece\endcsname{0.064}
\expandafter\def\csname res@asom_v2_vg.subset.ecev\endcsname{0.040}
\expandafter\def\csname res@asom_v2_vg.subset.ecevoracle\endcsname{0.009}
\expandafter\def\csname res@asom_v2_vg.subset.f1\endcsname{0.390}
\expandafter\def\csname res@asom_v2_vg.subset.f1ci\endcsname{[0.354, 0.424]}
\expandafter\def\csname res@asom_v2_vg.subset.f1off\endcsname{0.401}
\expandafter\def\csname res@asom_v2_vg.subset.f1offci\endcsname{[0.358, 0.443]}
\expandafter\def\csname res@asom_v2_vg.subset.gap\endcsname{-0.006}
\expandafter\def\csname res@asom_v2_vg.subset.gapci\endcsname{[-0.022, 0.008]}
\expandafter\def\csname res@asom_v2_vg.subset.ll\endcsname{1.502}
\expandafter\def\csname res@asom_v2_vg.subset.lloracle\endcsname{1.496}
\expandafter\def\csname res@asom_v2_vg.subset.toracle\endcsname{1.12}
\expandafter\def\csname res@asom_v2_vg_u.subset.delta\endcsname{-0.007}
\expandafter\def\csname res@asom_v2_vg_u.subset.deltaci\endcsname{[-0.023, +0.012]}
\expandafter\def\csname res@asom_v2_vg_u.subset.deltaoff\endcsname{+0.007}
\expandafter\def\csname res@asom_v2_vg_u.subset.deltaoffci\endcsname{[-0.011, +0.030]}
\expandafter\def\csname res@asom_v2_vg_u.subset.ece\endcsname{0.091}
\expandafter\def\csname res@asom_v2_vg_u.subset.ecev\endcsname{0.023}
\expandafter\def\csname res@asom_v2_vg_u.subset.ecevoracle\endcsname{0.013}
\expandafter\def\csname res@asom_v2_vg_u.subset.f1\endcsname{0.376}
\expandafter\def\csname res@asom_v2_vg_u.subset.f1ci\endcsname{[0.342, 0.410]}
\expandafter\def\csname res@asom_v2_vg_u.subset.f1off\endcsname{0.401}
\expandafter\def\csname res@asom_v2_vg_u.subset.f1offci\endcsname{[0.352, 0.449]}
\expandafter\def\csname res@asom_v2_vg_u.subset.gap\endcsname{0.007}
\expandafter\def\csname res@asom_v2_vg_u.subset.gapci\endcsname{[-0.012, 0.023]}
\expandafter\def\csname res@asom_v2_vg_u.subset.ll\endcsname{1.520}
\expandafter\def\csname res@asom_v2_vg_u.subset.lloracle\endcsname{1.519}
\expandafter\def\csname res@asom_v2_vg_u.subset.toracle\endcsname{1.05}
\expandafter\def\csname res@asom_v2na.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_v2na.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom_v2na.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2na.full.delta\endcsname{+0.001}
\expandafter\def\csname res@asom_v2na.full.deltaci\endcsname{[-0.004, +0.006]}
\expandafter\def\csname res@asom_v2na.full.deltaoff\endcsname{-0.003}
\expandafter\def\csname res@asom_v2na.full.deltaoffci\endcsname{[-0.007, +0.003]}
\expandafter\def\csname res@asom_v2na.full.ece\endcsname{0.054}
\expandafter\def\csname res@asom_v2na.full.ecev\endcsname{0.042}
\expandafter\def\csname res@asom_v2na.full.ecevoracle\endcsname{0.004}
\expandafter\def\csname res@asom_v2na.full.f1\endcsname{0.383}
\expandafter\def\csname res@asom_v2na.full.f1ci\endcsname{[0.355, 0.408]}
\expandafter\def\csname res@asom_v2na.full.f1off\endcsname{0.399}
\expandafter\def\csname res@asom_v2na.full.f1offci\endcsname{[0.367, 0.430]}
\expandafter\def\csname res@asom_v2na.full.gap\endcsname{-0.001}
\expandafter\def\csname res@asom_v2na.full.gapci\endcsname{[-0.006, 0.004]}
\expandafter\def\csname res@asom_v2na.full.ll\endcsname{1.505}
\expandafter\def\csname res@asom_v2na.full.lloracle\endcsname{1.498}
\expandafter\def\csname res@asom_v2na.full.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2na.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@asom_v2na.subset.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom_v2na.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2na.subset.delta\endcsname{-0.003}
\expandafter\def\csname res@asom_v2na.subset.deltaci\endcsname{[-0.015, +0.010]}
\expandafter\def\csname res@asom_v2na.subset.deltaoff\endcsname{-0.003}
\expandafter\def\csname res@asom_v2na.subset.deltaoffci\endcsname{[-0.017, +0.013]}
\expandafter\def\csname res@asom_v2na.subset.ece\endcsname{0.056}
\expandafter\def\csname res@asom_v2na.subset.ecev\endcsname{0.042}
\expandafter\def\csname res@asom_v2na.subset.ecevoracle\endcsname{0.009}
\expandafter\def\csname res@asom_v2na.subset.f1\endcsname{0.380}
\expandafter\def\csname res@asom_v2na.subset.f1ci\endcsname{[0.347, 0.412]}
\expandafter\def\csname res@asom_v2na.subset.f1off\endcsname{0.391}
\expandafter\def\csname res@asom_v2na.subset.f1offci\endcsname{[0.350, 0.431]}
\expandafter\def\csname res@asom_v2na.subset.gap\endcsname{0.003}
\expandafter\def\csname res@asom_v2na.subset.gapci\endcsname{[-0.010, 0.015]}
\expandafter\def\csname res@asom_v2na.subset.ll\endcsname{1.506}
\expandafter\def\csname res@asom_v2na.subset.lloracle\endcsname{1.500}
\expandafter\def\csname res@asom_v2na.subset.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2na_u.subset.delta\endcsname{-0.026}
\expandafter\def\csname res@asom_v2na_u.subset.deltaci\endcsname{[-0.041, -0.008]}
\expandafter\def\csname res@asom_v2na_u.subset.deltaoff\endcsname{-0.016}
\expandafter\def\csname res@asom_v2na_u.subset.deltaoffci\endcsname{[-0.036, +0.010]}
\expandafter\def\csname res@asom_v2na_u.subset.ece\endcsname{0.082}
\expandafter\def\csname res@asom_v2na_u.subset.ecev\endcsname{0.030}
\expandafter\def\csname res@asom_v2na_u.subset.ecevoracle\endcsname{0.015}
\expandafter\def\csname res@asom_v2na_u.subset.f1\endcsname{0.357}
\expandafter\def\csname res@asom_v2na_u.subset.f1ci\endcsname{[0.324, 0.391]}
\expandafter\def\csname res@asom_v2na_u.subset.f1off\endcsname{0.378}
\expandafter\def\csname res@asom_v2na_u.subset.f1offci\endcsname{[0.332, 0.425]}
\expandafter\def\csname res@asom_v2na_u.subset.gap\endcsname{0.026}
\expandafter\def\csname res@asom_v2na_u.subset.gapci\endcsname{[0.008, 0.041]}
\expandafter\def\csname res@asom_v2na_u.subset.ll\endcsname{1.531}
\expandafter\def\csname res@asom_v2na_u.subset.lloracle\endcsname{1.530}
\expandafter\def\csname res@asom_v2na_u.subset.toracle\endcsname{1.07}
\expandafter\def\csname res@asom_v2sp.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_v2sp.full.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@asom_v2sp.full.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2sp.full.delta\endcsname{+0.001}
\expandafter\def\csname res@asom_v2sp.full.deltaci\endcsname{[-0.003, +0.006]}
\expandafter\def\csname res@asom_v2sp.full.deltaoff\endcsname{-0.001}
\expandafter\def\csname res@asom_v2sp.full.deltaoffci\endcsname{[-0.005, +0.003]}
\expandafter\def\csname res@asom_v2sp.full.ece\endcsname{0.054}
\expandafter\def\csname res@asom_v2sp.full.ecev\endcsname{0.044}
\expandafter\def\csname res@asom_v2sp.full.ecevoracle\endcsname{0.005}
\expandafter\def\csname res@asom_v2sp.full.f1\endcsname{0.383}
\expandafter\def\csname res@asom_v2sp.full.f1ci\endcsname{[0.355, 0.409]}
\expandafter\def\csname res@asom_v2sp.full.f1off\endcsname{0.400}
\expandafter\def\csname res@asom_v2sp.full.f1offci\endcsname{[0.367, 0.431]}
\expandafter\def\csname res@asom_v2sp.full.gap\endcsname{-0.001}
\expandafter\def\csname res@asom_v2sp.full.gapci\endcsname{[-0.006, 0.003]}
\expandafter\def\csname res@asom_v2sp.full.ll\endcsname{1.503}
\expandafter\def\csname res@asom_v2sp.full.lloracle\endcsname{1.497}
\expandafter\def\csname res@asom_v2sp.full.toracle\endcsname{1.13}
\expandafter\def\csname res@asom_v2sp.subset.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@asom_v2sp.subset.ccc.dominance\endcsname{0.53}
\expandafter\def\csname res@asom_v2sp.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@asom_v2sp.subset.delta\endcsname{-0.005}
\expandafter\def\csname res@asom_v2sp.subset.deltaci\endcsname{[-0.016, +0.009]}
\expandafter\def\csname res@asom_v2sp.subset.deltaoff\endcsname{-0.002}
\expandafter\def\csname res@asom_v2sp.subset.deltaoffci\endcsname{[-0.014, +0.014]}
\expandafter\def\csname res@asom_v2sp.subset.ece\endcsname{0.054}
\expandafter\def\csname res@asom_v2sp.subset.ecev\endcsname{0.045}
\expandafter\def\csname res@asom_v2sp.subset.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@asom_v2sp.subset.f1\endcsname{0.378}
\expandafter\def\csname res@asom_v2sp.subset.f1ci\endcsname{[0.344, 0.409]}
\expandafter\def\csname res@asom_v2sp.subset.f1off\endcsname{0.392}
\expandafter\def\csname res@asom_v2sp.subset.f1offci\endcsname{[0.351, 0.433]}
\expandafter\def\csname res@asom_v2sp.subset.gap\endcsname{0.005}
\expandafter\def\csname res@asom_v2sp.subset.gapci\endcsname{[-0.009, 0.016]}
\expandafter\def\csname res@asom_v2sp.subset.ll\endcsname{1.505}
\expandafter\def\csname res@asom_v2sp.subset.lloracle\endcsname{1.499}
\expandafter\def\csname res@asom_v2sp.subset.toracle\endcsname{1.12}
\expandafter\def\csname res@asom_v2sp_em.subset.delta\endcsname{-0.151}
\expandafter\def\csname res@asom_v2sp_em.subset.deltaci\endcsname{[-0.173, -0.130]}
\expandafter\def\csname res@asom_v2sp_em.subset.deltaoff\endcsname{-0.141}
\expandafter\def\csname res@asom_v2sp_em.subset.deltaoffci\endcsname{[-0.163, -0.118]}
\expandafter\def\csname res@asom_v2sp_em.subset.ece\endcsname{0.163}
\expandafter\def\csname res@asom_v2sp_em.subset.ecev\endcsname{0.247}
\expandafter\def\csname res@asom_v2sp_em.subset.ecevoracle\endcsname{0.189}
\expandafter\def\csname res@asom_v2sp_em.subset.f1\endcsname{0.232}
\expandafter\def\csname res@asom_v2sp_em.subset.f1ci\endcsname{[0.214, 0.249]}
\expandafter\def\csname res@asom_v2sp_em.subset.f1off\endcsname{0.253}
\expandafter\def\csname res@asom_v2sp_em.subset.f1offci\endcsname{[0.229, 0.277]}
\expandafter\def\csname res@asom_v2sp_em.subset.gap\endcsname{0.151}
\expandafter\def\csname res@asom_v2sp_em.subset.gapci\endcsname{[0.130, 0.173]}
\expandafter\def\csname res@asom_v2sp_em.subset.ll\endcsname{7.748}
\expandafter\def\csname res@asom_v2sp_em.subset.lloracle\endcsname{1.818}
\expandafter\def\csname res@asom_v2sp_em.subset.toracle\endcsname{15.77}
\expandafter\def\csname res@asom_v2sp_u.subset.delta\endcsname{-0.026}
\expandafter\def\csname res@asom_v2sp_u.subset.deltaci\endcsname{[-0.040, -0.009]}
\expandafter\def\csname res@asom_v2sp_u.subset.deltaoff\endcsname{-0.017}
\expandafter\def\csname res@asom_v2sp_u.subset.deltaoffci\endcsname{[-0.036, +0.006]}
\expandafter\def\csname res@asom_v2sp_u.subset.ece\endcsname{0.080}
\expandafter\def\csname res@asom_v2sp_u.subset.ecev\endcsname{0.029}
\expandafter\def\csname res@asom_v2sp_u.subset.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@asom_v2sp_u.subset.f1\endcsname{0.358}
\expandafter\def\csname res@asom_v2sp_u.subset.f1ci\endcsname{[0.325, 0.390]}
\expandafter\def\csname res@asom_v2sp_u.subset.f1off\endcsname{0.377}
\expandafter\def\csname res@asom_v2sp_u.subset.f1offci\endcsname{[0.335, 0.419]}
\expandafter\def\csname res@asom_v2sp_u.subset.gap\endcsname{0.026}
\expandafter\def\csname res@asom_v2sp_u.subset.gapci\endcsname{[0.009, 0.040]}
\expandafter\def\csname res@asom_v2sp_u.subset.ll\endcsname{1.530}
\expandafter\def\csname res@asom_v2sp_u.subset.lloracle\endcsname{1.528}
\expandafter\def\csname res@asom_v2sp_u.subset.toracle\endcsname{1.06}
\expandafter\def\csname res@bestalm.full.f1\endcsname{0.259}
\expandafter\def\csname res@bestalm.full.gap\endcsname{0.123}
\expandafter\def\csname res@bestalm.full.gapci\endcsname{[0.101, 0.146]}
\expandafter\def\csname res@bestalm.full.name\endcsname{Qwen2.5-Omni-3B}
\expandafter\def\csname res@bestalm.subset.f1\endcsname{0.311}
\expandafter\def\csname res@bestalm.subset.gap\endcsname{0.072}
\expandafter\def\csname res@bestalm.subset.gapci\endcsname{[0.051, 0.097]}
\expandafter\def\csname res@bestalm.subset.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@bestalmcc.full.f1\endcsname{0.293}
\expandafter\def\csname res@bestalmcc.full.gap\endcsname{0.089}
\expandafter\def\csname res@bestalmcc.full.gapci\endcsname{[0.074, 0.107]}
\expandafter\def\csname res@bestalmcc.full.name\endcsname{Qwen2.5-Omni-3B + CC}
\expandafter\def\csname res@bestalmcc.subset.f1\endcsname{0.299}
\expandafter\def\csname res@bestalmcc.subset.gap\endcsname{0.084}
\expandafter\def\csname res@bestalmcc.subset.gapci\endcsname{[0.064, 0.111]}
\expandafter\def\csname res@bestalmcc.subset.name\endcsname{Qwen2.5-Omni-3B + CC}
\expandafter\def\csname res@clap_laion.full.delta\endcsname{-0.308}
\expandafter\def\csname res@clap_laion.full.deltaci\endcsname{[-0.328, -0.287]}
\expandafter\def\csname res@clap_laion.full.deltaoff\endcsname{-0.325}
\expandafter\def\csname res@clap_laion.full.deltaoffci\endcsname{[-0.351, -0.299]}
\expandafter\def\csname res@clap_laion.full.ece\endcsname{0.584}
\expandafter\def\csname res@clap_laion.full.ecev\endcsname{0.576}
\expandafter\def\csname res@clap_laion.full.ecevoracle\endcsname{0.041}
\expandafter\def\csname res@clap_laion.full.f1\endcsname{0.074}
\expandafter\def\csname res@clap_laion.full.f1ci\endcsname{[0.065, 0.085]}
\expandafter\def\csname res@clap_laion.full.f1off\endcsname{0.076}
\expandafter\def\csname res@clap_laion.full.f1offci\endcsname{[0.066, 0.086]}
\expandafter\def\csname res@clap_laion.full.gap\endcsname{0.308}
\expandafter\def\csname res@clap_laion.full.gapci\endcsname{[0.287, 0.328]}
\expandafter\def\csname res@clap_laion.full.ll\endcsname{4.069}
\expandafter\def\csname res@clap_laion.full.lloracle\endcsname{2.045}
\expandafter\def\csname res@clap_laion.full.toracle\endcsname{10.19}
\expandafter\def\csname res@clap_laion.subset.delta\endcsname{-0.306}
\expandafter\def\csname res@clap_laion.subset.deltaci\endcsname{[-0.333, -0.281]}
\expandafter\def\csname res@clap_laion.subset.deltaoff\endcsname{-0.313}
\expandafter\def\csname res@clap_laion.subset.deltaoffci\endcsname{[-0.348, -0.282]}
\expandafter\def\csname res@clap_laion.subset.ece\endcsname{0.581}
\expandafter\def\csname res@clap_laion.subset.ecev\endcsname{0.573}
\expandafter\def\csname res@clap_laion.subset.ecevoracle\endcsname{0.039}
\expandafter\def\csname res@clap_laion.subset.f1\endcsname{0.077}
\expandafter\def\csname res@clap_laion.subset.f1ci\endcsname{[0.066, 0.089]}
\expandafter\def\csname res@clap_laion.subset.f1off\endcsname{0.081}
\expandafter\def\csname res@clap_laion.subset.f1offci\endcsname{[0.068, 0.095]}
\expandafter\def\csname res@clap_laion.subset.gap\endcsname{0.306}
\expandafter\def\csname res@clap_laion.subset.gapci\endcsname{[0.281, 0.333]}
\expandafter\def\csname res@clap_laion.subset.ll\endcsname{4.085}
\expandafter\def\csname res@clap_laion.subset.lloracle\endcsname{2.046}
\expandafter\def\csname res@clap_laion.subset.toracle\endcsname{10.45}
\expandafter\def\csname res@clap_laion_desc.full.delta\endcsname{-0.287}
\expandafter\def\csname res@clap_laion_desc.full.deltaci\endcsname{[-0.306, -0.264]}
\expandafter\def\csname res@clap_laion_desc.full.deltaoff\endcsname{-0.300}
\expandafter\def\csname res@clap_laion_desc.full.deltaoffci\endcsname{[-0.327, -0.272]}
\expandafter\def\csname res@clap_laion_desc.full.ece\endcsname{0.440}
\expandafter\def\csname res@clap_laion_desc.full.ecev\endcsname{0.417}
\expandafter\def\csname res@clap_laion_desc.full.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@clap_laion_desc.full.f1\endcsname{0.095}
\expandafter\def\csname res@clap_laion_desc.full.f1ci\endcsname{[0.085, 0.106]}
\expandafter\def\csname res@clap_laion_desc.full.f1off\endcsname{0.101}
\expandafter\def\csname res@clap_laion_desc.full.f1offci\endcsname{[0.090, 0.112]}
\expandafter\def\csname res@clap_laion_desc.full.gap\endcsname{0.287}
\expandafter\def\csname res@clap_laion_desc.full.gapci\endcsname{[0.264, 0.306]}
\expandafter\def\csname res@clap_laion_desc.full.ll\endcsname{3.071}
\expandafter\def\csname res@clap_laion_desc.full.lloracle\endcsname{2.002}
\expandafter\def\csname res@clap_laion_desc.full.toracle\endcsname{5.35}
\expandafter\def\csname res@clap_laion_desc.subset.delta\endcsname{-0.284}
\expandafter\def\csname res@clap_laion_desc.subset.deltaci\endcsname{[-0.315, -0.255]}
\expandafter\def\csname res@clap_laion_desc.subset.deltaoff\endcsname{-0.288}
\expandafter\def\csname res@clap_laion_desc.subset.deltaoffci\endcsname{[-0.326, -0.251]}
\expandafter\def\csname res@clap_laion_desc.subset.ece\endcsname{0.437}
\expandafter\def\csname res@clap_laion_desc.subset.ecev\endcsname{0.414}
\expandafter\def\csname res@clap_laion_desc.subset.ecevoracle\endcsname{0.010}
\expandafter\def\csname res@clap_laion_desc.subset.f1\endcsname{0.099}
\expandafter\def\csname res@clap_laion_desc.subset.f1ci\endcsname{[0.086, 0.113]}
\expandafter\def\csname res@clap_laion_desc.subset.f1off\endcsname{0.106}
\expandafter\def\csname res@clap_laion_desc.subset.f1offci\endcsname{[0.091, 0.122]}
\expandafter\def\csname res@clap_laion_desc.subset.gap\endcsname{0.284}
\expandafter\def\csname res@clap_laion_desc.subset.gapci\endcsname{[0.255, 0.315]}
\expandafter\def\csname res@clap_laion_desc.subset.ll\endcsname{3.095}
\expandafter\def\csname res@clap_laion_desc.subset.lloracle\endcsname{2.003}
\expandafter\def\csname res@clap_laion_desc.subset.toracle\endcsname{5.43}
\expandafter\def\csname res@clap_mlp.full.ccc.arousal\endcsname{0.60}
\expandafter\def\csname res@clap_mlp.full.ccc.dominance\endcsname{0.48}
\expandafter\def\csname res@clap_mlp.full.ccc.valence\endcsname{0.46}
\expandafter\def\csname res@clap_mlp.full.delta\endcsname{-0.128}
\expandafter\def\csname res@clap_mlp.full.deltaci\endcsname{[-0.146, -0.114]}
\expandafter\def\csname res@clap_mlp.full.deltaoff\endcsname{-0.141}
\expandafter\def\csname res@clap_mlp.full.deltaoffci\endcsname{[-0.163, -0.125]}
\expandafter\def\csname res@clap_mlp.full.ece\endcsname{0.028}
\expandafter\def\csname res@clap_mlp.full.ecev\endcsname{0.031}
\expandafter\def\csname res@clap_mlp.full.ecevoracle\endcsname{0.011}
\expandafter\def\csname res@clap_mlp.full.f1\endcsname{0.254}
\expandafter\def\csname res@clap_mlp.full.f1ci\endcsname{[0.239, 0.270]}
\expandafter\def\csname res@clap_mlp.full.f1off\endcsname{0.261}
\expandafter\def\csname res@clap_mlp.full.f1offci\endcsname{[0.242, 0.279]}
\expandafter\def\csname res@clap_mlp.full.gap\endcsname{0.128}
\expandafter\def\csname res@clap_mlp.full.gapci\endcsname{[0.114, 0.146]}
\expandafter\def\csname res@clap_mlp.full.ll\endcsname{1.673}
\expandafter\def\csname res@clap_mlp.full.lloracle\endcsname{1.665}
\expandafter\def\csname res@clap_mlp.full.toracle\endcsname{1.16}
\expandafter\def\csname res@clap_mlp.subset.ccc.arousal\endcsname{0.61}
\expandafter\def\csname res@clap_mlp.subset.ccc.dominance\endcsname{0.50}
\expandafter\def\csname res@clap_mlp.subset.ccc.valence\endcsname{0.46}
\expandafter\def\csname res@clap_mlp.subset.delta\endcsname{-0.124}
\expandafter\def\csname res@clap_mlp.subset.deltaci\endcsname{[-0.152, -0.101]}
\expandafter\def\csname res@clap_mlp.subset.deltaoff\endcsname{-0.132}
\expandafter\def\csname res@clap_mlp.subset.deltaoffci\endcsname{[-0.164, -0.105]}
\expandafter\def\csname res@clap_mlp.subset.ece\endcsname{0.022}
\expandafter\def\csname res@clap_mlp.subset.ecev\endcsname{0.031}
\expandafter\def\csname res@clap_mlp.subset.ecevoracle\endcsname{0.012}
\expandafter\def\csname res@clap_mlp.subset.f1\endcsname{0.259}
\expandafter\def\csname res@clap_mlp.subset.f1ci\endcsname{[0.240, 0.277]}
\expandafter\def\csname res@clap_mlp.subset.f1off\endcsname{0.262}
\expandafter\def\csname res@clap_mlp.subset.f1offci\endcsname{[0.239, 0.290]}
\expandafter\def\csname res@clap_mlp.subset.gap\endcsname{0.124}
\expandafter\def\csname res@clap_mlp.subset.gapci\endcsname{[0.101, 0.152]}
\expandafter\def\csname res@clap_mlp.subset.ll\endcsname{1.672}
\expandafter\def\csname res@clap_mlp.subset.lloracle\endcsname{1.663}
\expandafter\def\csname res@clap_mlp.subset.toracle\endcsname{1.17}
\expandafter\def\csname res@clap_ms.full.delta\endcsname{-0.267}
\expandafter\def\csname res@clap_ms.full.deltaci\endcsname{[-0.290, -0.244]}
\expandafter\def\csname res@clap_ms.full.deltaoff\endcsname{-0.267}
\expandafter\def\csname res@clap_ms.full.deltaoffci\endcsname{[-0.296, -0.242]}
\expandafter\def\csname res@clap_ms.full.ece\endcsname{0.303}
\expandafter\def\csname res@clap_ms.full.ecev\endcsname{0.279}
\expandafter\def\csname res@clap_ms.full.ecevoracle\endcsname{0.019}
\expandafter\def\csname res@clap_ms.full.f1\endcsname{0.115}
\expandafter\def\csname res@clap_ms.full.f1ci\endcsname{[0.106, 0.122]}
\expandafter\def\csname res@clap_ms.full.f1off\endcsname{0.134}
\expandafter\def\csname res@clap_ms.full.f1offci\endcsname{[0.123, 0.143]}
\expandafter\def\csname res@clap_ms.full.gap\endcsname{0.267}
\expandafter\def\csname res@clap_ms.full.gapci\endcsname{[0.244, 0.290]}
\expandafter\def\csname res@clap_ms.full.ll\endcsname{2.241}
\expandafter\def\csname res@clap_ms.full.lloracle\endcsname{1.867}
\expandafter\def\csname res@clap_ms.full.toracle\endcsname{2.61}
\expandafter\def\csname res@clap_ms.subset.delta\endcsname{-0.271}
\expandafter\def\csname res@clap_ms.subset.deltaci\endcsname{[-0.299, -0.246]}
\expandafter\def\csname res@clap_ms.subset.deltaoff\endcsname{-0.260}
\expandafter\def\csname res@clap_ms.subset.deltaoffci\endcsname{[-0.293, -0.233]}
\expandafter\def\csname res@clap_ms.subset.ece\endcsname{0.314}
\expandafter\def\csname res@clap_ms.subset.ecev\endcsname{0.285}
\expandafter\def\csname res@clap_ms.subset.ecevoracle\endcsname{0.021}
\expandafter\def\csname res@clap_ms.subset.f1\endcsname{0.112}
\expandafter\def\csname res@clap_ms.subset.f1ci\endcsname{[0.099, 0.124]}
\expandafter\def\csname res@clap_ms.subset.f1off\endcsname{0.134}
\expandafter\def\csname res@clap_ms.subset.f1offci\endcsname{[0.117, 0.149]}
\expandafter\def\csname res@clap_ms.subset.gap\endcsname{0.271}
\expandafter\def\csname res@clap_ms.subset.gapci\endcsname{[0.246, 0.299]}
\expandafter\def\csname res@clap_ms.subset.ll\endcsname{2.264}
\expandafter\def\csname res@clap_ms.subset.lloracle\endcsname{1.876}
\expandafter\def\csname res@clap_ms.subset.toracle\endcsname{2.66}
\expandafter\def\csname res@clap_ms_desc.full.delta\endcsname{-0.356}
\expandafter\def\csname res@clap_ms_desc.full.deltaci\endcsname{[-0.385, -0.330]}
\expandafter\def\csname res@clap_ms_desc.full.deltaoff\endcsname{-0.372}
\expandafter\def\csname res@clap_ms_desc.full.deltaoffci\endcsname{[-0.409, -0.340]}
\expandafter\def\csname res@clap_ms_desc.full.ece\endcsname{0.701}
\expandafter\def\csname res@clap_ms_desc.full.ecev\endcsname{0.692}
\expandafter\def\csname res@clap_ms_desc.full.ecevoracle\endcsname{0.098}
\expandafter\def\csname res@clap_ms_desc.full.f1\endcsname{0.026}
\expandafter\def\csname res@clap_ms_desc.full.f1ci\endcsname{[0.015, 0.041]}
\expandafter\def\csname res@clap_ms_desc.full.f1off\endcsname{0.029}
\expandafter\def\csname res@clap_ms_desc.full.f1offci\endcsname{[0.016, 0.046]}
\expandafter\def\csname res@clap_ms_desc.full.gap\endcsname{0.356}
\expandafter\def\csname res@clap_ms_desc.full.gapci\endcsname{[0.330, 0.385]}
\expandafter\def\csname res@clap_ms_desc.full.ll\endcsname{3.526}
\expandafter\def\csname res@clap_ms_desc.full.lloracle\endcsname{2.085}
\expandafter\def\csname res@clap_ms_desc.full.toracle\endcsname{20.00}
\expandafter\def\csname res@clap_ms_desc.subset.delta\endcsname{-0.354}
\expandafter\def\csname res@clap_ms_desc.subset.deltaci\endcsname{[-0.386, -0.325]}
\expandafter\def\csname res@clap_ms_desc.subset.deltaoff\endcsname{-0.362}
\expandafter\def\csname res@clap_ms_desc.subset.deltaoffci\endcsname{[-0.402, -0.328]}
\expandafter\def\csname res@clap_ms_desc.subset.ece\endcsname{0.701}
\expandafter\def\csname res@clap_ms_desc.subset.ecev\endcsname{0.694}
\expandafter\def\csname res@clap_ms_desc.subset.ecevoracle\endcsname{0.095}
\expandafter\def\csname res@clap_ms_desc.subset.f1\endcsname{0.029}
\expandafter\def\csname res@clap_ms_desc.subset.f1ci\endcsname{[0.015, 0.045]}
\expandafter\def\csname res@clap_ms_desc.subset.f1off\endcsname{0.032}
\expandafter\def\csname res@clap_ms_desc.subset.f1offci\endcsname{[0.017, 0.051]}
\expandafter\def\csname res@clap_ms_desc.subset.gap\endcsname{0.354}
\expandafter\def\csname res@clap_ms_desc.subset.gapci\endcsname{[0.325, 0.386]}
\expandafter\def\csname res@clap_ms_desc.subset.ll\endcsname{3.532}
\expandafter\def\csname res@clap_ms_desc.subset.lloracle\endcsname{2.085}
\expandafter\def\csname res@clap_ms_desc.subset.toracle\endcsname{20.00}
\expandafter\def\csname res@clap_para.full.delta\endcsname{-0.108}
\expandafter\def\csname res@clap_para.full.deltaci\endcsname{[-0.127, -0.094]}
\expandafter\def\csname res@clap_para.full.deltaoff\endcsname{-0.116}
\expandafter\def\csname res@clap_para.full.deltaoffci\endcsname{[-0.136, -0.103]}
\expandafter\def\csname res@clap_para.full.ece\endcsname{0.265}
\expandafter\def\csname res@clap_para.full.ecev\endcsname{0.195}
\expandafter\def\csname res@clap_para.full.ecevoracle\endcsname{0.063}
\expandafter\def\csname res@clap_para.full.f1\endcsname{0.274}
\expandafter\def\csname res@clap_para.full.f1ci\endcsname{[0.257, 0.289]}
\expandafter\def\csname res@clap_para.full.f1off\endcsname{0.286}
\expandafter\def\csname res@clap_para.full.f1offci\endcsname{[0.263, 0.307]}
\expandafter\def\csname res@clap_para.full.gap\endcsname{0.108}
\expandafter\def\csname res@clap_para.full.gapci\endcsname{[0.094, 0.127]}
\expandafter\def\csname res@clap_para.full.ll\endcsname{2.021}
\expandafter\def\csname res@clap_para.full.lloracle\endcsname{1.885}
\expandafter\def\csname res@clap_para.full.toracle\endcsname{0.16}
\expandafter\def\csname res@clap_para.subset.delta\endcsname{-0.099}
\expandafter\def\csname res@clap_para.subset.deltaci\endcsname{[-0.127, -0.076]}
\expandafter\def\csname res@clap_para.subset.deltaoff\endcsname{-0.098}
\expandafter\def\csname res@clap_para.subset.deltaoffci\endcsname{[-0.129, -0.071]}
\expandafter\def\csname res@clap_para.subset.ece\endcsname{0.274}
\expandafter\def\csname res@clap_para.subset.ecev\endcsname{0.197}
\expandafter\def\csname res@clap_para.subset.ecevoracle\endcsname{0.065}
\expandafter\def\csname res@clap_para.subset.f1\endcsname{0.284}
\expandafter\def\csname res@clap_para.subset.f1ci\endcsname{[0.264, 0.306]}
\expandafter\def\csname res@clap_para.subset.f1off\endcsname{0.296}
\expandafter\def\csname res@clap_para.subset.f1offci\endcsname{[0.272, 0.322]}
\expandafter\def\csname res@clap_para.subset.gap\endcsname{0.099}
\expandafter\def\csname res@clap_para.subset.gapci\endcsname{[0.076, 0.127]}
\expandafter\def\csname res@clap_para.subset.ll\endcsname{2.021}
\expandafter\def\csname res@clap_para.subset.lloracle\endcsname{1.886}
\expandafter\def\csname res@clap_para.subset.toracle\endcsname{0.16}
\expandafter\def\csname res@clap_para_desc.full.delta\endcsname{-0.143}
\expandafter\def\csname res@clap_para_desc.full.deltaci\endcsname{[-0.158, -0.131]}
\expandafter\def\csname res@clap_para_desc.full.deltaoff\endcsname{-0.152}
\expandafter\def\csname res@clap_para_desc.full.deltaoffci\endcsname{[-0.175, -0.138]}
\expandafter\def\csname res@clap_para_desc.full.ece\endcsname{0.221}
\expandafter\def\csname res@clap_para_desc.full.ecev\endcsname{0.165}
\expandafter\def\csname res@clap_para_desc.full.ecevoracle\endcsname{0.058}
\expandafter\def\csname res@clap_para_desc.full.f1\endcsname{0.239}
\expandafter\def\csname res@clap_para_desc.full.f1ci\endcsname{[0.218, 0.257]}
\expandafter\def\csname res@clap_para_desc.full.f1off\endcsname{0.249}
\expandafter\def\csname res@clap_para_desc.full.f1offci\endcsname{[0.226, 0.267]}
\expandafter\def\csname res@clap_para_desc.full.gap\endcsname{0.143}
\expandafter\def\csname res@clap_para_desc.full.gapci\endcsname{[0.131, 0.158]}
\expandafter\def\csname res@clap_para_desc.full.ll\endcsname{2.043}
\expandafter\def\csname res@clap_para_desc.full.lloracle\endcsname{1.949}
\expandafter\def\csname res@clap_para_desc.full.toracle\endcsname{0.15}
\expandafter\def\csname res@clap_para_desc.subset.delta\endcsname{-0.153}
\expandafter\def\csname res@clap_para_desc.subset.deltaci\endcsname{[-0.180, -0.130]}
\expandafter\def\csname res@clap_para_desc.subset.deltaoff\endcsname{-0.150}
\expandafter\def\csname res@clap_para_desc.subset.deltaoffci\endcsname{[-0.185, -0.121]}
\expandafter\def\csname res@clap_para_desc.subset.ece\endcsname{0.213}
\expandafter\def\csname res@clap_para_desc.subset.ecev\endcsname{0.161}
\expandafter\def\csname res@clap_para_desc.subset.ecevoracle\endcsname{0.056}
\expandafter\def\csname res@clap_para_desc.subset.f1\endcsname{0.230}
\expandafter\def\csname res@clap_para_desc.subset.f1ci\endcsname{[0.212, 0.246]}
\expandafter\def\csname res@clap_para_desc.subset.f1off\endcsname{0.244}
\expandafter\def\csname res@clap_para_desc.subset.f1offci\endcsname{[0.226, 0.261]}
\expandafter\def\csname res@clap_para_desc.subset.gap\endcsname{0.153}
\expandafter\def\csname res@clap_para_desc.subset.gapci\endcsname{[0.130, 0.180]}
\expandafter\def\csname res@clap_para_desc.subset.ll\endcsname{2.044}
\expandafter\def\csname res@clap_para_desc.subset.lloracle\endcsname{1.953}
\expandafter\def\csname res@clap_para_desc.subset.toracle\endcsname{0.15}
\expandafter\def\csname res@deepser.full.delta\endcsname{+0.022}
\expandafter\def\csname res@deepser.full.deltaci\endcsname{[+0.015, +0.028]}
\expandafter\def\csname res@deepser.full.deltaoff\endcsname{+0.025}
\expandafter\def\csname res@deepser.full.deltaoffci\endcsname{[+0.017, +0.033]}
\expandafter\def\csname res@deepser.full.ece\endcsname{0.118}
\expandafter\def\csname res@deepser.full.ecev\endcsname{0.021}
\expandafter\def\csname res@deepser.full.ecevoracle\endcsname{0.032}
\expandafter\def\csname res@deepser.full.f1\endcsname{0.404}
\expandafter\def\csname res@deepser.full.f1ci\endcsname{[0.377, 0.427]}
\expandafter\def\csname res@deepser.full.f1off\endcsname{0.427}
\expandafter\def\csname res@deepser.full.f1offci\endcsname{[0.394, 0.456]}
\expandafter\def\csname res@deepser.full.gap\endcsname{-0.022}
\expandafter\def\csname res@deepser.full.gapci\endcsname{[-0.028, -0.015]}
\expandafter\def\csname res@deepser.full.ll\endcsname{1.542}
\expandafter\def\csname res@deepser.full.lloracle\endcsname{1.541}
\expandafter\def\csname res@deepser.full.toracle\endcsname{1.05}
\expandafter\def\csname res@deepser.subset.delta\endcsname{+0.017}
\expandafter\def\csname res@deepser.subset.deltaci\endcsname{[-0.001, +0.036]}
\expandafter\def\csname res@deepser.subset.deltaoff\endcsname{+0.026}
\expandafter\def\csname res@deepser.subset.deltaoffci\endcsname{[+0.006, +0.048]}
\expandafter\def\csname res@deepser.subset.ece\endcsname{0.118}
\expandafter\def\csname res@deepser.subset.ecev\endcsname{0.025}
\expandafter\def\csname res@deepser.subset.ecevoracle\endcsname{0.033}
\expandafter\def\csname res@deepser.subset.f1\endcsname{0.400}
\expandafter\def\csname res@deepser.subset.f1ci\endcsname{[0.369, 0.429]}
\expandafter\def\csname res@deepser.subset.f1off\endcsname{0.420}
\expandafter\def\csname res@deepser.subset.f1offci\endcsname{[0.380, 0.457]}
\expandafter\def\csname res@deepser.subset.gap\endcsname{-0.017}
\expandafter\def\csname res@deepser.subset.gapci\endcsname{[-0.036, 0.001]}
\expandafter\def\csname res@deepser.subset.ll\endcsname{1.544}
\expandafter\def\csname res@deepser.subset.lloracle\endcsname{1.542}
\expandafter\def\csname res@deepser.subset.toracle\endcsname{1.05}
\expandafter\def\csname res@e2v.full.delta\endcsname{-0.150}
\expandafter\def\csname res@e2v.full.deltaci\endcsname{[-0.165, -0.138]}
\expandafter\def\csname res@e2v.full.deltaoff\endcsname{-0.136}
\expandafter\def\csname res@e2v.full.deltaoffci\endcsname{[-0.151, -0.124]}
\expandafter\def\csname res@e2v.full.ece\endcsname{0.444}
\expandafter\def\csname res@e2v.full.ecev\endcsname{0.477}
\expandafter\def\csname res@e2v.full.ecevoracle\endcsname{0.044}
\expandafter\def\csname res@e2v.full.f1\endcsname{0.232}
\expandafter\def\csname res@e2v.full.f1ci\endcsname{[0.213, 0.249]}
\expandafter\def\csname res@e2v.full.f1off\endcsname{0.265}
\expandafter\def\csname res@e2v.full.f1offci\endcsname{[0.239, 0.290]}
\expandafter\def\csname res@e2v.full.gap\endcsname{0.150}
\expandafter\def\csname res@e2v.full.gapci\endcsname{[0.138, 0.165]}
\expandafter\def\csname res@e2v.full.ll\endcsname{4.437}
\expandafter\def\csname res@e2v.full.lloracle\endcsname{1.845}
\expandafter\def\csname res@e2v.full.toracle\endcsname{6.11}
\expandafter\def\csname res@e2v.subset.delta\endcsname{-0.149}
\expandafter\def\csname res@e2v.subset.deltaci\endcsname{[-0.175, -0.126]}
\expandafter\def\csname res@e2v.subset.deltaoff\endcsname{-0.120}
\expandafter\def\csname res@e2v.subset.deltaoffci\endcsname{[-0.144, -0.100]}
\expandafter\def\csname res@e2v.subset.ece\endcsname{0.443}
\expandafter\def\csname res@e2v.subset.ecev\endcsname{0.469}
\expandafter\def\csname res@e2v.subset.ecevoracle\endcsname{0.050}
\expandafter\def\csname res@e2v.subset.f1\endcsname{0.235}
\expandafter\def\csname res@e2v.subset.f1ci\endcsname{[0.211, 0.255]}
\expandafter\def\csname res@e2v.subset.f1off\endcsname{0.274}
\expandafter\def\csname res@e2v.subset.f1offci\endcsname{[0.241, 0.306]}
\expandafter\def\csname res@e2v.subset.gap\endcsname{0.149}
\expandafter\def\csname res@e2v.subset.gapci\endcsname{[0.126, 0.175]}
\expandafter\def\csname res@e2v.subset.ll\endcsname{4.361}
\expandafter\def\csname res@e2v.subset.lloracle\endcsname{1.831}
\expandafter\def\csname res@e2v.subset.toracle\endcsname{5.95}
\expandafter\def\csname res@ears.af3.acc\endcsname{0.097}
\expandafter\def\csname res@ears.af3.aucknown\endcsname{0.457}
\expandafter\def\csname res@ears.af3.aucnew\endcsname{0.542}
\expandafter\def\csname res@ears.af3.aucprimary\endcsname{0.435}
\expandafter\def\csname res@ears.af3.aucsecondary\endcsname{0.478}
\expandafter\def\csname res@ears.af3.f1\endcsname{0.077}
\expandafter\def\csname res@ears.af3.f1ci\endcsname{[0.070, 0.084]}
\expandafter\def\csname res@ears.af3.f1known\endcsname{0.069}
\expandafter\def\csname res@ears.af3.f1new\endcsname{0.083}
\expandafter\def\csname res@ears.af3.f1pm\endcsname{0.093}
\expandafter\def\csname res@ears.af3.f1primary\endcsname{0.086}
\expandafter\def\csname res@ears.af3.f1secondary\endcsname{0.052}
\expandafter\def\csname res@ears.af3.gap\endcsname{+0.139}
\expandafter\def\csname res@ears.af3.gapci\endcsname{[+0.125, +0.153]}
\expandafter\def\csname res@ears.af3_cc.acc\endcsname{0.109}
\expandafter\def\csname res@ears.af3_cc.aucknown\endcsname{0.467}
\expandafter\def\csname res@ears.af3_cc.aucnew\endcsname{0.552}
\expandafter\def\csname res@ears.af3_cc.aucprimary\endcsname{0.466}
\expandafter\def\csname res@ears.af3_cc.aucsecondary\endcsname{0.468}
\expandafter\def\csname res@ears.af3_cc.f1\endcsname{0.102}
\expandafter\def\csname res@ears.af3_cc.f1ci\endcsname{[0.095, 0.109]}
\expandafter\def\csname res@ears.af3_cc.f1known\endcsname{0.074}
\expandafter\def\csname res@ears.af3_cc.f1new\endcsname{0.124}
\expandafter\def\csname res@ears.af3_cc.f1pm\endcsname{0.103}
\expandafter\def\csname res@ears.af3_cc.f1primary\endcsname{0.102}
\expandafter\def\csname res@ears.af3_cc.f1secondary\endcsname{0.046}
\expandafter\def\csname res@ears.af3_cc.gap\endcsname{+0.114}
\expandafter\def\csname res@ears.af3_cc.gapci\endcsname{[+0.098, +0.129]}
\expandafter\def\csname res@ears.asom.acc\endcsname{0.296}
\expandafter\def\csname res@ears.asom.aucknown\endcsname{0.866}
\expandafter\def\csname res@ears.asom.aucnew\endcsname{0.785}
\expandafter\def\csname res@ears.asom.aucprimary\endcsname{0.963}
\expandafter\def\csname res@ears.asom.aucsecondary\endcsname{0.769}
\expandafter\def\csname res@ears.asom.f1\endcsname{0.216}
\expandafter\def\csname res@ears.asom.f1ci\endcsname{[0.203, 0.229]}
\expandafter\def\csname res@ears.asom.f1known\endcsname{0.264}
\expandafter\def\csname res@ears.asom.f1new\endcsname{0.182}
\expandafter\def\csname res@ears.asom.f1pm\endcsname{0.386}
\expandafter\def\csname res@ears.asom.f1primary\endcsname{0.528}
\expandafter\def\csname res@ears.asom.f1secondary\endcsname{0.000}
\expandafter\def\csname res@ears.asom_30s.acc\endcsname{0.295}
\expandafter\def\csname res@ears.asom_30s.aucknown\endcsname{0.868}
\expandafter\def\csname res@ears.asom_30s.aucnew\endcsname{0.787}
\expandafter\def\csname res@ears.asom_30s.aucprimary\endcsname{0.963}
\expandafter\def\csname res@ears.asom_30s.aucsecondary\endcsname{0.772}
\expandafter\def\csname res@ears.asom_30s.f1\endcsname{0.214}
\expandafter\def\csname res@ears.asom_30s.f1ci\endcsname{[0.201, 0.226]}
\expandafter\def\csname res@ears.asom_30s.f1known\endcsname{0.267}
\expandafter\def\csname res@ears.asom_30s.f1new\endcsname{0.176}
\expandafter\def\csname res@ears.asom_30s.f1pm\endcsname{0.392}
\expandafter\def\csname res@ears.asom_30s.f1primary\endcsname{0.534}
\expandafter\def\csname res@ears.asom_30s.f1secondary\endcsname{0.000}
\expandafter\def\csname res@ears.asom_30s.gap\endcsname{+0.002}
\expandafter\def\csname res@ears.asom_30s.gapci\endcsname{[-0.003, +0.007]}
\expandafter\def\csname res@ears.asom_cc.acc\endcsname{0.318}
\expandafter\def\csname res@ears.asom_cc.aucknown\endcsname{0.883}
\expandafter\def\csname res@ears.asom_cc.aucnew\endcsname{0.763}
\expandafter\def\csname res@ears.asom_cc.aucprimary\endcsname{0.962}
\expandafter\def\csname res@ears.asom_cc.aucsecondary\endcsname{0.805}
\expandafter\def\csname res@ears.asom_cc.f1\endcsname{0.257}
\expandafter\def\csname res@ears.asom_cc.f1ci\endcsname{[0.246, 0.268]}
\expandafter\def\csname res@ears.asom_cc.f1known\endcsname{0.263}
\expandafter\def\csname res@ears.asom_cc.f1new\endcsname{0.255}
\expandafter\def\csname res@ears.asom_cc.f1pm\endcsname{0.386}
\expandafter\def\csname res@ears.asom_cc.f1primary\endcsname{0.464}
\expandafter\def\csname res@ears.asom_cc.f1secondary\endcsname{0.063}
\expandafter\def\csname res@ears.asom_cc.gap\endcsname{-0.041}
\expandafter\def\csname res@ears.asom_cc.gapci\endcsname{[-0.056, -0.026]}
\expandafter\def\csname res@ears.asom_em.acc\endcsname{0.193}
\expandafter\def\csname res@ears.asom_em.aucknown\endcsname{0.813}
\expandafter\def\csname res@ears.asom_em.aucnew\endcsname{0.749}
\expandafter\def\csname res@ears.asom_em.aucprimary\endcsname{0.937}
\expandafter\def\csname res@ears.asom_em.aucsecondary\endcsname{0.690}
\expandafter\def\csname res@ears.asom_em.f1\endcsname{0.091}
\expandafter\def\csname res@ears.asom_em.f1ci\endcsname{[0.085, 0.097]}
\expandafter\def\csname res@ears.asom_em.f1known\endcsname{0.106}
\expandafter\def\csname res@ears.asom_em.f1new\endcsname{0.082}
\expandafter\def\csname res@ears.asom_em.f1pm\endcsname{0.145}
\expandafter\def\csname res@ears.asom_em.f1primary\endcsname{0.212}
\expandafter\def\csname res@ears.asom_em.f1secondary\endcsname{0.000}
\expandafter\def\csname res@ears.asom_em.gap\endcsname{+0.125}
\expandafter\def\csname res@ears.asom_em.gapci\endcsname{[+0.115, +0.135]}
\expandafter\def\csname res@ears.asom_u.acc\endcsname{0.325}
\expandafter\def\csname res@ears.asom_u.aucknown\endcsname{0.871}
\expandafter\def\csname res@ears.asom_u.aucnew\endcsname{0.784}
\expandafter\def\csname res@ears.asom_u.aucprimary\endcsname{0.964}
\expandafter\def\csname res@ears.asom_u.aucsecondary\endcsname{0.778}
\expandafter\def\csname res@ears.asom_u.f1\endcsname{0.255}
\expandafter\def\csname res@ears.asom_u.f1ci\endcsname{[0.241, 0.270]}
\expandafter\def\csname res@ears.asom_u.f1known\endcsname{0.303}
\expandafter\def\csname res@ears.asom_u.f1new\endcsname{0.221}
\expandafter\def\csname res@ears.asom_u.f1pm\endcsname{0.389}
\expandafter\def\csname res@ears.asom_u.f1primary\endcsname{0.607}
\expandafter\def\csname res@ears.asom_u.f1secondary\endcsname{0.000}
\expandafter\def\csname res@ears.asom_u.gap\endcsname{-0.039}
\expandafter\def\csname res@ears.asom_u.gapci\endcsname{[-0.046, -0.033]}
\expandafter\def\csname res@ears.asom_v2sp.acc\endcsname{0.305}
\expandafter\def\csname res@ears.asom_v2sp.aucknown\endcsname{0.850}
\expandafter\def\csname res@ears.asom_v2sp.aucnew\endcsname{0.771}
\expandafter\def\csname res@ears.asom_v2sp.aucprimary\endcsname{0.962}
\expandafter\def\csname res@ears.asom_v2sp.aucsecondary\endcsname{0.739}
\expandafter\def\csname res@ears.asom_v2sp.f1\endcsname{0.246}
\expandafter\def\csname res@ears.asom_v2sp.f1ci\endcsname{[0.230, 0.260]}
\expandafter\def\csname res@ears.asom_v2sp.f1known\endcsname{0.280}
\expandafter\def\csname res@ears.asom_v2sp.f1new\endcsname{0.219}
\expandafter\def\csname res@ears.asom_v2sp.f1pm\endcsname{0.356}
\expandafter\def\csname res@ears.asom_v2sp.f1primary\endcsname{0.506}
\expandafter\def\csname res@ears.asom_v2sp.f1secondary\endcsname{0.055}
\expandafter\def\csname res@ears.asom_v2sp.gap\endcsname{-0.030}
\expandafter\def\csname res@ears.asom_v2sp.gapci\endcsname{[-0.039, -0.020]}
\expandafter\def\csname res@ears.asom_v2sp_em.acc\endcsname{0.166}
\expandafter\def\csname res@ears.asom_v2sp_em.aucknown\endcsname{0.793}
\expandafter\def\csname res@ears.asom_v2sp_em.aucnew\endcsname{0.710}
\expandafter\def\csname res@ears.asom_v2sp_em.aucprimary\endcsname{0.940}
\expandafter\def\csname res@ears.asom_v2sp_em.aucsecondary\endcsname{0.646}
\expandafter\def\csname res@ears.asom_v2sp_em.f1\endcsname{0.073}
\expandafter\def\csname res@ears.asom_v2sp_em.f1ci\endcsname{[0.068, 0.079]}
\expandafter\def\csname res@ears.asom_v2sp_em.f1known\endcsname{0.054}
\expandafter\def\csname res@ears.asom_v2sp_em.f1new\endcsname{0.090}
\expandafter\def\csname res@ears.asom_v2sp_em.f1pm\endcsname{0.189}
\expandafter\def\csname res@ears.asom_v2sp_em.f1primary\endcsname{0.107}
\expandafter\def\csname res@ears.asom_v2sp_em.f1secondary\endcsname{0.000}
\expandafter\def\csname res@ears.asom_v2sp_em.gap\endcsname{+0.142}
\expandafter\def\csname res@ears.asom_v2sp_em.gapci\endcsname{[+0.131, +0.155]}
\expandafter\def\csname res@ears.asom_v2sp_s43.acc\endcsname{0.308}
\expandafter\def\csname res@ears.asom_v2sp_s43.aucknown\endcsname{0.833}
\expandafter\def\csname res@ears.asom_v2sp_s43.aucnew\endcsname{0.773}
\expandafter\def\csname res@ears.asom_v2sp_s43.aucprimary\endcsname{0.956}
\expandafter\def\csname res@ears.asom_v2sp_s43.aucsecondary\endcsname{0.711}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1\endcsname{0.252}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1ci\endcsname{[0.236, 0.266]}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1known\endcsname{0.282}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1new\endcsname{0.229}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1pm\endcsname{0.357}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1primary\endcsname{0.526}
\expandafter\def\csname res@ears.asom_v2sp_s43.f1secondary\endcsname{0.038}
\expandafter\def\csname res@ears.asom_v2sp_s43.gap\endcsname{-0.036}
\expandafter\def\csname res@ears.asom_v2sp_s43.gapci\endcsname{[-0.046, -0.024]}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.acc\endcsname{0.330}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.aucknown\endcsname{0.838}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.aucnew\endcsname{0.772}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.aucprimary\endcsname{0.956}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.aucsecondary\endcsname{0.719}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1\endcsname{0.282}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1ci\endcsname{[0.266, 0.296]}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1known\endcsname{0.320}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1new\endcsname{0.251}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1pm\endcsname{0.360}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1primary\endcsname{0.567}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.f1secondary\endcsname{0.073}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.gap\endcsname{-0.066}
\expandafter\def\csname res@ears.asom_v2sp_s43_noprior.gapci\endcsname{[-0.077, -0.054]}
\expandafter\def\csname res@ears.asom_v2sp_s44.acc\endcsname{0.309}
\expandafter\def\csname res@ears.asom_v2sp_s44.aucknown\endcsname{0.853}
\expandafter\def\csname res@ears.asom_v2sp_s44.aucnew\endcsname{0.769}
\expandafter\def\csname res@ears.asom_v2sp_s44.aucprimary\endcsname{0.963}
\expandafter\def\csname res@ears.asom_v2sp_s44.aucsecondary\endcsname{0.742}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1\endcsname{0.247}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1ci\endcsname{[0.229, 0.264]}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1known\endcsname{0.293}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1new\endcsname{0.213}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1pm\endcsname{0.359}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1primary\endcsname{0.508}
\expandafter\def\csname res@ears.asom_v2sp_s44.f1secondary\endcsname{0.077}
\expandafter\def\csname res@ears.asom_v2sp_s44.gap\endcsname{-0.031}
\expandafter\def\csname res@ears.asom_v2sp_s44.gapci\endcsname{[-0.043, -0.019]}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.acc\endcsname{0.329}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.aucknown\endcsname{0.857}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.aucnew\endcsname{0.768}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.aucprimary\endcsname{0.964}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.aucsecondary\endcsname{0.750}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1\endcsname{0.281}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1ci\endcsname{[0.266, 0.295]}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1known\endcsname{0.339}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1new\endcsname{0.235}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1pm\endcsname{0.359}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1primary\endcsname{0.564}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.f1secondary\endcsname{0.114}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.gap\endcsname{-0.065}
\expandafter\def\csname res@ears.asom_v2sp_s44_noprior.gapci\endcsname{[-0.075, -0.054]}
\expandafter\def\csname res@ears.asom_v2sp_s45.acc\endcsname{0.298}
\expandafter\def\csname res@ears.asom_v2sp_s45.aucknown\endcsname{0.849}
\expandafter\def\csname res@ears.asom_v2sp_s45.aucnew\endcsname{0.765}
\expandafter\def\csname res@ears.asom_v2sp_s45.aucprimary\endcsname{0.956}
\expandafter\def\csname res@ears.asom_v2sp_s45.aucsecondary\endcsname{0.742}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1\endcsname{0.238}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1ci\endcsname{[0.224, 0.252]}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1known\endcsname{0.267}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1new\endcsname{0.217}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1pm\endcsname{0.352}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1primary\endcsname{0.485}
\expandafter\def\csname res@ears.asom_v2sp_s45.f1secondary\endcsname{0.049}
\expandafter\def\csname res@ears.asom_v2sp_s45.gap\endcsname{-0.022}
\expandafter\def\csname res@ears.asom_v2sp_s45.gapci\endcsname{[-0.033, -0.011]}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.acc\endcsname{0.315}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.aucknown\endcsname{0.853}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.aucnew\endcsname{0.764}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.aucprimary\endcsname{0.956}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.aucsecondary\endcsname{0.750}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1\endcsname{0.269}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1ci\endcsname{[0.252, 0.285]}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1known\endcsname{0.304}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1new\endcsname{0.240}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1pm\endcsname{0.351}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1primary\endcsname{0.533}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.f1secondary\endcsname{0.075}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.gap\endcsname{-0.053}
\expandafter\def\csname res@ears.asom_v2sp_s45_noprior.gapci\endcsname{[-0.065, -0.041]}
\expandafter\def\csname res@ears.asom_v2sp_u.acc\endcsname{0.325}
\expandafter\def\csname res@ears.asom_v2sp_u.aucknown\endcsname{0.854}
\expandafter\def\csname res@ears.asom_v2sp_u.aucnew\endcsname{0.770}
\expandafter\def\csname res@ears.asom_v2sp_u.aucprimary\endcsname{0.962}
\expandafter\def\csname res@ears.asom_v2sp_u.aucsecondary\endcsname{0.747}
\expandafter\def\csname res@ears.asom_v2sp_u.f1\endcsname{0.277}
\expandafter\def\csname res@ears.asom_v2sp_u.f1ci\endcsname{[0.262, 0.291]}
\expandafter\def\csname res@ears.asom_v2sp_u.f1known\endcsname{0.321}
\expandafter\def\csname res@ears.asom_v2sp_u.f1new\endcsname{0.242}
\expandafter\def\csname res@ears.asom_v2sp_u.f1pm\endcsname{0.357}
\expandafter\def\csname res@ears.asom_v2sp_u.f1primary\endcsname{0.554}
\expandafter\def\csname res@ears.asom_v2sp_u.f1secondary\endcsname{0.087}
\expandafter\def\csname res@ears.asom_v2sp_u.gap\endcsname{-0.061}
\expandafter\def\csname res@ears.asom_v2sp_u.gapci\endcsname{[-0.071, -0.051]}
\expandafter\def\csname res@ears.basic.af3.acc\endcsname{0.140}
\expandafter\def\csname res@ears.basic.af3.aucknown\endcsname{0.447}
\expandafter\def\csname res@ears.basic.af3.aucprimary\endcsname{0.447}
\expandafter\def\csname res@ears.basic.af3.f1\endcsname{0.128}
\expandafter\def\csname res@ears.basic.af3.f1ci\endcsname{[0.106, 0.148]}
\expandafter\def\csname res@ears.basic.af3.f1known\endcsname{0.128}
\expandafter\def\csname res@ears.basic.af3.f1pm\endcsname{0.147}
\expandafter\def\csname res@ears.basic.af3.f1primary\endcsname{0.128}
\expandafter\def\csname res@ears.basic.af3.gap\endcsname{+0.493}
\expandafter\def\csname res@ears.basic.af3.gapci\endcsname{[+0.456, +0.531]}
\expandafter\def\csname res@ears.basic.af3_cc.acc\endcsname{0.155}
\expandafter\def\csname res@ears.basic.af3_cc.aucknown\endcsname{0.447}
\expandafter\def\csname res@ears.basic.af3_cc.aucprimary\endcsname{0.447}
\expandafter\def\csname res@ears.basic.af3_cc.f1\endcsname{0.150}
\expandafter\def\csname res@ears.basic.af3_cc.f1ci\endcsname{[0.125, 0.173]}
\expandafter\def\csname res@ears.basic.af3_cc.f1known\endcsname{0.150}
\expandafter\def\csname res@ears.basic.af3_cc.f1pm\endcsname{0.157}
\expandafter\def\csname res@ears.basic.af3_cc.f1primary\endcsname{0.150}
\expandafter\def\csname res@ears.basic.af3_cc.gap\endcsname{+0.471}
\expandafter\def\csname res@ears.basic.af3_cc.gapci\endcsname{[+0.431, +0.512]}
\expandafter\def\csname res@ears.basic.asom.acc\endcsname{0.652}
\expandafter\def\csname res@ears.basic.asom.aucknown\endcsname{0.965}
\expandafter\def\csname res@ears.basic.asom.aucprimary\endcsname{0.965}
\expandafter\def\csname res@ears.basic.asom.f1\endcsname{0.621}
\expandafter\def\csname res@ears.basic.asom.f1ci\endcsname{[0.586, 0.656]}
\expandafter\def\csname res@ears.basic.asom.f1known\endcsname{0.621}
\expandafter\def\csname res@ears.basic.asom.f1pm\endcsname{0.808}
\expandafter\def\csname res@ears.basic.asom.f1primary\endcsname{0.621}
\expandafter\def\csname res@ears.basic.asom_30s.acc\endcsname{0.663}
\expandafter\def\csname res@ears.basic.asom_30s.aucknown\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_30s.aucprimary\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_30s.f1\endcsname{0.630}
\expandafter\def\csname res@ears.basic.asom_30s.f1ci\endcsname{[0.592, 0.667]}
\expandafter\def\csname res@ears.basic.asom_30s.f1known\endcsname{0.630}
\expandafter\def\csname res@ears.basic.asom_30s.f1pm\endcsname{0.817}
\expandafter\def\csname res@ears.basic.asom_30s.f1primary\endcsname{0.630}
\expandafter\def\csname res@ears.basic.asom_30s.gap\endcsname{-0.009}
\expandafter\def\csname res@ears.basic.asom_30s.gapci\endcsname{[-0.029, +0.011]}
\expandafter\def\csname res@ears.basic.asom_cc.acc\endcsname{0.637}
\expandafter\def\csname res@ears.basic.asom_cc.aucknown\endcsname{0.961}
\expandafter\def\csname res@ears.basic.asom_cc.aucprimary\endcsname{0.961}
\expandafter\def\csname res@ears.basic.asom_cc.f1\endcsname{0.588}
\expandafter\def\csname res@ears.basic.asom_cc.f1ci\endcsname{[0.563, 0.612]}
\expandafter\def\csname res@ears.basic.asom_cc.f1known\endcsname{0.588}
\expandafter\def\csname res@ears.basic.asom_cc.f1pm\endcsname{0.830}
\expandafter\def\csname res@ears.basic.asom_cc.f1primary\endcsname{0.588}
\expandafter\def\csname res@ears.basic.asom_cc.gap\endcsname{+0.033}
\expandafter\def\csname res@ears.basic.asom_cc.gapci\endcsname{[-0.005, +0.070]}
\expandafter\def\csname res@ears.basic.asom_em.acc\endcsname{0.332}
\expandafter\def\csname res@ears.basic.asom_em.aucknown\endcsname{0.930}
\expandafter\def\csname res@ears.basic.asom_em.aucprimary\endcsname{0.930}
\expandafter\def\csname res@ears.basic.asom_em.f1\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_em.f1ci\endcsname{[0.209, 0.238]}
\expandafter\def\csname res@ears.basic.asom_em.f1known\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_em.f1pm\endcsname{0.488}
\expandafter\def\csname res@ears.basic.asom_em.f1primary\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_em.gap\endcsname{+0.397}
\expandafter\def\csname res@ears.basic.asom_em.gapci\endcsname{[+0.364, +0.428]}
\expandafter\def\csname res@ears.basic.asom_u.acc\endcsname{0.703}
\expandafter\def\csname res@ears.basic.asom_u.aucknown\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_u.aucprimary\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_u.f1\endcsname{0.702}
\expandafter\def\csname res@ears.basic.asom_u.f1ci\endcsname{[0.666, 0.735]}
\expandafter\def\csname res@ears.basic.asom_u.f1known\endcsname{0.702}
\expandafter\def\csname res@ears.basic.asom_u.f1pm\endcsname{0.824}
\expandafter\def\csname res@ears.basic.asom_u.f1primary\endcsname{0.702}
\expandafter\def\csname res@ears.basic.asom_u.gap\endcsname{-0.081}
\expandafter\def\csname res@ears.basic.asom_u.gapci\endcsname{[-0.106, -0.057]}
\expandafter\def\csname res@ears.basic.asom_v2sp.acc\endcsname{0.631}
\expandafter\def\csname res@ears.basic.asom_v2sp.aucknown\endcsname{0.965}
\expandafter\def\csname res@ears.basic.asom_v2sp.aucprimary\endcsname{0.965}
\expandafter\def\csname res@ears.basic.asom_v2sp.f1\endcsname{0.596}
\expandafter\def\csname res@ears.basic.asom_v2sp.f1ci\endcsname{[0.555, 0.638]}
\expandafter\def\csname res@ears.basic.asom_v2sp.f1known\endcsname{0.596}
\expandafter\def\csname res@ears.basic.asom_v2sp.f1pm\endcsname{0.797}
\expandafter\def\csname res@ears.basic.asom_v2sp.f1primary\endcsname{0.596}
\expandafter\def\csname res@ears.basic.asom_v2sp.gap\endcsname{+0.024}
\expandafter\def\csname res@ears.basic.asom_v2sp.gapci\endcsname{[-0.001, +0.047]}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.acc\endcsname{0.336}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.aucknown\endcsname{0.919}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.aucprimary\endcsname{0.919}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.f1\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.f1ci\endcsname{[0.209, 0.238]}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.f1known\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.f1pm\endcsname{0.490}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.f1primary\endcsname{0.224}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.gap\endcsname{+0.396}
\expandafter\def\csname res@ears.basic.asom_v2sp_em.gapci\endcsname{[+0.364, +0.428]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.acc\endcsname{0.638}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.aucknown\endcsname{0.963}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.aucprimary\endcsname{0.963}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.f1\endcsname{0.604}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.f1ci\endcsname{[0.561, 0.645]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.f1known\endcsname{0.604}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.f1pm\endcsname{0.790}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.f1primary\endcsname{0.604}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.gap\endcsname{+0.017}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43.gapci\endcsname{[-0.012, +0.046]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.acc\endcsname{0.668}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.aucknown\endcsname{0.966}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.aucprimary\endcsname{0.966}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.f1\endcsname{0.665}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.f1ci\endcsname{[0.624, 0.705]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.f1known\endcsname{0.665}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.f1pm\endcsname{0.808}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.f1primary\endcsname{0.665}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.gap\endcsname{-0.044}
\expandafter\def\csname res@ears.basic.asom_v2sp_s43_noprior.gapci\endcsname{[-0.075, -0.015]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.acc\endcsname{0.643}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.aucknown\endcsname{0.964}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.aucprimary\endcsname{0.964}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.f1\endcsname{0.615}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.f1ci\endcsname{[0.574, 0.658]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.f1known\endcsname{0.615}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.f1pm\endcsname{0.804}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.f1primary\endcsname{0.615}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.gap\endcsname{+0.006}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44.gapci\endcsname{[-0.019, +0.030]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.acc\endcsname{0.655}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.aucknown\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.aucprimary\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.f1\endcsname{0.649}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.f1ci\endcsname{[0.607, 0.690]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.f1known\endcsname{0.649}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.f1pm\endcsname{0.816}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.f1primary\endcsname{0.649}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.gap\endcsname{-0.029}
\expandafter\def\csname res@ears.basic.asom_v2sp_s44_noprior.gapci\endcsname{[-0.058, -0.003]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.acc\endcsname{0.610}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.aucknown\endcsname{0.960}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.aucprimary\endcsname{0.960}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.f1\endcsname{0.571}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.f1ci\endcsname{[0.529, 0.616]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.f1known\endcsname{0.571}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.f1pm\endcsname{0.796}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.f1primary\endcsname{0.571}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.gap\endcsname{+0.050}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45.gapci\endcsname{[+0.022, +0.074]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.acc\endcsname{0.642}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.aucknown\endcsname{0.963}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.aucprimary\endcsname{0.963}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.f1\endcsname{0.631}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.f1ci\endcsname{[0.590, 0.672]}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.f1known\endcsname{0.631}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.f1pm\endcsname{0.809}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.f1primary\endcsname{0.631}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.gap\endcsname{-0.010}
\expandafter\def\csname res@ears.basic.asom_v2sp_s45_noprior.gapci\endcsname{[-0.039, +0.017]}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.acc\endcsname{0.655}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.aucknown\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.aucprimary\endcsname{0.968}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.f1\endcsname{0.649}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.f1ci\endcsname{[0.608, 0.688]}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.f1known\endcsname{0.648}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.f1pm\endcsname{0.811}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.f1primary\endcsname{0.648}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.gap\endcsname{-0.028}
\expandafter\def\csname res@ears.basic.asom_v2sp_u.gapci\endcsname{[-0.053, -0.004]}
\expandafter\def\csname res@ears.basic.bestalm.f1\endcsname{0.970}
\expandafter\def\csname res@ears.basic.bestalm.f1.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@ears.basic.bestalmcc.f1\endcsname{0.967}
\expandafter\def\csname res@ears.basic.bestalmcc.f1.name\endcsname{Qwen2.5-Omni-3B + CC}
\expandafter\def\csname res@ears.basic.bestclap.f1\endcsname{0.371}
\expandafter\def\csname res@ears.basic.bestclap.name\endcsname{ParaCLAP}
\expandafter\def\csname res@ears.basic.chance\endcsname{0.200}
\expandafter\def\csname res@ears.basic.clap_laion.acc\endcsname{0.317}
\expandafter\def\csname res@ears.basic.clap_laion.aucknown\endcsname{0.650}
\expandafter\def\csname res@ears.basic.clap_laion.aucprimary\endcsname{0.650}
\expandafter\def\csname res@ears.basic.clap_laion.f1\endcsname{0.246}
\expandafter\def\csname res@ears.basic.clap_laion.f1ci\endcsname{[0.217, 0.273]}
\expandafter\def\csname res@ears.basic.clap_laion.f1known\endcsname{0.246}
\expandafter\def\csname res@ears.basic.clap_laion.f1pm\endcsname{0.333}
\expandafter\def\csname res@ears.basic.clap_laion.f1primary\endcsname{0.246}
\expandafter\def\csname res@ears.basic.clap_laion.gap\endcsname{+0.375}
\expandafter\def\csname res@ears.basic.clap_laion.gapci\endcsname{[+0.328, +0.419]}
\expandafter\def\csname res@ears.basic.clap_laion_desc.acc\endcsname{0.270}
\expandafter\def\csname res@ears.basic.clap_laion_desc.aucknown\endcsname{0.618}
\expandafter\def\csname res@ears.basic.clap_laion_desc.aucprimary\endcsname{0.618}
\expandafter\def\csname res@ears.basic.clap_laion_desc.f1\endcsname{0.186}
\expandafter\def\csname res@ears.basic.clap_laion_desc.f1ci\endcsname{[0.163, 0.208]}
\expandafter\def\csname res@ears.basic.clap_laion_desc.f1known\endcsname{0.186}
\expandafter\def\csname res@ears.basic.clap_laion_desc.f1pm\endcsname{0.303}
\expandafter\def\csname res@ears.basic.clap_laion_desc.f1primary\endcsname{0.186}
\expandafter\def\csname res@ears.basic.clap_laion_desc.gap\endcsname{+0.435}
\expandafter\def\csname res@ears.basic.clap_laion_desc.gapci\endcsname{[+0.394, +0.475]}
\expandafter\def\csname res@ears.basic.clap_ms.acc\endcsname{0.335}
\expandafter\def\csname res@ears.basic.clap_ms.aucknown\endcsname{0.751}
\expandafter\def\csname res@ears.basic.clap_ms.aucprimary\endcsname{0.751}
\expandafter\def\csname res@ears.basic.clap_ms.f1\endcsname{0.268}
\expandafter\def\csname res@ears.basic.clap_ms.f1ci\endcsname{[0.231, 0.302]}
\expandafter\def\csname res@ears.basic.clap_ms.f1known\endcsname{0.268}
\expandafter\def\csname res@ears.basic.clap_ms.f1pm\endcsname{0.409}
\expandafter\def\csname res@ears.basic.clap_ms.f1primary\endcsname{0.268}
\expandafter\def\csname res@ears.basic.clap_ms.gap\endcsname{+0.353}
\expandafter\def\csname res@ears.basic.clap_ms.gapci\endcsname{[+0.310, +0.395]}
\expandafter\def\csname res@ears.basic.clap_ms_desc.acc\endcsname{0.212}
\expandafter\def\csname res@ears.basic.clap_ms_desc.aucknown\endcsname{0.669}
\expandafter\def\csname res@ears.basic.clap_ms_desc.aucprimary\endcsname{0.669}
\expandafter\def\csname res@ears.basic.clap_ms_desc.f1\endcsname{0.095}
\expandafter\def\csname res@ears.basic.clap_ms_desc.f1ci\endcsname{[0.081, 0.110]}
\expandafter\def\csname res@ears.basic.clap_ms_desc.f1known\endcsname{0.095}
\expandafter\def\csname res@ears.basic.clap_ms_desc.f1pm\endcsname{0.342}
\expandafter\def\csname res@ears.basic.clap_ms_desc.f1primary\endcsname{0.095}
\expandafter\def\csname res@ears.basic.clap_ms_desc.gap\endcsname{+0.525}
\expandafter\def\csname res@ears.basic.clap_ms_desc.gapci\endcsname{[+0.485, +0.565]}
\expandafter\def\csname res@ears.basic.clap_para.acc\endcsname{0.413}
\expandafter\def\csname res@ears.basic.clap_para.aucknown\endcsname{0.797}
\expandafter\def\csname res@ears.basic.clap_para.aucprimary\endcsname{0.797}
\expandafter\def\csname res@ears.basic.clap_para.f1\endcsname{0.371}
\expandafter\def\csname res@ears.basic.clap_para.f1ci\endcsname{[0.334, 0.406]}
\expandafter\def\csname res@ears.basic.clap_para.f1known\endcsname{0.371}
\expandafter\def\csname res@ears.basic.clap_para.f1pm\endcsname{0.456}
\expandafter\def\csname res@ears.basic.clap_para.f1primary\endcsname{0.371}
\expandafter\def\csname res@ears.basic.clap_para.gap\endcsname{+0.250}
\expandafter\def\csname res@ears.basic.clap_para.gapci\endcsname{[+0.203, +0.296]}
\expandafter\def\csname res@ears.basic.clap_para_desc.acc\endcsname{0.297}
\expandafter\def\csname res@ears.basic.clap_para_desc.aucknown\endcsname{0.701}
\expandafter\def\csname res@ears.basic.clap_para_desc.aucprimary\endcsname{0.701}
\expandafter\def\csname res@ears.basic.clap_para_desc.f1\endcsname{0.258}
\expandafter\def\csname res@ears.basic.clap_para_desc.f1ci\endcsname{[0.228, 0.287]}
\expandafter\def\csname res@ears.basic.clap_para_desc.f1known\endcsname{0.258}
\expandafter\def\csname res@ears.basic.clap_para_desc.f1pm\endcsname{0.350}
\expandafter\def\csname res@ears.basic.clap_para_desc.f1primary\endcsname{0.258}
\expandafter\def\csname res@ears.basic.clap_para_desc.gap\endcsname{+0.363}
\expandafter\def\csname res@ears.basic.clap_para_desc.gapci\endcsname{[+0.320, +0.402]}
\expandafter\def\csname res@ears.basic.clips\endcsname{600}
\expandafter\def\csname res@ears.basic.e2v.acc\endcsname{0.613}
\expandafter\def\csname res@ears.basic.e2v.aucknown\endcsname{0.877}
\expandafter\def\csname res@ears.basic.e2v.aucprimary\endcsname{0.877}
\expandafter\def\csname res@ears.basic.e2v.f1\endcsname{0.578}
\expandafter\def\csname res@ears.basic.e2v.f1ci\endcsname{[0.535, 0.619]}
\expandafter\def\csname res@ears.basic.e2v.f1known\endcsname{0.578}
\expandafter\def\csname res@ears.basic.e2v.f1pm\endcsname{0.666}
\expandafter\def\csname res@ears.basic.e2v.f1primary\endcsname{0.578}
\expandafter\def\csname res@ears.basic.e2v.gap\endcsname{+0.043}
\expandafter\def\csname res@ears.basic.e2v.gapci\endcsname{[-0.004, +0.087]}
\expandafter\def\csname res@ears.basic.labels\endcsname{anger, disgust, fear, neutral, sadness}
\expandafter\def\csname res@ears.basic.omni3b.acc\endcsname{0.948}
\expandafter\def\csname res@ears.basic.omni3b.aucknown\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni3b.aucprimary\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni3b.f1\endcsname{0.948}
\expandafter\def\csname res@ears.basic.omni3b.f1ci\endcsname{[0.932, 0.965]}
\expandafter\def\csname res@ears.basic.omni3b.f1known\endcsname{0.948}
\expandafter\def\csname res@ears.basic.omni3b.f1pm\endcsname{0.952}
\expandafter\def\csname res@ears.basic.omni3b.f1primary\endcsname{0.948}
\expandafter\def\csname res@ears.basic.omni3b.gap\endcsname{-0.328}
\expandafter\def\csname res@ears.basic.omni3b.gapci\endcsname{[-0.363, -0.294]}
\expandafter\def\csname res@ears.basic.omni3b_cc.acc\endcsname{0.967}
\expandafter\def\csname res@ears.basic.omni3b_cc.aucknown\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni3b_cc.aucprimary\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni3b_cc.f1\endcsname{0.967}
\expandafter\def\csname res@ears.basic.omni3b_cc.f1ci\endcsname{[0.953, 0.978]}
\expandafter\def\csname res@ears.basic.omni3b_cc.f1known\endcsname{0.967}
\expandafter\def\csname res@ears.basic.omni3b_cc.f1pm\endcsname{0.967}
\expandafter\def\csname res@ears.basic.omni3b_cc.f1primary\endcsname{0.967}
\expandafter\def\csname res@ears.basic.omni3b_cc.gap\endcsname{-0.346}
\expandafter\def\csname res@ears.basic.omni3b_cc.gapci\endcsname{[-0.381, -0.312]}
\expandafter\def\csname res@ears.basic.omni3b_ft.acc\endcsname{0.930}
\expandafter\def\csname res@ears.basic.omni3b_ft.aucknown\endcsname{0.996}
\expandafter\def\csname res@ears.basic.omni3b_ft.aucprimary\endcsname{0.996}
\expandafter\def\csname res@ears.basic.omni3b_ft.f1\endcsname{0.930}
\expandafter\def\csname res@ears.basic.omni3b_ft.f1ci\endcsname{[0.906, 0.954]}
\expandafter\def\csname res@ears.basic.omni3b_ft.f1known\endcsname{0.930}
\expandafter\def\csname res@ears.basic.omni3b_ft.f1pm\endcsname{0.943}
\expandafter\def\csname res@ears.basic.omni3b_ft.f1primary\endcsname{0.930}
\expandafter\def\csname res@ears.basic.omni3b_ft.gap\endcsname{-0.310}
\expandafter\def\csname res@ears.basic.omni3b_ft.gapci\endcsname{[-0.347, -0.274]}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.acc\endcsname{0.903}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.aucknown\endcsname{0.993}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.f1\endcsname{0.902}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.f1ci\endcsname{[0.878, 0.924]}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.f1known\endcsname{0.902}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.f1pm\endcsname{0.920}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.f1primary\endcsname{0.902}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.gap\endcsname{-0.281}
\expandafter\def\csname res@ears.basic.omni3b_ftfull.gapci\endcsname{[-0.316, -0.245]}
\expandafter\def\csname res@ears.basic.omni7b.acc\endcsname{0.970}
\expandafter\def\csname res@ears.basic.omni7b.aucknown\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b.aucprimary\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b.f1\endcsname{0.970}
\expandafter\def\csname res@ears.basic.omni7b.f1ci\endcsname{[0.957, 0.983]}
\expandafter\def\csname res@ears.basic.omni7b.f1known\endcsname{0.970}
\expandafter\def\csname res@ears.basic.omni7b.f1pm\endcsname{0.972}
\expandafter\def\csname res@ears.basic.omni7b.f1primary\endcsname{0.970}
\expandafter\def\csname res@ears.basic.omni7b.gap\endcsname{-0.349}
\expandafter\def\csname res@ears.basic.omni7b.gapci\endcsname{[-0.384, -0.317]}
\expandafter\def\csname res@ears.basic.omni7b_cc.acc\endcsname{0.963}
\expandafter\def\csname res@ears.basic.omni7b_cc.aucknown\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b_cc.aucprimary\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b_cc.f1\endcsname{0.963}
\expandafter\def\csname res@ears.basic.omni7b_cc.f1ci\endcsname{[0.947, 0.978]}
\expandafter\def\csname res@ears.basic.omni7b_cc.f1known\endcsname{0.963}
\expandafter\def\csname res@ears.basic.omni7b_cc.f1pm\endcsname{0.963}
\expandafter\def\csname res@ears.basic.omni7b_cc.f1primary\endcsname{0.963}
\expandafter\def\csname res@ears.basic.omni7b_cc.gap\endcsname{-0.343}
\expandafter\def\csname res@ears.basic.omni7b_cc.gapci\endcsname{[-0.377, -0.310]}
\expandafter\def\csname res@ears.basic.omni7b_text.acc\endcsname{0.958}
\expandafter\def\csname res@ears.basic.omni7b_text.aucknown\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b_text.aucprimary\endcsname{0.998}
\expandafter\def\csname res@ears.basic.omni7b_text.f1\endcsname{0.959}
\expandafter\def\csname res@ears.basic.omni7b_text.f1ci\endcsname{[0.941, 0.975]}
\expandafter\def\csname res@ears.basic.omni7b_text.f1known\endcsname{0.959}
\expandafter\def\csname res@ears.basic.omni7b_text.f1pm\endcsname{0.960}
\expandafter\def\csname res@ears.basic.omni7b_text.f1primary\endcsname{0.959}
\expandafter\def\csname res@ears.basic.omni7b_text.gap\endcsname{-0.338}
\expandafter\def\csname res@ears.basic.omni7b_text.gapci\endcsname{[-0.373, -0.305]}
\expandafter\def\csname res@ears.basic.phi4mm.acc\endcsname{0.835}
\expandafter\def\csname res@ears.basic.phi4mm.aucknown\endcsname{0.974}
\expandafter\def\csname res@ears.basic.phi4mm.aucprimary\endcsname{0.974}
\expandafter\def\csname res@ears.basic.phi4mm.f1\endcsname{0.843}
\expandafter\def\csname res@ears.basic.phi4mm.f1ci\endcsname{[0.815, 0.871]}
\expandafter\def\csname res@ears.basic.phi4mm.f1known\endcsname{0.843}
\expandafter\def\csname res@ears.basic.phi4mm.f1pm\endcsname{0.880}
\expandafter\def\csname res@ears.basic.phi4mm.f1primary\endcsname{0.843}
\expandafter\def\csname res@ears.basic.phi4mm.gap\endcsname{-0.222}
\expandafter\def\csname res@ears.basic.phi4mm.gapci\endcsname{[-0.257, -0.188]}
\expandafter\def\csname res@ears.basic.phi4mm_cc.acc\endcsname{0.752}
\expandafter\def\csname res@ears.basic.phi4mm_cc.aucknown\endcsname{0.969}
\expandafter\def\csname res@ears.basic.phi4mm_cc.aucprimary\endcsname{0.969}
\expandafter\def\csname res@ears.basic.phi4mm_cc.f1\endcsname{0.758}
\expandafter\def\csname res@ears.basic.phi4mm_cc.f1ci\endcsname{[0.725, 0.791]}
\expandafter\def\csname res@ears.basic.phi4mm_cc.f1known\endcsname{0.758}
\expandafter\def\csname res@ears.basic.phi4mm_cc.f1pm\endcsname{0.859}
\expandafter\def\csname res@ears.basic.phi4mm_cc.f1primary\endcsname{0.758}
\expandafter\def\csname res@ears.basic.phi4mm_cc.gap\endcsname{-0.137}
\expandafter\def\csname res@ears.basic.phi4mm_cc.gapci\endcsname{[-0.174, -0.100]}
\expandafter\def\csname res@ears.basic.qwen2audio7b.acc\endcsname{0.945}
\expandafter\def\csname res@ears.basic.qwen2audio7b.aucknown\endcsname{0.992}
\expandafter\def\csname res@ears.basic.qwen2audio7b.aucprimary\endcsname{0.992}
\expandafter\def\csname res@ears.basic.qwen2audio7b.f1\endcsname{0.945}
\expandafter\def\csname res@ears.basic.qwen2audio7b.f1ci\endcsname{[0.927, 0.962]}
\expandafter\def\csname res@ears.basic.qwen2audio7b.f1known\endcsname{0.945}
\expandafter\def\csname res@ears.basic.qwen2audio7b.f1pm\endcsname{0.943}
\expandafter\def\csname res@ears.basic.qwen2audio7b.f1primary\endcsname{0.945}
\expandafter\def\csname res@ears.basic.qwen2audio7b.gap\endcsname{-0.324}
\expandafter\def\csname res@ears.basic.qwen2audio7b.gapci\endcsname{[-0.364, -0.289]}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.acc\endcsname{0.930}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.aucknown\endcsname{0.991}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.aucprimary\endcsname{0.991}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.f1\endcsname{0.930}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.f1ci\endcsname{[0.911, 0.947]}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.f1known\endcsname{0.930}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.f1pm\endcsname{0.942}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.f1primary\endcsname{0.930}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.gap\endcsname{-0.310}
\expandafter\def\csname res@ears.basic.qwen2audio7b_cc.gapci\endcsname{[-0.348, -0.272]}
\expandafter\def\csname res@ears.basic.voxtral3b.acc\endcsname{0.950}
\expandafter\def\csname res@ears.basic.voxtral3b.aucknown\endcsname{0.995}
\expandafter\def\csname res@ears.basic.voxtral3b.aucprimary\endcsname{0.995}
\expandafter\def\csname res@ears.basic.voxtral3b.f1\endcsname{0.950}
\expandafter\def\csname res@ears.basic.voxtral3b.f1ci\endcsname{[0.933, 0.967]}
\expandafter\def\csname res@ears.basic.voxtral3b.f1known\endcsname{0.950}
\expandafter\def\csname res@ears.basic.voxtral3b.f1pm\endcsname{0.952}
\expandafter\def\csname res@ears.basic.voxtral3b.f1primary\endcsname{0.950}
\expandafter\def\csname res@ears.basic.voxtral3b.gap\endcsname{-0.329}
\expandafter\def\csname res@ears.basic.voxtral3b.gapci\endcsname{[-0.368, -0.294]}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.acc\endcsname{0.937}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.aucknown\endcsname{0.991}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.aucprimary\endcsname{0.991}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.f1\endcsname{0.937}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.f1ci\endcsname{[0.918, 0.957]}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.f1known\endcsname{0.937}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.f1pm\endcsname{0.937}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.f1primary\endcsname{0.937}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.gap\endcsname{-0.316}
\expandafter\def\csname res@ears.basic.voxtral3b_cc.gapci\endcsname{[-0.354, -0.282]}
\expandafter\def\csname res@ears.basic.whisper_mlp.acc\endcsname{0.638}
\expandafter\def\csname res@ears.basic.whisper_mlp.aucknown\endcsname{0.962}
\expandafter\def\csname res@ears.basic.whisper_mlp.aucprimary\endcsname{0.962}
\expandafter\def\csname res@ears.basic.whisper_mlp.f1\endcsname{0.590}
\expandafter\def\csname res@ears.basic.whisper_mlp.f1ci\endcsname{[0.557, 0.623]}
\expandafter\def\csname res@ears.basic.whisper_mlp.f1known\endcsname{0.590}
\expandafter\def\csname res@ears.basic.whisper_mlp.f1pm\endcsname{0.810}
\expandafter\def\csname res@ears.basic.whisper_mlp.f1primary\endcsname{0.590}
\expandafter\def\csname res@ears.basic.whisper_mlp.gap\endcsname{+0.031}
\expandafter\def\csname res@ears.basic.whisper_mlp.gapci\endcsname{[+0.013, +0.048]}
\expandafter\def\csname res@ears.bestalm.aucnew\endcsname{0.987}
\expandafter\def\csname res@ears.bestalm.aucnew.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@ears.bestalm.f1\endcsname{0.849}
\expandafter\def\csname res@ears.bestalm.f1.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@ears.bestalm.f1new\endcsname{0.833}
\expandafter\def\csname res@ears.bestalm.f1new.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@ears.bestalmcc.aucnew\endcsname{0.987}
\expandafter\def\csname res@ears.bestalmcc.aucnew.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@ears.bestalmcc.f1\endcsname{0.848}
\expandafter\def\csname res@ears.bestalmcc.f1.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@ears.bestalmcc.f1new\endcsname{0.826}
\expandafter\def\csname res@ears.bestalmcc.f1new.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@ears.bestclap.f1\endcsname{0.127}
\expandafter\def\csname res@ears.bestclap.name\endcsname{ParaCLAP}
\expandafter\def\csname res@ears.chance\endcsname{0.087}
\expandafter\def\csname res@ears.clap_laion.acc\endcsname{0.105}
\expandafter\def\csname res@ears.clap_laion.aucknown\endcsname{0.592}
\expandafter\def\csname res@ears.clap_laion.aucnew\endcsname{0.565}
\expandafter\def\csname res@ears.clap_laion.aucprimary\endcsname{0.629}
\expandafter\def\csname res@ears.clap_laion.aucsecondary\endcsname{0.555}
\expandafter\def\csname res@ears.clap_laion.f1\endcsname{0.048}
\expandafter\def\csname res@ears.clap_laion.f1ci\endcsname{[0.041, 0.056]}
\expandafter\def\csname res@ears.clap_laion.f1known\endcsname{0.019}
\expandafter\def\csname res@ears.clap_laion.f1new\endcsname{0.070}
\expandafter\def\csname res@ears.clap_laion.f1pm\endcsname{0.125}
\expandafter\def\csname res@ears.clap_laion.f1primary\endcsname{0.023}
\expandafter\def\csname res@ears.clap_laion.f1secondary\endcsname{0.015}
\expandafter\def\csname res@ears.clap_laion.gap\endcsname{+0.168}
\expandafter\def\csname res@ears.clap_laion.gapci\endcsname{[+0.152, +0.183]}
\expandafter\def\csname res@ears.clap_laion_desc.acc\endcsname{0.124}
\expandafter\def\csname res@ears.clap_laion_desc.aucknown\endcsname{0.585}
\expandafter\def\csname res@ears.clap_laion_desc.aucnew\endcsname{0.573}
\expandafter\def\csname res@ears.clap_laion_desc.aucprimary\endcsname{0.592}
\expandafter\def\csname res@ears.clap_laion_desc.aucsecondary\endcsname{0.578}
\expandafter\def\csname res@ears.clap_laion_desc.f1\endcsname{0.084}
\expandafter\def\csname res@ears.clap_laion_desc.f1ci\endcsname{[0.074, 0.093]}
\expandafter\def\csname res@ears.clap_laion_desc.f1known\endcsname{0.084}
\expandafter\def\csname res@ears.clap_laion_desc.f1new\endcsname{0.083}
\expandafter\def\csname res@ears.clap_laion_desc.f1pm\endcsname{0.110}
\expandafter\def\csname res@ears.clap_laion_desc.f1primary\endcsname{0.014}
\expandafter\def\csname res@ears.clap_laion_desc.f1secondary\endcsname{0.153}
\expandafter\def\csname res@ears.clap_laion_desc.gap\endcsname{+0.132}
\expandafter\def\csname res@ears.clap_laion_desc.gapci\endcsname{[+0.118, +0.147]}
\expandafter\def\csname res@ears.clap_ms.acc\endcsname{0.136}
\expandafter\def\csname res@ears.clap_ms.aucknown\endcsname{0.707}
\expandafter\def\csname res@ears.clap_ms.aucnew\endcsname{0.580}
\expandafter\def\csname res@ears.clap_ms.aucprimary\endcsname{0.776}
\expandafter\def\csname res@ears.clap_ms.aucsecondary\endcsname{0.639}
\expandafter\def\csname res@ears.clap_ms.f1\endcsname{0.086}
\expandafter\def\csname res@ears.clap_ms.f1ci\endcsname{[0.074, 0.098]}
\expandafter\def\csname res@ears.clap_ms.f1known\endcsname{0.113}
\expandafter\def\csname res@ears.clap_ms.f1new\endcsname{0.066}
\expandafter\def\csname res@ears.clap_ms.f1pm\endcsname{0.184}
\expandafter\def\csname res@ears.clap_ms.f1primary\endcsname{0.169}
\expandafter\def\csname res@ears.clap_ms.f1secondary\endcsname{0.057}
\expandafter\def\csname res@ears.clap_ms.gap\endcsname{+0.130}
\expandafter\def\csname res@ears.clap_ms.gapci\endcsname{[+0.118, +0.142]}
\expandafter\def\csname res@ears.clap_ms_desc.acc\endcsname{0.132}
\expandafter\def\csname res@ears.clap_ms_desc.aucknown\endcsname{0.608}
\expandafter\def\csname res@ears.clap_ms_desc.aucnew\endcsname{0.597}
\expandafter\def\csname res@ears.clap_ms_desc.aucprimary\endcsname{0.629}
\expandafter\def\csname res@ears.clap_ms_desc.aucsecondary\endcsname{0.587}
\expandafter\def\csname res@ears.clap_ms_desc.f1\endcsname{0.064}
\expandafter\def\csname res@ears.clap_ms_desc.f1ci\endcsname{[0.057, 0.071]}
\expandafter\def\csname res@ears.clap_ms_desc.f1known\endcsname{0.085}
\expandafter\def\csname res@ears.clap_ms_desc.f1new\endcsname{0.051}
\expandafter\def\csname res@ears.clap_ms_desc.f1pm\endcsname{0.153}
\expandafter\def\csname res@ears.clap_ms_desc.f1primary\endcsname{0.163}
\expandafter\def\csname res@ears.clap_ms_desc.f1secondary\endcsname{0.006}
\expandafter\def\csname res@ears.clap_ms_desc.gap\endcsname{+0.152}
\expandafter\def\csname res@ears.clap_ms_desc.gapci\endcsname{[+0.138, +0.166]}
\expandafter\def\csname res@ears.clap_para.acc\endcsname{0.182}
\expandafter\def\csname res@ears.clap_para.aucknown\endcsname{0.744}
\expandafter\def\csname res@ears.clap_para.aucnew\endcsname{0.621}
\expandafter\def\csname res@ears.clap_para.aucprimary\endcsname{0.821}
\expandafter\def\csname res@ears.clap_para.aucsecondary\endcsname{0.666}
\expandafter\def\csname res@ears.clap_para.f1\endcsname{0.127}
\expandafter\def\csname res@ears.clap_para.f1ci\endcsname{[0.117, 0.135]}
\expandafter\def\csname res@ears.clap_para.f1known\endcsname{0.197}
\expandafter\def\csname res@ears.clap_para.f1new\endcsname{0.073}
\expandafter\def\csname res@ears.clap_para.f1pm\endcsname{0.149}
\expandafter\def\csname res@ears.clap_para.f1primary\endcsname{0.333}
\expandafter\def\csname res@ears.clap_para.f1secondary\endcsname{0.061}
\expandafter\def\csname res@ears.clap_para.gap\endcsname{+0.089}
\expandafter\def\csname res@ears.clap_para.gapci\endcsname{[+0.077, +0.101]}
\expandafter\def\csname res@ears.clap_para_desc.acc\endcsname{0.149}
\expandafter\def\csname res@ears.clap_para_desc.aucknown\endcsname{0.697}
\expandafter\def\csname res@ears.clap_para_desc.aucnew\endcsname{0.654}
\expandafter\def\csname res@ears.clap_para_desc.aucprimary\endcsname{0.723}
\expandafter\def\csname res@ears.clap_para_desc.aucsecondary\endcsname{0.671}
\expandafter\def\csname res@ears.clap_para_desc.f1\endcsname{0.108}
\expandafter\def\csname res@ears.clap_para_desc.f1ci\endcsname{[0.096, 0.119]}
\expandafter\def\csname res@ears.clap_para_desc.f1known\endcsname{0.140}
\expandafter\def\csname res@ears.clap_para_desc.f1new\endcsname{0.083}
\expandafter\def\csname res@ears.clap_para_desc.f1pm\endcsname{0.142}
\expandafter\def\csname res@ears.clap_para_desc.f1primary\endcsname{0.180}
\expandafter\def\csname res@ears.clap_para_desc.f1secondary\endcsname{0.100}
\expandafter\def\csname res@ears.clap_para_desc.gap\endcsname{+0.108}
\expandafter\def\csname res@ears.clap_para_desc.gapci\endcsname{[+0.092, +0.126]}
\expandafter\def\csname res@ears.clips\endcsname{2,760}
\expandafter\def\csname res@ears.emotions\endcsname{23}
\expandafter\def\csname res@ears.known\endcsname{10}
\expandafter\def\csname res@ears.menus\endcsname{2}
\expandafter\def\csname res@ears.new\endcsname{13}
\expandafter\def\csname res@ears.omni3b.acc\endcsname{0.802}
\expandafter\def\csname res@ears.omni3b.aucknown\endcsname{0.990}
\expandafter\def\csname res@ears.omni3b.aucnew\endcsname{0.970}
\expandafter\def\csname res@ears.omni3b.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.omni3b.aucsecondary\endcsname{0.988}
\expandafter\def\csname res@ears.omni3b.f1\endcsname{0.807}
\expandafter\def\csname res@ears.omni3b.f1ci\endcsname{[0.791, 0.822]}
\expandafter\def\csname res@ears.omni3b.f1known\endcsname{0.845}
\expandafter\def\csname res@ears.omni3b.f1new\endcsname{0.783}
\expandafter\def\csname res@ears.omni3b.f1pm\endcsname{0.849}
\expandafter\def\csname res@ears.omni3b.f1primary\endcsname{0.809}
\expandafter\def\csname res@ears.omni3b.f1secondary\endcsname{0.880}
\expandafter\def\csname res@ears.omni3b.gap\endcsname{-0.591}
\expandafter\def\csname res@ears.omni3b.gapci\endcsname{[-0.609, -0.573]}
\expandafter\def\csname res@ears.omni3b_cc.acc\endcsname{0.844}
\expandafter\def\csname res@ears.omni3b_cc.aucknown\endcsname{0.990}
\expandafter\def\csname res@ears.omni3b_cc.aucnew\endcsname{0.976}
\expandafter\def\csname res@ears.omni3b_cc.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.omni3b_cc.aucsecondary\endcsname{0.987}
\expandafter\def\csname res@ears.omni3b_cc.f1\endcsname{0.845}
\expandafter\def\csname res@ears.omni3b_cc.f1ci\endcsname{[0.830, 0.860]}
\expandafter\def\csname res@ears.omni3b_cc.f1known\endcsname{0.872}
\expandafter\def\csname res@ears.omni3b_cc.f1new\endcsname{0.826}
\expandafter\def\csname res@ears.omni3b_cc.f1pm\endcsname{0.854}
\expandafter\def\csname res@ears.omni3b_cc.f1primary\endcsname{0.864}
\expandafter\def\csname res@ears.omni3b_cc.f1secondary\endcsname{0.881}
\expandafter\def\csname res@ears.omni3b_cc.gap\endcsname{-0.629}
\expandafter\def\csname res@ears.omni3b_cc.gapci\endcsname{[-0.647, -0.612]}
\expandafter\def\csname res@ears.omni3b_ft.acc\endcsname{0.778}
\expandafter\def\csname res@ears.omni3b_ft.aucknown\endcsname{0.988}
\expandafter\def\csname res@ears.omni3b_ft.aucnew\endcsname{0.974}
\expandafter\def\csname res@ears.omni3b_ft.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.omni3b_ft.aucsecondary\endcsname{0.983}
\expandafter\def\csname res@ears.omni3b_ft.f1\endcsname{0.765}
\expandafter\def\csname res@ears.omni3b_ft.f1ci\endcsname{[0.746, 0.782]}
\expandafter\def\csname res@ears.omni3b_ft.f1known\endcsname{0.822}
\expandafter\def\csname res@ears.omni3b_ft.f1new\endcsname{0.722}
\expandafter\def\csname res@ears.omni3b_ft.f1pm\endcsname{0.849}
\expandafter\def\csname res@ears.omni3b_ft.f1primary\endcsname{0.877}
\expandafter\def\csname res@ears.omni3b_ft.f1secondary\endcsname{0.767}
\expandafter\def\csname res@ears.omni3b_ft.gap\endcsname{-0.549}
\expandafter\def\csname res@ears.omni3b_ft.gapci\endcsname{[-0.570, -0.527]}
\expandafter\def\csname res@ears.omni3b_ftfull.acc\endcsname{0.707}
\expandafter\def\csname res@ears.omni3b_ftfull.aucknown\endcsname{0.988}
\expandafter\def\csname res@ears.omni3b_ftfull.aucnew\endcsname{0.967}
\expandafter\def\csname res@ears.omni3b_ftfull.aucprimary\endcsname{0.991}
\expandafter\def\csname res@ears.omni3b_ftfull.aucsecondary\endcsname{0.984}
\expandafter\def\csname res@ears.omni3b_ftfull.f1\endcsname{0.683}
\expandafter\def\csname res@ears.omni3b_ftfull.f1ci\endcsname{[0.663, 0.702]}
\expandafter\def\csname res@ears.omni3b_ftfull.f1known\endcsname{0.758}
\expandafter\def\csname res@ears.omni3b_ftfull.f1new\endcsname{0.628}
\expandafter\def\csname res@ears.omni3b_ftfull.f1pm\endcsname{0.827}
\expandafter\def\csname res@ears.omni3b_ftfull.f1primary\endcsname{0.855}
\expandafter\def\csname res@ears.omni3b_ftfull.f1secondary\endcsname{0.661}
\expandafter\def\csname res@ears.omni3b_ftfull.gap\endcsname{-0.467}
\expandafter\def\csname res@ears.omni3b_ftfull.gapci\endcsname{[-0.488, -0.446]}
\expandafter\def\csname res@ears.omni7b.acc\endcsname{0.851}
\expandafter\def\csname res@ears.omni7b.aucknown\endcsname{0.992}
\expandafter\def\csname res@ears.omni7b.aucnew\endcsname{0.987}
\expandafter\def\csname res@ears.omni7b.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.omni7b.aucsecondary\endcsname{0.991}
\expandafter\def\csname res@ears.omni7b.f1\endcsname{0.849}
\expandafter\def\csname res@ears.omni7b.f1ci\endcsname{[0.832, 0.865]}
\expandafter\def\csname res@ears.omni7b.f1known\endcsname{0.871}
\expandafter\def\csname res@ears.omni7b.f1new\endcsname{0.833}
\expandafter\def\csname res@ears.omni7b.f1pm\endcsname{0.875}
\expandafter\def\csname res@ears.omni7b.f1primary\endcsname{0.870}
\expandafter\def\csname res@ears.omni7b.f1secondary\endcsname{0.871}
\expandafter\def\csname res@ears.omni7b.gap\endcsname{-0.633}
\expandafter\def\csname res@ears.omni7b.gapci\endcsname{[-0.651, -0.614]}
\expandafter\def\csname res@ears.omni7b_cc.acc\endcsname{0.852}
\expandafter\def\csname res@ears.omni7b_cc.aucknown\endcsname{0.992}
\expandafter\def\csname res@ears.omni7b_cc.aucnew\endcsname{0.987}
\expandafter\def\csname res@ears.omni7b_cc.aucprimary\endcsname{0.995}
\expandafter\def\csname res@ears.omni7b_cc.aucsecondary\endcsname{0.990}
\expandafter\def\csname res@ears.omni7b_cc.f1\endcsname{0.848}
\expandafter\def\csname res@ears.omni7b_cc.f1ci\endcsname{[0.831, 0.863]}
\expandafter\def\csname res@ears.omni7b_cc.f1known\endcsname{0.876}
\expandafter\def\csname res@ears.omni7b_cc.f1new\endcsname{0.826}
\expandafter\def\csname res@ears.omni7b_cc.f1pm\endcsname{0.877}
\expandafter\def\csname res@ears.omni7b_cc.f1primary\endcsname{0.894}
\expandafter\def\csname res@ears.omni7b_cc.f1secondary\endcsname{0.859}
\expandafter\def\csname res@ears.omni7b_cc.gap\endcsname{-0.632}
\expandafter\def\csname res@ears.omni7b_cc.gapci\endcsname{[-0.650, -0.614]}
\expandafter\def\csname res@ears.omni7b_text.acc\endcsname{0.812}
\expandafter\def\csname res@ears.omni7b_text.aucknown\endcsname{0.989}
\expandafter\def\csname res@ears.omni7b_text.aucnew\endcsname{0.984}
\expandafter\def\csname res@ears.omni7b_text.aucprimary\endcsname{0.993}
\expandafter\def\csname res@ears.omni7b_text.aucsecondary\endcsname{0.985}
\expandafter\def\csname res@ears.omni7b_text.f1\endcsname{0.798}
\expandafter\def\csname res@ears.omni7b_text.f1ci\endcsname{[0.783, 0.813]}
\expandafter\def\csname res@ears.omni7b_text.f1known\endcsname{0.829}
\expandafter\def\csname res@ears.omni7b_text.f1new\endcsname{0.776}
\expandafter\def\csname res@ears.omni7b_text.f1pm\endcsname{0.851}
\expandafter\def\csname res@ears.omni7b_text.f1primary\endcsname{0.814}
\expandafter\def\csname res@ears.omni7b_text.f1secondary\endcsname{0.844}
\expandafter\def\csname res@ears.omni7b_text.gap\endcsname{-0.582}
\expandafter\def\csname res@ears.omni7b_text.gapci\endcsname{[-0.601, -0.564]}
\expandafter\def\csname res@ears.phi4mm.acc\endcsname{0.746}
\expandafter\def\csname res@ears.phi4mm.aucknown\endcsname{0.959}
\expandafter\def\csname res@ears.phi4mm.aucnew\endcsname{0.964}
\expandafter\def\csname res@ears.phi4mm.aucprimary\endcsname{0.945}
\expandafter\def\csname res@ears.phi4mm.aucsecondary\endcsname{0.973}
\expandafter\def\csname res@ears.phi4mm.f1\endcsname{0.742}
\expandafter\def\csname res@ears.phi4mm.f1ci\endcsname{[0.724, 0.759]}
\expandafter\def\csname res@ears.phi4mm.f1known\endcsname{0.722}
\expandafter\def\csname res@ears.phi4mm.f1new\endcsname{0.761}
\expandafter\def\csname res@ears.phi4mm.f1pm\endcsname{0.785}
\expandafter\def\csname res@ears.phi4mm.f1primary\endcsname{0.688}
\expandafter\def\csname res@ears.phi4mm.f1secondary\endcsname{0.756}
\expandafter\def\csname res@ears.phi4mm.gap\endcsname{-0.526}
\expandafter\def\csname res@ears.phi4mm.gapci\endcsname{[-0.545, -0.505]}
\expandafter\def\csname res@ears.phi4mm_cc.acc\endcsname{0.725}
\expandafter\def\csname res@ears.phi4mm_cc.aucknown\endcsname{0.964}
\expandafter\def\csname res@ears.phi4mm_cc.aucnew\endcsname{0.964}
\expandafter\def\csname res@ears.phi4mm_cc.aucprimary\endcsname{0.954}
\expandafter\def\csname res@ears.phi4mm_cc.aucsecondary\endcsname{0.974}
\expandafter\def\csname res@ears.phi4mm_cc.f1\endcsname{0.705}
\expandafter\def\csname res@ears.phi4mm_cc.f1ci\endcsname{[0.687, 0.723]}
\expandafter\def\csname res@ears.phi4mm_cc.f1known\endcsname{0.695}
\expandafter\def\csname res@ears.phi4mm_cc.f1new\endcsname{0.718}
\expandafter\def\csname res@ears.phi4mm_cc.f1pm\endcsname{0.786}
\expandafter\def\csname res@ears.phi4mm_cc.f1primary\endcsname{0.605}
\expandafter\def\csname res@ears.phi4mm_cc.f1secondary\endcsname{0.784}
\expandafter\def\csname res@ears.phi4mm_cc.gap\endcsname{-0.490}
\expandafter\def\csname res@ears.phi4mm_cc.gapci\endcsname{[-0.510, -0.469]}
\expandafter\def\csname res@ears.primary\endcsname{5}
\expandafter\def\csname res@ears.qwen2audio7b.acc\endcsname{0.691}
\expandafter\def\csname res@ears.qwen2audio7b.aucknown\endcsname{0.962}
\expandafter\def\csname res@ears.qwen2audio7b.aucnew\endcsname{0.933}
\expandafter\def\csname res@ears.qwen2audio7b.aucprimary\endcsname{0.975}
\expandafter\def\csname res@ears.qwen2audio7b.aucsecondary\endcsname{0.948}
\expandafter\def\csname res@ears.qwen2audio7b.f1\endcsname{0.691}
\expandafter\def\csname res@ears.qwen2audio7b.f1ci\endcsname{[0.674, 0.706]}
\expandafter\def\csname res@ears.qwen2audio7b.f1known\endcsname{0.651}
\expandafter\def\csname res@ears.qwen2audio7b.f1new\endcsname{0.720}
\expandafter\def\csname res@ears.qwen2audio7b.f1pm\endcsname{0.757}
\expandafter\def\csname res@ears.qwen2audio7b.f1primary\endcsname{0.647}
\expandafter\def\csname res@ears.qwen2audio7b.f1secondary\endcsname{0.655}
\expandafter\def\csname res@ears.qwen2audio7b.gap\endcsname{-0.475}
\expandafter\def\csname res@ears.qwen2audio7b.gapci\endcsname{[-0.492, -0.455]}
\expandafter\def\csname res@ears.qwen2audio7b_cc.acc\endcsname{0.659}
\expandafter\def\csname res@ears.qwen2audio7b_cc.aucknown\endcsname{0.961}
\expandafter\def\csname res@ears.qwen2audio7b_cc.aucnew\endcsname{0.943}
\expandafter\def\csname res@ears.qwen2audio7b_cc.aucprimary\endcsname{0.970}
\expandafter\def\csname res@ears.qwen2audio7b_cc.aucsecondary\endcsname{0.952}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1\endcsname{0.655}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1ci\endcsname{[0.635, 0.675]}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1known\endcsname{0.606}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1new\endcsname{0.695}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1pm\endcsname{0.757}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1primary\endcsname{0.569}
\expandafter\def\csname res@ears.qwen2audio7b_cc.f1secondary\endcsname{0.644}
\expandafter\def\csname res@ears.qwen2audio7b_cc.gap\endcsname{-0.439}
\expandafter\def\csname res@ears.qwen2audio7b_cc.gapci\endcsname{[-0.459, -0.417]}
\expandafter\def\csname res@ears.secondary\endcsname{5}
\expandafter\def\csname res@ears.speakers\endcsname{60}
\expandafter\def\csname res@ears.voxtral3b.acc\endcsname{0.809}
\expandafter\def\csname res@ears.voxtral3b.aucknown\endcsname{0.981}
\expandafter\def\csname res@ears.voxtral3b.aucnew\endcsname{0.971}
\expandafter\def\csname res@ears.voxtral3b.aucprimary\endcsname{0.987}
\expandafter\def\csname res@ears.voxtral3b.aucsecondary\endcsname{0.975}
\expandafter\def\csname res@ears.voxtral3b.f1\endcsname{0.808}
\expandafter\def\csname res@ears.voxtral3b.f1ci\endcsname{[0.791, 0.823]}
\expandafter\def\csname res@ears.voxtral3b.f1known\endcsname{0.823}
\expandafter\def\csname res@ears.voxtral3b.f1new\endcsname{0.799}
\expandafter\def\csname res@ears.voxtral3b.f1pm\endcsname{0.822}
\expandafter\def\csname res@ears.voxtral3b.f1primary\endcsname{0.857}
\expandafter\def\csname res@ears.voxtral3b.f1secondary\endcsname{0.789}
\expandafter\def\csname res@ears.voxtral3b.gap\endcsname{-0.592}
\expandafter\def\csname res@ears.voxtral3b.gapci\endcsname{[-0.611, -0.571]}
\expandafter\def\csname res@ears.voxtral3b_cc.acc\endcsname{0.815}
\expandafter\def\csname res@ears.voxtral3b_cc.aucknown\endcsname{0.980}
\expandafter\def\csname res@ears.voxtral3b_cc.aucnew\endcsname{0.968}
\expandafter\def\csname res@ears.voxtral3b_cc.aucprimary\endcsname{0.985}
\expandafter\def\csname res@ears.voxtral3b_cc.aucsecondary\endcsname{0.976}
\expandafter\def\csname res@ears.voxtral3b_cc.f1\endcsname{0.808}
\expandafter\def\csname res@ears.voxtral3b_cc.f1ci\endcsname{[0.792, 0.823]}
\expandafter\def\csname res@ears.voxtral3b_cc.f1known\endcsname{0.819}
\expandafter\def\csname res@ears.voxtral3b_cc.f1new\endcsname{0.801}
\expandafter\def\csname res@ears.voxtral3b_cc.f1pm\endcsname{0.815}
\expandafter\def\csname res@ears.voxtral3b_cc.f1primary\endcsname{0.868}
\expandafter\def\csname res@ears.voxtral3b_cc.f1secondary\endcsname{0.771}
\expandafter\def\csname res@ears.voxtral3b_cc.gap\endcsname{-0.592}
\expandafter\def\csname res@ears.voxtral3b_cc.gapci\endcsname{[-0.610, -0.572]}
\expandafter\def\csname res@flex.af3.bare_names.agree\endcsname{28.3}
\expandafter\def\csname res@flex.af3.bare_names.delta\endcsname{-0.019}
\expandafter\def\csname res@flex.af3.bare_names.deltaci\endcsname{[-0.043, +0.004]}
\expandafter\def\csname res@flex.af3.bare_names.f1\endcsname{0.142}
\expandafter\def\csname res@flex.af3.ccc.arousal\endcsname{0.044}
\expandafter\def\csname res@flex.af3.ccc.arousalci\endcsname{[-0.001, 0.090]}
\expandafter\def\csname res@flex.af3.ccc.dominance\endcsname{0.023}
\expandafter\def\csname res@flex.af3.ccc.dominanceci\endcsname{[-0.006, 0.074]}
\expandafter\def\csname res@flex.af3.ccc.valence\endcsname{0.187}
\expandafter\def\csname res@flex.af3.ccc.valenceci\endcsname{[0.098, 0.239]}
\expandafter\def\csname res@flex.af3.ccc2.arousal\endcsname{0.04}
\expandafter\def\csname res@flex.af3.ccc2.dominance\endcsname{0.02}
\expandafter\def\csname res@flex.af3.ccc2.valence\endcsname{0.19}
\expandafter\def\csname res@flex.af3.gender\endcsname{0.553}
\expandafter\def\csname res@flex.af3.genderref\endcsname{0.682}
\expandafter\def\csname res@flex.af3.genderrefci\endcsname{[0.617, 0.744]}
\expandafter\def\csname res@flex.af3.instr2.agree\endcsname{32.1}
\expandafter\def\csname res@flex.af3.instr2.delta\endcsname{-0.016}
\expandafter\def\csname res@flex.af3.instr2.deltaci\endcsname{[-0.047, +0.013]}
\expandafter\def\csname res@flex.af3.instr2.f1\endcsname{0.145}
\expandafter\def\csname res@flex.af3.native.f1\endcsname{0.161}
\expandafter\def\csname res@flex.af3.newwords_above\endcsname{4}
\expandafter\def\csname res@flex.af3.newwords_oracle\endcsname{0.553}
\expandafter\def\csname res@flex.af3.para1.agree\endcsname{36.3}
\expandafter\def\csname res@flex.af3.para1.delta\endcsname{-0.034}
\expandafter\def\csname res@flex.af3.para1.deltaci\endcsname{[-0.059, -0.013]}
\expandafter\def\csname res@flex.af3.para1.f1\endcsname{0.127}
\expandafter\def\csname res@flex.af3.para2.agree\endcsname{36.8}
\expandafter\def\csname res@flex.af3.para2.delta\endcsname{-0.030}
\expandafter\def\csname res@flex.af3.para2.deltaci\endcsname{[-0.059, -0.001]}
\expandafter\def\csname res@flex.af3.para2.f1\endcsname{0.131}
\expandafter\def\csname res@flex.af3.redagree\endcsname{43.0}
\expandafter\def\csname res@flex.af3.synpara.agree\endcsname{33.8}
\expandafter\def\csname res@flex.af3.synpara.delta\endcsname{-0.009}
\expandafter\def\csname res@flex.af3.synpara.deltaci\endcsname{[-0.043, +0.026]}
\expandafter\def\csname res@flex.af3.synpara.f1\endcsname{0.152}
\expandafter\def\csname res@flex.af3.tenth\endcsname{0.551}
\expandafter\def\csname res@flex.af3.tv\endcsname{0.380}
\expandafter\def\csname res@flex.af3.yesno_native\endcsname{0.550}
\expandafter\def\csname res@flex.af3.yesno_nativeci\endcsname{[0.533, 0.567]}
\expandafter\def\csname res@flex.af3.yesno_new_words\endcsname{0.542}
\expandafter\def\csname res@flex.af3.yesno_new_wordsci\endcsname{[0.522, 0.562]}
\expandafter\def\csname res@flex.af3_cc.bare_names.agree\endcsname{22.2}
\expandafter\def\csname res@flex.af3_cc.bare_names.delta\endcsname{+0.011}
\expandafter\def\csname res@flex.af3_cc.bare_names.deltaci\endcsname{[-0.022, +0.041]}
\expandafter\def\csname res@flex.af3_cc.bare_names.f1\endcsname{0.146}
\expandafter\def\csname res@flex.af3_cc.ccc.arousal\endcsname{0.061}
\expandafter\def\csname res@flex.af3_cc.ccc.arousalci\endcsname{[-0.007, 0.124]}
\expandafter\def\csname res@flex.af3_cc.ccc.dominance\endcsname{0.018}
\expandafter\def\csname res@flex.af3_cc.ccc.dominanceci\endcsname{[-0.014, 0.075]}
\expandafter\def\csname res@flex.af3_cc.ccc.valence\endcsname{0.178}
\expandafter\def\csname res@flex.af3_cc.ccc.valenceci\endcsname{[0.095, 0.228]}
\expandafter\def\csname res@flex.af3_cc.ccc2.arousal\endcsname{0.06}
\expandafter\def\csname res@flex.af3_cc.ccc2.dominance\endcsname{0.02}
\expandafter\def\csname res@flex.af3_cc.ccc2.valence\endcsname{0.18}
\expandafter\def\csname res@flex.af3_cc.gender\endcsname{0.560}
\expandafter\def\csname res@flex.af3_cc.genderref\endcsname{0.682}
\expandafter\def\csname res@flex.af3_cc.genderrefci\endcsname{[0.617, 0.744]}
\expandafter\def\csname res@flex.af3_cc.instr2.agree\endcsname{20.0}
\expandafter\def\csname res@flex.af3_cc.instr2.delta\endcsname{+0.012}
\expandafter\def\csname res@flex.af3_cc.instr2.deltaci\endcsname{[-0.019, +0.040]}
\expandafter\def\csname res@flex.af3_cc.instr2.f1\endcsname{0.147}
\expandafter\def\csname res@flex.af3_cc.native.f1\endcsname{0.135}
\expandafter\def\csname res@flex.af3_cc.newwords_above\endcsname{5}
\expandafter\def\csname res@flex.af3_cc.newwords_oracle\endcsname{0.551}
\expandafter\def\csname res@flex.af3_cc.para1.agree\endcsname{21.3}
\expandafter\def\csname res@flex.af3_cc.para1.delta\endcsname{+0.030}
\expandafter\def\csname res@flex.af3_cc.para1.deltaci\endcsname{[-0.005, +0.061]}
\expandafter\def\csname res@flex.af3_cc.para1.f1\endcsname{0.165}
\expandafter\def\csname res@flex.af3_cc.para2.agree\endcsname{22.6}
\expandafter\def\csname res@flex.af3_cc.para2.delta\endcsname{+0.030}
\expandafter\def\csname res@flex.af3_cc.para2.deltaci\endcsname{[-0.002, +0.063]}
\expandafter\def\csname res@flex.af3_cc.para2.f1\endcsname{0.165}
\expandafter\def\csname res@flex.af3_cc.redagree\endcsname{48.7}
\expandafter\def\csname res@flex.af3_cc.synpara.agree\endcsname{20.0}
\expandafter\def\csname res@flex.af3_cc.synpara.delta\endcsname{+0.032}
\expandafter\def\csname res@flex.af3_cc.synpara.deltaci\endcsname{[+0.000, +0.064]}
\expandafter\def\csname res@flex.af3_cc.synpara.f1\endcsname{0.167}
\expandafter\def\csname res@flex.af3_cc.tenth\endcsname{0.550}
\expandafter\def\csname res@flex.af3_cc.tv\endcsname{0.302}
\expandafter\def\csname res@flex.af3_cc.yesno_native\endcsname{0.550}
\expandafter\def\csname res@flex.af3_cc.yesno_nativeci\endcsname{[0.533, 0.567]}
\expandafter\def\csname res@flex.af3_cc.yesno_new_words\endcsname{0.542}
\expandafter\def\csname res@flex.af3_cc.yesno_new_wordsci\endcsname{[0.522, 0.562]}
\expandafter\def\csname res@flex.asom.bare_names.agree\endcsname{79.1}
\expandafter\def\csname res@flex.asom.bare_names.delta\endcsname{-0.063}
\expandafter\def\csname res@flex.asom.bare_names.deltaci\endcsname{[-0.096, -0.033]}
\expandafter\def\csname res@flex.asom.bare_names.f1\endcsname{0.335}
\expandafter\def\csname res@flex.asom.ccc.arousal\endcsname{0.674}
\expandafter\def\csname res@flex.asom.ccc.arousalci\endcsname{[0.581, 0.753]}
\expandafter\def\csname res@flex.asom.ccc.dominance\endcsname{0.584}
\expandafter\def\csname res@flex.asom.ccc.dominanceci\endcsname{[0.476, 0.715]}
\expandafter\def\csname res@flex.asom.ccc.valence\endcsname{0.735}
\expandafter\def\csname res@flex.asom.ccc.valenceci\endcsname{[0.674, 0.782]}
\expandafter\def\csname res@flex.asom.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flex.asom.gender\endcsname{0.685}
\expandafter\def\csname res@flex.asom.genderref\endcsname{0.873}
\expandafter\def\csname res@flex.asom.genderrefci\endcsname{[0.780, 0.935]}
\expandafter\def\csname res@flex.asom.instr2.agree\endcsname{88.9}
\expandafter\def\csname res@flex.asom.instr2.delta\endcsname{-0.035}
\expandafter\def\csname res@flex.asom.instr2.deltaci\endcsname{[-0.064, -0.007]}
\expandafter\def\csname res@flex.asom.instr2.f1\endcsname{0.363}
\expandafter\def\csname res@flex.asom.listener.bare_names.agree\endcsname{84.8}
\expandafter\def\csname res@flex.asom.listener.bare_names.delta\endcsname{-0.069}
\expandafter\def\csname res@flex.asom.listener.bare_names.deltaci\endcsname{[-0.098, -0.047]}
\expandafter\def\csname res@flex.asom.listener.bare_names.f1\endcsname{0.278}
\expandafter\def\csname res@flex.asom.listener.instr2.agree\endcsname{85.4}
\expandafter\def\csname res@flex.asom.listener.instr2.delta\endcsname{+0.017}
\expandafter\def\csname res@flex.asom.listener.instr2.deltaci\endcsname{[-0.003, +0.044]}
\expandafter\def\csname res@flex.asom.listener.instr2.f1\endcsname{0.364}
\expandafter\def\csname res@flex.asom.listener.native.f1\endcsname{0.347}
\expandafter\def\csname res@flex.asom.listener.para1.agree\endcsname{94.8}
\expandafter\def\csname res@flex.asom.listener.para1.delta\endcsname{+0.003}
\expandafter\def\csname res@flex.asom.listener.para1.deltaci\endcsname{[-0.009, +0.020]}
\expandafter\def\csname res@flex.asom.listener.para1.f1\endcsname{0.350}
\expandafter\def\csname res@flex.asom.listener.para2.agree\endcsname{91.3}
\expandafter\def\csname res@flex.asom.listener.para2.delta\endcsname{-0.007}
\expandafter\def\csname res@flex.asom.listener.para2.deltaci\endcsname{[-0.021, +0.009]}
\expandafter\def\csname res@flex.asom.listener.para2.f1\endcsname{0.340}
\expandafter\def\csname res@flex.asom.listener.synpara.agree\endcsname{91.2}
\expandafter\def\csname res@flex.asom.listener.synpara.delta\endcsname{+0.004}
\expandafter\def\csname res@flex.asom.listener.synpara.deltaci\endcsname{[-0.011, +0.027]}
\expandafter\def\csname res@flex.asom.listener.synpara.f1\endcsname{0.351}
\expandafter\def\csname res@flex.asom.native.f1\endcsname{0.398}
\expandafter\def\csname res@flex.asom.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom.newwords_oracle\endcsname{0.742}
\expandafter\def\csname res@flex.asom.para1.agree\endcsname{90.1}
\expandafter\def\csname res@flex.asom.para1.delta\endcsname{-0.017}
\expandafter\def\csname res@flex.asom.para1.deltaci\endcsname{[-0.046, +0.009]}
\expandafter\def\csname res@flex.asom.para1.f1\endcsname{0.381}
\expandafter\def\csname res@flex.asom.para2.agree\endcsname{89.9}
\expandafter\def\csname res@flex.asom.para2.delta\endcsname{-0.017}
\expandafter\def\csname res@flex.asom.para2.deltaci\endcsname{[-0.033, -0.003]}
\expandafter\def\csname res@flex.asom.para2.f1\endcsname{0.381}
\expandafter\def\csname res@flex.asom.redagree\endcsname{99.3}
\expandafter\def\csname res@flex.asom.synpara.agree\endcsname{86.7}
\expandafter\def\csname res@flex.asom.synpara.delta\endcsname{-0.038}
\expandafter\def\csname res@flex.asom.synpara.deltaci\endcsname{[-0.063, -0.012]}
\expandafter\def\csname res@flex.asom.synpara.f1\endcsname{0.360}
\expandafter\def\csname res@flex.asom.tenth\endcsname{0.699}
\expandafter\def\csname res@flex.asom.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom.yesno_nativeci\endcsname{[0.743, 0.784]}
\expandafter\def\csname res@flex.asom.yesno_new_words\endcsname{0.714}
\expandafter\def\csname res@flex.asom.yesno_new_wordsci\endcsname{[0.686, 0.742]}
\expandafter\def\csname res@flex.asom_30s.bare_names.agree\endcsname{84.7}
\expandafter\def\csname res@flex.asom_30s.bare_names.delta\endcsname{-0.061}
\expandafter\def\csname res@flex.asom_30s.bare_names.deltaci\endcsname{[-0.081, -0.044]}
\expandafter\def\csname res@flex.asom_30s.bare_names.f1\endcsname{0.286}
\expandafter\def\csname res@flex.asom_30s.ccc.arousal\endcsname{0.667}
\expandafter\def\csname res@flex.asom_30s.ccc.arousalci\endcsname{[0.568, 0.756]}
\expandafter\def\csname res@flex.asom_30s.ccc.dominance\endcsname{0.577}
\expandafter\def\csname res@flex.asom_30s.ccc.dominanceci\endcsname{[0.463, 0.715]}
\expandafter\def\csname res@flex.asom_30s.ccc.valence\endcsname{0.741}
\expandafter\def\csname res@flex.asom_30s.ccc.valenceci\endcsname{[0.687, 0.784]}
\expandafter\def\csname res@flex.asom_30s.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_30s.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_30s.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_30s.gender\endcsname{0.683}
\expandafter\def\csname res@flex.asom_30s.genderref\endcsname{0.893}
\expandafter\def\csname res@flex.asom_30s.genderrefci\endcsname{[0.818, 0.944]}
\expandafter\def\csname res@flex.asom_30s.instr2.agree\endcsname{84.7}
\expandafter\def\csname res@flex.asom_30s.instr2.delta\endcsname{+0.010}
\expandafter\def\csname res@flex.asom_30s.instr2.deltaci\endcsname{[-0.010, +0.038]}
\expandafter\def\csname res@flex.asom_30s.instr2.f1\endcsname{0.357}
\expandafter\def\csname res@flex.asom_30s.native.f1\endcsname{0.347}
\expandafter\def\csname res@flex.asom_30s.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom_30s.newwords_oracle\endcsname{0.742}
\expandafter\def\csname res@flex.asom_30s.para1.agree\endcsname{94.1}
\expandafter\def\csname res@flex.asom_30s.para1.delta\endcsname{+0.005}
\expandafter\def\csname res@flex.asom_30s.para1.deltaci\endcsname{[-0.008, +0.026]}
\expandafter\def\csname res@flex.asom_30s.para1.f1\endcsname{0.351}
\expandafter\def\csname res@flex.asom_30s.para2.agree\endcsname{91.1}
\expandafter\def\csname res@flex.asom_30s.para2.delta\endcsname{-0.005}
\expandafter\def\csname res@flex.asom_30s.para2.deltaci\endcsname{[-0.022, +0.018]}
\expandafter\def\csname res@flex.asom_30s.para2.f1\endcsname{0.341}
\expandafter\def\csname res@flex.asom_30s.redagree\endcsname{99.2}
\expandafter\def\csname res@flex.asom_30s.synpara.agree\endcsname{91.4}
\expandafter\def\csname res@flex.asom_30s.synpara.delta\endcsname{+0.006}
\expandafter\def\csname res@flex.asom_30s.synpara.deltaci\endcsname{[-0.010, +0.029]}
\expandafter\def\csname res@flex.asom_30s.synpara.f1\endcsname{0.352}
\expandafter\def\csname res@flex.asom_30s.tenth\endcsname{0.698}
\expandafter\def\csname res@flex.asom_30s.tv\endcsname{0.005}
\expandafter\def\csname res@flex.asom_30s.yesno_native\endcsname{0.763}
\expandafter\def\csname res@flex.asom_30s.yesno_nativeci\endcsname{[0.744, 0.785]}
\expandafter\def\csname res@flex.asom_30s.yesno_new_words\endcsname{0.713}
\expandafter\def\csname res@flex.asom_30s.yesno_new_wordsci\endcsname{[0.684, 0.741]}
\expandafter\def\csname res@flex.asom_cc.bare_names.agree\endcsname{77.9}
\expandafter\def\csname res@flex.asom_cc.bare_names.delta\endcsname{+0.026}
\expandafter\def\csname res@flex.asom_cc.bare_names.deltaci\endcsname{[+0.006, +0.041]}
\expandafter\def\csname res@flex.asom_cc.bare_names.f1\endcsname{0.303}
\expandafter\def\csname res@flex.asom_cc.gender\endcsname{0.685}
\expandafter\def\csname res@flex.asom_cc.genderref\endcsname{0.873}
\expandafter\def\csname res@flex.asom_cc.genderrefci\endcsname{[0.780, 0.935]}
\expandafter\def\csname res@flex.asom_cc.instr2.agree\endcsname{91.9}
\expandafter\def\csname res@flex.asom_cc.instr2.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.asom_cc.instr2.deltaci\endcsname{[-0.015, +0.002]}
\expandafter\def\csname res@flex.asom_cc.instr2.f1\endcsname{0.272}
\expandafter\def\csname res@flex.asom_cc.native.f1\endcsname{0.277}
\expandafter\def\csname res@flex.asom_cc.newwords_above\endcsname{3}
\expandafter\def\csname res@flex.asom_cc.newwords_oracle\endcsname{0.719}
\expandafter\def\csname res@flex.asom_cc.para1.agree\endcsname{75.1}
\expandafter\def\csname res@flex.asom_cc.para1.delta\endcsname{+0.013}
\expandafter\def\csname res@flex.asom_cc.para1.deltaci\endcsname{[-0.006, +0.027]}
\expandafter\def\csname res@flex.asom_cc.para1.f1\endcsname{0.290}
\expandafter\def\csname res@flex.asom_cc.para2.agree\endcsname{84.7}
\expandafter\def\csname res@flex.asom_cc.para2.delta\endcsname{-0.023}
\expandafter\def\csname res@flex.asom_cc.para2.deltaci\endcsname{[-0.036, -0.013]}
\expandafter\def\csname res@flex.asom_cc.para2.f1\endcsname{0.254}
\expandafter\def\csname res@flex.asom_cc.redagree\endcsname{99.4}
\expandafter\def\csname res@flex.asom_cc.synpara.agree\endcsname{83.0}
\expandafter\def\csname res@flex.asom_cc.synpara.delta\endcsname{+0.011}
\expandafter\def\csname res@flex.asom_cc.synpara.deltaci\endcsname{[-0.004, +0.026]}
\expandafter\def\csname res@flex.asom_cc.synpara.f1\endcsname{0.288}
\expandafter\def\csname res@flex.asom_cc.tenth\endcsname{0.672}
\expandafter\def\csname res@flex.asom_cc.tv\endcsname{0.005}
\expandafter\def\csname res@flex.asom_cc.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_cc.yesno_nativeci\endcsname{[0.743, 0.783]}
\expandafter\def\csname res@flex.asom_cc.yesno_new_words\endcsname{0.714}
\expandafter\def\csname res@flex.asom_cc.yesno_new_wordsci\endcsname{[0.687, 0.742]}
\expandafter\def\csname res@flex.asom_clip.bare_names.agree\endcsname{73.8}
\expandafter\def\csname res@flex.asom_clip.bare_names.delta\endcsname{-0.010}
\expandafter\def\csname res@flex.asom_clip.bare_names.deltaci\endcsname{[-0.039, +0.014]}
\expandafter\def\csname res@flex.asom_clip.bare_names.f1\endcsname{0.353}
\expandafter\def\csname res@flex.asom_clip.ccc.arousal\endcsname{0.686}
\expandafter\def\csname res@flex.asom_clip.ccc.arousalci\endcsname{[0.637, 0.734]}
\expandafter\def\csname res@flex.asom_clip.ccc.dominance\endcsname{0.568}
\expandafter\def\csname res@flex.asom_clip.ccc.dominanceci\endcsname{[0.492, 0.637]}
\expandafter\def\csname res@flex.asom_clip.ccc.valence\endcsname{0.747}
\expandafter\def\csname res@flex.asom_clip.ccc.valenceci\endcsname{[0.716, 0.767]}
\expandafter\def\csname res@flex.asom_clip.ccc2.arousal\endcsname{0.69}
\expandafter\def\csname res@flex.asom_clip.ccc2.dominance\endcsname{0.57}
\expandafter\def\csname res@flex.asom_clip.ccc2.valence\endcsname{0.75}
\expandafter\def\csname res@flex.asom_clip.gender\endcsname{0.736}
\expandafter\def\csname res@flex.asom_clip.instr2.agree\endcsname{86.2}
\expandafter\def\csname res@flex.asom_clip.instr2.delta\endcsname{+0.009}
\expandafter\def\csname res@flex.asom_clip.instr2.deltaci\endcsname{[-0.007, +0.025]}
\expandafter\def\csname res@flex.asom_clip.instr2.f1\endcsname{0.371}
\expandafter\def\csname res@flex.asom_clip.native.f1\endcsname{0.362}
\expandafter\def\csname res@flex.asom_clip.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom_clip.newwords_oracle\endcsname{0.732}
\expandafter\def\csname res@flex.asom_clip.para1.agree\endcsname{88.7}
\expandafter\def\csname res@flex.asom_clip.para1.delta\endcsname{-0.004}
\expandafter\def\csname res@flex.asom_clip.para1.deltaci\endcsname{[-0.017, +0.009]}
\expandafter\def\csname res@flex.asom_clip.para1.f1\endcsname{0.359}
\expandafter\def\csname res@flex.asom_clip.para2.agree\endcsname{77.5}
\expandafter\def\csname res@flex.asom_clip.para2.delta\endcsname{-0.044}
\expandafter\def\csname res@flex.asom_clip.para2.deltaci\endcsname{[-0.071, -0.023]}
\expandafter\def\csname res@flex.asom_clip.para2.f1\endcsname{0.318}
\expandafter\def\csname res@flex.asom_clip.redagree\endcsname{99.2}
\expandafter\def\csname res@flex.asom_clip.synpara.agree\endcsname{80.6}
\expandafter\def\csname res@flex.asom_clip.synpara.delta\endcsname{-0.025}
\expandafter\def\csname res@flex.asom_clip.synpara.deltaci\endcsname{[-0.050, -0.005]}
\expandafter\def\csname res@flex.asom_clip.synpara.f1\endcsname{0.337}
\expandafter\def\csname res@flex.asom_clip.tenth\endcsname{0.694}
\expandafter\def\csname res@flex.asom_clip.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_clip.yesno_native\endcsname{0.596}
\expandafter\def\csname res@flex.asom_clip.yesno_nativeci\endcsname{[0.579, 0.612]}
\expandafter\def\csname res@flex.asom_clip.yesno_new_words\endcsname{0.556}
\expandafter\def\csname res@flex.asom_clip.yesno_new_wordsci\endcsname{[0.543, 0.573]}
\expandafter\def\csname res@flex.asom_em.bare_names.agree\endcsname{82.5}
\expandafter\def\csname res@flex.asom_em.bare_names.delta\endcsname{-0.028}
\expandafter\def\csname res@flex.asom_em.bare_names.deltaci\endcsname{[-0.057, -0.005]}
\expandafter\def\csname res@flex.asom_em.bare_names.f1\endcsname{0.336}
\expandafter\def\csname res@flex.asom_em.ccc.arousal\endcsname{0.674}
\expandafter\def\csname res@flex.asom_em.ccc.arousalci\endcsname{[0.581, 0.753]}
\expandafter\def\csname res@flex.asom_em.ccc.dominance\endcsname{0.584}
\expandafter\def\csname res@flex.asom_em.ccc.dominanceci\endcsname{[0.476, 0.715]}
\expandafter\def\csname res@flex.asom_em.ccc.valence\endcsname{0.735}
\expandafter\def\csname res@flex.asom_em.ccc.valenceci\endcsname{[0.674, 0.782]}
\expandafter\def\csname res@flex.asom_em.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_em.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_em.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flex.asom_em.gender\endcsname{0.686}
\expandafter\def\csname res@flex.asom_em.instr2.agree\endcsname{88.0}
\expandafter\def\csname res@flex.asom_em.instr2.delta\endcsname{+0.013}
\expandafter\def\csname res@flex.asom_em.instr2.deltaci\endcsname{[-0.011, +0.037]}
\expandafter\def\csname res@flex.asom_em.instr2.f1\endcsname{0.376}
\expandafter\def\csname res@flex.asom_em.native.f1\endcsname{0.363}
\expandafter\def\csname res@flex.asom_em.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_em.newwords_oracle\endcsname{0.739}
\expandafter\def\csname res@flex.asom_em.para1.agree\endcsname{92.7}
\expandafter\def\csname res@flex.asom_em.para1.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.asom_em.para1.deltaci\endcsname{[-0.021, +0.017]}
\expandafter\def\csname res@flex.asom_em.para1.f1\endcsname{0.364}
\expandafter\def\csname res@flex.asom_em.para2.agree\endcsname{90.4}
\expandafter\def\csname res@flex.asom_em.para2.delta\endcsname{+0.009}
\expandafter\def\csname res@flex.asom_em.para2.deltaci\endcsname{[-0.014, +0.029]}
\expandafter\def\csname res@flex.asom_em.para2.f1\endcsname{0.372}
\expandafter\def\csname res@flex.asom_em.redagree\endcsname{99.5}
\expandafter\def\csname res@flex.asom_em.synpara.agree\endcsname{91.0}
\expandafter\def\csname res@flex.asom_em.synpara.delta\endcsname{+0.004}
\expandafter\def\csname res@flex.asom_em.synpara.deltaci\endcsname{[-0.022, +0.033]}
\expandafter\def\csname res@flex.asom_em.synpara.f1\endcsname{0.368}
\expandafter\def\csname res@flex.asom_em.tenth\endcsname{0.701}
\expandafter\def\csname res@flex.asom_em.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_em.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_em.yesno_nativeci\endcsname{[0.743, 0.784]}
\expandafter\def\csname res@flex.asom_em.yesno_new_words\endcsname{0.714}
\expandafter\def\csname res@flex.asom_em.yesno_new_wordsci\endcsname{[0.686, 0.742]}
\expandafter\def\csname res@flex.asom_u.bare_names.agree\endcsname{82.5}
\expandafter\def\csname res@flex.asom_u.bare_names.delta\endcsname{-0.028}
\expandafter\def\csname res@flex.asom_u.bare_names.deltaci\endcsname{[-0.057, -0.005]}
\expandafter\def\csname res@flex.asom_u.bare_names.f1\endcsname{0.336}
\expandafter\def\csname res@flex.asom_u.ccc.arousal\endcsname{0.674}
\expandafter\def\csname res@flex.asom_u.ccc.arousalci\endcsname{[0.581, 0.753]}
\expandafter\def\csname res@flex.asom_u.ccc.dominance\endcsname{0.584}
\expandafter\def\csname res@flex.asom_u.ccc.dominanceci\endcsname{[0.476, 0.715]}
\expandafter\def\csname res@flex.asom_u.ccc.valence\endcsname{0.735}
\expandafter\def\csname res@flex.asom_u.ccc.valenceci\endcsname{[0.674, 0.782]}
\expandafter\def\csname res@flex.asom_u.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_u.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_u.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flex.asom_u.gender\endcsname{0.686}
\expandafter\def\csname res@flex.asom_u.instr2.agree\endcsname{88.0}
\expandafter\def\csname res@flex.asom_u.instr2.delta\endcsname{+0.013}
\expandafter\def\csname res@flex.asom_u.instr2.deltaci\endcsname{[-0.011, +0.037]}
\expandafter\def\csname res@flex.asom_u.instr2.f1\endcsname{0.376}
\expandafter\def\csname res@flex.asom_u.native.f1\endcsname{0.363}
\expandafter\def\csname res@flex.asom_u.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_u.newwords_oracle\endcsname{0.739}
\expandafter\def\csname res@flex.asom_u.para1.agree\endcsname{92.7}
\expandafter\def\csname res@flex.asom_u.para1.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.asom_u.para1.deltaci\endcsname{[-0.021, +0.017]}
\expandafter\def\csname res@flex.asom_u.para1.f1\endcsname{0.364}
\expandafter\def\csname res@flex.asom_u.para2.agree\endcsname{90.4}
\expandafter\def\csname res@flex.asom_u.para2.delta\endcsname{+0.009}
\expandafter\def\csname res@flex.asom_u.para2.deltaci\endcsname{[-0.014, +0.029]}
\expandafter\def\csname res@flex.asom_u.para2.f1\endcsname{0.372}
\expandafter\def\csname res@flex.asom_u.redagree\endcsname{99.5}
\expandafter\def\csname res@flex.asom_u.synpara.agree\endcsname{91.0}
\expandafter\def\csname res@flex.asom_u.synpara.delta\endcsname{+0.004}
\expandafter\def\csname res@flex.asom_u.synpara.deltaci\endcsname{[-0.022, +0.033]}
\expandafter\def\csname res@flex.asom_u.synpara.f1\endcsname{0.368}
\expandafter\def\csname res@flex.asom_u.tenth\endcsname{0.701}
\expandafter\def\csname res@flex.asom_u.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_u.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_u.yesno_nativeci\endcsname{[0.743, 0.784]}
\expandafter\def\csname res@flex.asom_u.yesno_new_words\endcsname{0.714}
\expandafter\def\csname res@flex.asom_u.yesno_new_wordsci\endcsname{[0.686, 0.742]}
\expandafter\def\csname res@flex.asom_v2.bare_names.agree\endcsname{89.1}
\expandafter\def\csname res@flex.asom_v2.bare_names.delta\endcsname{-0.021}
\expandafter\def\csname res@flex.asom_v2.bare_names.deltaci\endcsname{[-0.040, -0.007]}
\expandafter\def\csname res@flex.asom_v2.bare_names.f1\endcsname{0.321}
\expandafter\def\csname res@flex.asom_v2.ccc.arousal\endcsname{0.670}
\expandafter\def\csname res@flex.asom_v2.ccc.arousalci\endcsname{[0.577, 0.753]}
\expandafter\def\csname res@flex.asom_v2.ccc.dominance\endcsname{0.578}
\expandafter\def\csname res@flex.asom_v2.ccc.dominanceci\endcsname{[0.468, 0.712]}
\expandafter\def\csname res@flex.asom_v2.ccc.valence\endcsname{0.733}
\expandafter\def\csname res@flex.asom_v2.ccc.valenceci\endcsname{[0.677, 0.777]}
\expandafter\def\csname res@flex.asom_v2.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flex.asom_v2.gender\endcsname{0.686}
\expandafter\def\csname res@flex.asom_v2.genderref\endcsname{0.904}
\expandafter\def\csname res@flex.asom_v2.genderrefci\endcsname{[0.824, 0.955]}
\expandafter\def\csname res@flex.asom_v2.instr2.agree\endcsname{86.9}
\expandafter\def\csname res@flex.asom_v2.instr2.delta\endcsname{+0.019}
\expandafter\def\csname res@flex.asom_v2.instr2.deltaci\endcsname{[-0.003, +0.047]}
\expandafter\def\csname res@flex.asom_v2.instr2.f1\endcsname{0.361}
\expandafter\def\csname res@flex.asom_v2.native.f1\endcsname{0.342}
\expandafter\def\csname res@flex.asom_v2.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2.newwords_oracle\endcsname{0.740}
\expandafter\def\csname res@flex.asom_v2.para1.agree\endcsname{90.1}
\expandafter\def\csname res@flex.asom_v2.para1.delta\endcsname{+0.018}
\expandafter\def\csname res@flex.asom_v2.para1.deltaci\endcsname{[+0.001, +0.040]}
\expandafter\def\csname res@flex.asom_v2.para1.f1\endcsname{0.359}
\expandafter\def\csname res@flex.asom_v2.para2.agree\endcsname{88.5}
\expandafter\def\csname res@flex.asom_v2.para2.delta\endcsname{+0.003}
\expandafter\def\csname res@flex.asom_v2.para2.deltaci\endcsname{[-0.012, +0.026]}
\expandafter\def\csname res@flex.asom_v2.para2.f1\endcsname{0.345}
\expandafter\def\csname res@flex.asom_v2.redagree\endcsname{99.4}
\expandafter\def\csname res@flex.asom_v2.synpara.agree\endcsname{86.5}
\expandafter\def\csname res@flex.asom_v2.synpara.delta\endcsname{+0.010}
\expandafter\def\csname res@flex.asom_v2.synpara.deltaci\endcsname{[-0.008, +0.034]}
\expandafter\def\csname res@flex.asom_v2.synpara.f1\endcsname{0.351}
\expandafter\def\csname res@flex.asom_v2.tenth\endcsname{0.694}
\expandafter\def\csname res@flex.asom_v2.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_v2.yesno_native\endcsname{0.758}
\expandafter\def\csname res@flex.asom_v2.yesno_nativeci\endcsname{[0.738, 0.783]}
\expandafter\def\csname res@flex.asom_v2.yesno_new_words\endcsname{0.707}
\expandafter\def\csname res@flex.asom_v2.yesno_new_wordsci\endcsname{[0.665, 0.745]}
\expandafter\def\csname res@flex.asom_v2_u.bare_names.agree\endcsname{88.6}
\expandafter\def\csname res@flex.asom_v2_u.bare_names.delta\endcsname{-0.029}
\expandafter\def\csname res@flex.asom_v2_u.bare_names.deltaci\endcsname{[-0.057, -0.008]}
\expandafter\def\csname res@flex.asom_v2_u.bare_names.f1\endcsname{0.344}
\expandafter\def\csname res@flex.asom_v2_u.ccc.arousal\endcsname{0.670}
\expandafter\def\csname res@flex.asom_v2_u.ccc.arousalci\endcsname{[0.577, 0.753]}
\expandafter\def\csname res@flex.asom_v2_u.ccc.dominance\endcsname{0.578}
\expandafter\def\csname res@flex.asom_v2_u.ccc.dominanceci\endcsname{[0.468, 0.712]}
\expandafter\def\csname res@flex.asom_v2_u.ccc.valence\endcsname{0.733}
\expandafter\def\csname res@flex.asom_v2_u.ccc.valenceci\endcsname{[0.677, 0.777]}
\expandafter\def\csname res@flex.asom_v2_u.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2_u.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2_u.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flex.asom_v2_u.gender\endcsname{0.688}
\expandafter\def\csname res@flex.asom_v2_u.instr2.agree\endcsname{90.5}
\expandafter\def\csname res@flex.asom_v2_u.instr2.delta\endcsname{-0.004}
\expandafter\def\csname res@flex.asom_v2_u.instr2.deltaci\endcsname{[-0.016, +0.009]}
\expandafter\def\csname res@flex.asom_v2_u.instr2.f1\endcsname{0.368}
\expandafter\def\csname res@flex.asom_v2_u.native.f1\endcsname{0.373}
\expandafter\def\csname res@flex.asom_v2_u.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2_u.newwords_oracle\endcsname{0.738}
\expandafter\def\csname res@flex.asom_v2_u.para1.agree\endcsname{91.5}
\expandafter\def\csname res@flex.asom_v2_u.para1.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.asom_v2_u.para1.deltaci\endcsname{[-0.017, +0.017]}
\expandafter\def\csname res@flex.asom_v2_u.para1.f1\endcsname{0.373}
\expandafter\def\csname res@flex.asom_v2_u.para2.agree\endcsname{92.0}
\expandafter\def\csname res@flex.asom_v2_u.para2.delta\endcsname{-0.007}
\expandafter\def\csname res@flex.asom_v2_u.para2.deltaci\endcsname{[-0.022, +0.013]}
\expandafter\def\csname res@flex.asom_v2_u.para2.f1\endcsname{0.366}
\expandafter\def\csname res@flex.asom_v2_u.redagree\endcsname{99.6}
\expandafter\def\csname res@flex.asom_v2_u.synpara.agree\endcsname{89.1}
\expandafter\def\csname res@flex.asom_v2_u.synpara.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.asom_v2_u.synpara.deltaci\endcsname{[-0.020, +0.021]}
\expandafter\def\csname res@flex.asom_v2_u.synpara.f1\endcsname{0.373}
\expandafter\def\csname res@flex.asom_v2_u.tenth\endcsname{0.699}
\expandafter\def\csname res@flex.asom_v2_u.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2_u.yesno_native\endcsname{0.758}
\expandafter\def\csname res@flex.asom_v2_u.yesno_nativeci\endcsname{[0.738, 0.783]}
\expandafter\def\csname res@flex.asom_v2_u.yesno_new_words\endcsname{0.707}
\expandafter\def\csname res@flex.asom_v2_u.yesno_new_wordsci\endcsname{[0.665, 0.745]}
\expandafter\def\csname res@flex.asom_v2_vg.bare_names.agree\endcsname{87.7}
\expandafter\def\csname res@flex.asom_v2_vg.bare_names.delta\endcsname{-0.045}
\expandafter\def\csname res@flex.asom_v2_vg.bare_names.deltaci\endcsname{[-0.072, -0.018]}
\expandafter\def\csname res@flex.asom_v2_vg.bare_names.f1\endcsname{0.321}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.arousal\endcsname{0.675}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.arousalci\endcsname{[0.586, 0.757]}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.dominance\endcsname{0.583}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.dominanceci\endcsname{[0.476, 0.717]}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.valence\endcsname{0.739}
\expandafter\def\csname res@flex.asom_v2_vg.ccc.valenceci\endcsname{[0.682, 0.784]}
\expandafter\def\csname res@flex.asom_v2_vg.ccc2.arousal\endcsname{0.68}
\expandafter\def\csname res@flex.asom_v2_vg.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2_vg.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2_vg.gender\endcsname{0.503}
\expandafter\def\csname res@flex.asom_v2_vg.genderref\endcsname{0.844}
\expandafter\def\csname res@flex.asom_v2_vg.genderrefci\endcsname{[0.788, 0.895]}
\expandafter\def\csname res@flex.asom_v2_vg.instr2.agree\endcsname{84.4}
\expandafter\def\csname res@flex.asom_v2_vg.instr2.delta\endcsname{+0.028}
\expandafter\def\csname res@flex.asom_v2_vg.instr2.deltaci\endcsname{[-0.005, +0.067]}
\expandafter\def\csname res@flex.asom_v2_vg.instr2.f1\endcsname{0.394}
\expandafter\def\csname res@flex.asom_v2_vg.native.f1\endcsname{0.365}
\expandafter\def\csname res@flex.asom_v2_vg.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2_vg.newwords_oracle\endcsname{0.740}
\expandafter\def\csname res@flex.asom_v2_vg.para1.agree\endcsname{90.2}
\expandafter\def\csname res@flex.asom_v2_vg.para1.delta\endcsname{+0.020}
\expandafter\def\csname res@flex.asom_v2_vg.para1.deltaci\endcsname{[-0.010, +0.058]}
\expandafter\def\csname res@flex.asom_v2_vg.para1.f1\endcsname{0.385}
\expandafter\def\csname res@flex.asom_v2_vg.para2.agree\endcsname{84.1}
\expandafter\def\csname res@flex.asom_v2_vg.para2.delta\endcsname{+0.006}
\expandafter\def\csname res@flex.asom_v2_vg.para2.deltaci\endcsname{[-0.022, +0.044]}
\expandafter\def\csname res@flex.asom_v2_vg.para2.f1\endcsname{0.372}
\expandafter\def\csname res@flex.asom_v2_vg.redagree\endcsname{99.3}
\expandafter\def\csname res@flex.asom_v2_vg.synpara.agree\endcsname{84.5}
\expandafter\def\csname res@flex.asom_v2_vg.synpara.delta\endcsname{+0.014}
\expandafter\def\csname res@flex.asom_v2_vg.synpara.deltaci\endcsname{[-0.017, +0.055]}
\expandafter\def\csname res@flex.asom_v2_vg.synpara.f1\endcsname{0.379}
\expandafter\def\csname res@flex.asom_v2_vg.tenth\endcsname{0.700}
\expandafter\def\csname res@flex.asom_v2_vg.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_v2_vg.yesno_native\endcsname{0.757}
\expandafter\def\csname res@flex.asom_v2_vg.yesno_nativeci\endcsname{[0.737, 0.781]}
\expandafter\def\csname res@flex.asom_v2_vg.yesno_new_words\endcsname{0.713}
\expandafter\def\csname res@flex.asom_v2_vg.yesno_new_wordsci\endcsname{[0.679, 0.745]}
\expandafter\def\csname res@flex.asom_v2_vg_u.bare_names.agree\endcsname{85.7}
\expandafter\def\csname res@flex.asom_v2_vg_u.bare_names.delta\endcsname{-0.019}
\expandafter\def\csname res@flex.asom_v2_vg_u.bare_names.deltaci\endcsname{[-0.053, +0.009]}
\expandafter\def\csname res@flex.asom_v2_vg_u.bare_names.f1\endcsname{0.372}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.arousal\endcsname{0.675}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.arousalci\endcsname{[0.586, 0.757]}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.dominance\endcsname{0.583}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.dominanceci\endcsname{[0.476, 0.717]}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.valence\endcsname{0.739}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc.valenceci\endcsname{[0.682, 0.784]}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc2.arousal\endcsname{0.68}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2_vg_u.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2_vg_u.gender\endcsname{0.565}
\expandafter\def\csname res@flex.asom_v2_vg_u.instr2.agree\endcsname{90.3}
\expandafter\def\csname res@flex.asom_v2_vg_u.instr2.delta\endcsname{-0.002}
\expandafter\def\csname res@flex.asom_v2_vg_u.instr2.deltaci\endcsname{[-0.020, +0.020]}
\expandafter\def\csname res@flex.asom_v2_vg_u.instr2.f1\endcsname{0.388}
\expandafter\def\csname res@flex.asom_v2_vg_u.native.f1\endcsname{0.391}
\expandafter\def\csname res@flex.asom_v2_vg_u.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2_vg_u.newwords_oracle\endcsname{0.739}
\expandafter\def\csname res@flex.asom_v2_vg_u.para1.agree\endcsname{92.2}
\expandafter\def\csname res@flex.asom_v2_vg_u.para1.delta\endcsname{-0.004}
\expandafter\def\csname res@flex.asom_v2_vg_u.para1.deltaci\endcsname{[-0.028, +0.018]}
\expandafter\def\csname res@flex.asom_v2_vg_u.para1.f1\endcsname{0.386}
\expandafter\def\csname res@flex.asom_v2_vg_u.para2.agree\endcsname{89.9}
\expandafter\def\csname res@flex.asom_v2_vg_u.para2.delta\endcsname{-0.002}
\expandafter\def\csname res@flex.asom_v2_vg_u.para2.deltaci\endcsname{[-0.017, +0.015]}
\expandafter\def\csname res@flex.asom_v2_vg_u.para2.f1\endcsname{0.388}
\expandafter\def\csname res@flex.asom_v2_vg_u.redagree\endcsname{99.5}
\expandafter\def\csname res@flex.asom_v2_vg_u.synpara.agree\endcsname{88.2}
\expandafter\def\csname res@flex.asom_v2_vg_u.synpara.delta\endcsname{-0.012}
\expandafter\def\csname res@flex.asom_v2_vg_u.synpara.deltaci\endcsname{[-0.037, +0.012]}
\expandafter\def\csname res@flex.asom_v2_vg_u.synpara.f1\endcsname{0.378}
\expandafter\def\csname res@flex.asom_v2_vg_u.tenth\endcsname{0.704}
\expandafter\def\csname res@flex.asom_v2_vg_u.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2_vg_u.yesno_native\endcsname{0.757}
\expandafter\def\csname res@flex.asom_v2_vg_u.yesno_nativeci\endcsname{[0.737, 0.781]}
\expandafter\def\csname res@flex.asom_v2_vg_u.yesno_new_words\endcsname{0.713}
\expandafter\def\csname res@flex.asom_v2_vg_u.yesno_new_wordsci\endcsname{[0.679, 0.745]}
\expandafter\def\csname res@flex.asom_v2na.bare_names.agree\endcsname{87.9}
\expandafter\def\csname res@flex.asom_v2na.bare_names.delta\endcsname{-0.046}
\expandafter\def\csname res@flex.asom_v2na.bare_names.deltaci\endcsname{[-0.075, -0.025]}
\expandafter\def\csname res@flex.asom_v2na.bare_names.f1\endcsname{0.306}
\expandafter\def\csname res@flex.asom_v2na.ccc.arousal\endcsname{0.669}
\expandafter\def\csname res@flex.asom_v2na.ccc.arousalci\endcsname{[0.577, 0.753]}
\expandafter\def\csname res@flex.asom_v2na.ccc.dominance\endcsname{0.582}
\expandafter\def\csname res@flex.asom_v2na.ccc.dominanceci\endcsname{[0.474, 0.716]}
\expandafter\def\csname res@flex.asom_v2na.ccc.valence\endcsname{0.737}
\expandafter\def\csname res@flex.asom_v2na.ccc.valenceci\endcsname{[0.683, 0.780]}
\expandafter\def\csname res@flex.asom_v2na.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2na.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2na.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2na.gender\endcsname{0.689}
\expandafter\def\csname res@flex.asom_v2na.genderref\endcsname{0.899}
\expandafter\def\csname res@flex.asom_v2na.genderrefci\endcsname{[0.799, 0.960]}
\expandafter\def\csname res@flex.asom_v2na.instr2.agree\endcsname{87.5}
\expandafter\def\csname res@flex.asom_v2na.instr2.delta\endcsname{+0.010}
\expandafter\def\csname res@flex.asom_v2na.instr2.deltaci\endcsname{[-0.007, +0.033]}
\expandafter\def\csname res@flex.asom_v2na.instr2.f1\endcsname{0.361}
\expandafter\def\csname res@flex.asom_v2na.native.f1\endcsname{0.351}
\expandafter\def\csname res@flex.asom_v2na.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom_v2na.newwords_oracle\endcsname{0.742}
\expandafter\def\csname res@flex.asom_v2na.para1.agree\endcsname{91.5}
\expandafter\def\csname res@flex.asom_v2na.para1.delta\endcsname{+0.013}
\expandafter\def\csname res@flex.asom_v2na.para1.deltaci\endcsname{[-0.001, +0.030]}
\expandafter\def\csname res@flex.asom_v2na.para1.f1\endcsname{0.364}
\expandafter\def\csname res@flex.asom_v2na.para2.agree\endcsname{89.1}
\expandafter\def\csname res@flex.asom_v2na.para2.delta\endcsname{-0.002}
\expandafter\def\csname res@flex.asom_v2na.para2.deltaci\endcsname{[-0.015, +0.017]}
\expandafter\def\csname res@flex.asom_v2na.para2.f1\endcsname{0.349}
\expandafter\def\csname res@flex.asom_v2na.redagree\endcsname{99.3}
\expandafter\def\csname res@flex.asom_v2na.synpara.agree\endcsname{88.2}
\expandafter\def\csname res@flex.asom_v2na.synpara.delta\endcsname{+0.008}
\expandafter\def\csname res@flex.asom_v2na.synpara.deltaci\endcsname{[-0.006, +0.028]}
\expandafter\def\csname res@flex.asom_v2na.synpara.f1\endcsname{0.360}
\expandafter\def\csname res@flex.asom_v2na.tenth\endcsname{0.700}
\expandafter\def\csname res@flex.asom_v2na.tv\endcsname{0.004}
\expandafter\def\csname res@flex.asom_v2na.yesno_native\endcsname{0.760}
\expandafter\def\csname res@flex.asom_v2na.yesno_nativeci\endcsname{[0.740, 0.783]}
\expandafter\def\csname res@flex.asom_v2na.yesno_new_words\endcsname{0.709}
\expandafter\def\csname res@flex.asom_v2na.yesno_new_wordsci\endcsname{[0.673, 0.743]}
\expandafter\def\csname res@flex.asom_v2na_u.bare_names.agree\endcsname{86.2}
\expandafter\def\csname res@flex.asom_v2na_u.bare_names.delta\endcsname{-0.025}
\expandafter\def\csname res@flex.asom_v2na_u.bare_names.deltaci\endcsname{[-0.051, -0.007]}
\expandafter\def\csname res@flex.asom_v2na_u.bare_names.f1\endcsname{0.343}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.arousal\endcsname{0.669}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.arousalci\endcsname{[0.577, 0.753]}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.dominance\endcsname{0.582}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.dominanceci\endcsname{[0.474, 0.716]}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.valence\endcsname{0.737}
\expandafter\def\csname res@flex.asom_v2na_u.ccc.valenceci\endcsname{[0.683, 0.780]}
\expandafter\def\csname res@flex.asom_v2na_u.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2na_u.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2na_u.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2na_u.gender\endcsname{0.694}
\expandafter\def\csname res@flex.asom_v2na_u.instr2.agree\endcsname{91.9}
\expandafter\def\csname res@flex.asom_v2na_u.instr2.delta\endcsname{+0.004}
\expandafter\def\csname res@flex.asom_v2na_u.instr2.deltaci\endcsname{[-0.010, +0.018]}
\expandafter\def\csname res@flex.asom_v2na_u.instr2.f1\endcsname{0.372}
\expandafter\def\csname res@flex.asom_v2na_u.native.f1\endcsname{0.368}
\expandafter\def\csname res@flex.asom_v2na_u.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom_v2na_u.newwords_oracle\endcsname{0.740}
\expandafter\def\csname res@flex.asom_v2na_u.para1.agree\endcsname{93.2}
\expandafter\def\csname res@flex.asom_v2na_u.para1.delta\endcsname{+0.015}
\expandafter\def\csname res@flex.asom_v2na_u.para1.deltaci\endcsname{[-0.003, +0.030]}
\expandafter\def\csname res@flex.asom_v2na_u.para1.f1\endcsname{0.383}
\expandafter\def\csname res@flex.asom_v2na_u.para2.agree\endcsname{92.8}
\expandafter\def\csname res@flex.asom_v2na_u.para2.delta\endcsname{-0.005}
\expandafter\def\csname res@flex.asom_v2na_u.para2.deltaci\endcsname{[-0.023, +0.011]}
\expandafter\def\csname res@flex.asom_v2na_u.para2.f1\endcsname{0.363}
\expandafter\def\csname res@flex.asom_v2na_u.redagree\endcsname{99.6}
\expandafter\def\csname res@flex.asom_v2na_u.synpara.agree\endcsname{91.0}
\expandafter\def\csname res@flex.asom_v2na_u.synpara.delta\endcsname{+0.013}
\expandafter\def\csname res@flex.asom_v2na_u.synpara.deltaci\endcsname{[-0.005, +0.028]}
\expandafter\def\csname res@flex.asom_v2na_u.synpara.f1\endcsname{0.381}
\expandafter\def\csname res@flex.asom_v2na_u.tenth\endcsname{0.703}
\expandafter\def\csname res@flex.asom_v2na_u.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2na_u.yesno_native\endcsname{0.760}
\expandafter\def\csname res@flex.asom_v2na_u.yesno_nativeci\endcsname{[0.740, 0.783]}
\expandafter\def\csname res@flex.asom_v2na_u.yesno_new_words\endcsname{0.709}
\expandafter\def\csname res@flex.asom_v2na_u.yesno_new_wordsci\endcsname{[0.673, 0.743]}
\expandafter\def\csname res@flex.asom_v2sp.bare_names.agree\endcsname{84.8}
\expandafter\def\csname res@flex.asom_v2sp.bare_names.delta\endcsname{-0.063}
\expandafter\def\csname res@flex.asom_v2sp.bare_names.deltaci\endcsname{[-0.108, -0.036]}
\expandafter\def\csname res@flex.asom_v2sp.bare_names.f1\endcsname{0.279}
\expandafter\def\csname res@flex.asom_v2sp.ccc.arousal\endcsname{0.669}
\expandafter\def\csname res@flex.asom_v2sp.ccc.arousalci\endcsname{[0.574, 0.755]}
\expandafter\def\csname res@flex.asom_v2sp.ccc.dominance\endcsname{0.583}
\expandafter\def\csname res@flex.asom_v2sp.ccc.dominanceci\endcsname{[0.474, 0.717]}
\expandafter\def\csname res@flex.asom_v2sp.ccc.valence\endcsname{0.738}
\expandafter\def\csname res@flex.asom_v2sp.ccc.valenceci\endcsname{[0.683, 0.780]}
\expandafter\def\csname res@flex.asom_v2sp.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2sp.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2sp.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2sp.gender\endcsname{0.685}
\expandafter\def\csname res@flex.asom_v2sp.genderref\endcsname{0.900}
\expandafter\def\csname res@flex.asom_v2sp.genderrefci\endcsname{[0.807, 0.959]}
\expandafter\def\csname res@flex.asom_v2sp.instr2.agree\endcsname{87.0}
\expandafter\def\csname res@flex.asom_v2sp.instr2.delta\endcsname{+0.024}
\expandafter\def\csname res@flex.asom_v2sp.instr2.deltaci\endcsname{[+0.003, +0.049]}
\expandafter\def\csname res@flex.asom_v2sp.instr2.f1\endcsname{0.366}
\expandafter\def\csname res@flex.asom_v2sp.native.f1\endcsname{0.342}
\expandafter\def\csname res@flex.asom_v2sp.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.asom_v2sp.newwords_oracle\endcsname{0.741}
\expandafter\def\csname res@flex.asom_v2sp.para1.agree\endcsname{93.6}
\expandafter\def\csname res@flex.asom_v2sp.para1.delta\endcsname{+0.005}
\expandafter\def\csname res@flex.asom_v2sp.para1.deltaci\endcsname{[-0.007, +0.019]}
\expandafter\def\csname res@flex.asom_v2sp.para1.f1\endcsname{0.347}
\expandafter\def\csname res@flex.asom_v2sp.para2.agree\endcsname{88.8}
\expandafter\def\csname res@flex.asom_v2sp.para2.delta\endcsname{+0.003}
\expandafter\def\csname res@flex.asom_v2sp.para2.deltaci\endcsname{[-0.013, +0.022]}
\expandafter\def\csname res@flex.asom_v2sp.para2.f1\endcsname{0.345}
\expandafter\def\csname res@flex.asom_v2sp.redagree\endcsname{99.5}
\expandafter\def\csname res@flex.asom_v2sp.synpara.agree\endcsname{88.8}
\expandafter\def\csname res@flex.asom_v2sp.synpara.delta\endcsname{+0.018}
\expandafter\def\csname res@flex.asom_v2sp.synpara.deltaci\endcsname{[-0.002, +0.040]}
\expandafter\def\csname res@flex.asom_v2sp.synpara.f1\endcsname{0.360}
\expandafter\def\csname res@flex.asom_v2sp.tenth\endcsname{0.692}
\expandafter\def\csname res@flex.asom_v2sp.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2sp.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_v2sp.yesno_nativeci\endcsname{[0.742, 0.786]}
\expandafter\def\csname res@flex.asom_v2sp.yesno_new_words\endcsname{0.708}
\expandafter\def\csname res@flex.asom_v2sp.yesno_new_wordsci\endcsname{[0.670, 0.744]}
\expandafter\def\csname res@flex.asom_v2sp_em.bare_names.agree\endcsname{83.9}
\expandafter\def\csname res@flex.asom_v2sp_em.bare_names.delta\endcsname{-0.036}
\expandafter\def\csname res@flex.asom_v2sp_em.bare_names.deltaci\endcsname{[-0.069, -0.006]}
\expandafter\def\csname res@flex.asom_v2sp_em.bare_names.f1\endcsname{0.334}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.arousal\endcsname{0.669}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.arousalci\endcsname{[0.574, 0.755]}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.dominance\endcsname{0.583}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.dominanceci\endcsname{[0.474, 0.717]}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.valence\endcsname{0.738}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc.valenceci\endcsname{[0.683, 0.780]}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2sp_em.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2sp_em.gender\endcsname{0.690}
\expandafter\def\csname res@flex.asom_v2sp_em.instr2.agree\endcsname{91.0}
\expandafter\def\csname res@flex.asom_v2sp_em.instr2.delta\endcsname{+0.012}
\expandafter\def\csname res@flex.asom_v2sp_em.instr2.deltaci\endcsname{[-0.002, +0.028]}
\expandafter\def\csname res@flex.asom_v2sp_em.instr2.f1\endcsname{0.383}
\expandafter\def\csname res@flex.asom_v2sp_em.native.f1\endcsname{0.371}
\expandafter\def\csname res@flex.asom_v2sp_em.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2sp_em.newwords_oracle\endcsname{0.739}
\expandafter\def\csname res@flex.asom_v2sp_em.para1.agree\endcsname{92.8}
\expandafter\def\csname res@flex.asom_v2sp_em.para1.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.asom_v2sp_em.para1.deltaci\endcsname{[-0.028, +0.013]}
\expandafter\def\csname res@flex.asom_v2sp_em.para1.f1\endcsname{0.365}
\expandafter\def\csname res@flex.asom_v2sp_em.para2.agree\endcsname{91.6}
\expandafter\def\csname res@flex.asom_v2sp_em.para2.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.asom_v2sp_em.para2.deltaci\endcsname{[-0.021, +0.010]}
\expandafter\def\csname res@flex.asom_v2sp_em.para2.f1\endcsname{0.365}
\expandafter\def\csname res@flex.asom_v2sp_em.redagree\endcsname{99.6}
\expandafter\def\csname res@flex.asom_v2sp_em.synpara.agree\endcsname{89.1}
\expandafter\def\csname res@flex.asom_v2sp_em.synpara.delta\endcsname{-0.000}
\expandafter\def\csname res@flex.asom_v2sp_em.synpara.deltaci\endcsname{[-0.028, +0.025]}
\expandafter\def\csname res@flex.asom_v2sp_em.synpara.f1\endcsname{0.371}
\expandafter\def\csname res@flex.asom_v2sp_em.tenth\endcsname{0.693}
\expandafter\def\csname res@flex.asom_v2sp_em.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2sp_em.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_v2sp_em.yesno_nativeci\endcsname{[0.742, 0.786]}
\expandafter\def\csname res@flex.asom_v2sp_em.yesno_new_words\endcsname{0.709}
\expandafter\def\csname res@flex.asom_v2sp_em.yesno_new_wordsci\endcsname{[0.671, 0.744]}
\expandafter\def\csname res@flex.asom_v2sp_u.bare_names.agree\endcsname{83.9}
\expandafter\def\csname res@flex.asom_v2sp_u.bare_names.delta\endcsname{-0.036}
\expandafter\def\csname res@flex.asom_v2sp_u.bare_names.deltaci\endcsname{[-0.069, -0.006]}
\expandafter\def\csname res@flex.asom_v2sp_u.bare_names.f1\endcsname{0.334}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.arousal\endcsname{0.669}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.arousalci\endcsname{[0.574, 0.755]}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.dominance\endcsname{0.583}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.dominanceci\endcsname{[0.474, 0.717]}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.valence\endcsname{0.738}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc.valenceci\endcsname{[0.683, 0.780]}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.asom_v2sp_u.ccc2.valence\endcsname{0.74}
\expandafter\def\csname res@flex.asom_v2sp_u.gender\endcsname{0.690}
\expandafter\def\csname res@flex.asom_v2sp_u.instr2.agree\endcsname{91.0}
\expandafter\def\csname res@flex.asom_v2sp_u.instr2.delta\endcsname{+0.012}
\expandafter\def\csname res@flex.asom_v2sp_u.instr2.deltaci\endcsname{[-0.002, +0.028]}
\expandafter\def\csname res@flex.asom_v2sp_u.instr2.f1\endcsname{0.383}
\expandafter\def\csname res@flex.asom_v2sp_u.native.f1\endcsname{0.371}
\expandafter\def\csname res@flex.asom_v2sp_u.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.asom_v2sp_u.newwords_oracle\endcsname{0.739}
\expandafter\def\csname res@flex.asom_v2sp_u.para1.agree\endcsname{92.8}
\expandafter\def\csname res@flex.asom_v2sp_u.para1.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.asom_v2sp_u.para1.deltaci\endcsname{[-0.028, +0.013]}
\expandafter\def\csname res@flex.asom_v2sp_u.para1.f1\endcsname{0.365}
\expandafter\def\csname res@flex.asom_v2sp_u.para2.agree\endcsname{91.6}
\expandafter\def\csname res@flex.asom_v2sp_u.para2.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.asom_v2sp_u.para2.deltaci\endcsname{[-0.021, +0.010]}
\expandafter\def\csname res@flex.asom_v2sp_u.para2.f1\endcsname{0.365}
\expandafter\def\csname res@flex.asom_v2sp_u.redagree\endcsname{99.6}
\expandafter\def\csname res@flex.asom_v2sp_u.synpara.agree\endcsname{89.1}
\expandafter\def\csname res@flex.asom_v2sp_u.synpara.delta\endcsname{-0.000}
\expandafter\def\csname res@flex.asom_v2sp_u.synpara.deltaci\endcsname{[-0.028, +0.025]}
\expandafter\def\csname res@flex.asom_v2sp_u.synpara.f1\endcsname{0.371}
\expandafter\def\csname res@flex.asom_v2sp_u.tenth\endcsname{0.693}
\expandafter\def\csname res@flex.asom_v2sp_u.tv\endcsname{0.003}
\expandafter\def\csname res@flex.asom_v2sp_u.yesno_native\endcsname{0.762}
\expandafter\def\csname res@flex.asom_v2sp_u.yesno_nativeci\endcsname{[0.742, 0.786]}
\expandafter\def\csname res@flex.asom_v2sp_u.yesno_new_words\endcsname{0.709}
\expandafter\def\csname res@flex.asom_v2sp_u.yesno_new_wordsci\endcsname{[0.671, 0.744]}
\expandafter\def\csname res@flex.clap_laion.bare_names.agree\endcsname{99.7}
\expandafter\def\csname res@flex.clap_laion.bare_names.delta\endcsname{-0.000}
\expandafter\def\csname res@flex.clap_laion.bare_names.deltaci\endcsname{[-0.002, +0.000]}
\expandafter\def\csname res@flex.clap_laion.bare_names.f1\endcsname{0.086}
\expandafter\def\csname res@flex.clap_laion.ccc.arousal\endcsname{0.281}
\expandafter\def\csname res@flex.clap_laion.ccc.arousalci\endcsname{[0.234, 0.315]}
\expandafter\def\csname res@flex.clap_laion.ccc.dominance\endcsname{-0.028}
\expandafter\def\csname res@flex.clap_laion.ccc.dominanceci\endcsname{[-0.052, 0.011]}
\expandafter\def\csname res@flex.clap_laion.ccc.valence\endcsname{-0.018}
\expandafter\def\csname res@flex.clap_laion.ccc.valenceci\endcsname{[-0.051, 0.032]}
\expandafter\def\csname res@flex.clap_laion.ccc2.arousal\endcsname{0.28}
\expandafter\def\csname res@flex.clap_laion.ccc2.dominance\endcsname{-0.03}
\expandafter\def\csname res@flex.clap_laion.ccc2.valence\endcsname{-0.02}
\expandafter\def\csname res@flex.clap_laion.gender\endcsname{0.685}
\expandafter\def\csname res@flex.clap_laion.genderref\endcsname{0.858}
\expandafter\def\csname res@flex.clap_laion.genderrefci\endcsname{[0.806, 0.900]}
\expandafter\def\csname res@flex.clap_laion.instr2.agree\endcsname{99.7}
\expandafter\def\csname res@flex.clap_laion.instr2.delta\endcsname{-0.000}
\expandafter\def\csname res@flex.clap_laion.instr2.deltaci\endcsname{[-0.002, +0.000]}
\expandafter\def\csname res@flex.clap_laion.instr2.f1\endcsname{0.086}
\expandafter\def\csname res@flex.clap_laion.native.f1\endcsname{0.086}
\expandafter\def\csname res@flex.clap_laion.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.clap_laion.newwords_oracle\endcsname{0.561}
\expandafter\def\csname res@flex.clap_laion.para1.agree\endcsname{99.7}
\expandafter\def\csname res@flex.clap_laion.para1.delta\endcsname{-0.000}
\expandafter\def\csname res@flex.clap_laion.para1.deltaci\endcsname{[-0.002, +0.000]}
\expandafter\def\csname res@flex.clap_laion.para1.f1\endcsname{0.086}
\expandafter\def\csname res@flex.clap_laion.para2.agree\endcsname{21.6}
\expandafter\def\csname res@flex.clap_laion.para2.delta\endcsname{-0.012}
\expandafter\def\csname res@flex.clap_laion.para2.deltaci\endcsname{[-0.036, +0.008]}
\expandafter\def\csname res@flex.clap_laion.para2.f1\endcsname{0.074}
\expandafter\def\csname res@flex.clap_laion.redagree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_laion.synpara.agree\endcsname{21.6}
\expandafter\def\csname res@flex.clap_laion.synpara.delta\endcsname{-0.012}
\expandafter\def\csname res@flex.clap_laion.synpara.deltaci\endcsname{[-0.036, +0.008]}
\expandafter\def\csname res@flex.clap_laion.synpara.f1\endcsname{0.074}
\expandafter\def\csname res@flex.clap_laion.tenth\endcsname{0.494}
\expandafter\def\csname res@flex.clap_laion.tv\endcsname{0.000}
\expandafter\def\csname res@flex.clap_laion.yesno_native\endcsname{0.521}
\expandafter\def\csname res@flex.clap_laion.yesno_nativeci\endcsname{[0.498, 0.542]}
\expandafter\def\csname res@flex.clap_laion.yesno_new_words\endcsname{0.508}
\expandafter\def\csname res@flex.clap_laion.yesno_new_wordsci\endcsname{[0.490, 0.524]}
\expandafter\def\csname res@flex.clap_laion_desc.bare_names.agree\endcsname{10.6}
\expandafter\def\csname res@flex.clap_laion_desc.bare_names.delta\endcsname{-0.018}
\expandafter\def\csname res@flex.clap_laion_desc.bare_names.deltaci\endcsname{[-0.043, +0.011]}
\expandafter\def\csname res@flex.clap_laion_desc.bare_names.f1\endcsname{0.088}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.arousal\endcsname{0.281}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.arousalci\endcsname{[0.234, 0.315]}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.dominance\endcsname{-0.028}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.dominanceci\endcsname{[-0.052, 0.011]}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.valence\endcsname{-0.018}
\expandafter\def\csname res@flex.clap_laion_desc.ccc.valenceci\endcsname{[-0.051, 0.032]}
\expandafter\def\csname res@flex.clap_laion_desc.ccc2.arousal\endcsname{0.28}
\expandafter\def\csname res@flex.clap_laion_desc.ccc2.dominance\endcsname{-0.03}
\expandafter\def\csname res@flex.clap_laion_desc.ccc2.valence\endcsname{-0.02}
\expandafter\def\csname res@flex.clap_laion_desc.gender\endcsname{0.685}
\expandafter\def\csname res@flex.clap_laion_desc.genderref\endcsname{0.858}
\expandafter\def\csname res@flex.clap_laion_desc.genderrefci\endcsname{[0.806, 0.900]}
\expandafter\def\csname res@flex.clap_laion_desc.instr2.agree\endcsname{99.8}
\expandafter\def\csname res@flex.clap_laion_desc.instr2.delta\endcsname{+0.001}
\expandafter\def\csname res@flex.clap_laion_desc.instr2.deltaci\endcsname{[-0.000, +0.004]}
\expandafter\def\csname res@flex.clap_laion_desc.instr2.f1\endcsname{0.107}
\expandafter\def\csname res@flex.clap_laion_desc.native.f1\endcsname{0.106}
\expandafter\def\csname res@flex.clap_laion_desc.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.clap_laion_desc.newwords_oracle\endcsname{0.556}
\expandafter\def\csname res@flex.clap_laion_desc.para1.agree\endcsname{27.0}
\expandafter\def\csname res@flex.clap_laion_desc.para1.delta\endcsname{+0.033}
\expandafter\def\csname res@flex.clap_laion_desc.para1.deltaci\endcsname{[+0.001, +0.070]}
\expandafter\def\csname res@flex.clap_laion_desc.para1.f1\endcsname{0.138}
\expandafter\def\csname res@flex.clap_laion_desc.para2.agree\endcsname{99.8}
\expandafter\def\csname res@flex.clap_laion_desc.para2.delta\endcsname{+0.001}
\expandafter\def\csname res@flex.clap_laion_desc.para2.deltaci\endcsname{[-0.000, +0.004]}
\expandafter\def\csname res@flex.clap_laion_desc.para2.f1\endcsname{0.107}
\expandafter\def\csname res@flex.clap_laion_desc.redagree\endcsname{99.9}
\expandafter\def\csname res@flex.clap_laion_desc.synpara.agree\endcsname{27.0}
\expandafter\def\csname res@flex.clap_laion_desc.synpara.delta\endcsname{+0.033}
\expandafter\def\csname res@flex.clap_laion_desc.synpara.deltaci\endcsname{[+0.001, +0.070]}
\expandafter\def\csname res@flex.clap_laion_desc.synpara.f1\endcsname{0.138}
\expandafter\def\csname res@flex.clap_laion_desc.tenth\endcsname{0.512}
\expandafter\def\csname res@flex.clap_laion_desc.tv\endcsname{0.001}
\expandafter\def\csname res@flex.clap_laion_desc.yesno_native\endcsname{0.514}
\expandafter\def\csname res@flex.clap_laion_desc.yesno_nativeci\endcsname{[0.496, 0.535]}
\expandafter\def\csname res@flex.clap_laion_desc.yesno_new_words\endcsname{0.529}
\expandafter\def\csname res@flex.clap_laion_desc.yesno_new_wordsci\endcsname{[0.502, 0.553]}
\expandafter\def\csname res@flex.clap_mlp.ccc.arousal\endcsname{0.638}
\expandafter\def\csname res@flex.clap_mlp.ccc.arousalci\endcsname{[0.540, 0.729]}
\expandafter\def\csname res@flex.clap_mlp.ccc.dominance\endcsname{0.540}
\expandafter\def\csname res@flex.clap_mlp.ccc.dominanceci\endcsname{[0.446, 0.659]}
\expandafter\def\csname res@flex.clap_mlp.ccc.valence\endcsname{0.404}
\expandafter\def\csname res@flex.clap_mlp.ccc.valenceci\endcsname{[0.325, 0.442]}
\expandafter\def\csname res@flex.clap_mlp.ccc2.arousal\endcsname{0.64}
\expandafter\def\csname res@flex.clap_mlp.ccc2.dominance\endcsname{0.54}
\expandafter\def\csname res@flex.clap_mlp.ccc2.valence\endcsname{0.40}
\expandafter\def\csname res@flex.clap_ms.bare_names.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms.bare_names.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_ms.bare_names.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_ms.bare_names.f1\endcsname{0.097}
\expandafter\def\csname res@flex.clap_ms.ccc.arousal\endcsname{0.480}
\expandafter\def\csname res@flex.clap_ms.ccc.arousalci\endcsname{[0.445, 0.510]}
\expandafter\def\csname res@flex.clap_ms.ccc.dominance\endcsname{0.071}
\expandafter\def\csname res@flex.clap_ms.ccc.dominanceci\endcsname{[-0.003, 0.169]}
\expandafter\def\csname res@flex.clap_ms.ccc.valence\endcsname{0.135}
\expandafter\def\csname res@flex.clap_ms.ccc.valenceci\endcsname{[0.081, 0.191]}
\expandafter\def\csname res@flex.clap_ms.ccc2.arousal\endcsname{0.48}
\expandafter\def\csname res@flex.clap_ms.ccc2.dominance\endcsname{0.07}
\expandafter\def\csname res@flex.clap_ms.ccc2.valence\endcsname{0.13}
\expandafter\def\csname res@flex.clap_ms.gender\endcsname{0.716}
\expandafter\def\csname res@flex.clap_ms.genderref\endcsname{0.907}
\expandafter\def\csname res@flex.clap_ms.genderrefci\endcsname{[0.872, 0.940]}
\expandafter\def\csname res@flex.clap_ms.instr2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms.instr2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_ms.instr2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_ms.instr2.f1\endcsname{0.097}
\expandafter\def\csname res@flex.clap_ms.native.f1\endcsname{0.097}
\expandafter\def\csname res@flex.clap_ms.newwords_above\endcsname{3}
\expandafter\def\csname res@flex.clap_ms.newwords_oracle\endcsname{0.616}
\expandafter\def\csname res@flex.clap_ms.para1.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms.para1.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_ms.para1.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_ms.para1.f1\endcsname{0.097}
\expandafter\def\csname res@flex.clap_ms.para2.agree\endcsname{40.2}
\expandafter\def\csname res@flex.clap_ms.para2.delta\endcsname{-0.017}
\expandafter\def\csname res@flex.clap_ms.para2.deltaci\endcsname{[-0.035, +0.002]}
\expandafter\def\csname res@flex.clap_ms.para2.f1\endcsname{0.080}
\expandafter\def\csname res@flex.clap_ms.redagree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms.synpara.agree\endcsname{40.2}
\expandafter\def\csname res@flex.clap_ms.synpara.delta\endcsname{-0.017}
\expandafter\def\csname res@flex.clap_ms.synpara.deltaci\endcsname{[-0.035, +0.002]}
\expandafter\def\csname res@flex.clap_ms.synpara.f1\endcsname{0.080}
\expandafter\def\csname res@flex.clap_ms.tenth\endcsname{0.579}
\expandafter\def\csname res@flex.clap_ms.tv\endcsname{0.000}
\expandafter\def\csname res@flex.clap_ms.yesno_native\endcsname{0.580}
\expandafter\def\csname res@flex.clap_ms.yesno_nativeci\endcsname{[0.554, 0.599]}
\expandafter\def\csname res@flex.clap_ms.yesno_new_words\endcsname{0.549}
\expandafter\def\csname res@flex.clap_ms.yesno_new_wordsci\endcsname{[0.520, 0.578]}
\expandafter\def\csname res@flex.clap_ms_desc.bare_names.agree\endcsname{4.7}
\expandafter\def\csname res@flex.clap_ms_desc.bare_names.delta\endcsname{+0.072}
\expandafter\def\csname res@flex.clap_ms_desc.bare_names.deltaci\endcsname{[+0.050, +0.089]}
\expandafter\def\csname res@flex.clap_ms_desc.bare_names.f1\endcsname{0.091}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.arousal\endcsname{0.480}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.arousalci\endcsname{[0.445, 0.510]}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.dominance\endcsname{0.071}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.dominanceci\endcsname{[-0.003, 0.169]}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.valence\endcsname{0.135}
\expandafter\def\csname res@flex.clap_ms_desc.ccc.valenceci\endcsname{[0.081, 0.191]}
\expandafter\def\csname res@flex.clap_ms_desc.ccc2.arousal\endcsname{0.48}
\expandafter\def\csname res@flex.clap_ms_desc.ccc2.dominance\endcsname{0.07}
\expandafter\def\csname res@flex.clap_ms_desc.ccc2.valence\endcsname{0.13}
\expandafter\def\csname res@flex.clap_ms_desc.gender\endcsname{0.716}
\expandafter\def\csname res@flex.clap_ms_desc.genderref\endcsname{0.907}
\expandafter\def\csname res@flex.clap_ms_desc.genderrefci\endcsname{[0.872, 0.940]}
\expandafter\def\csname res@flex.clap_ms_desc.instr2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms_desc.instr2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_ms_desc.instr2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_ms_desc.instr2.f1\endcsname{0.020}
\expandafter\def\csname res@flex.clap_ms_desc.native.f1\endcsname{0.020}
\expandafter\def\csname res@flex.clap_ms_desc.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.clap_ms_desc.newwords_oracle\endcsname{0.606}
\expandafter\def\csname res@flex.clap_ms_desc.para1.agree\endcsname{2.2}
\expandafter\def\csname res@flex.clap_ms_desc.para1.delta\endcsname{+0.093}
\expandafter\def\csname res@flex.clap_ms_desc.para1.deltaci\endcsname{[+0.078, +0.106]}
\expandafter\def\csname res@flex.clap_ms_desc.para1.f1\endcsname{0.113}
\expandafter\def\csname res@flex.clap_ms_desc.para2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms_desc.para2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_ms_desc.para2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_ms_desc.para2.f1\endcsname{0.020}
\expandafter\def\csname res@flex.clap_ms_desc.redagree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_ms_desc.synpara.agree\endcsname{2.2}
\expandafter\def\csname res@flex.clap_ms_desc.synpara.delta\endcsname{+0.093}
\expandafter\def\csname res@flex.clap_ms_desc.synpara.deltaci\endcsname{[+0.078, +0.106]}
\expandafter\def\csname res@flex.clap_ms_desc.synpara.f1\endcsname{0.113}
\expandafter\def\csname res@flex.clap_ms_desc.tenth\endcsname{0.573}
\expandafter\def\csname res@flex.clap_ms_desc.tv\endcsname{0.000}
\expandafter\def\csname res@flex.clap_ms_desc.yesno_native\endcsname{0.606}
\expandafter\def\csname res@flex.clap_ms_desc.yesno_nativeci\endcsname{[0.581, 0.624]}
\expandafter\def\csname res@flex.clap_ms_desc.yesno_new_words\endcsname{0.545}
\expandafter\def\csname res@flex.clap_ms_desc.yesno_new_wordsci\endcsname{[0.527, 0.562]}
\expandafter\def\csname res@flex.clap_para.bare_names.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para.bare_names.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_para.bare_names.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_para.bare_names.f1\endcsname{0.294}
\expandafter\def\csname res@flex.clap_para.ccc.arousal\endcsname{0.168}
\expandafter\def\csname res@flex.clap_para.ccc.arousalci\endcsname{[0.092, 0.256]}
\expandafter\def\csname res@flex.clap_para.ccc.dominance\endcsname{-0.007}
\expandafter\def\csname res@flex.clap_para.ccc.dominanceci\endcsname{[-0.032, 0.006]}
\expandafter\def\csname res@flex.clap_para.ccc.valence\endcsname{0.171}
\expandafter\def\csname res@flex.clap_para.ccc.valenceci\endcsname{[0.124, 0.219]}
\expandafter\def\csname res@flex.clap_para.ccc2.arousal\endcsname{0.17}
\expandafter\def\csname res@flex.clap_para.ccc2.dominance\endcsname{-0.01}
\expandafter\def\csname res@flex.clap_para.ccc2.valence\endcsname{0.17}
\expandafter\def\csname res@flex.clap_para.gender\endcsname{0.684}
\expandafter\def\csname res@flex.clap_para.genderref\endcsname{0.905}
\expandafter\def\csname res@flex.clap_para.genderrefci\endcsname{[0.833, 0.956]}
\expandafter\def\csname res@flex.clap_para.instr2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para.instr2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_para.instr2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_para.instr2.f1\endcsname{0.294}
\expandafter\def\csname res@flex.clap_para.native.f1\endcsname{0.294}
\expandafter\def\csname res@flex.clap_para.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.clap_para.newwords_oracle\endcsname{0.676}
\expandafter\def\csname res@flex.clap_para.para1.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para.para1.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_para.para1.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_para.para1.f1\endcsname{0.294}
\expandafter\def\csname res@flex.clap_para.para2.agree\endcsname{44.0}
\expandafter\def\csname res@flex.clap_para.para2.delta\endcsname{-0.088}
\expandafter\def\csname res@flex.clap_para.para2.deltaci\endcsname{[-0.118, -0.062]}
\expandafter\def\csname res@flex.clap_para.para2.f1\endcsname{0.205}
\expandafter\def\csname res@flex.clap_para.redagree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para.synpara.agree\endcsname{44.0}
\expandafter\def\csname res@flex.clap_para.synpara.delta\endcsname{-0.088}
\expandafter\def\csname res@flex.clap_para.synpara.deltaci\endcsname{[-0.118, -0.062]}
\expandafter\def\csname res@flex.clap_para.synpara.f1\endcsname{0.205}
\expandafter\def\csname res@flex.clap_para.tenth\endcsname{0.599}
\expandafter\def\csname res@flex.clap_para.tv\endcsname{0.000}
\expandafter\def\csname res@flex.clap_para.yesno_native\endcsname{0.638}
\expandafter\def\csname res@flex.clap_para.yesno_nativeci\endcsname{[0.612, 0.665]}
\expandafter\def\csname res@flex.clap_para.yesno_new_words\endcsname{0.567}
\expandafter\def\csname res@flex.clap_para.yesno_new_wordsci\endcsname{[0.533, 0.597]}
\expandafter\def\csname res@flex.clap_para_desc.bare_names.agree\endcsname{42.8}
\expandafter\def\csname res@flex.clap_para_desc.bare_names.delta\endcsname{+0.060}
\expandafter\def\csname res@flex.clap_para_desc.bare_names.deltaci\endcsname{[+0.029, +0.090]}
\expandafter\def\csname res@flex.clap_para_desc.bare_names.f1\endcsname{0.291}
\expandafter\def\csname res@flex.clap_para_desc.ccc.arousal\endcsname{0.168}
\expandafter\def\csname res@flex.clap_para_desc.ccc.arousalci\endcsname{[0.092, 0.256]}
\expandafter\def\csname res@flex.clap_para_desc.ccc.dominance\endcsname{-0.007}
\expandafter\def\csname res@flex.clap_para_desc.ccc.dominanceci\endcsname{[-0.032, 0.006]}
\expandafter\def\csname res@flex.clap_para_desc.ccc.valence\endcsname{0.171}
\expandafter\def\csname res@flex.clap_para_desc.ccc.valenceci\endcsname{[0.124, 0.219]}
\expandafter\def\csname res@flex.clap_para_desc.ccc2.arousal\endcsname{0.17}
\expandafter\def\csname res@flex.clap_para_desc.ccc2.dominance\endcsname{-0.01}
\expandafter\def\csname res@flex.clap_para_desc.ccc2.valence\endcsname{0.17}
\expandafter\def\csname res@flex.clap_para_desc.gender\endcsname{0.684}
\expandafter\def\csname res@flex.clap_para_desc.genderref\endcsname{0.905}
\expandafter\def\csname res@flex.clap_para_desc.genderrefci\endcsname{[0.833, 0.956]}
\expandafter\def\csname res@flex.clap_para_desc.instr2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para_desc.instr2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_para_desc.instr2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_para_desc.instr2.f1\endcsname{0.230}
\expandafter\def\csname res@flex.clap_para_desc.native.f1\endcsname{0.230}
\expandafter\def\csname res@flex.clap_para_desc.newwords_above\endcsname{0}
\expandafter\def\csname res@flex.clap_para_desc.newwords_oracle\endcsname{0.680}
\expandafter\def\csname res@flex.clap_para_desc.para1.agree\endcsname{44.1}
\expandafter\def\csname res@flex.clap_para_desc.para1.delta\endcsname{+0.012}
\expandafter\def\csname res@flex.clap_para_desc.para1.deltaci\endcsname{[-0.015, +0.041]}
\expandafter\def\csname res@flex.clap_para_desc.para1.f1\endcsname{0.242}
\expandafter\def\csname res@flex.clap_para_desc.para2.agree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para_desc.para2.delta\endcsname{+0.000}
\expandafter\def\csname res@flex.clap_para_desc.para2.deltaci\endcsname{[+0.000, +0.000]}
\expandafter\def\csname res@flex.clap_para_desc.para2.f1\endcsname{0.230}
\expandafter\def\csname res@flex.clap_para_desc.redagree\endcsname{100.0}
\expandafter\def\csname res@flex.clap_para_desc.synpara.agree\endcsname{44.1}
\expandafter\def\csname res@flex.clap_para_desc.synpara.delta\endcsname{+0.012}
\expandafter\def\csname res@flex.clap_para_desc.synpara.deltaci\endcsname{[-0.015, +0.041]}
\expandafter\def\csname res@flex.clap_para_desc.synpara.f1\endcsname{0.242}
\expandafter\def\csname res@flex.clap_para_desc.tenth\endcsname{0.574}
\expandafter\def\csname res@flex.clap_para_desc.tv\endcsname{0.000}
\expandafter\def\csname res@flex.clap_para_desc.yesno_native\endcsname{0.573}
\expandafter\def\csname res@flex.clap_para_desc.yesno_nativeci\endcsname{[0.548, 0.604]}
\expandafter\def\csname res@flex.clap_para_desc.yesno_new_words\endcsname{0.536}
\expandafter\def\csname res@flex.clap_para_desc.yesno_new_wordsci\endcsname{[0.492, 0.573]}
\expandafter\def\csname res@flex.omni3b.bare_names.agree\endcsname{68.7}
\expandafter\def\csname res@flex.omni3b.bare_names.delta\endcsname{+0.038}
\expandafter\def\csname res@flex.omni3b.bare_names.deltaci\endcsname{[+0.015, +0.063]}
\expandafter\def\csname res@flex.omni3b.bare_names.f1\endcsname{0.299}
\expandafter\def\csname res@flex.omni3b.ccc.arousal\endcsname{0.102}
\expandafter\def\csname res@flex.omni3b.ccc.arousalci\endcsname{[0.044, 0.168]}
\expandafter\def\csname res@flex.omni3b.ccc.dominance\endcsname{0.112}
\expandafter\def\csname res@flex.omni3b.ccc.dominanceci\endcsname{[0.064, 0.188]}
\expandafter\def\csname res@flex.omni3b.ccc.valence\endcsname{0.462}
\expandafter\def\csname res@flex.omni3b.ccc.valenceci\endcsname{[0.387, 0.532]}
\expandafter\def\csname res@flex.omni3b.ccc2.arousal\endcsname{0.10}
\expandafter\def\csname res@flex.omni3b.ccc2.dominance\endcsname{0.11}
\expandafter\def\csname res@flex.omni3b.ccc2.valence\endcsname{0.46}
\expandafter\def\csname res@flex.omni3b.gender\endcsname{0.679}
\expandafter\def\csname res@flex.omni3b.genderref\endcsname{0.887}
\expandafter\def\csname res@flex.omni3b.genderrefci\endcsname{[0.859, 0.913]}
\expandafter\def\csname res@flex.omni3b.instr2.agree\endcsname{85.8}
\expandafter\def\csname res@flex.omni3b.instr2.delta\endcsname{-0.004}
\expandafter\def\csname res@flex.omni3b.instr2.deltaci\endcsname{[-0.028, +0.021]}
\expandafter\def\csname res@flex.omni3b.instr2.f1\endcsname{0.258}
\expandafter\def\csname res@flex.omni3b.native.f1\endcsname{0.261}
\expandafter\def\csname res@flex.omni3b.newwords_above\endcsname{8}
\expandafter\def\csname res@flex.omni3b.newwords_oracle\endcsname{0.651}
\expandafter\def\csname res@flex.omni3b.para1.agree\endcsname{89.5}
\expandafter\def\csname res@flex.omni3b.para1.delta\endcsname{-0.005}
\expandafter\def\csname res@flex.omni3b.para1.deltaci\endcsname{[-0.023, +0.017]}
\expandafter\def\csname res@flex.omni3b.para1.f1\endcsname{0.256}
\expandafter\def\csname res@flex.omni3b.para2.agree\endcsname{72.5}
\expandafter\def\csname res@flex.omni3b.para2.delta\endcsname{-0.044}
\expandafter\def\csname res@flex.omni3b.para2.deltaci\endcsname{[-0.081, -0.010]}
\expandafter\def\csname res@flex.omni3b.para2.f1\endcsname{0.217}
\expandafter\def\csname res@flex.omni3b.redagree\endcsname{86.8}
\expandafter\def\csname res@flex.omni3b.synpara.agree\endcsname{72.9}
\expandafter\def\csname res@flex.omni3b.synpara.delta\endcsname{-0.041}
\expandafter\def\csname res@flex.omni3b.synpara.deltaci\endcsname{[-0.075, -0.003]}
\expandafter\def\csname res@flex.omni3b.synpara.f1\endcsname{0.221}
\expandafter\def\csname res@flex.omni3b.tenth\endcsname{0.626}
\expandafter\def\csname res@flex.omni3b.tv\endcsname{0.116}
\expandafter\def\csname res@flex.omni3b.yesno_native\endcsname{0.687}
\expandafter\def\csname res@flex.omni3b.yesno_nativeci\endcsname{[0.666, 0.708]}
\expandafter\def\csname res@flex.omni3b.yesno_new_words\endcsname{0.707}
\expandafter\def\csname res@flex.omni3b.yesno_new_wordsci\endcsname{[0.684, 0.729]}
\expandafter\def\csname res@flex.omni3b_cc.bare_names.agree\endcsname{74.9}
\expandafter\def\csname res@flex.omni3b_cc.bare_names.delta\endcsname{-0.009}
\expandafter\def\csname res@flex.omni3b_cc.bare_names.deltaci\endcsname{[-0.035, +0.016]}
\expandafter\def\csname res@flex.omni3b_cc.bare_names.f1\endcsname{0.299}
\expandafter\def\csname res@flex.omni3b_cc.ccc.arousal\endcsname{0.160}
\expandafter\def\csname res@flex.omni3b_cc.ccc.arousalci\endcsname{[0.071, 0.263]}
\expandafter\def\csname res@flex.omni3b_cc.ccc.dominance\endcsname{0.139}
\expandafter\def\csname res@flex.omni3b_cc.ccc.dominanceci\endcsname{[0.079, 0.234]}
\expandafter\def\csname res@flex.omni3b_cc.ccc.valence\endcsname{0.576}
\expandafter\def\csname res@flex.omni3b_cc.ccc.valenceci\endcsname{[0.521, 0.642]}
\expandafter\def\csname res@flex.omni3b_cc.ccc2.arousal\endcsname{0.16}
\expandafter\def\csname res@flex.omni3b_cc.ccc2.dominance\endcsname{0.14}
\expandafter\def\csname res@flex.omni3b_cc.ccc2.valence\endcsname{0.58}
\expandafter\def\csname res@flex.omni3b_cc.gender\endcsname{0.690}
\expandafter\def\csname res@flex.omni3b_cc.genderref\endcsname{0.887}
\expandafter\def\csname res@flex.omni3b_cc.genderrefci\endcsname{[0.859, 0.913]}
\expandafter\def\csname res@flex.omni3b_cc.instr2.agree\endcsname{78.9}
\expandafter\def\csname res@flex.omni3b_cc.instr2.delta\endcsname{-0.012}
\expandafter\def\csname res@flex.omni3b_cc.instr2.deltaci\endcsname{[-0.035, +0.008]}
\expandafter\def\csname res@flex.omni3b_cc.instr2.f1\endcsname{0.297}
\expandafter\def\csname res@flex.omni3b_cc.native.f1\endcsname{0.308}
\expandafter\def\csname res@flex.omni3b_cc.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.omni3b_cc.newwords_oracle\endcsname{0.667}
\expandafter\def\csname res@flex.omni3b_cc.para1.agree\endcsname{84.5}
\expandafter\def\csname res@flex.omni3b_cc.para1.delta\endcsname{-0.014}
\expandafter\def\csname res@flex.omni3b_cc.para1.deltaci\endcsname{[-0.034, +0.007]}
\expandafter\def\csname res@flex.omni3b_cc.para1.f1\endcsname{0.294}
\expandafter\def\csname res@flex.omni3b_cc.para2.agree\endcsname{63.8}
\expandafter\def\csname res@flex.omni3b_cc.para2.delta\endcsname{-0.071}
\expandafter\def\csname res@flex.omni3b_cc.para2.deltaci\endcsname{[-0.095, -0.045]}
\expandafter\def\csname res@flex.omni3b_cc.para2.f1\endcsname{0.238}
\expandafter\def\csname res@flex.omni3b_cc.redagree\endcsname{79.4}
\expandafter\def\csname res@flex.omni3b_cc.synpara.agree\endcsname{62.5}
\expandafter\def\csname res@flex.omni3b_cc.synpara.delta\endcsname{-0.075}
\expandafter\def\csname res@flex.omni3b_cc.synpara.deltaci\endcsname{[-0.099, -0.048]}
\expandafter\def\csname res@flex.omni3b_cc.synpara.f1\endcsname{0.234}
\expandafter\def\csname res@flex.omni3b_cc.tenth\endcsname{0.631}
\expandafter\def\csname res@flex.omni3b_cc.tv\endcsname{0.123}
\expandafter\def\csname res@flex.omni3b_cc.yesno_native\endcsname{0.687}
\expandafter\def\csname res@flex.omni3b_cc.yesno_nativeci\endcsname{[0.666, 0.708]}
\expandafter\def\csname res@flex.omni3b_cc.yesno_new_words\endcsname{0.707}
\expandafter\def\csname res@flex.omni3b_cc.yesno_new_wordsci\endcsname{[0.684, 0.729]}
\expandafter\def\csname res@flex.omni3b_ft.bare_names.agree\endcsname{92.1}
\expandafter\def\csname res@flex.omni3b_ft.bare_names.delta\endcsname{+0.037}
\expandafter\def\csname res@flex.omni3b_ft.bare_names.deltaci\endcsname{[+0.005, +0.086]}
\expandafter\def\csname res@flex.omni3b_ft.bare_names.f1\endcsname{0.365}
\expandafter\def\csname res@flex.omni3b_ft.ccc.arousal\endcsname{0.430}
\expandafter\def\csname res@flex.omni3b_ft.ccc.arousalci\endcsname{[0.362, 0.513]}
\expandafter\def\csname res@flex.omni3b_ft.ccc.dominance\endcsname{0.398}
\expandafter\def\csname res@flex.omni3b_ft.ccc.dominanceci\endcsname{[0.295, 0.538]}
\expandafter\def\csname res@flex.omni3b_ft.ccc.valence\endcsname{0.667}
\expandafter\def\csname res@flex.omni3b_ft.ccc.valenceci\endcsname{[0.601, 0.721]}
\expandafter\def\csname res@flex.omni3b_ft.ccc2.arousal\endcsname{0.43}
\expandafter\def\csname res@flex.omni3b_ft.ccc2.dominance\endcsname{0.40}
\expandafter\def\csname res@flex.omni3b_ft.ccc2.valence\endcsname{0.67}
\expandafter\def\csname res@flex.omni3b_ft.gender\endcsname{0.746}
\expandafter\def\csname res@flex.omni3b_ft.genderref\endcsname{0.932}
\expandafter\def\csname res@flex.omni3b_ft.genderrefci\endcsname{[0.905, 0.954]}
\expandafter\def\csname res@flex.omni3b_ft.instr2.agree\endcsname{94.6}
\expandafter\def\csname res@flex.omni3b_ft.instr2.delta\endcsname{-0.018}
\expandafter\def\csname res@flex.omni3b_ft.instr2.deltaci\endcsname{[-0.043, +0.004]}
\expandafter\def\csname res@flex.omni3b_ft.instr2.f1\endcsname{0.311}
\expandafter\def\csname res@flex.omni3b_ft.native.f1\endcsname{0.328}
\expandafter\def\csname res@flex.omni3b_ft.newwords_above\endcsname{4}
\expandafter\def\csname res@flex.omni3b_ft.newwords_oracle\endcsname{0.741}
\expandafter\def\csname res@flex.omni3b_ft.para1.agree\endcsname{94.9}
\expandafter\def\csname res@flex.omni3b_ft.para1.delta\endcsname{+0.006}
\expandafter\def\csname res@flex.omni3b_ft.para1.deltaci\endcsname{[-0.008, +0.027]}
\expandafter\def\csname res@flex.omni3b_ft.para1.f1\endcsname{0.334}
\expandafter\def\csname res@flex.omni3b_ft.para2.agree\endcsname{89.1}
\expandafter\def\csname res@flex.omni3b_ft.para2.delta\endcsname{+0.037}
\expandafter\def\csname res@flex.omni3b_ft.para2.deltaci\endcsname{[+0.009, +0.068]}
\expandafter\def\csname res@flex.omni3b_ft.para2.f1\endcsname{0.365}
\expandafter\def\csname res@flex.omni3b_ft.redagree\endcsname{86.8}
\expandafter\def\csname res@flex.omni3b_ft.synpara.agree\endcsname{89.7}
\expandafter\def\csname res@flex.omni3b_ft.synpara.delta\endcsname{+0.062}
\expandafter\def\csname res@flex.omni3b_ft.synpara.deltaci\endcsname{[+0.030, +0.100]}
\expandafter\def\csname res@flex.omni3b_ft.synpara.f1\endcsname{0.391}
\expandafter\def\csname res@flex.omni3b_ft.tenth\endcsname{0.734}
\expandafter\def\csname res@flex.omni3b_ft.tv\endcsname{0.095}
\expandafter\def\csname res@flex.omni3b_ft.yesno_native\endcsname{0.741}
\expandafter\def\csname res@flex.omni3b_ft.yesno_nativeci\endcsname{[0.724, 0.761]}
\expandafter\def\csname res@flex.omni3b_ft.yesno_new_words\endcsname{0.755}
\expandafter\def\csname res@flex.omni3b_ft.yesno_new_wordsci\endcsname{[0.728, 0.782]}
\expandafter\def\csname res@flex.omni3b_ftfull.bare_names.agree\endcsname{96.1}
\expandafter\def\csname res@flex.omni3b_ftfull.bare_names.delta\endcsname{-0.002}
\expandafter\def\csname res@flex.omni3b_ftfull.bare_names.deltaci\endcsname{[-0.029, +0.012]}
\expandafter\def\csname res@flex.omni3b_ftfull.bare_names.f1\endcsname{0.363}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.arousal\endcsname{0.534}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.arousalci\endcsname{[0.459, 0.615]}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.dominance\endcsname{0.304}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.dominanceci\endcsname{[0.192, 0.445]}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.valence\endcsname{0.701}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc.valenceci\endcsname{[0.644, 0.750]}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc2.arousal\endcsname{0.53}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc2.dominance\endcsname{0.30}
\expandafter\def\csname res@flex.omni3b_ftfull.ccc2.valence\endcsname{0.70}
\expandafter\def\csname res@flex.omni3b_ftfull.gender\endcsname{0.734}
\expandafter\def\csname res@flex.omni3b_ftfull.genderref\endcsname{0.927}
\expandafter\def\csname res@flex.omni3b_ftfull.genderrefci\endcsname{[0.900, 0.949]}
\expandafter\def\csname res@flex.omni3b_ftfull.instr2.agree\endcsname{97.0}
\expandafter\def\csname res@flex.omni3b_ftfull.instr2.delta\endcsname{-0.013}
\expandafter\def\csname res@flex.omni3b_ftfull.instr2.deltaci\endcsname{[-0.033, +0.001]}
\expandafter\def\csname res@flex.omni3b_ftfull.instr2.f1\endcsname{0.352}
\expandafter\def\csname res@flex.omni3b_ftfull.native.f1\endcsname{0.365}
\expandafter\def\csname res@flex.omni3b_ftfull.newwords_above\endcsname{4}
\expandafter\def\csname res@flex.omni3b_ftfull.newwords_oracle\endcsname{0.747}
\expandafter\def\csname res@flex.omni3b_ftfull.para1.agree\endcsname{96.9}
\expandafter\def\csname res@flex.omni3b_ftfull.para1.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.omni3b_ftfull.para1.deltaci\endcsname{[-0.016, +0.005]}
\expandafter\def\csname res@flex.omni3b_ftfull.para1.f1\endcsname{0.359}
\expandafter\def\csname res@flex.omni3b_ftfull.para2.agree\endcsname{92.3}
\expandafter\def\csname res@flex.omni3b_ftfull.para2.delta\endcsname{-0.018}
\expandafter\def\csname res@flex.omni3b_ftfull.para2.deltaci\endcsname{[-0.035, -0.001]}
\expandafter\def\csname res@flex.omni3b_ftfull.para2.f1\endcsname{0.347}
\expandafter\def\csname res@flex.omni3b_ftfull.redagree\endcsname{80.9}
\expandafter\def\csname res@flex.omni3b_ftfull.synpara.agree\endcsname{93.0}
\expandafter\def\csname res@flex.omni3b_ftfull.synpara.delta\endcsname{-0.017}
\expandafter\def\csname res@flex.omni3b_ftfull.synpara.deltaci\endcsname{[-0.030, -0.002]}
\expandafter\def\csname res@flex.omni3b_ftfull.synpara.f1\endcsname{0.349}
\expandafter\def\csname res@flex.omni3b_ftfull.tenth\endcsname{0.692}
\expandafter\def\csname res@flex.omni3b_ftfull.tv\endcsname{0.124}
\expandafter\def\csname res@flex.omni3b_ftfull.yesno_native\endcsname{0.758}
\expandafter\def\csname res@flex.omni3b_ftfull.yesno_nativeci\endcsname{[0.741, 0.781]}
\expandafter\def\csname res@flex.omni3b_ftfull.yesno_new_words\endcsname{0.760}
\expandafter\def\csname res@flex.omni3b_ftfull.yesno_new_wordsci\endcsname{[0.733, 0.786]}
\expandafter\def\csname res@flex.omni7b.bare_names.agree\endcsname{80.0}
\expandafter\def\csname res@flex.omni7b.bare_names.delta\endcsname{-0.034}
\expandafter\def\csname res@flex.omni7b.bare_names.deltaci\endcsname{[-0.057, -0.011]}
\expandafter\def\csname res@flex.omni7b.bare_names.f1\endcsname{0.278}
\expandafter\def\csname res@flex.omni7b.ccc.arousal\endcsname{0.090}
\expandafter\def\csname res@flex.omni7b.ccc.arousalci\endcsname{[0.062, 0.129]}
\expandafter\def\csname res@flex.omni7b.ccc.dominance\endcsname{0.111}
\expandafter\def\csname res@flex.omni7b.ccc.dominanceci\endcsname{[0.086, 0.150]}
\expandafter\def\csname res@flex.omni7b.ccc.valence\endcsname{0.604}
\expandafter\def\csname res@flex.omni7b.ccc.valenceci\endcsname{[0.565, 0.643]}
\expandafter\def\csname res@flex.omni7b.ccc2.arousal\endcsname{0.09}
\expandafter\def\csname res@flex.omni7b.ccc2.dominance\endcsname{0.11}
\expandafter\def\csname res@flex.omni7b.ccc2.valence\endcsname{0.60}
\expandafter\def\csname res@flex.omni7b.gender\endcsname{0.710}
\expandafter\def\csname res@flex.omni7b.genderref\endcsname{0.927}
\expandafter\def\csname res@flex.omni7b.genderrefci\endcsname{[0.907, 0.947]}
\expandafter\def\csname res@flex.omni7b.instr2.agree\endcsname{89.3}
\expandafter\def\csname res@flex.omni7b.instr2.delta\endcsname{-0.008}
\expandafter\def\csname res@flex.omni7b.instr2.deltaci\endcsname{[-0.025, +0.008]}
\expandafter\def\csname res@flex.omni7b.instr2.f1\endcsname{0.304}
\expandafter\def\csname res@flex.omni7b.native.f1\endcsname{0.312}
\expandafter\def\csname res@flex.omni7b.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.omni7b.newwords_oracle\endcsname{0.685}
\expandafter\def\csname res@flex.omni7b.para1.agree\endcsname{88.8}
\expandafter\def\csname res@flex.omni7b.para1.delta\endcsname{-0.013}
\expandafter\def\csname res@flex.omni7b.para1.deltaci\endcsname{[-0.034, +0.007]}
\expandafter\def\csname res@flex.omni7b.para1.f1\endcsname{0.299}
\expandafter\def\csname res@flex.omni7b.para2.agree\endcsname{75.8}
\expandafter\def\csname res@flex.omni7b.para2.delta\endcsname{-0.029}
\expandafter\def\csname res@flex.omni7b.para2.deltaci\endcsname{[-0.053, -0.004]}
\expandafter\def\csname res@flex.omni7b.para2.f1\endcsname{0.283}
\expandafter\def\csname res@flex.omni7b.redagree\endcsname{82.1}
\expandafter\def\csname res@flex.omni7b.synpara.agree\endcsname{77.0}
\expandafter\def\csname res@flex.omni7b.synpara.delta\endcsname{-0.030}
\expandafter\def\csname res@flex.omni7b.synpara.deltaci\endcsname{[-0.052, -0.006]}
\expandafter\def\csname res@flex.omni7b.synpara.f1\endcsname{0.282}
\expandafter\def\csname res@flex.omni7b.tenth\endcsname{0.668}
\expandafter\def\csname res@flex.omni7b.tv\endcsname{0.147}
\expandafter\def\csname res@flex.omni7b.yesno_native\endcsname{0.697}
\expandafter\def\csname res@flex.omni7b.yesno_nativeci\endcsname{[0.677, 0.717]}
\expandafter\def\csname res@flex.omni7b.yesno_new_words\endcsname{0.720}
\expandafter\def\csname res@flex.omni7b.yesno_new_wordsci\endcsname{[0.700, 0.744]}
\expandafter\def\csname res@flex.omni7b_cc.bare_names.agree\endcsname{81.7}
\expandafter\def\csname res@flex.omni7b_cc.bare_names.delta\endcsname{-0.022}
\expandafter\def\csname res@flex.omni7b_cc.bare_names.deltaci\endcsname{[-0.037, -0.005]}
\expandafter\def\csname res@flex.omni7b_cc.bare_names.f1\endcsname{0.253}
\expandafter\def\csname res@flex.omni7b_cc.ccc.arousal\endcsname{0.273}
\expandafter\def\csname res@flex.omni7b_cc.ccc.arousalci\endcsname{[0.198, 0.368]}
\expandafter\def\csname res@flex.omni7b_cc.ccc.dominance\endcsname{0.242}
\expandafter\def\csname res@flex.omni7b_cc.ccc.dominanceci\endcsname{[0.196, 0.314]}
\expandafter\def\csname res@flex.omni7b_cc.ccc.valence\endcsname{0.592}
\expandafter\def\csname res@flex.omni7b_cc.ccc.valenceci\endcsname{[0.555, 0.623]}
\expandafter\def\csname res@flex.omni7b_cc.ccc2.arousal\endcsname{0.27}
\expandafter\def\csname res@flex.omni7b_cc.ccc2.dominance\endcsname{0.24}
\expandafter\def\csname res@flex.omni7b_cc.ccc2.valence\endcsname{0.59}
\expandafter\def\csname res@flex.omni7b_cc.gender\endcsname{0.727}
\expandafter\def\csname res@flex.omni7b_cc.genderref\endcsname{0.927}
\expandafter\def\csname res@flex.omni7b_cc.genderrefci\endcsname{[0.907, 0.947]}
\expandafter\def\csname res@flex.omni7b_cc.instr2.agree\endcsname{81.7}
\expandafter\def\csname res@flex.omni7b_cc.instr2.delta\endcsname{-0.022}
\expandafter\def\csname res@flex.omni7b_cc.instr2.deltaci\endcsname{[-0.038, -0.006]}
\expandafter\def\csname res@flex.omni7b_cc.instr2.f1\endcsname{0.253}
\expandafter\def\csname res@flex.omni7b_cc.native.f1\endcsname{0.275}
\expandafter\def\csname res@flex.omni7b_cc.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.omni7b_cc.newwords_oracle\endcsname{0.673}
\expandafter\def\csname res@flex.omni7b_cc.para1.agree\endcsname{86.4}
\expandafter\def\csname res@flex.omni7b_cc.para1.delta\endcsname{+0.007}
\expandafter\def\csname res@flex.omni7b_cc.para1.deltaci\endcsname{[-0.008, +0.023]}
\expandafter\def\csname res@flex.omni7b_cc.para1.f1\endcsname{0.282}
\expandafter\def\csname res@flex.omni7b_cc.para2.agree\endcsname{76.7}
\expandafter\def\csname res@flex.omni7b_cc.para2.delta\endcsname{-0.013}
\expandafter\def\csname res@flex.omni7b_cc.para2.deltaci\endcsname{[-0.031, +0.009]}
\expandafter\def\csname res@flex.omni7b_cc.para2.f1\endcsname{0.262}
\expandafter\def\csname res@flex.omni7b_cc.redagree\endcsname{88.2}
\expandafter\def\csname res@flex.omni7b_cc.synpara.agree\endcsname{76.7}
\expandafter\def\csname res@flex.omni7b_cc.synpara.delta\endcsname{-0.012}
\expandafter\def\csname res@flex.omni7b_cc.synpara.deltaci\endcsname{[-0.029, +0.009]}
\expandafter\def\csname res@flex.omni7b_cc.synpara.f1\endcsname{0.263}
\expandafter\def\csname res@flex.omni7b_cc.tenth\endcsname{0.632}
\expandafter\def\csname res@flex.omni7b_cc.tv\endcsname{0.091}
\expandafter\def\csname res@flex.omni7b_cc.yesno_native\endcsname{0.697}
\expandafter\def\csname res@flex.omni7b_cc.yesno_nativeci\endcsname{[0.677, 0.717]}
\expandafter\def\csname res@flex.omni7b_cc.yesno_new_words\endcsname{0.720}
\expandafter\def\csname res@flex.omni7b_cc.yesno_new_wordsci\endcsname{[0.700, 0.744]}
\expandafter\def\csname res@flex.phi4mm.bare_names.agree\endcsname{78.8}
\expandafter\def\csname res@flex.phi4mm.bare_names.delta\endcsname{-0.003}
\expandafter\def\csname res@flex.phi4mm.bare_names.deltaci\endcsname{[-0.016, +0.014]}
\expandafter\def\csname res@flex.phi4mm.bare_names.f1\endcsname{0.238}
\expandafter\def\csname res@flex.phi4mm.ccc.arousal\endcsname{0.080}
\expandafter\def\csname res@flex.phi4mm.ccc.arousalci\endcsname{[0.051, 0.111]}
\expandafter\def\csname res@flex.phi4mm.ccc.dominance\endcsname{0.060}
\expandafter\def\csname res@flex.phi4mm.ccc.dominanceci\endcsname{[0.035, 0.089]}
\expandafter\def\csname res@flex.phi4mm.ccc.valence\endcsname{0.309}
\expandafter\def\csname res@flex.phi4mm.ccc.valenceci\endcsname{[0.258, 0.356]}
\expandafter\def\csname res@flex.phi4mm.ccc2.arousal\endcsname{0.08}
\expandafter\def\csname res@flex.phi4mm.ccc2.dominance\endcsname{0.06}
\expandafter\def\csname res@flex.phi4mm.ccc2.valence\endcsname{0.31}
\expandafter\def\csname res@flex.phi4mm.gender\endcsname{0.699}
\expandafter\def\csname res@flex.phi4mm.genderref\endcsname{0.714}
\expandafter\def\csname res@flex.phi4mm.genderrefci\endcsname{[0.649, 0.772]}
\expandafter\def\csname res@flex.phi4mm.instr2.agree\endcsname{80.0}
\expandafter\def\csname res@flex.phi4mm.instr2.delta\endcsname{+0.005}
\expandafter\def\csname res@flex.phi4mm.instr2.deltaci\endcsname{[-0.015, +0.018]}
\expandafter\def\csname res@flex.phi4mm.instr2.f1\endcsname{0.247}
\expandafter\def\csname res@flex.phi4mm.native.f1\endcsname{0.242}
\expandafter\def\csname res@flex.phi4mm.newwords_above\endcsname{1}
\expandafter\def\csname res@flex.phi4mm.newwords_oracle\endcsname{0.665}
\expandafter\def\csname res@flex.phi4mm.para1.agree\endcsname{68.3}
\expandafter\def\csname res@flex.phi4mm.para1.delta\endcsname{+0.008}
\expandafter\def\csname res@flex.phi4mm.para1.deltaci\endcsname{[-0.025, +0.035]}
\expandafter\def\csname res@flex.phi4mm.para1.f1\endcsname{0.250}
\expandafter\def\csname res@flex.phi4mm.para2.agree\endcsname{69.0}
\expandafter\def\csname res@flex.phi4mm.para2.delta\endcsname{-0.023}
\expandafter\def\csname res@flex.phi4mm.para2.deltaci\endcsname{[-0.043, +0.002]}
\expandafter\def\csname res@flex.phi4mm.para2.f1\endcsname{0.219}
\expandafter\def\csname res@flex.phi4mm.redagree\endcsname{77.0}
\expandafter\def\csname res@flex.phi4mm.synpara.agree\endcsname{68.9}
\expandafter\def\csname res@flex.phi4mm.synpara.delta\endcsname{-0.004}
\expandafter\def\csname res@flex.phi4mm.synpara.deltaci\endcsname{[-0.024, +0.018]}
\expandafter\def\csname res@flex.phi4mm.synpara.f1\endcsname{0.238}
\expandafter\def\csname res@flex.phi4mm.tenth\endcsname{0.623}
\expandafter\def\csname res@flex.phi4mm.tv\endcsname{0.187}
\expandafter\def\csname res@flex.phi4mm.yesno_native\endcsname{0.624}
\expandafter\def\csname res@flex.phi4mm.yesno_nativeci\endcsname{[0.608, 0.643]}
\expandafter\def\csname res@flex.phi4mm.yesno_new_words\endcsname{0.640}
\expandafter\def\csname res@flex.phi4mm.yesno_new_wordsci\endcsname{[0.616, 0.666]}
\expandafter\def\csname res@flex.phi4mm_cc.bare_names.agree\endcsname{71.7}
\expandafter\def\csname res@flex.phi4mm_cc.bare_names.delta\endcsname{-0.010}
\expandafter\def\csname res@flex.phi4mm_cc.bare_names.deltaci\endcsname{[-0.041, +0.028]}
\expandafter\def\csname res@flex.phi4mm_cc.bare_names.f1\endcsname{0.214}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.arousal\endcsname{0.342}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.arousalci\endcsname{[0.250, 0.436]}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.dominance\endcsname{0.259}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.dominanceci\endcsname{[0.163, 0.372]}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.valence\endcsname{0.440}
\expandafter\def\csname res@flex.phi4mm_cc.ccc.valenceci\endcsname{[0.389, 0.488]}
\expandafter\def\csname res@flex.phi4mm_cc.ccc2.arousal\endcsname{0.34}
\expandafter\def\csname res@flex.phi4mm_cc.ccc2.dominance\endcsname{0.26}
\expandafter\def\csname res@flex.phi4mm_cc.ccc2.valence\endcsname{0.44}
\expandafter\def\csname res@flex.phi4mm_cc.gender\endcsname{0.698}
\expandafter\def\csname res@flex.phi4mm_cc.genderref\endcsname{0.714}
\expandafter\def\csname res@flex.phi4mm_cc.genderrefci\endcsname{[0.649, 0.772]}
\expandafter\def\csname res@flex.phi4mm_cc.instr2.agree\endcsname{71.7}
\expandafter\def\csname res@flex.phi4mm_cc.instr2.delta\endcsname{-0.002}
\expandafter\def\csname res@flex.phi4mm_cc.instr2.deltaci\endcsname{[-0.026, +0.023]}
\expandafter\def\csname res@flex.phi4mm_cc.instr2.f1\endcsname{0.222}
\expandafter\def\csname res@flex.phi4mm_cc.native.f1\endcsname{0.224}
\expandafter\def\csname res@flex.phi4mm_cc.newwords_above\endcsname{4}
\expandafter\def\csname res@flex.phi4mm_cc.newwords_oracle\endcsname{0.657}
\expandafter\def\csname res@flex.phi4mm_cc.para1.agree\endcsname{75.8}
\expandafter\def\csname res@flex.phi4mm_cc.para1.delta\endcsname{+0.018}
\expandafter\def\csname res@flex.phi4mm_cc.para1.deltaci\endcsname{[-0.003, +0.042]}
\expandafter\def\csname res@flex.phi4mm_cc.para1.f1\endcsname{0.242}
\expandafter\def\csname res@flex.phi4mm_cc.para2.agree\endcsname{71.2}
\expandafter\def\csname res@flex.phi4mm_cc.para2.delta\endcsname{+0.005}
\expandafter\def\csname res@flex.phi4mm_cc.para2.deltaci\endcsname{[-0.017, +0.029]}
\expandafter\def\csname res@flex.phi4mm_cc.para2.f1\endcsname{0.230}
\expandafter\def\csname res@flex.phi4mm_cc.redagree\endcsname{83.2}
\expandafter\def\csname res@flex.phi4mm_cc.synpara.agree\endcsname{64.1}
\expandafter\def\csname res@flex.phi4mm_cc.synpara.delta\endcsname{+0.001}
\expandafter\def\csname res@flex.phi4mm_cc.synpara.deltaci\endcsname{[-0.022, +0.027]}
\expandafter\def\csname res@flex.phi4mm_cc.synpara.f1\endcsname{0.225}
\expandafter\def\csname res@flex.phi4mm_cc.tenth\endcsname{0.606}
\expandafter\def\csname res@flex.phi4mm_cc.tv\endcsname{0.161}
\expandafter\def\csname res@flex.phi4mm_cc.yesno_native\endcsname{0.624}
\expandafter\def\csname res@flex.phi4mm_cc.yesno_nativeci\endcsname{[0.608, 0.643]}
\expandafter\def\csname res@flex.phi4mm_cc.yesno_new_words\endcsname{0.640}
\expandafter\def\csname res@flex.phi4mm_cc.yesno_new_wordsci\endcsname{[0.616, 0.666]}
\expandafter\def\csname res@flex.qwen2audio7b.bare_names.agree\endcsname{66.5}
\expandafter\def\csname res@flex.qwen2audio7b.bare_names.delta\endcsname{+0.009}
\expandafter\def\csname res@flex.qwen2audio7b.bare_names.deltaci\endcsname{[-0.007, +0.028]}
\expandafter\def\csname res@flex.qwen2audio7b.bare_names.f1\endcsname{0.297}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.arousal\endcsname{0.231}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.arousalci\endcsname{[0.172, 0.270]}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.dominance\endcsname{0.311}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.dominanceci\endcsname{[0.209, 0.369]}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.valence\endcsname{0.230}
\expandafter\def\csname res@flex.qwen2audio7b.ccc.valenceci\endcsname{[0.132, 0.331]}
\expandafter\def\csname res@flex.qwen2audio7b.ccc2.arousal\endcsname{0.23}
\expandafter\def\csname res@flex.qwen2audio7b.ccc2.dominance\endcsname{0.31}
\expandafter\def\csname res@flex.qwen2audio7b.ccc2.valence\endcsname{0.23}
\expandafter\def\csname res@flex.qwen2audio7b.gender\endcsname{0.660}
\expandafter\def\csname res@flex.qwen2audio7b.genderref\endcsname{0.831}
\expandafter\def\csname res@flex.qwen2audio7b.genderrefci\endcsname{[0.776, 0.880]}
\expandafter\def\csname res@flex.qwen2audio7b.instr2.agree\endcsname{83.0}
\expandafter\def\csname res@flex.qwen2audio7b.instr2.delta\endcsname{-0.003}
\expandafter\def\csname res@flex.qwen2audio7b.instr2.deltaci\endcsname{[-0.024, +0.014]}
\expandafter\def\csname res@flex.qwen2audio7b.instr2.f1\endcsname{0.285}
\expandafter\def\csname res@flex.qwen2audio7b.native.f1\endcsname{0.288}
\expandafter\def\csname res@flex.qwen2audio7b.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.qwen2audio7b.newwords_oracle\endcsname{0.673}
\expandafter\def\csname res@flex.qwen2audio7b.para1.agree\endcsname{37.5}
\expandafter\def\csname res@flex.qwen2audio7b.para1.delta\endcsname{-0.067}
\expandafter\def\csname res@flex.qwen2audio7b.para1.deltaci\endcsname{[-0.099, -0.037]}
\expandafter\def\csname res@flex.qwen2audio7b.para1.f1\endcsname{0.220}
\expandafter\def\csname res@flex.qwen2audio7b.para2.agree\endcsname{67.9}
\expandafter\def\csname res@flex.qwen2audio7b.para2.delta\endcsname{-0.043}
\expandafter\def\csname res@flex.qwen2audio7b.para2.deltaci\endcsname{[-0.070, -0.013]}
\expandafter\def\csname res@flex.qwen2audio7b.para2.f1\endcsname{0.245}
\expandafter\def\csname res@flex.qwen2audio7b.redagree\endcsname{58.6}
\expandafter\def\csname res@flex.qwen2audio7b.synpara.agree\endcsname{45.8}
\expandafter\def\csname res@flex.qwen2audio7b.synpara.delta\endcsname{-0.079}
\expandafter\def\csname res@flex.qwen2audio7b.synpara.deltaci\endcsname{[-0.107, -0.050]}
\expandafter\def\csname res@flex.qwen2audio7b.synpara.f1\endcsname{0.208}
\expandafter\def\csname res@flex.qwen2audio7b.tenth\endcsname{0.583}
\expandafter\def\csname res@flex.qwen2audio7b.tv\endcsname{0.319}
\expandafter\def\csname res@flex.qwen2audio7b.yesno_native\endcsname{0.700}
\expandafter\def\csname res@flex.qwen2audio7b.yesno_nativeci\endcsname{[0.679, 0.718]}
\expandafter\def\csname res@flex.qwen2audio7b.yesno_new_words\endcsname{0.696}
\expandafter\def\csname res@flex.qwen2audio7b.yesno_new_wordsci\endcsname{[0.670, 0.724]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.bare_names.agree\endcsname{69.3}
\expandafter\def\csname res@flex.qwen2audio7b_cc.bare_names.delta\endcsname{-0.021}
\expandafter\def\csname res@flex.qwen2audio7b_cc.bare_names.deltaci\endcsname{[-0.049, +0.005]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.bare_names.f1\endcsname{0.281}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.arousal\endcsname{0.300}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.arousalci\endcsname{[0.244, 0.350]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.dominance\endcsname{0.256}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.dominanceci\endcsname{[0.161, 0.317]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.valence\endcsname{0.299}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc.valenceci\endcsname{[0.249, 0.348]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc2.arousal\endcsname{0.30}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc2.dominance\endcsname{0.26}
\expandafter\def\csname res@flex.qwen2audio7b_cc.ccc2.valence\endcsname{0.30}
\expandafter\def\csname res@flex.qwen2audio7b_cc.gender\endcsname{0.710}
\expandafter\def\csname res@flex.qwen2audio7b_cc.genderref\endcsname{0.831}
\expandafter\def\csname res@flex.qwen2audio7b_cc.genderrefci\endcsname{[0.776, 0.880]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.instr2.agree\endcsname{82.9}
\expandafter\def\csname res@flex.qwen2audio7b_cc.instr2.delta\endcsname{-0.003}
\expandafter\def\csname res@flex.qwen2audio7b_cc.instr2.deltaci\endcsname{[-0.021, +0.013]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.instr2.f1\endcsname{0.300}
\expandafter\def\csname res@flex.qwen2audio7b_cc.native.f1\endcsname{0.302}
\expandafter\def\csname res@flex.qwen2audio7b_cc.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.qwen2audio7b_cc.newwords_oracle\endcsname{0.671}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para1.agree\endcsname{63.9}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para1.delta\endcsname{-0.058}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para1.deltaci\endcsname{[-0.088, -0.033]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para1.f1\endcsname{0.244}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para2.agree\endcsname{76.3}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para2.delta\endcsname{-0.022}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para2.deltaci\endcsname{[-0.050, +0.005]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.para2.f1\endcsname{0.280}
\expandafter\def\csname res@flex.qwen2audio7b_cc.redagree\endcsname{68.2}
\expandafter\def\csname res@flex.qwen2audio7b_cc.synpara.agree\endcsname{67.5}
\expandafter\def\csname res@flex.qwen2audio7b_cc.synpara.delta\endcsname{-0.044}
\expandafter\def\csname res@flex.qwen2audio7b_cc.synpara.deltaci\endcsname{[-0.070, -0.019]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.synpara.f1\endcsname{0.259}
\expandafter\def\csname res@flex.qwen2audio7b_cc.tenth\endcsname{0.599}
\expandafter\def\csname res@flex.qwen2audio7b_cc.tv\endcsname{0.217}
\expandafter\def\csname res@flex.qwen2audio7b_cc.yesno_native\endcsname{0.700}
\expandafter\def\csname res@flex.qwen2audio7b_cc.yesno_nativeci\endcsname{[0.679, 0.718]}
\expandafter\def\csname res@flex.qwen2audio7b_cc.yesno_new_words\endcsname{0.696}
\expandafter\def\csname res@flex.qwen2audio7b_cc.yesno_new_wordsci\endcsname{[0.670, 0.724]}
\expandafter\def\csname res@flex.voxtral3b.bare_names.agree\endcsname{84.4}
\expandafter\def\csname res@flex.voxtral3b.bare_names.delta\endcsname{+0.003}
\expandafter\def\csname res@flex.voxtral3b.bare_names.deltaci\endcsname{[-0.020, +0.026]}
\expandafter\def\csname res@flex.voxtral3b.bare_names.f1\endcsname{0.214}
\expandafter\def\csname res@flex.voxtral3b.ccc.arousal\endcsname{0.137}
\expandafter\def\csname res@flex.voxtral3b.ccc.arousalci\endcsname{[0.095, 0.192]}
\expandafter\def\csname res@flex.voxtral3b.ccc.dominance\endcsname{0.024}
\expandafter\def\csname res@flex.voxtral3b.ccc.dominanceci\endcsname{[0.011, 0.041]}
\expandafter\def\csname res@flex.voxtral3b.ccc.valence\endcsname{0.584}
\expandafter\def\csname res@flex.voxtral3b.ccc.valenceci\endcsname{[0.534, 0.637]}
\expandafter\def\csname res@flex.voxtral3b.ccc2.arousal\endcsname{0.14}
\expandafter\def\csname res@flex.voxtral3b.ccc2.dominance\endcsname{0.02}
\expandafter\def\csname res@flex.voxtral3b.ccc2.valence\endcsname{0.58}
\expandafter\def\csname res@flex.voxtral3b.gender\endcsname{0.594}
\expandafter\def\csname res@flex.voxtral3b.genderref\endcsname{0.483}
\expandafter\def\csname res@flex.voxtral3b.genderrefci\endcsname{[0.359, 0.606]}
\expandafter\def\csname res@flex.voxtral3b.instr2.agree\endcsname{85.0}
\expandafter\def\csname res@flex.voxtral3b.instr2.delta\endcsname{-0.038}
\expandafter\def\csname res@flex.voxtral3b.instr2.deltaci\endcsname{[-0.061, -0.018]}
\expandafter\def\csname res@flex.voxtral3b.instr2.f1\endcsname{0.174}
\expandafter\def\csname res@flex.voxtral3b.native.f1\endcsname{0.211}
\expandafter\def\csname res@flex.voxtral3b.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.voxtral3b.newwords_oracle\endcsname{0.597}
\expandafter\def\csname res@flex.voxtral3b.para1.agree\endcsname{85.9}
\expandafter\def\csname res@flex.voxtral3b.para1.delta\endcsname{-0.043}
\expandafter\def\csname res@flex.voxtral3b.para1.deltaci\endcsname{[-0.058, -0.027]}
\expandafter\def\csname res@flex.voxtral3b.para1.f1\endcsname{0.168}
\expandafter\def\csname res@flex.voxtral3b.para2.agree\endcsname{56.3}
\expandafter\def\csname res@flex.voxtral3b.para2.delta\endcsname{-0.019}
\expandafter\def\csname res@flex.voxtral3b.para2.deltaci\endcsname{[-0.045, +0.017]}
\expandafter\def\csname res@flex.voxtral3b.para2.f1\endcsname{0.192}
\expandafter\def\csname res@flex.voxtral3b.redagree\endcsname{74.1}
\expandafter\def\csname res@flex.voxtral3b.synpara.agree\endcsname{83.4}
\expandafter\def\csname res@flex.voxtral3b.synpara.delta\endcsname{-0.001}
\expandafter\def\csname res@flex.voxtral3b.synpara.deltaci\endcsname{[-0.020, +0.024]}
\expandafter\def\csname res@flex.voxtral3b.synpara.f1\endcsname{0.210}
\expandafter\def\csname res@flex.voxtral3b.tenth\endcsname{0.637}
\expandafter\def\csname res@flex.voxtral3b.tv\endcsname{0.241}
\expandafter\def\csname res@flex.voxtral3b.yesno_native\endcsname{0.651}
\expandafter\def\csname res@flex.voxtral3b.yesno_nativeci\endcsname{[0.633, 0.671]}
\expandafter\def\csname res@flex.voxtral3b.yesno_new_words\endcsname{0.675}
\expandafter\def\csname res@flex.voxtral3b.yesno_new_wordsci\endcsname{[0.647, 0.705]}
\expandafter\def\csname res@flex.voxtral3b_cc.bare_names.agree\endcsname{76.5}
\expandafter\def\csname res@flex.voxtral3b_cc.bare_names.delta\endcsname{+0.011}
\expandafter\def\csname res@flex.voxtral3b_cc.bare_names.deltaci\endcsname{[-0.014, +0.041]}
\expandafter\def\csname res@flex.voxtral3b_cc.bare_names.f1\endcsname{0.223}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.arousal\endcsname{0.112}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.arousalci\endcsname{[0.086, 0.148]}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.dominance\endcsname{0.018}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.dominanceci\endcsname{[0.008, 0.030]}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.valence\endcsname{0.369}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc.valenceci\endcsname{[0.326, 0.407]}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc2.arousal\endcsname{0.11}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc2.dominance\endcsname{0.02}
\expandafter\def\csname res@flex.voxtral3b_cc.ccc2.valence\endcsname{0.37}
\expandafter\def\csname res@flex.voxtral3b_cc.gender\endcsname{0.712}
\expandafter\def\csname res@flex.voxtral3b_cc.genderref\endcsname{0.483}
\expandafter\def\csname res@flex.voxtral3b_cc.genderrefci\endcsname{[0.359, 0.606]}
\expandafter\def\csname res@flex.voxtral3b_cc.instr2.agree\endcsname{74.4}
\expandafter\def\csname res@flex.voxtral3b_cc.instr2.delta\endcsname{-0.049}
\expandafter\def\csname res@flex.voxtral3b_cc.instr2.deltaci\endcsname{[-0.073, -0.019]}
\expandafter\def\csname res@flex.voxtral3b_cc.instr2.f1\endcsname{0.164}
\expandafter\def\csname res@flex.voxtral3b_cc.native.f1\endcsname{0.213}
\expandafter\def\csname res@flex.voxtral3b_cc.newwords_above\endcsname{7}
\expandafter\def\csname res@flex.voxtral3b_cc.newwords_oracle\endcsname{0.599}
\expandafter\def\csname res@flex.voxtral3b_cc.para1.agree\endcsname{81.5}
\expandafter\def\csname res@flex.voxtral3b_cc.para1.delta\endcsname{-0.047}
\expandafter\def\csname res@flex.voxtral3b_cc.para1.deltaci\endcsname{[-0.064, -0.027]}
\expandafter\def\csname res@flex.voxtral3b_cc.para1.f1\endcsname{0.166}
\expandafter\def\csname res@flex.voxtral3b_cc.para2.agree\endcsname{64.7}
\expandafter\def\csname res@flex.voxtral3b_cc.para2.delta\endcsname{-0.006}
\expandafter\def\csname res@flex.voxtral3b_cc.para2.deltaci\endcsname{[-0.028, +0.022]}
\expandafter\def\csname res@flex.voxtral3b_cc.para2.f1\endcsname{0.207}
\expandafter\def\csname res@flex.voxtral3b_cc.redagree\endcsname{65.0}
\expandafter\def\csname res@flex.voxtral3b_cc.synpara.agree\endcsname{63.5}
\expandafter\def\csname res@flex.voxtral3b_cc.synpara.delta\endcsname{-0.014}
\expandafter\def\csname res@flex.voxtral3b_cc.synpara.deltaci\endcsname{[-0.036, +0.012]}
\expandafter\def\csname res@flex.voxtral3b_cc.synpara.f1\endcsname{0.198}
\expandafter\def\csname res@flex.voxtral3b_cc.tenth\endcsname{0.631}
\expandafter\def\csname res@flex.voxtral3b_cc.tv\endcsname{0.265}
\expandafter\def\csname res@flex.voxtral3b_cc.yesno_native\endcsname{0.651}
\expandafter\def\csname res@flex.voxtral3b_cc.yesno_nativeci\endcsname{[0.633, 0.671]}
\expandafter\def\csname res@flex.voxtral3b_cc.yesno_new_words\endcsname{0.675}
\expandafter\def\csname res@flex.voxtral3b_cc.yesno_new_wordsci\endcsname{[0.647, 0.705]}
\expandafter\def\csname res@flex.whisper_mlp.ccc.arousal\endcsname{0.672}
\expandafter\def\csname res@flex.whisper_mlp.ccc.arousalci\endcsname{[0.577, 0.755]}
\expandafter\def\csname res@flex.whisper_mlp.ccc.dominance\endcsname{0.579}
\expandafter\def\csname res@flex.whisper_mlp.ccc.dominanceci\endcsname{[0.468, 0.716]}
\expandafter\def\csname res@flex.whisper_mlp.ccc.valence\endcsname{0.730}
\expandafter\def\csname res@flex.whisper_mlp.ccc.valenceci\endcsname{[0.667, 0.780]}
\expandafter\def\csname res@flex.whisper_mlp.ccc2.arousal\endcsname{0.67}
\expandafter\def\csname res@flex.whisper_mlp.ccc2.dominance\endcsname{0.58}
\expandafter\def\csname res@flex.whisper_mlp.ccc2.valence\endcsname{0.73}
\expandafter\def\csname res@flexalm.ccc.arousal\endcsname{0.231}
\expandafter\def\csname res@flexalm.ccc.arousal.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@flexalm.ccc.dominance\endcsname{0.311}
\expandafter\def\csname res@flexalm.ccc.dominance.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@flexalm.ccc.valence\endcsname{0.604}
\expandafter\def\csname res@flexalm.ccc.valence.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@flexalm.gender\endcsname{0.710}
\expandafter\def\csname res@flexalm.gender.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@flexalm.genderref\endcsname{0.927}
\expandafter\def\csname res@flexalm.genderref.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@flexalm.native\endcsname{0.312}
\expandafter\def\csname res@flexalm.native.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@flexalm.newwords\endcsname{0.720}
\expandafter\def\csname res@flexalm.newwords.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@flexalm.redagreemax\endcsname{86.8}
\expandafter\def\csname res@flexalm.redagreemax.name\endcsname{Qwen2.5-Omni-3B}
\expandafter\def\csname res@flexalm.synparamin\endcsname{-0.079}
\expandafter\def\csname res@flexalm.synparamin.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@flexalm.tvmax\endcsname{0.380}
\expandafter\def\csname res@flexalm.tvmax.name\endcsname{Audio Flamingo 3}
\expandafter\def\csname res@flexalm.tvmin\endcsname{0.116}
\expandafter\def\csname res@flexalm.tvmin.name\endcsname{Qwen2.5-Omni-3B}
\expandafter\def\csname res@flexalm.yesno\endcsname{0.700}
\expandafter\def\csname res@flexalm.yesno.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@lat.af3.1q\endcsname{81.0}
\expandafter\def\csname res@lat.af3.20q\endcsname{527}
\expandafter\def\csname res@lat.af3.20q_plain\endcsname{1677}
\expandafter\def\csname res@lat.af3.20q_shared\endcsname{527}
\expandafter\def\csname res@lat.af3.generate_1q\endcsname{104}
\expandafter\def\csname res@lat.asom.1q\endcsname{27.1}
\expandafter\def\csname res@lat.asom.20q\endcsname{27.3}
\expandafter\def\csname res@lat.asom2_paper.1q\endcsname{22.7}
\expandafter\def\csname res@lat.asom2_paper.20q\endcsname{23.3}
\expandafter\def\csname res@lat.asom2_paper.frontend\endcsname{1.0}
\expandafter\def\csname res@lat.asom2_paper.reader\endcsname{0.6}
\expandafter\def\csname res@lat.asom2_paper.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom2_paper.whisper\endcsname{21.0}
\expandafter\def\csname res@lat.asom2_paper_cpufe_encode.1q\endcsname{41.8}
\expandafter\def\csname res@lat.asom2_paper_cpufe_encode.frontend\endcsname{4.8}
\expandafter\def\csname res@lat.asom2_paper_encode.1q\endcsname{38.0}
\expandafter\def\csname res@lat.asom2_paper_encode.20q\endcsname{143}
\expandafter\def\csname res@lat.asom2_paper_encode.frontend\endcsname{1.0}
\expandafter\def\csname res@lat.asom2_paper_encode.reader\endcsname{0.6}
\expandafter\def\csname res@lat.asom2_paper_encode.text\endcsname{15.7}
\expandafter\def\csname res@lat.asom2_paper_encode.whisper\endcsname{20.5}
\expandafter\def\csname res@lat.asom2_paper_encode_local.1q\endcsname{41.0}
\expandafter\def\csname res@lat.asom2_paper_encode_local.20q\endcsname{142}
\expandafter\def\csname res@lat.asom2_t14.1q\endcsname{22.6}
\expandafter\def\csname res@lat.asom2_t14.20q\endcsname{23.0}
\expandafter\def\csname res@lat.asom2_t14.frontend\endcsname{1.0}
\expandafter\def\csname res@lat.asom2_t14.reader\endcsname{0.6}
\expandafter\def\csname res@lat.asom2_t14.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom2_t14.whisper\endcsname{21.0}
\expandafter\def\csname res@lat.asom2_t14_encode.1q\endcsname{32.0}
\expandafter\def\csname res@lat.asom2_t14_encode.20q\endcsname{85.6}
\expandafter\def\csname res@lat.asom2_t14_encode.frontend\endcsname{1.0}
\expandafter\def\csname res@lat.asom2_t14_encode.reader\endcsname{0.6}
\expandafter\def\csname res@lat.asom2_t14_encode.text\endcsname{10.5}
\expandafter\def\csname res@lat.asom2_t14_encode.whisper\endcsname{20.1}
\expandafter\def\csname res@lat.asom2_t7.1q\endcsname{22.5}
\expandafter\def\csname res@lat.asom2_t7.20q\endcsname{23.0}
\expandafter\def\csname res@lat.asom2_t7.frontend\endcsname{1.0}
\expandafter\def\csname res@lat.asom2_t7.reader\endcsname{0.5}
\expandafter\def\csname res@lat.asom2_t7.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom2_t7.whisper\endcsname{20.9}
\expandafter\def\csname res@lat.asom2_t7_encode.1q\endcsname{28.0}
\expandafter\def\csname res@lat.asom2_t7_encode.20q\endcsname{54.9}
\expandafter\def\csname res@lat.asom2_t7_encode.frontend\endcsname{1.1}
\expandafter\def\csname res@lat.asom2_t7_encode.reader\endcsname{0.6}
\expandafter\def\csname res@lat.asom2_t7_encode.text\endcsname{6.7}
\expandafter\def\csname res@lat.asom2_t7_encode.whisper\endcsname{19.6}
\expandafter\def\csname res@lat.asom_bkt.1q\endcsname{12.5}
\expandafter\def\csname res@lat.asom_bkt.20q\endcsname{13.1}
\expandafter\def\csname res@lat.asom_bkt.frontend\endcsname{1.3}
\expandafter\def\csname res@lat.asom_bkt.reader\endcsname{1.2}
\expandafter\def\csname res@lat.asom_bkt.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom_bkt.whisper\endcsname{10.6}
\expandafter\def\csname res@lat.asom_bkt_encode.1q\endcsname{32.2}
\expandafter\def\csname res@lat.asom_bkt_encode.20q\endcsname{129}
\expandafter\def\csname res@lat.asom_bkt_encode.frontend\endcsname{1.6}
\expandafter\def\csname res@lat.asom_bkt_encode.reader\endcsname{1.4}
\expandafter\def\csname res@lat.asom_bkt_encode.text\endcsname{113}
\expandafter\def\csname res@lat.asom_bkt_encode.whisper\endcsname{14.1}
\expandafter\def\csname res@lat.asom_bkt_graph.1q\endcsname{10.4}
\expandafter\def\csname res@lat.asom_bkt_graph.20q\endcsname{11.0}
\expandafter\def\csname res@lat.asom_bkt_graph.frontend\endcsname{1.3}
\expandafter\def\csname res@lat.asom_bkt_graph.reader\endcsname{1.2}
\expandafter\def\csname res@lat.asom_bkt_graph.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom_bkt_graph.whisper\endcsname{8.4}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.1q\endcsname{29.5}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.20q\endcsname{132}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.frontend\endcsname{1.6}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.reader\endcsname{1.5}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.text\endcsname{115}
\expandafter\def\csname res@lat.asom_bkt_graph_encode.whisper\endcsname{13.9}
\expandafter\def\csname res@lat.asom_dyn.1q\endcsname{12.0}
\expandafter\def\csname res@lat.asom_dyn.20q\endcsname{12.5}
\expandafter\def\csname res@lat.asom_dyn.frontend\endcsname{1.2}
\expandafter\def\csname res@lat.asom_dyn.reader\endcsname{1.2}
\expandafter\def\csname res@lat.asom_dyn.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom_dyn.whisper\endcsname{10.0}
\expandafter\def\csname res@lat.asom_dyn_encode.1q\endcsname{31.3}
\expandafter\def\csname res@lat.asom_dyn_encode.20q\endcsname{130}
\expandafter\def\csname res@lat.asom_dyn_encode.frontend\endcsname{1.6}
\expandafter\def\csname res@lat.asom_dyn_encode.reader\endcsname{1.3}
\expandafter\def\csname res@lat.asom_dyn_encode.text\endcsname{117}
\expandafter\def\csname res@lat.asom_dyn_encode.whisper\endcsname{10.7}
\expandafter\def\csname res@lat.asom_encode.1q\endcsname{47.5}
\expandafter\def\csname res@lat.asom_encode.20q\endcsname{145}
\expandafter\def\csname res@lat.asom_r1_local.1q\endcsname{23.6}
\expandafter\def\csname res@lat.asom_r1_local.20q\endcsname{24.1}
\expandafter\def\csname res@lat.asom_r1_local.frontend\endcsname{0.9}
\expandafter\def\csname res@lat.asom_r1_local.reader\endcsname{1.3}
\expandafter\def\csname res@lat.asom_r1_local.text\endcsname{0.1}
\expandafter\def\csname res@lat.asom_r1_local.whisper\endcsname{21.9}
\expandafter\def\csname res@lat.asom_r1_local_encode.1q\endcsname{41.0}
\expandafter\def\csname res@lat.asom_r1_local_encode.20q\endcsname{149}
\expandafter\def\csname res@lat.asom_r1_local_encode.frontend\endcsname{1.4}
\expandafter\def\csname res@lat.asom_r1_local_encode.reader\endcsname{1.4}
\expandafter\def\csname res@lat.asom_r1_local_encode.text\endcsname{117}
\expandafter\def\csname res@lat.asom_r1_local_encode.whisper\endcsname{28.8}
\expandafter\def\csname res@lat.asom_served.1q\endcsname{23.6}
\expandafter\def\csname res@lat.asom_served.20q\endcsname{23.3}
\expandafter\def\csname res@lat.asom_served_encode.1q\endcsname{38.6}
\expandafter\def\csname res@lat.asom_served_encode.20q\endcsname{146}
\expandafter\def\csname res@lat.asom_served_local.1q\endcsname{23.9}
\expandafter\def\csname res@lat.asom_served_local.20q\endcsname{24.3}
\expandafter\def\csname res@lat.asom_served_local_encode.1q\endcsname{41.7}
\expandafter\def\csname res@lat.asom_served_local_encode.20q\endcsname{150}
\expandafter\def\csname res@lat.asom_text.1q\endcsname{27.0}
\expandafter\def\csname res@lat.asom_text.20q\endcsname{27.0}
\expandafter\def\csname res@lat.clap_laion.1q\endcsname{35.1}
\expandafter\def\csname res@lat.clap_laion.20q\endcsname{35.5}
\expandafter\def\csname res@lat.clap_laion_encode.1q\endcsname{41.0}
\expandafter\def\csname res@lat.clap_laion_encode.20q\endcsname{45.6}
\expandafter\def\csname res@lat.clap_mlp.1q\endcsname{22.6}
\expandafter\def\csname res@lat.clap_mlp.20q\endcsname{22.6}
\expandafter\def\csname res@lat.clap_ms.1q\endcsname{8.0}
\expandafter\def\csname res@lat.clap_ms.20q\endcsname{8.2}
\expandafter\def\csname res@lat.clap_ms_encode.1q\endcsname{15.0}
\expandafter\def\csname res@lat.clap_ms_encode.20q\endcsname{44.6}
\expandafter\def\csname res@lat.clap_para.1q\endcsname{7.6}
\expandafter\def\csname res@lat.clap_para.20q\endcsname{7.8}
\expandafter\def\csname res@lat.clap_para_encode.1q\endcsname{13.0}
\expandafter\def\csname res@lat.clap_para_encode.20q\endcsname{18.6}
\expandafter\def\csname res@lat.clap_para_r1.1q\endcsname{7.7}
\expandafter\def\csname res@lat.clap_para_r1.20q\endcsname{7.9}
\expandafter\def\csname res@lat.deepser.1q\endcsname{329}
\expandafter\def\csname res@lat.deepser.20q\endcsname{329}
\expandafter\def\csname res@lat.e2v.1q\endcsname{10.3}
\expandafter\def\csname res@lat.e2v.20q\endcsname{10.3}
\expandafter\def\csname res@lat.omni3b.1q\endcsname{35.7}
\expandafter\def\csname res@lat.omni3b.20q\endcsname{230}
\expandafter\def\csname res@lat.omni3b.20q_plain\endcsname{698}
\expandafter\def\csname res@lat.omni3b.20q_shared\endcsname{230}
\expandafter\def\csname res@lat.omni3b.generate_1q\endcsname{130}
\expandafter\def\csname res@lat.omni7b.1q\endcsname{63.9}
\expandafter\def\csname res@lat.omni7b.20q\endcsname{500}
\expandafter\def\csname res@lat.omni7b.20q_plain\endcsname{1278}
\expandafter\def\csname res@lat.omni7b.20q_shared\endcsname{500}
\expandafter\def\csname res@lat.omni7b.generate_1q\endcsname{202}
\expandafter\def\csname res@lat.phi4mm.1q\endcsname{38.2}
\expandafter\def\csname res@lat.phi4mm.20q\endcsname{311}
\expandafter\def\csname res@lat.phi4mm.20q_plain\endcsname{462}
\expandafter\def\csname res@lat.phi4mm.20q_shared\endcsname{311}
\expandafter\def\csname res@lat.phi4mm.generate_1q\endcsname{58.0}
\expandafter\def\csname res@lat.qwen2audio7b.1q\endcsname{82.1}
\expandafter\def\csname res@lat.qwen2audio7b.20q\endcsname{545}
\expandafter\def\csname res@lat.qwen2audio7b.20q_plain\endcsname{1686}
\expandafter\def\csname res@lat.qwen2audio7b.20q_shared\endcsname{545}
\expandafter\def\csname res@lat.qwen2audio7b.generate_1q\endcsname{108}
\expandafter\def\csname res@lat.voxtral3b.1q\endcsname{65.4}
\expandafter\def\csname res@lat.voxtral3b.20q\endcsname{327}
\expandafter\def\csname res@lat.voxtral3b.20q_plain\endcsname{1502}
\expandafter\def\csname res@lat.voxtral3b.20q_shared\endcsname{327}
\expandafter\def\csname res@lat.voxtral3b.generate_1q\endcsname{98.9}
\expandafter\def\csname res@lat.wavlm_ft.1q\endcsname{10.6}
\expandafter\def\csname res@lat.wavlm_ft.20q\endcsname{10.6}
\expandafter\def\csname res@lat.whisper_decoder.1q\endcsname{75.7}
\expandafter\def\csname res@lat.whisper_decoder.c14\endcsname{104}
\expandafter\def\csname res@lat.whisper_decoder.c40\endcsname{270}
\expandafter\def\csname res@lat.whisper_decoder.c9\endcsname{75.7}
\expandafter\def\csname res@lat.whisper_decoder.encoder\endcsname{23.0}
\expandafter\def\csname res@lat.whisper_decoder.vram\endcsname{22}
\expandafter\def\csname res@lat.whisper_mlp.1q\endcsname{12.5}
\expandafter\def\csname res@lat.whisper_mlp.20q\endcsname{12.5}
\expandafter\def\csname res@lat.whisper_mlp_30s.1q\endcsname{23.6}
\expandafter\def\csname res@lat.whisper_mlp_30s.20q\endcsname{23.6}
\expandafter\def\csname res@latalm.max20q\endcsname{545}
\expandafter\def\csname res@latalm.max20q.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@latalm.min20q\endcsname{230}
\expandafter\def\csname res@latalm.min20q.name\endcsname{Qwen2.5-Omni-3B}
\expandafter\def\csname res@latalm.plainmax20q\endcsname{1686}
\expandafter\def\csname res@latalm.plainmin20q\endcsname{462}
\expandafter\def\csname res@latalm.ratiomax\endcsname{41}
\expandafter\def\csname res@latalm.ratiomin\endcsname{17}
\expandafter\def\csname res@latalm.sharedagree\endcsname{95}
\expandafter\def\csname res@latalm.sharedtv\endcsname{0.06}
\expandafter\def\csname res@msp.dur.le10\endcsname{95}
\expandafter\def\csname res@msp.dur.median\endcsname{5.1}
\expandafter\def\csname res@msp.seg.ms\endcsname{80}
\expandafter\def\csname res@n.dev\endcsname{28,759}
\expandafter\def\csname res@n.genderref\endcsname{10,011}
\expandafter\def\csname res@n.official.full\endcsname{22,763}
\expandafter\def\csname res@n.official.subset\endcsname{2,435}
\expandafter\def\csname res@n.subset\endcsname{3,113}
\expandafter\def\csname res@n.v2acted\endcsname{9,314}
\expandafter\def\csname res@n.v2clips\endcsname{32,187}
\expandafter\def\csname res@nc.af3.acc\endcsname{0.253}
\expandafter\def\csname res@nc.af3.aucknown\endcsname{0.693}
\expandafter\def\csname res@nc.af3.aucnew\endcsname{0.720}
\expandafter\def\csname res@nc.af3.aucprimary\endcsname{0.710}
\expandafter\def\csname res@nc.af3.aucsecondary\endcsname{0.680}
\expandafter\def\csname res@nc.af3.f1\endcsname{0.226}
\expandafter\def\csname res@nc.af3.f1ci\endcsname{[0.214, 0.237]}
\expandafter\def\csname res@nc.af3.f1known\endcsname{0.226}
\expandafter\def\csname res@nc.af3.f1new\endcsname{0.227}
\expandafter\def\csname res@nc.af3.f1pm\endcsname{0.293}
\expandafter\def\csname res@nc.af3.f1primary\endcsname{0.269}
\expandafter\def\csname res@nc.af3.f1secondary\endcsname{0.192}
\expandafter\def\csname res@nc.af3.gap\endcsname{-0.091}
\expandafter\def\csname res@nc.af3.gapci\endcsname{[-0.104, -0.077]}
\expandafter\def\csname res@nc.af3_cc.acc\endcsname{0.282}
\expandafter\def\csname res@nc.af3_cc.aucknown\endcsname{0.691}
\expandafter\def\csname res@nc.af3_cc.aucnew\endcsname{0.717}
\expandafter\def\csname res@nc.af3_cc.aucprimary\endcsname{0.701}
\expandafter\def\csname res@nc.af3_cc.aucsecondary\endcsname{0.682}
\expandafter\def\csname res@nc.af3_cc.f1\endcsname{0.269}
\expandafter\def\csname res@nc.af3_cc.f1ci\endcsname{[0.256, 0.282]}
\expandafter\def\csname res@nc.af3_cc.f1known\endcsname{0.230}
\expandafter\def\csname res@nc.af3_cc.f1new\endcsname{0.297}
\expandafter\def\csname res@nc.af3_cc.f1pm\endcsname{0.298}
\expandafter\def\csname res@nc.af3_cc.f1primary\endcsname{0.259}
\expandafter\def\csname res@nc.af3_cc.f1secondary\endcsname{0.207}
\expandafter\def\csname res@nc.af3_cc.gap\endcsname{-0.134}
\expandafter\def\csname res@nc.af3_cc.gapci\endcsname{[-0.149, -0.119]}
\expandafter\def\csname res@nc.asom.acc\endcsname{0.192}
\expandafter\def\csname res@nc.asom.aucknown\endcsname{0.666}
\expandafter\def\csname res@nc.asom.aucnew\endcsname{0.648}
\expandafter\def\csname res@nc.asom.aucprimary\endcsname{0.675}
\expandafter\def\csname res@nc.asom.aucsecondary\endcsname{0.660}
\expandafter\def\csname res@nc.asom.f1\endcsname{0.135}
\expandafter\def\csname res@nc.asom.f1ci\endcsname{[0.127, 0.143]}
\expandafter\def\csname res@nc.asom.f1known\endcsname{0.143}
\expandafter\def\csname res@nc.asom.f1new\endcsname{0.128}
\expandafter\def\csname res@nc.asom.f1pm\endcsname{0.201}
\expandafter\def\csname res@nc.asom.f1primary\endcsname{0.231}
\expandafter\def\csname res@nc.asom.f1secondary\endcsname{0.075}
\expandafter\def\csname res@nc.asom_30s.acc\endcsname{0.196}
\expandafter\def\csname res@nc.asom_30s.aucknown\endcsname{0.669}
\expandafter\def\csname res@nc.asom_30s.aucnew\endcsname{0.652}
\expandafter\def\csname res@nc.asom_30s.aucprimary\endcsname{0.683}
\expandafter\def\csname res@nc.asom_30s.aucsecondary\endcsname{0.658}
\expandafter\def\csname res@nc.asom_30s.f1\endcsname{0.138}
\expandafter\def\csname res@nc.asom_30s.f1ci\endcsname{[0.130, 0.146]}
\expandafter\def\csname res@nc.asom_30s.f1known\endcsname{0.144}
\expandafter\def\csname res@nc.asom_30s.f1new\endcsname{0.133}
\expandafter\def\csname res@nc.asom_30s.f1pm\endcsname{0.202}
\expandafter\def\csname res@nc.asom_30s.f1primary\endcsname{0.244}
\expandafter\def\csname res@nc.asom_30s.f1secondary\endcsname{0.067}
\expandafter\def\csname res@nc.asom_30s.gap\endcsname{-0.003}
\expandafter\def\csname res@nc.asom_30s.gapci\endcsname{[-0.008, +0.002]}
\expandafter\def\csname res@nc.asom_cc.acc\endcsname{0.178}
\expandafter\def\csname res@nc.asom_cc.aucknown\endcsname{0.668}
\expandafter\def\csname res@nc.asom_cc.aucnew\endcsname{0.649}
\expandafter\def\csname res@nc.asom_cc.aucprimary\endcsname{0.661}
\expandafter\def\csname res@nc.asom_cc.aucsecondary\endcsname{0.674}
\expandafter\def\csname res@nc.asom_cc.f1\endcsname{0.121}
\expandafter\def\csname res@nc.asom_cc.f1ci\endcsname{[0.114, 0.128]}
\expandafter\def\csname res@nc.asom_cc.f1known\endcsname{0.153}
\expandafter\def\csname res@nc.asom_cc.f1new\endcsname{0.097}
\expandafter\def\csname res@nc.asom_cc.f1pm\endcsname{0.200}
\expandafter\def\csname res@nc.asom_cc.f1primary\endcsname{0.202}
\expandafter\def\csname res@nc.asom_cc.f1secondary\endcsname{0.115}
\expandafter\def\csname res@nc.asom_cc.gap\endcsname{+0.014}
\expandafter\def\csname res@nc.asom_cc.gapci\endcsname{[+0.005, +0.023]}
\expandafter\def\csname res@nc.asom_em.acc\endcsname{0.149}
\expandafter\def\csname res@nc.asom_em.aucknown\endcsname{0.645}
\expandafter\def\csname res@nc.asom_em.aucnew\endcsname{0.632}
\expandafter\def\csname res@nc.asom_em.aucprimary\endcsname{0.649}
\expandafter\def\csname res@nc.asom_em.aucsecondary\endcsname{0.641}
\expandafter\def\csname res@nc.asom_em.f1\endcsname{0.068}
\expandafter\def\csname res@nc.asom_em.f1ci\endcsname{[0.063, 0.072]}
\expandafter\def\csname res@nc.asom_em.f1known\endcsname{0.079}
\expandafter\def\csname res@nc.asom_em.f1new\endcsname{0.059}
\expandafter\def\csname res@nc.asom_em.f1pm\endcsname{0.111}
\expandafter\def\csname res@nc.asom_em.f1primary\endcsname{0.164}
\expandafter\def\csname res@nc.asom_em.f1secondary\endcsname{0.012}
\expandafter\def\csname res@nc.asom_em.gap\endcsname{+0.068}
\expandafter\def\csname res@nc.asom_em.gapci\endcsname{[+0.060, +0.075]}
\expandafter\def\csname res@nc.asom_u.acc\endcsname{0.191}
\expandafter\def\csname res@nc.asom_u.aucknown\endcsname{0.669}
\expandafter\def\csname res@nc.asom_u.aucnew\endcsname{0.651}
\expandafter\def\csname res@nc.asom_u.aucprimary\endcsname{0.675}
\expandafter\def\csname res@nc.asom_u.aucsecondary\endcsname{0.665}
\expandafter\def\csname res@nc.asom_u.f1\endcsname{0.144}
\expandafter\def\csname res@nc.asom_u.f1ci\endcsname{[0.136, 0.152]}
\expandafter\def\csname res@nc.asom_u.f1known\endcsname{0.153}
\expandafter\def\csname res@nc.asom_u.f1new\endcsname{0.137}
\expandafter\def\csname res@nc.asom_u.f1pm\endcsname{0.202}
\expandafter\def\csname res@nc.asom_u.f1primary\endcsname{0.232}
\expandafter\def\csname res@nc.asom_u.f1secondary\endcsname{0.092}
\expandafter\def\csname res@nc.asom_u.gap\endcsname{-0.009}
\expandafter\def\csname res@nc.asom_u.gapci\endcsname{[-0.014, -0.005]}
\expandafter\def\csname res@nc.asom_v2sp.acc\endcsname{0.191}
\expandafter\def\csname res@nc.asom_v2sp.aucknown\endcsname{0.647}
\expandafter\def\csname res@nc.asom_v2sp.aucnew\endcsname{0.635}
\expandafter\def\csname res@nc.asom_v2sp.aucprimary\endcsname{0.675}
\expandafter\def\csname res@nc.asom_v2sp.aucsecondary\endcsname{0.624}
\expandafter\def\csname res@nc.asom_v2sp.f1\endcsname{0.150}
\expandafter\def\csname res@nc.asom_v2sp.f1ci\endcsname{[0.141, 0.157]}
\expandafter\def\csname res@nc.asom_v2sp.f1known\endcsname{0.162}
\expandafter\def\csname res@nc.asom_v2sp.f1new\endcsname{0.140}
\expandafter\def\csname res@nc.asom_v2sp.f1pm\endcsname{0.186}
\expandafter\def\csname res@nc.asom_v2sp.f1primary\endcsname{0.240}
\expandafter\def\csname res@nc.asom_v2sp.f1secondary\endcsname{0.101}
\expandafter\def\csname res@nc.asom_v2sp.gap\endcsname{-0.015}
\expandafter\def\csname res@nc.asom_v2sp.gapci\endcsname{[-0.022, -0.007]}
\expandafter\def\csname res@nc.asom_v2sp_em.acc\endcsname{0.158}
\expandafter\def\csname res@nc.asom_v2sp_em.aucknown\endcsname{0.641}
\expandafter\def\csname res@nc.asom_v2sp_em.aucnew\endcsname{0.620}
\expandafter\def\csname res@nc.asom_v2sp_em.aucprimary\endcsname{0.653}
\expandafter\def\csname res@nc.asom_v2sp_em.aucsecondary\endcsname{0.633}
\expandafter\def\csname res@nc.asom_v2sp_em.f1\endcsname{0.076}
\expandafter\def\csname res@nc.asom_v2sp_em.f1ci\endcsname{[0.071, 0.081]}
\expandafter\def\csname res@nc.asom_v2sp_em.f1known\endcsname{0.082}
\expandafter\def\csname res@nc.asom_v2sp_em.f1new\endcsname{0.071}
\expandafter\def\csname res@nc.asom_v2sp_em.f1pm\endcsname{0.115}
\expandafter\def\csname res@nc.asom_v2sp_em.f1primary\endcsname{0.148}
\expandafter\def\csname res@nc.asom_v2sp_em.f1secondary\endcsname{0.032}
\expandafter\def\csname res@nc.asom_v2sp_em.gap\endcsname{+0.059}
\expandafter\def\csname res@nc.asom_v2sp_em.gapci\endcsname{[+0.051, +0.066]}
\expandafter\def\csname res@nc.asom_v2sp_s43.acc\endcsname{0.188}
\expandafter\def\csname res@nc.asom_v2sp_s43.aucknown\endcsname{0.644}
\expandafter\def\csname res@nc.asom_v2sp_s43.aucnew\endcsname{0.631}
\expandafter\def\csname res@nc.asom_v2sp_s43.aucprimary\endcsname{0.673}
\expandafter\def\csname res@nc.asom_v2sp_s43.aucsecondary\endcsname{0.621}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1\endcsname{0.147}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1ci\endcsname{[0.137, 0.156]}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1known\endcsname{0.161}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1new\endcsname{0.135}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1pm\endcsname{0.188}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1primary\endcsname{0.244}
\expandafter\def\csname res@nc.asom_v2sp_s43.f1secondary\endcsname{0.097}
\expandafter\def\csname res@nc.asom_v2sp_s43.gap\endcsname{-0.012}
\expandafter\def\csname res@nc.asom_v2sp_s43.gapci\endcsname{[-0.020, -0.003]}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.acc\endcsname{0.192}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.aucknown\endcsname{0.646}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.aucnew\endcsname{0.632}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.aucprimary\endcsname{0.673}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.aucsecondary\endcsname{0.625}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1\endcsname{0.158}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1ci\endcsname{[0.149, 0.168]}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1known\endcsname{0.166}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1new\endcsname{0.151}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1pm\endcsname{0.190}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1primary\endcsname{0.235}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.f1secondary\endcsname{0.113}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.gap\endcsname{-0.023}
\expandafter\def\csname res@nc.asom_v2sp_s43_noprior.gapci\endcsname{[-0.032, -0.014]}
\expandafter\def\csname res@nc.asom_v2sp_s44.acc\endcsname{0.195}
\expandafter\def\csname res@nc.asom_v2sp_s44.aucknown\endcsname{0.644}
\expandafter\def\csname res@nc.asom_v2sp_s44.aucnew\endcsname{0.634}
\expandafter\def\csname res@nc.asom_v2sp_s44.aucprimary\endcsname{0.675}
\expandafter\def\csname res@nc.asom_v2sp_s44.aucsecondary\endcsname{0.620}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1\endcsname{0.154}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1ci\endcsname{[0.144, 0.163]}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1known\endcsname{0.166}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1new\endcsname{0.144}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1pm\endcsname{0.184}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1primary\endcsname{0.241}
\expandafter\def\csname res@nc.asom_v2sp_s44.f1secondary\endcsname{0.107}
\expandafter\def\csname res@nc.asom_v2sp_s44.gap\endcsname{-0.019}
\expandafter\def\csname res@nc.asom_v2sp_s44.gapci\endcsname{[-0.027, -0.010]}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.acc\endcsname{0.196}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.aucknown\endcsname{0.646}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.aucnew\endcsname{0.635}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.aucprimary\endcsname{0.674}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.aucsecondary\endcsname{0.624}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1\endcsname{0.161}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1ci\endcsname{[0.151, 0.171]}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1known\endcsname{0.174}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1new\endcsname{0.151}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1pm\endcsname{0.187}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1primary\endcsname{0.234}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.f1secondary\endcsname{0.127}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.gap\endcsname{-0.026}
\expandafter\def\csname res@nc.asom_v2sp_s44_noprior.gapci\endcsname{[-0.035, -0.017]}
\expandafter\def\csname res@nc.asom_v2sp_s45.acc\endcsname{0.191}
\expandafter\def\csname res@nc.asom_v2sp_s45.aucknown\endcsname{0.645}
\expandafter\def\csname res@nc.asom_v2sp_s45.aucnew\endcsname{0.633}
\expandafter\def\csname res@nc.asom_v2sp_s45.aucprimary\endcsname{0.671}
\expandafter\def\csname res@nc.asom_v2sp_s45.aucsecondary\endcsname{0.625}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1\endcsname{0.149}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1ci\endcsname{[0.139, 0.157]}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1known\endcsname{0.158}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1new\endcsname{0.141}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1pm\endcsname{0.187}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1primary\endcsname{0.236}
\expandafter\def\csname res@nc.asom_v2sp_s45.f1secondary\endcsname{0.098}
\expandafter\def\csname res@nc.asom_v2sp_s45.gap\endcsname{-0.013}
\expandafter\def\csname res@nc.asom_v2sp_s45.gapci\endcsname{[-0.022, -0.005]}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.acc\endcsname{0.191}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.aucknown\endcsname{0.647}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.aucnew\endcsname{0.635}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.aucprimary\endcsname{0.671}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.aucsecondary\endcsname{0.629}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1\endcsname{0.155}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1ci\endcsname{[0.145, 0.165]}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1known\endcsname{0.157}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1new\endcsname{0.153}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1pm\endcsname{0.186}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1primary\endcsname{0.223}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.f1secondary\endcsname{0.106}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.gap\endcsname{-0.020}
\expandafter\def\csname res@nc.asom_v2sp_s45_noprior.gapci\endcsname{[-0.029, -0.011]}
\expandafter\def\csname res@nc.asom_v2sp_u.acc\endcsname{0.193}
\expandafter\def\csname res@nc.asom_v2sp_u.aucknown\endcsname{0.649}
\expandafter\def\csname res@nc.asom_v2sp_u.aucnew\endcsname{0.636}
\expandafter\def\csname res@nc.asom_v2sp_u.aucprimary\endcsname{0.675}
\expandafter\def\csname res@nc.asom_v2sp_u.aucsecondary\endcsname{0.628}
\expandafter\def\csname res@nc.asom_v2sp_u.f1\endcsname{0.158}
\expandafter\def\csname res@nc.asom_v2sp_u.f1ci\endcsname{[0.149, 0.167]}
\expandafter\def\csname res@nc.asom_v2sp_u.f1known\endcsname{0.166}
\expandafter\def\csname res@nc.asom_v2sp_u.f1new\endcsname{0.152}
\expandafter\def\csname res@nc.asom_v2sp_u.f1pm\endcsname{0.188}
\expandafter\def\csname res@nc.asom_v2sp_u.f1primary\endcsname{0.231}
\expandafter\def\csname res@nc.asom_v2sp_u.f1secondary\endcsname{0.115}
\expandafter\def\csname res@nc.asom_v2sp_u.gap\endcsname{-0.023}
\expandafter\def\csname res@nc.asom_v2sp_u.gapci\endcsname{[-0.031, -0.015]}
\expandafter\def\csname res@nc.bestalm.aucnew\endcsname{0.772}
\expandafter\def\csname res@nc.bestalm.aucnew.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@nc.bestalm.f1\endcsname{0.349}
\expandafter\def\csname res@nc.bestalm.f1.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@nc.bestalm.f1new\endcsname{0.368}
\expandafter\def\csname res@nc.bestalm.f1new.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@nc.bestalmcc.aucnew\endcsname{0.762}
\expandafter\def\csname res@nc.bestalmcc.aucnew.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@nc.bestalmcc.f1\endcsname{0.354}
\expandafter\def\csname res@nc.bestalmcc.f1.name\endcsname{Qwen2.5-Omni-3B + CC}
\expandafter\def\csname res@nc.bestalmcc.f1new\endcsname{0.372}
\expandafter\def\csname res@nc.bestalmcc.f1new.name\endcsname{Qwen2.5-Omni-3B + CC}
\expandafter\def\csname res@nc.bestclap.f1\endcsname{0.110}
\expandafter\def\csname res@nc.bestclap.name\endcsname{ParaCLAP}
\expandafter\def\csname res@nc.chance\endcsname{0.106}
\expandafter\def\csname res@nc.clap_laion.acc\endcsname{0.104}
\expandafter\def\csname res@nc.clap_laion.aucknown\endcsname{0.495}
\expandafter\def\csname res@nc.clap_laion.aucnew\endcsname{0.511}
\expandafter\def\csname res@nc.clap_laion.aucprimary\endcsname{0.479}
\expandafter\def\csname res@nc.clap_laion.aucsecondary\endcsname{0.506}
\expandafter\def\csname res@nc.clap_laion.f1\endcsname{0.060}
\expandafter\def\csname res@nc.clap_laion.f1ci\endcsname{[0.053, 0.066]}
\expandafter\def\csname res@nc.clap_laion.f1known\endcsname{0.038}
\expandafter\def\csname res@nc.clap_laion.f1new\endcsname{0.076}
\expandafter\def\csname res@nc.clap_laion.f1pm\endcsname{0.109}
\expandafter\def\csname res@nc.clap_laion.f1primary\endcsname{0.067}
\expandafter\def\csname res@nc.clap_laion.f1secondary\endcsname{0.015}
\expandafter\def\csname res@nc.clap_laion.gap\endcsname{+0.075}
\expandafter\def\csname res@nc.clap_laion.gapci\endcsname{[+0.065, +0.085]}
\expandafter\def\csname res@nc.clap_laion_desc.acc\endcsname{0.110}
\expandafter\def\csname res@nc.clap_laion_desc.aucknown\endcsname{0.516}
\expandafter\def\csname res@nc.clap_laion_desc.aucnew\endcsname{0.514}
\expandafter\def\csname res@nc.clap_laion_desc.aucprimary\endcsname{0.515}
\expandafter\def\csname res@nc.clap_laion_desc.aucsecondary\endcsname{0.517}
\expandafter\def\csname res@nc.clap_laion_desc.f1\endcsname{0.076}
\expandafter\def\csname res@nc.clap_laion_desc.f1ci\endcsname{[0.068, 0.083]}
\expandafter\def\csname res@nc.clap_laion_desc.f1known\endcsname{0.099}
\expandafter\def\csname res@nc.clap_laion_desc.f1new\endcsname{0.058}
\expandafter\def\csname res@nc.clap_laion_desc.f1pm\endcsname{0.110}
\expandafter\def\csname res@nc.clap_laion_desc.f1primary\endcsname{0.089}
\expandafter\def\csname res@nc.clap_laion_desc.f1secondary\endcsname{0.107}
\expandafter\def\csname res@nc.clap_laion_desc.gap\endcsname{+0.059}
\expandafter\def\csname res@nc.clap_laion_desc.gapci\endcsname{[+0.049, +0.070]}
\expandafter\def\csname res@nc.clap_ms.acc\endcsname{0.122}
\expandafter\def\csname res@nc.clap_ms.aucknown\endcsname{0.564}
\expandafter\def\csname res@nc.clap_ms.aucnew\endcsname{0.521}
\expandafter\def\csname res@nc.clap_ms.aucprimary\endcsname{0.554}
\expandafter\def\csname res@nc.clap_ms.aucsecondary\endcsname{0.572}
\expandafter\def\csname res@nc.clap_ms.f1\endcsname{0.074}
\expandafter\def\csname res@nc.clap_ms.f1ci\endcsname{[0.067, 0.080]}
\expandafter\def\csname res@nc.clap_ms.f1known\endcsname{0.095}
\expandafter\def\csname res@nc.clap_ms.f1new\endcsname{0.057}
\expandafter\def\csname res@nc.clap_ms.f1pm\endcsname{0.126}
\expandafter\def\csname res@nc.clap_ms.f1primary\endcsname{0.049}
\expandafter\def\csname res@nc.clap_ms.f1secondary\endcsname{0.130}
\expandafter\def\csname res@nc.clap_ms.gap\endcsname{+0.061}
\expandafter\def\csname res@nc.clap_ms.gapci\endcsname{[+0.051, +0.071]}
\expandafter\def\csname res@nc.clap_ms_desc.acc\endcsname{0.113}
\expandafter\def\csname res@nc.clap_ms_desc.aucknown\endcsname{0.540}
\expandafter\def\csname res@nc.clap_ms_desc.aucnew\endcsname{0.518}
\expandafter\def\csname res@nc.clap_ms_desc.aucprimary\endcsname{0.553}
\expandafter\def\csname res@nc.clap_ms_desc.aucsecondary\endcsname{0.530}
\expandafter\def\csname res@nc.clap_ms_desc.f1\endcsname{0.049}
\expandafter\def\csname res@nc.clap_ms_desc.f1ci\endcsname{[0.044, 0.054]}
\expandafter\def\csname res@nc.clap_ms_desc.f1known\endcsname{0.075}
\expandafter\def\csname res@nc.clap_ms_desc.f1new\endcsname{0.030}
\expandafter\def\csname res@nc.clap_ms_desc.f1pm\endcsname{0.127}
\expandafter\def\csname res@nc.clap_ms_desc.f1primary\endcsname{0.142}
\expandafter\def\csname res@nc.clap_ms_desc.f1secondary\endcsname{0.022}
\expandafter\def\csname res@nc.clap_ms_desc.gap\endcsname{+0.086}
\expandafter\def\csname res@nc.clap_ms_desc.gapci\endcsname{[+0.077, +0.095]}
\expandafter\def\csname res@nc.clap_para.acc\endcsname{0.140}
\expandafter\def\csname res@nc.clap_para.aucknown\endcsname{0.576}
\expandafter\def\csname res@nc.clap_para.aucnew\endcsname{0.561}
\expandafter\def\csname res@nc.clap_para.aucprimary\endcsname{0.594}
\expandafter\def\csname res@nc.clap_para.aucsecondary\endcsname{0.561}
\expandafter\def\csname res@nc.clap_para.f1\endcsname{0.110}
\expandafter\def\csname res@nc.clap_para.f1ci\endcsname{[0.101, 0.118]}
\expandafter\def\csname res@nc.clap_para.f1known\endcsname{0.128}
\expandafter\def\csname res@nc.clap_para.f1new\endcsname{0.096}
\expandafter\def\csname res@nc.clap_para.f1pm\endcsname{0.117}
\expandafter\def\csname res@nc.clap_para.f1primary\endcsname{0.151}
\expandafter\def\csname res@nc.clap_para.f1secondary\endcsname{0.111}
\expandafter\def\csname res@nc.clap_para.gap\endcsname{+0.025}
\expandafter\def\csname res@nc.clap_para.gapci\endcsname{[+0.014, +0.036]}
\expandafter\def\csname res@nc.clap_para_desc.acc\endcsname{0.128}
\expandafter\def\csname res@nc.clap_para_desc.aucknown\endcsname{0.547}
\expandafter\def\csname res@nc.clap_para_desc.aucnew\endcsname{0.534}
\expandafter\def\csname res@nc.clap_para_desc.aucprimary\endcsname{0.540}
\expandafter\def\csname res@nc.clap_para_desc.aucsecondary\endcsname{0.552}
\expandafter\def\csname res@nc.clap_para_desc.f1\endcsname{0.094}
\expandafter\def\csname res@nc.clap_para_desc.f1ci\endcsname{[0.086, 0.102]}
\expandafter\def\csname res@nc.clap_para_desc.f1known\endcsname{0.103}
\expandafter\def\csname res@nc.clap_para_desc.f1new\endcsname{0.087}
\expandafter\def\csname res@nc.clap_para_desc.f1pm\endcsname{0.099}
\expandafter\def\csname res@nc.clap_para_desc.f1primary\endcsname{0.105}
\expandafter\def\csname res@nc.clap_para_desc.f1secondary\endcsname{0.101}
\expandafter\def\csname res@nc.clap_para_desc.gap\endcsname{+0.041}
\expandafter\def\csname res@nc.clap_para_desc.gapci\endcsname{[+0.031, +0.052]}
\expandafter\def\csname res@nc.clips\endcsname{4,560}
\expandafter\def\csname res@nc.emotions\endcsname{38}
\expandafter\def\csname res@nc.known\endcsname{16}
\expandafter\def\csname res@nc.menus\endcsname{4}
\expandafter\def\csname res@nc.new\endcsname{22}
\expandafter\def\csname res@nc.omni3b.acc\endcsname{0.334}
\expandafter\def\csname res@nc.omni3b.aucknown\endcsname{0.725}
\expandafter\def\csname res@nc.omni3b.aucnew\endcsname{0.739}
\expandafter\def\csname res@nc.omni3b.aucprimary\endcsname{0.730}
\expandafter\def\csname res@nc.omni3b.aucsecondary\endcsname{0.721}
\expandafter\def\csname res@nc.omni3b.f1\endcsname{0.328}
\expandafter\def\csname res@nc.omni3b.f1ci\endcsname{[0.314, 0.341]}
\expandafter\def\csname res@nc.omni3b.f1known\endcsname{0.307}
\expandafter\def\csname res@nc.omni3b.f1new\endcsname{0.343}
\expandafter\def\csname res@nc.omni3b.f1pm\endcsname{0.356}
\expandafter\def\csname res@nc.omni3b.f1primary\endcsname{0.314}
\expandafter\def\csname res@nc.omni3b.f1secondary\endcsname{0.302}
\expandafter\def\csname res@nc.omni3b.gap\endcsname{-0.193}
\expandafter\def\csname res@nc.omni3b.gapci\endcsname{[-0.207, -0.178]}
\expandafter\def\csname res@nc.omni3b_cc.acc\endcsname{0.359}
\expandafter\def\csname res@nc.omni3b_cc.aucknown\endcsname{0.728}
\expandafter\def\csname res@nc.omni3b_cc.aucnew\endcsname{0.739}
\expandafter\def\csname res@nc.omni3b_cc.aucprimary\endcsname{0.733}
\expandafter\def\csname res@nc.omni3b_cc.aucsecondary\endcsname{0.724}
\expandafter\def\csname res@nc.omni3b_cc.f1\endcsname{0.354}
\expandafter\def\csname res@nc.omni3b_cc.f1ci\endcsname{[0.339, 0.366]}
\expandafter\def\csname res@nc.omni3b_cc.f1known\endcsname{0.326}
\expandafter\def\csname res@nc.omni3b_cc.f1new\endcsname{0.372}
\expandafter\def\csname res@nc.omni3b_cc.f1pm\endcsname{0.365}
\expandafter\def\csname res@nc.omni3b_cc.f1primary\endcsname{0.338}
\expandafter\def\csname res@nc.omni3b_cc.f1secondary\endcsname{0.316}
\expandafter\def\csname res@nc.omni3b_cc.gap\endcsname{-0.219}
\expandafter\def\csname res@nc.omni3b_cc.gapci\endcsname{[-0.232, -0.203]}
\expandafter\def\csname res@nc.omni3b_ft.acc\endcsname{0.307}
\expandafter\def\csname res@nc.omni3b_ft.aucknown\endcsname{0.759}
\expandafter\def\csname res@nc.omni3b_ft.aucnew\endcsname{0.777}
\expandafter\def\csname res@nc.omni3b_ft.aucprimary\endcsname{0.775}
\expandafter\def\csname res@nc.omni3b_ft.aucsecondary\endcsname{0.746}
\expandafter\def\csname res@nc.omni3b_ft.f1\endcsname{0.282}
\expandafter\def\csname res@nc.omni3b_ft.f1ci\endcsname{[0.269, 0.295]}
\expandafter\def\csname res@nc.omni3b_ft.f1known\endcsname{0.275}
\expandafter\def\csname res@nc.omni3b_ft.f1new\endcsname{0.289}
\expandafter\def\csname res@nc.omni3b_ft.f1pm\endcsname{0.367}
\expandafter\def\csname res@nc.omni3b_ft.f1primary\endcsname{0.318}
\expandafter\def\csname res@nc.omni3b_ft.f1secondary\endcsname{0.241}
\expandafter\def\csname res@nc.omni3b_ft.gap\endcsname{-0.147}
\expandafter\def\csname res@nc.omni3b_ft.gapci\endcsname{[-0.160, -0.133]}
\expandafter\def\csname res@nc.omni3b_ftfull.acc\endcsname{0.290}
\expandafter\def\csname res@nc.omni3b_ftfull.aucknown\endcsname{0.744}
\expandafter\def\csname res@nc.omni3b_ftfull.aucnew\endcsname{0.758}
\expandafter\def\csname res@nc.omni3b_ftfull.aucprimary\endcsname{0.759}
\expandafter\def\csname res@nc.omni3b_ftfull.aucsecondary\endcsname{0.733}
\expandafter\def\csname res@nc.omni3b_ftfull.f1\endcsname{0.258}
\expandafter\def\csname res@nc.omni3b_ftfull.f1ci\endcsname{[0.245, 0.269]}
\expandafter\def\csname res@nc.omni3b_ftfull.f1known\endcsname{0.249}
\expandafter\def\csname res@nc.omni3b_ftfull.f1new\endcsname{0.264}
\expandafter\def\csname res@nc.omni3b_ftfull.f1pm\endcsname{0.346}
\expandafter\def\csname res@nc.omni3b_ftfull.f1primary\endcsname{0.307}
\expandafter\def\csname res@nc.omni3b_ftfull.f1secondary\endcsname{0.204}
\expandafter\def\csname res@nc.omni3b_ftfull.gap\endcsname{-0.123}
\expandafter\def\csname res@nc.omni3b_ftfull.gapci\endcsname{[-0.135, -0.109]}
\expandafter\def\csname res@nc.omni7b.acc\endcsname{0.359}
\expandafter\def\csname res@nc.omni7b.aucknown\endcsname{0.746}
\expandafter\def\csname res@nc.omni7b.aucnew\endcsname{0.772}
\expandafter\def\csname res@nc.omni7b.aucprimary\endcsname{0.749}
\expandafter\def\csname res@nc.omni7b.aucsecondary\endcsname{0.744}
\expandafter\def\csname res@nc.omni7b.f1\endcsname{0.349}
\expandafter\def\csname res@nc.omni7b.f1ci\endcsname{[0.335, 0.362]}
\expandafter\def\csname res@nc.omni7b.f1known\endcsname{0.324}
\expandafter\def\csname res@nc.omni7b.f1new\endcsname{0.368}
\expandafter\def\csname res@nc.omni7b.f1pm\endcsname{0.364}
\expandafter\def\csname res@nc.omni7b.f1primary\endcsname{0.331}
\expandafter\def\csname res@nc.omni7b.f1secondary\endcsname{0.319}
\expandafter\def\csname res@nc.omni7b.gap\endcsname{-0.214}
\expandafter\def\csname res@nc.omni7b.gapci\endcsname{[-0.228, -0.199]}
\expandafter\def\csname res@nc.omni7b_cc.acc\endcsname{0.359}
\expandafter\def\csname res@nc.omni7b_cc.aucknown\endcsname{0.748}
\expandafter\def\csname res@nc.omni7b_cc.aucnew\endcsname{0.762}
\expandafter\def\csname res@nc.omni7b_cc.aucprimary\endcsname{0.749}
\expandafter\def\csname res@nc.omni7b_cc.aucsecondary\endcsname{0.747}
\expandafter\def\csname res@nc.omni7b_cc.f1\endcsname{0.348}
\expandafter\def\csname res@nc.omni7b_cc.f1ci\endcsname{[0.335, 0.361]}
\expandafter\def\csname res@nc.omni7b_cc.f1known\endcsname{0.325}
\expandafter\def\csname res@nc.omni7b_cc.f1new\endcsname{0.366}
\expandafter\def\csname res@nc.omni7b_cc.f1pm\endcsname{0.364}
\expandafter\def\csname res@nc.omni7b_cc.f1primary\endcsname{0.328}
\expandafter\def\csname res@nc.omni7b_cc.f1secondary\endcsname{0.323}
\expandafter\def\csname res@nc.omni7b_cc.gap\endcsname{-0.213}
\expandafter\def\csname res@nc.omni7b_cc.gapci\endcsname{[-0.227, -0.198]}
\expandafter\def\csname res@nc.omni7b_text.acc\endcsname{0.354}
\expandafter\def\csname res@nc.omni7b_text.aucknown\endcsname{0.736}
\expandafter\def\csname res@nc.omni7b_text.aucnew\endcsname{0.770}
\expandafter\def\csname res@nc.omni7b_text.aucprimary\endcsname{0.749}
\expandafter\def\csname res@nc.omni7b_text.aucsecondary\endcsname{0.726}
\expandafter\def\csname res@nc.omni7b_text.f1\endcsname{0.342}
\expandafter\def\csname res@nc.omni7b_text.f1ci\endcsname{[0.328, 0.356]}
\expandafter\def\csname res@nc.omni7b_text.f1known\endcsname{0.309}
\expandafter\def\csname res@nc.omni7b_text.f1new\endcsname{0.368}
\expandafter\def\csname res@nc.omni7b_text.f1pm\endcsname{0.355}
\expandafter\def\csname res@nc.omni7b_text.f1primary\endcsname{0.339}
\expandafter\def\csname res@nc.omni7b_text.f1secondary\endcsname{0.285}
\expandafter\def\csname res@nc.omni7b_text.gap\endcsname{-0.207}
\expandafter\def\csname res@nc.omni7b_text.gapci\endcsname{[-0.221, -0.192]}
\expandafter\def\csname res@nc.phi4mm.acc\endcsname{0.287}
\expandafter\def\csname res@nc.phi4mm.aucknown\endcsname{0.693}
\expandafter\def\csname res@nc.phi4mm.aucnew\endcsname{0.705}
\expandafter\def\csname res@nc.phi4mm.aucprimary\endcsname{0.725}
\expandafter\def\csname res@nc.phi4mm.aucsecondary\endcsname{0.667}
\expandafter\def\csname res@nc.phi4mm.f1\endcsname{0.271}
\expandafter\def\csname res@nc.phi4mm.f1ci\endcsname{[0.258, 0.283]}
\expandafter\def\csname res@nc.phi4mm.f1known\endcsname{0.290}
\expandafter\def\csname res@nc.phi4mm.f1new\endcsname{0.259}
\expandafter\def\csname res@nc.phi4mm.f1pm\endcsname{0.312}
\expandafter\def\csname res@nc.phi4mm.f1primary\endcsname{0.308}
\expandafter\def\csname res@nc.phi4mm.f1secondary\endcsname{0.276}
\expandafter\def\csname res@nc.phi4mm.gap\endcsname{-0.136}
\expandafter\def\csname res@nc.phi4mm.gapci\endcsname{[-0.150, -0.122]}
\expandafter\def\csname res@nc.phi4mm_cc.acc\endcsname{0.301}
\expandafter\def\csname res@nc.phi4mm_cc.aucknown\endcsname{0.699}
\expandafter\def\csname res@nc.phi4mm_cc.aucnew\endcsname{0.712}
\expandafter\def\csname res@nc.phi4mm_cc.aucprimary\endcsname{0.706}
\expandafter\def\csname res@nc.phi4mm_cc.aucsecondary\endcsname{0.693}
\expandafter\def\csname res@nc.phi4mm_cc.f1\endcsname{0.283}
\expandafter\def\csname res@nc.phi4mm_cc.f1ci\endcsname{[0.269, 0.294]}
\expandafter\def\csname res@nc.phi4mm_cc.f1known\endcsname{0.280}
\expandafter\def\csname res@nc.phi4mm_cc.f1new\endcsname{0.284}
\expandafter\def\csname res@nc.phi4mm_cc.f1pm\endcsname{0.319}
\expandafter\def\csname res@nc.phi4mm_cc.f1primary\endcsname{0.278}
\expandafter\def\csname res@nc.phi4mm_cc.f1secondary\endcsname{0.282}
\expandafter\def\csname res@nc.phi4mm_cc.gap\endcsname{-0.147}
\expandafter\def\csname res@nc.phi4mm_cc.gapci\endcsname{[-0.161, -0.133]}
\expandafter\def\csname res@nc.primary\endcsname{7}
\expandafter\def\csname res@nc.qwen2audio7b.acc\endcsname{0.273}
\expandafter\def\csname res@nc.qwen2audio7b.aucknown\endcsname{0.678}
\expandafter\def\csname res@nc.qwen2audio7b.aucnew\endcsname{0.680}
\expandafter\def\csname res@nc.qwen2audio7b.aucprimary\endcsname{0.698}
\expandafter\def\csname res@nc.qwen2audio7b.aucsecondary\endcsname{0.662}
\expandafter\def\csname res@nc.qwen2audio7b.f1\endcsname{0.257}
\expandafter\def\csname res@nc.qwen2audio7b.f1ci\endcsname{[0.244, 0.269]}
\expandafter\def\csname res@nc.qwen2audio7b.f1known\endcsname{0.269}
\expandafter\def\csname res@nc.qwen2audio7b.f1new\endcsname{0.249}
\expandafter\def\csname res@nc.qwen2audio7b.f1pm\endcsname{0.293}
\expandafter\def\csname res@nc.qwen2audio7b.f1primary\endcsname{0.299}
\expandafter\def\csname res@nc.qwen2audio7b.f1secondary\endcsname{0.246}
\expandafter\def\csname res@nc.qwen2audio7b.gap\endcsname{-0.122}
\expandafter\def\csname res@nc.qwen2audio7b.gapci\endcsname{[-0.135, -0.108]}
\expandafter\def\csname res@nc.qwen2audio7b_cc.acc\endcsname{0.272}
\expandafter\def\csname res@nc.qwen2audio7b_cc.aucknown\endcsname{0.683}
\expandafter\def\csname res@nc.qwen2audio7b_cc.aucnew\endcsname{0.687}
\expandafter\def\csname res@nc.qwen2audio7b_cc.aucprimary\endcsname{0.688}
\expandafter\def\csname res@nc.qwen2audio7b_cc.aucsecondary\endcsname{0.679}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1\endcsname{0.256}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1ci\endcsname{[0.242, 0.267]}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1known\endcsname{0.285}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1new\endcsname{0.233}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1pm\endcsname{0.297}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1primary\endcsname{0.308}
\expandafter\def\csname res@nc.qwen2audio7b_cc.f1secondary\endcsname{0.267}
\expandafter\def\csname res@nc.qwen2audio7b_cc.gap\endcsname{-0.120}
\expandafter\def\csname res@nc.qwen2audio7b_cc.gapci\endcsname{[-0.134, -0.106]}
\expandafter\def\csname res@nc.secondary\endcsname{9}
\expandafter\def\csname res@nc.voxtral3b.acc\endcsname{0.319}
\expandafter\def\csname res@nc.voxtral3b.aucknown\endcsname{0.700}
\expandafter\def\csname res@nc.voxtral3b.aucnew\endcsname{0.716}
\expandafter\def\csname res@nc.voxtral3b.aucprimary\endcsname{0.701}
\expandafter\def\csname res@nc.voxtral3b.aucsecondary\endcsname{0.700}
\expandafter\def\csname res@nc.voxtral3b.f1\endcsname{0.318}
\expandafter\def\csname res@nc.voxtral3b.f1ci\endcsname{[0.304, 0.330]}
\expandafter\def\csname res@nc.voxtral3b.f1known\endcsname{0.320}
\expandafter\def\csname res@nc.voxtral3b.f1new\endcsname{0.316}
\expandafter\def\csname res@nc.voxtral3b.f1pm\endcsname{0.333}
\expandafter\def\csname res@nc.voxtral3b.f1primary\endcsname{0.322}
\expandafter\def\csname res@nc.voxtral3b.f1secondary\endcsname{0.318}
\expandafter\def\csname res@nc.voxtral3b.gap\endcsname{-0.183}
\expandafter\def\csname res@nc.voxtral3b.gapci\endcsname{[-0.197, -0.167]}
\expandafter\def\csname res@nc.voxtral3b_cc.acc\endcsname{0.338}
\expandafter\def\csname res@nc.voxtral3b_cc.aucknown\endcsname{0.706}
\expandafter\def\csname res@nc.voxtral3b_cc.aucnew\endcsname{0.714}
\expandafter\def\csname res@nc.voxtral3b_cc.aucprimary\endcsname{0.705}
\expandafter\def\csname res@nc.voxtral3b_cc.aucsecondary\endcsname{0.707}
\expandafter\def\csname res@nc.voxtral3b_cc.f1\endcsname{0.335}
\expandafter\def\csname res@nc.voxtral3b_cc.f1ci\endcsname{[0.320, 0.348]}
\expandafter\def\csname res@nc.voxtral3b_cc.f1known\endcsname{0.321}
\expandafter\def\csname res@nc.voxtral3b_cc.f1new\endcsname{0.345}
\expandafter\def\csname res@nc.voxtral3b_cc.f1pm\endcsname{0.342}
\expandafter\def\csname res@nc.voxtral3b_cc.f1primary\endcsname{0.322}
\expandafter\def\csname res@nc.voxtral3b_cc.f1secondary\endcsname{0.321}
\expandafter\def\csname res@nc.voxtral3b_cc.gap\endcsname{-0.200}
\expandafter\def\csname res@nc.voxtral3b_cc.gapci\endcsname{[-0.214, -0.185]}
\expandafter\def\csname res@omni3b.full.delta\endcsname{-0.123}
\expandafter\def\csname res@omni3b.full.deltaci\endcsname{[-0.146, -0.101]}
\expandafter\def\csname res@omni3b.full.deltaoff\endcsname{-0.124}
\expandafter\def\csname res@omni3b.full.deltaoffci\endcsname{[-0.148, -0.103]}
\expandafter\def\csname res@omni3b.full.ece\endcsname{0.215}
\expandafter\def\csname res@omni3b.full.ecev\endcsname{0.281}
\expandafter\def\csname res@omni3b.full.ecevoracle\endcsname{0.021}
\expandafter\def\csname res@omni3b.full.f1\endcsname{0.259}
\expandafter\def\csname res@omni3b.full.f1ci\endcsname{[0.248, 0.269]}
\expandafter\def\csname res@omni3b.full.f1off\endcsname{0.277}
\expandafter\def\csname res@omni3b.full.f1offci\endcsname{[0.262, 0.294]}
\expandafter\def\csname res@omni3b.full.gap\endcsname{0.123}
\expandafter\def\csname res@omni3b.full.gapci\endcsname{[0.101, 0.146]}
\expandafter\def\csname res@omni3b.full.ll\endcsname{2.257}
\expandafter\def\csname res@omni3b.full.lloracle\endcsname{1.878}
\expandafter\def\csname res@omni3b.full.toracle\endcsname{2.55}
\expandafter\def\csname res@omni3b.subset.delta\endcsname{-0.128}
\expandafter\def\csname res@omni3b.subset.deltaci\endcsname{[-0.162, -0.099]}
\expandafter\def\csname res@omni3b.subset.deltaoff\endcsname{-0.109}
\expandafter\def\csname res@omni3b.subset.deltaoffci\endcsname{[-0.146, -0.076]}
\expandafter\def\csname res@omni3b.subset.ece\endcsname{0.215}
\expandafter\def\csname res@omni3b.subset.ecev\endcsname{0.284}
\expandafter\def\csname res@omni3b.subset.ecevoracle\endcsname{0.022}
\expandafter\def\csname res@omni3b.subset.f1\endcsname{0.256}
\expandafter\def\csname res@omni3b.subset.f1ci\endcsname{[0.235, 0.273]}
\expandafter\def\csname res@omni3b.subset.f1off\endcsname{0.285}
\expandafter\def\csname res@omni3b.subset.f1offci\endcsname{[0.261, 0.312]}
\expandafter\def\csname res@omni3b.subset.gap\endcsname{0.128}
\expandafter\def\csname res@omni3b.subset.gapci\endcsname{[0.099, 0.162]}
\expandafter\def\csname res@omni3b.subset.ll\endcsname{2.283}
\expandafter\def\csname res@omni3b.subset.lloracle\endcsname{1.886}
\expandafter\def\csname res@omni3b.subset.toracle\endcsname{2.60}
\expandafter\def\csname res@omni3b_cc.full.delta\endcsname{-0.089}
\expandafter\def\csname res@omni3b_cc.full.deltaci\endcsname{[-0.107, -0.074]}
\expandafter\def\csname res@omni3b_cc.full.deltaoff\endcsname{-0.093}
\expandafter\def\csname res@omni3b_cc.full.deltaoffci\endcsname{[-0.114, -0.076]}
\expandafter\def\csname res@omni3b_cc.full.ece\endcsname{0.125}
\expandafter\def\csname res@omni3b_cc.full.ecev\endcsname{0.165}
\expandafter\def\csname res@omni3b_cc.full.ecevoracle\endcsname{0.067}
\expandafter\def\csname res@omni3b_cc.full.f1\endcsname{0.293}
\expandafter\def\csname res@omni3b_cc.full.f1ci\endcsname{[0.279, 0.303]}
\expandafter\def\csname res@omni3b_cc.full.f1off\endcsname{0.309}
\expandafter\def\csname res@omni3b_cc.full.f1offci\endcsname{[0.291, 0.323]}
\expandafter\def\csname res@omni3b_cc.full.gap\endcsname{0.089}
\expandafter\def\csname res@omni3b_cc.full.gapci\endcsname{[0.074, 0.107]}
\expandafter\def\csname res@omni3b_cc.full.ll\endcsname{2.081}
\expandafter\def\csname res@omni3b_cc.full.lloracle\endcsname{1.893}
\expandafter\def\csname res@omni3b_cc.full.toracle\endcsname{2.15}
\expandafter\def\csname res@omni3b_cc.subset.delta\endcsname{-0.084}
\expandafter\def\csname res@omni3b_cc.subset.deltaci\endcsname{[-0.111, -0.064]}
\expandafter\def\csname res@omni3b_cc.subset.deltaoff\endcsname{-0.074}
\expandafter\def\csname res@omni3b_cc.subset.deltaoffci\endcsname{[-0.100, -0.049]}
\expandafter\def\csname res@omni3b_cc.subset.ece\endcsname{0.131}
\expandafter\def\csname res@omni3b_cc.subset.ecev\endcsname{0.169}
\expandafter\def\csname res@omni3b_cc.subset.ecevoracle\endcsname{0.065}
\expandafter\def\csname res@omni3b_cc.subset.f1\endcsname{0.299}
\expandafter\def\csname res@omni3b_cc.subset.f1ci\endcsname{[0.278, 0.319]}
\expandafter\def\csname res@omni3b_cc.subset.f1off\endcsname{0.320}
\expandafter\def\csname res@omni3b_cc.subset.f1offci\endcsname{[0.295, 0.347]}
\expandafter\def\csname res@omni3b_cc.subset.gap\endcsname{0.084}
\expandafter\def\csname res@omni3b_cc.subset.gapci\endcsname{[0.064, 0.111]}
\expandafter\def\csname res@omni3b_cc.subset.ll\endcsname{2.090}
\expandafter\def\csname res@omni3b_cc.subset.lloracle\endcsname{1.897}
\expandafter\def\csname res@omni3b_cc.subset.toracle\endcsname{2.16}
\expandafter\def\csname res@omni3b_ft.subset.delta\endcsname{-0.061}
\expandafter\def\csname res@omni3b_ft.subset.deltaci\endcsname{[-0.083, -0.039]}
\expandafter\def\csname res@omni3b_ft.subset.deltaoff\endcsname{-0.026}
\expandafter\def\csname res@omni3b_ft.subset.deltaoffci\endcsname{[-0.049, +0.009]}
\expandafter\def\csname res@omni3b_ft.subset.ece\endcsname{0.046}
\expandafter\def\csname res@omni3b_ft.subset.ecev\endcsname{0.058}
\expandafter\def\csname res@omni3b_ft.subset.ecevoracle\endcsname{0.010}
\expandafter\def\csname res@omni3b_ft.subset.f1\endcsname{0.322}
\expandafter\def\csname res@omni3b_ft.subset.f1ci\endcsname{[0.299, 0.348]}
\expandafter\def\csname res@omni3b_ft.subset.f1off\endcsname{0.368}
\expandafter\def\csname res@omni3b_ft.subset.f1offci\endcsname{[0.328, 0.424]}
\expandafter\def\csname res@omni3b_ft.subset.gap\endcsname{0.061}
\expandafter\def\csname res@omni3b_ft.subset.gapci\endcsname{[0.039, 0.083]}
\expandafter\def\csname res@omni3b_ft.subset.ll\endcsname{1.513}
\expandafter\def\csname res@omni3b_ft.subset.lloracle\endcsname{1.497}
\expandafter\def\csname res@omni3b_ft.subset.toracle\endcsname{1.21}
\expandafter\def\csname res@omni3b_ftfull.subset.delta\endcsname{-0.026}
\expandafter\def\csname res@omni3b_ftfull.subset.deltaci\endcsname{[-0.050, -0.006]}
\expandafter\def\csname res@omni3b_ftfull.subset.deltaoff\endcsname{+0.010}
\expandafter\def\csname res@omni3b_ftfull.subset.deltaoffci\endcsname{[-0.017, +0.042]}
\expandafter\def\csname res@omni3b_ftfull.subset.ece\endcsname{0.049}
\expandafter\def\csname res@omni3b_ftfull.subset.ecev\endcsname{0.053}
\expandafter\def\csname res@omni3b_ftfull.subset.ecevoracle\endcsname{0.014}
\expandafter\def\csname res@omni3b_ftfull.subset.f1\endcsname{0.357}
\expandafter\def\csname res@omni3b_ftfull.subset.f1ci\endcsname{[0.332, 0.382]}
\expandafter\def\csname res@omni3b_ftfull.subset.f1off\endcsname{0.404}
\expandafter\def\csname res@omni3b_ftfull.subset.f1offci\endcsname{[0.359, 0.457]}
\expandafter\def\csname res@omni3b_ftfull.subset.gap\endcsname{0.026}
\expandafter\def\csname res@omni3b_ftfull.subset.gapci\endcsname{[0.006, 0.050]}
\expandafter\def\csname res@omni3b_ftfull.subset.ll\endcsname{1.485}
\expandafter\def\csname res@omni3b_ftfull.subset.lloracle\endcsname{1.472}
\expandafter\def\csname res@omni3b_ftfull.subset.toracle\endcsname{1.19}
\expandafter\def\csname res@omni7b.subset.delta\endcsname{-0.072}
\expandafter\def\csname res@omni7b.subset.deltaci\endcsname{[-0.097, -0.051]}
\expandafter\def\csname res@omni7b.subset.deltaoff\endcsname{-0.048}
\expandafter\def\csname res@omni7b.subset.deltaoffci\endcsname{[-0.072, -0.025]}
\expandafter\def\csname res@omni7b.subset.ece\endcsname{0.292}
\expandafter\def\csname res@omni7b.subset.ecev\endcsname{0.331}
\expandafter\def\csname res@omni7b.subset.ecevoracle\endcsname{0.020}
\expandafter\def\csname res@omni7b.subset.f1\endcsname{0.311}
\expandafter\def\csname res@omni7b.subset.f1ci\endcsname{[0.287, 0.334]}
\expandafter\def\csname res@omni7b.subset.f1off\endcsname{0.346}
\expandafter\def\csname res@omni7b.subset.f1offci\endcsname{[0.311, 0.379]}
\expandafter\def\csname res@omni7b.subset.gap\endcsname{0.072}
\expandafter\def\csname res@omni7b.subset.gapci\endcsname{[0.051, 0.097]}
\expandafter\def\csname res@omni7b.subset.ll\endcsname{2.332}
\expandafter\def\csname res@omni7b.subset.lloracle\endcsname{1.751}
\expandafter\def\csname res@omni7b.subset.toracle\endcsname{2.71}
\expandafter\def\csname res@omni7b_cc.subset.delta\endcsname{-0.105}
\expandafter\def\csname res@omni7b_cc.subset.deltaci\endcsname{[-0.127, -0.086]}
\expandafter\def\csname res@omni7b_cc.subset.deltaoff\endcsname{-0.088}
\expandafter\def\csname res@omni7b_cc.subset.deltaoffci\endcsname{[-0.114, -0.065]}
\expandafter\def\csname res@omni7b_cc.subset.ece\endcsname{0.319}
\expandafter\def\csname res@omni7b_cc.subset.ecev\endcsname{0.351}
\expandafter\def\csname res@omni7b_cc.subset.ecevoracle\endcsname{0.042}
\expandafter\def\csname res@omni7b_cc.subset.f1\endcsname{0.278}
\expandafter\def\csname res@omni7b_cc.subset.f1ci\endcsname{[0.255, 0.300]}
\expandafter\def\csname res@omni7b_cc.subset.f1off\endcsname{0.306}
\expandafter\def\csname res@omni7b_cc.subset.f1offci\endcsname{[0.275, 0.336]}
\expandafter\def\csname res@omni7b_cc.subset.gap\endcsname{0.105}
\expandafter\def\csname res@omni7b_cc.subset.gapci\endcsname{[0.086, 0.127]}
\expandafter\def\csname res@omni7b_cc.subset.ll\endcsname{2.612}
\expandafter\def\csname res@omni7b_cc.subset.lloracle\endcsname{1.886}
\expandafter\def\csname res@omni7b_cc.subset.toracle\endcsname{3.39}
\expandafter\def\csname res@omni7b_text.subset.delta\endcsname{-0.122}
\expandafter\def\csname res@omni7b_text.subset.deltaci\endcsname{[-0.148, -0.099]}
\expandafter\def\csname res@omni7b_text.subset.deltaoff\endcsname{-0.100}
\expandafter\def\csname res@omni7b_text.subset.deltaoffci\endcsname{[-0.128, -0.072]}
\expandafter\def\csname res@omni7b_text.subset.ece\endcsname{0.446}
\expandafter\def\csname res@omni7b_text.subset.ecev\endcsname{0.459}
\expandafter\def\csname res@omni7b_text.subset.ecevoracle\endcsname{0.023}
\expandafter\def\csname res@omni7b_text.subset.f1\endcsname{0.261}
\expandafter\def\csname res@omni7b_text.subset.f1ci\endcsname{[0.240, 0.283]}
\expandafter\def\csname res@omni7b_text.subset.f1off\endcsname{0.294}
\expandafter\def\csname res@omni7b_text.subset.f1offci\endcsname{[0.264, 0.328]}
\expandafter\def\csname res@omni7b_text.subset.gap\endcsname{0.122}
\expandafter\def\csname res@omni7b_text.subset.gapci\endcsname{[0.099, 0.148]}
\expandafter\def\csname res@omni7b_text.subset.ll\endcsname{3.083}
\expandafter\def\csname res@omni7b_text.subset.lloracle\endcsname{1.843}
\expandafter\def\csname res@omni7b_text.subset.toracle\endcsname{3.89}
\expandafter\def\csname res@phi4mm.subset.delta\endcsname{-0.144}
\expandafter\def\csname res@phi4mm.subset.deltaci\endcsname{[-0.166, -0.121]}
\expandafter\def\csname res@phi4mm.subset.deltaoff\endcsname{-0.140}
\expandafter\def\csname res@phi4mm.subset.deltaoffci\endcsname{[-0.166, -0.112]}
\expandafter\def\csname res@phi4mm.subset.ece\endcsname{0.262}
\expandafter\def\csname res@phi4mm.subset.ecev\endcsname{0.335}
\expandafter\def\csname res@phi4mm.subset.ecevoracle\endcsname{0.033}
\expandafter\def\csname res@phi4mm.subset.f1\endcsname{0.239}
\expandafter\def\csname res@phi4mm.subset.f1ci\endcsname{[0.219, 0.263]}
\expandafter\def\csname res@phi4mm.subset.f1off\endcsname{0.254}
\expandafter\def\csname res@phi4mm.subset.f1offci\endcsname{[0.225, 0.298]}
\expandafter\def\csname res@phi4mm.subset.gap\endcsname{0.144}
\expandafter\def\csname res@phi4mm.subset.gapci\endcsname{[0.121, 0.166]}
\expandafter\def\csname res@phi4mm.subset.ll\endcsname{2.466}
\expandafter\def\csname res@phi4mm.subset.lloracle\endcsname{1.849}
\expandafter\def\csname res@phi4mm.subset.toracle\endcsname{2.95}
\expandafter\def\csname res@phi4mm_cc.subset.delta\endcsname{-0.161}
\expandafter\def\csname res@phi4mm_cc.subset.deltaci\endcsname{[-0.183, -0.142]}
\expandafter\def\csname res@phi4mm_cc.subset.deltaoff\endcsname{-0.164}
\expandafter\def\csname res@phi4mm_cc.subset.deltaoffci\endcsname{[-0.188, -0.140]}
\expandafter\def\csname res@phi4mm_cc.subset.ece\endcsname{0.219}
\expandafter\def\csname res@phi4mm_cc.subset.ecev\endcsname{0.276}
\expandafter\def\csname res@phi4mm_cc.subset.ecevoracle\endcsname{0.105}
\expandafter\def\csname res@phi4mm_cc.subset.f1\endcsname{0.222}
\expandafter\def\csname res@phi4mm_cc.subset.f1ci\endcsname{[0.202, 0.242]}
\expandafter\def\csname res@phi4mm_cc.subset.f1off\endcsname{0.231}
\expandafter\def\csname res@phi4mm_cc.subset.f1offci\endcsname{[0.206, 0.259]}
\expandafter\def\csname res@phi4mm_cc.subset.gap\endcsname{0.161}
\expandafter\def\csname res@phi4mm_cc.subset.gapci\endcsname{[0.142, 0.183]}
\expandafter\def\csname res@phi4mm_cc.subset.ll\endcsname{2.917}
\expandafter\def\csname res@phi4mm_cc.subset.lloracle\endcsname{2.057}
\expandafter\def\csname res@phi4mm_cc.subset.toracle\endcsname{7.79}
\expandafter\def\csname res@prior.full.ecev\endcsname{0.058}
\expandafter\def\csname res@prior.full.ll\endcsname{1.869}
\expandafter\def\csname res@prior.subset.ecev\endcsname{0.058}
\expandafter\def\csname res@prior.subset.ll\endcsname{1.863}
\expandafter\def\csname res@qwen2audio7b.subset.delta\endcsname{-0.100}
\expandafter\def\csname res@qwen2audio7b.subset.deltaci\endcsname{[-0.123, -0.081]}
\expandafter\def\csname res@qwen2audio7b.subset.deltaoff\endcsname{-0.089}
\expandafter\def\csname res@qwen2audio7b.subset.deltaoffci\endcsname{[-0.117, -0.067]}
\expandafter\def\csname res@qwen2audio7b.subset.ece\endcsname{0.119}
\expandafter\def\csname res@qwen2audio7b.subset.ecev\endcsname{0.187}
\expandafter\def\csname res@qwen2audio7b.subset.ecevoracle\endcsname{0.054}
\expandafter\def\csname res@qwen2audio7b.subset.f1\endcsname{0.283}
\expandafter\def\csname res@qwen2audio7b.subset.f1ci\endcsname{[0.259, 0.307]}
\expandafter\def\csname res@qwen2audio7b.subset.f1off\endcsname{0.305}
\expandafter\def\csname res@qwen2audio7b.subset.f1offci\endcsname{[0.275, 0.333]}
\expandafter\def\csname res@qwen2audio7b.subset.gap\endcsname{0.100}
\expandafter\def\csname res@qwen2audio7b.subset.gapci\endcsname{[0.081, 0.123]}
\expandafter\def\csname res@qwen2audio7b.subset.ll\endcsname{2.097}
\expandafter\def\csname res@qwen2audio7b.subset.lloracle\endcsname{1.853}
\expandafter\def\csname res@qwen2audio7b.subset.toracle\endcsname{2.22}
\expandafter\def\csname res@qwen2audio7b_cc.subset.delta\endcsname{-0.092}
\expandafter\def\csname res@qwen2audio7b_cc.subset.deltaci\endcsname{[-0.114, -0.072]}
\expandafter\def\csname res@qwen2audio7b_cc.subset.deltaoff\endcsname{-0.084}
\expandafter\def\csname res@qwen2audio7b_cc.subset.deltaoffci\endcsname{[-0.110, -0.059]}
\expandafter\def\csname res@qwen2audio7b_cc.subset.ece\endcsname{0.110}
\expandafter\def\csname res@qwen2audio7b_cc.subset.ecev\endcsname{0.185}
\expandafter\def\csname res@qwen2audio7b_cc.subset.ecevoracle\endcsname{0.039}
\expandafter\def\csname res@qwen2audio7b_cc.subset.f1\endcsname{0.291}
\expandafter\def\csname res@qwen2audio7b_cc.subset.f1ci\endcsname{[0.269, 0.316]}
\expandafter\def\csname res@qwen2audio7b_cc.subset.f1off\endcsname{0.310}
\expandafter\def\csname res@qwen2audio7b_cc.subset.f1offci\endcsname{[0.280, 0.345]}
\expandafter\def\csname res@qwen2audio7b_cc.subset.gap\endcsname{0.092}
\expandafter\def\csname res@qwen2audio7b_cc.subset.gapci\endcsname{[0.072, 0.114]}
\expandafter\def\csname res@qwen2audio7b_cc.subset.ll\endcsname{2.069}
\expandafter\def\csname res@qwen2audio7b_cc.subset.lloracle\endcsname{1.865}
\expandafter\def\csname res@qwen2audio7b_cc.subset.toracle\endcsname{2.11}
\expandafter\def\csname res@uniform.ll8\endcsname{2.079}
\expandafter\def\csname res@voxtral3b.subset.delta\endcsname{-0.181}
\expandafter\def\csname res@voxtral3b.subset.deltaci\endcsname{[-0.216, -0.150]}
\expandafter\def\csname res@voxtral3b.subset.deltaoff\endcsname{-0.152}
\expandafter\def\csname res@voxtral3b.subset.deltaoffci\endcsname{[-0.189, -0.119]}
\expandafter\def\csname res@voxtral3b.subset.ece\endcsname{0.452}
\expandafter\def\csname res@voxtral3b.subset.ecev\endcsname{0.448}
\expandafter\def\csname res@voxtral3b.subset.ecevoracle\endcsname{0.038}
\expandafter\def\csname res@voxtral3b.subset.f1\endcsname{0.202}
\expandafter\def\csname res@voxtral3b.subset.f1ci\endcsname{[0.182, 0.219]}
\expandafter\def\csname res@voxtral3b.subset.f1off\endcsname{0.243}
\expandafter\def\csname res@voxtral3b.subset.f1offci\endcsname{[0.220, 0.267]}
\expandafter\def\csname res@voxtral3b.subset.gap\endcsname{0.181}
\expandafter\def\csname res@voxtral3b.subset.gapci\endcsname{[0.150, 0.216]}
\expandafter\def\csname res@voxtral3b.subset.ll\endcsname{2.864}
\expandafter\def\csname res@voxtral3b.subset.lloracle\endcsname{1.885}
\expandafter\def\csname res@voxtral3b.subset.toracle\endcsname{3.56}
\expandafter\def\csname res@voxtral3b_cc.subset.delta\endcsname{-0.172}
\expandafter\def\csname res@voxtral3b_cc.subset.deltaci\endcsname{[-0.207, -0.140]}
\expandafter\def\csname res@voxtral3b_cc.subset.deltaoff\endcsname{-0.149}
\expandafter\def\csname res@voxtral3b_cc.subset.deltaoffci\endcsname{[-0.185, -0.113]}
\expandafter\def\csname res@voxtral3b_cc.subset.ece\endcsname{0.310}
\expandafter\def\csname res@voxtral3b_cc.subset.ecev\endcsname{0.302}
\expandafter\def\csname res@voxtral3b_cc.subset.ecevoracle\endcsname{0.099}
\expandafter\def\csname res@voxtral3b_cc.subset.f1\endcsname{0.211}
\expandafter\def\csname res@voxtral3b_cc.subset.f1ci\endcsname{[0.190, 0.227]}
\expandafter\def\csname res@voxtral3b_cc.subset.f1off\endcsname{0.245}
\expandafter\def\csname res@voxtral3b_cc.subset.f1offci\endcsname{[0.223, 0.269]}
\expandafter\def\csname res@voxtral3b_cc.subset.gap\endcsname{0.172}
\expandafter\def\csname res@voxtral3b_cc.subset.gapci\endcsname{[0.140, 0.207]}
\expandafter\def\csname res@voxtral3b_cc.subset.ll\endcsname{2.539}
\expandafter\def\csname res@voxtral3b_cc.subset.lloracle\endcsname{1.982}
\expandafter\def\csname res@voxtral3b_cc.subset.toracle\endcsname{3.65}
\expandafter\def\csname res@wavlm_ft.full.delta\endcsname{-0.049}
\expandafter\def\csname res@wavlm_ft.full.deltaci\endcsname{[-0.056, -0.041]}
\expandafter\def\csname res@wavlm_ft.full.deltaoff\endcsname{-0.039}
\expandafter\def\csname res@wavlm_ft.full.deltaoffci\endcsname{[-0.046, -0.028]}
\expandafter\def\csname res@wavlm_ft.full.ece\endcsname{0.051}
\expandafter\def\csname res@wavlm_ft.full.ecev\endcsname{0.036}
\expandafter\def\csname res@wavlm_ft.full.ecevoracle\endcsname{0.011}
\expandafter\def\csname res@wavlm_ft.full.f1\endcsname{0.333}
\expandafter\def\csname res@wavlm_ft.full.f1ci\endcsname{[0.307, 0.358]}
\expandafter\def\csname res@wavlm_ft.full.f1off\endcsname{0.362}
\expandafter\def\csname res@wavlm_ft.full.f1offci\endcsname{[0.328, 0.395]}
\expandafter\def\csname res@wavlm_ft.full.gap\endcsname{0.049}
\expandafter\def\csname res@wavlm_ft.full.gapci\endcsname{[0.041, 0.056]}
\expandafter\def\csname res@wavlm_ft.full.ll\endcsname{1.527}
\expandafter\def\csname res@wavlm_ft.full.lloracle\endcsname{1.520}
\expandafter\def\csname res@wavlm_ft.full.toracle\endcsname{1.14}
\expandafter\def\csname res@wavlm_ft.subset.delta\endcsname{-0.050}
\expandafter\def\csname res@wavlm_ft.subset.deltaci\endcsname{[-0.067, -0.029]}
\expandafter\def\csname res@wavlm_ft.subset.deltaoff\endcsname{-0.032}
\expandafter\def\csname res@wavlm_ft.subset.deltaoffci\endcsname{[-0.053, -0.005]}
\expandafter\def\csname res@wavlm_ft.subset.ece\endcsname{0.062}
\expandafter\def\csname res@wavlm_ft.subset.ecev\endcsname{0.035}
\expandafter\def\csname res@wavlm_ft.subset.ecevoracle\endcsname{0.019}
\expandafter\def\csname res@wavlm_ft.subset.f1\endcsname{0.333}
\expandafter\def\csname res@wavlm_ft.subset.f1ci\endcsname{[0.302, 0.364]}
\expandafter\def\csname res@wavlm_ft.subset.f1off\endcsname{0.362}
\expandafter\def\csname res@wavlm_ft.subset.f1offci\endcsname{[0.324, 0.403]}
\expandafter\def\csname res@wavlm_ft.subset.gap\endcsname{0.050}
\expandafter\def\csname res@wavlm_ft.subset.gapci\endcsname{[0.029, 0.067]}
\expandafter\def\csname res@wavlm_ft.subset.ll\endcsname{1.528}
\expandafter\def\csname res@wavlm_ft.subset.lloracle\endcsname{1.521}
\expandafter\def\csname res@wavlm_ft.subset.toracle\endcsname{1.14}
\expandafter\def\csname res@whisper_mlp.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@whisper_mlp.full.ccc.dominance\endcsname{0.50}
\expandafter\def\csname res@whisper_mlp.full.ccc.valence\endcsname{0.70}
\expandafter\def\csname res@whisper_mlp.full.delta\endcsname{-0.003}
\expandafter\def\csname res@whisper_mlp.full.deltaci\endcsname{[-0.005, +0.002]}
\expandafter\def\csname res@whisper_mlp.full.deltaoff\endcsname{-0.002}
\expandafter\def\csname res@whisper_mlp.full.deltaoffci\endcsname{[-0.005, +0.002]}
\expandafter\def\csname res@whisper_mlp.full.ece\endcsname{0.061}
\expandafter\def\csname res@whisper_mlp.full.ecev\endcsname{0.037}
\expandafter\def\csname res@whisper_mlp.full.ecevoracle\endcsname{0.004}
\expandafter\def\csname res@whisper_mlp.full.f1\endcsname{0.379}
\expandafter\def\csname res@whisper_mlp.full.f1ci\endcsname{[0.353, 0.403]}
\expandafter\def\csname res@whisper_mlp.full.f1off\endcsname{0.399}
\expandafter\def\csname res@whisper_mlp.full.f1offci\endcsname{[0.367, 0.429]}
\expandafter\def\csname res@whisper_mlp.full.gap\endcsname{0.003}
\expandafter\def\csname res@whisper_mlp.full.gapci\endcsname{[-0.002, 0.005]}
\expandafter\def\csname res@whisper_mlp.full.ll\endcsname{1.502}
\expandafter\def\csname res@whisper_mlp.full.lloracle\endcsname{1.497}
\expandafter\def\csname res@whisper_mlp.full.toracle\endcsname{1.11}
\expandafter\def\csname res@whisper_mlp.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@whisper_mlp.subset.ccc.dominance\endcsname{0.52}
\expandafter\def\csname res@whisper_mlp.subset.ccc.valence\endcsname{0.71}
\expandafter\def\csname res@whisper_mlp.subset.delta\endcsname{-0.004}
\expandafter\def\csname res@whisper_mlp.subset.deltaci\endcsname{[-0.017, +0.006]}
\expandafter\def\csname res@whisper_mlp.subset.deltaoff\endcsname{-0.005}
\expandafter\def\csname res@whisper_mlp.subset.deltaoffci\endcsname{[-0.019, +0.006]}
\expandafter\def\csname res@whisper_mlp.subset.ece\endcsname{0.065}
\expandafter\def\csname res@whisper_mlp.subset.ecev\endcsname{0.034}
\expandafter\def\csname res@whisper_mlp.subset.ecevoracle\endcsname{0.010}
\expandafter\def\csname res@whisper_mlp.subset.f1\endcsname{0.379}
\expandafter\def\csname res@whisper_mlp.subset.f1ci\endcsname{[0.352, 0.403]}
\expandafter\def\csname res@whisper_mlp.subset.f1off\endcsname{0.389}
\expandafter\def\csname res@whisper_mlp.subset.f1offci\endcsname{[0.358, 0.419]}
\expandafter\def\csname res@whisper_mlp.subset.gap\endcsname{0.004}
\expandafter\def\csname res@whisper_mlp.subset.gapci\endcsname{[-0.006, 0.017]}
\expandafter\def\csname res@whisper_mlp.subset.ll\endcsname{1.504}
\expandafter\def\csname res@whisper_mlp.subset.lloracle\endcsname{1.499}
\expandafter\def\csname res@whisper_mlp.subset.toracle\endcsname{1.11}
\expandafter\def\csname res@whisper_mlp_msp.full.ccc.arousal\endcsname{0.63}
\expandafter\def\csname res@whisper_mlp_msp.full.ccc.dominance\endcsname{0.50}
\expandafter\def\csname res@whisper_mlp_msp.full.ccc.valence\endcsname{0.68}
\expandafter\def\csname res@whisper_mlp_msp.full.delta\endcsname{-0.021}
\expandafter\def\csname res@whisper_mlp_msp.full.deltaci\endcsname{[-0.028, -0.013]}
\expandafter\def\csname res@whisper_mlp_msp.full.deltaoff\endcsname{-0.022}
\expandafter\def\csname res@whisper_mlp_msp.full.deltaoffci\endcsname{[-0.029, -0.014]}
\expandafter\def\csname res@whisper_mlp_msp.full.ece\endcsname{0.072}
\expandafter\def\csname res@whisper_mlp_msp.full.ecev\endcsname{0.019}
\expandafter\def\csname res@whisper_mlp_msp.full.ecevoracle\endcsname{0.006}
\expandafter\def\csname res@whisper_mlp_msp.full.f1\endcsname{0.361}
\expandafter\def\csname res@whisper_mlp_msp.full.f1ci\endcsname{[0.332, 0.387]}
\expandafter\def\csname res@whisper_mlp_msp.full.f1off\endcsname{0.379}
\expandafter\def\csname res@whisper_mlp_msp.full.f1offci\endcsname{[0.345, 0.411]}
\expandafter\def\csname res@whisper_mlp_msp.full.gap\endcsname{0.021}
\expandafter\def\csname res@whisper_mlp_msp.full.gapci\endcsname{[0.013, 0.028]}
\expandafter\def\csname res@whisper_mlp_msp.full.ll\endcsname{1.508}
\expandafter\def\csname res@whisper_mlp_msp.full.lloracle\endcsname{1.507}
\expandafter\def\csname res@whisper_mlp_msp.full.toracle\endcsname{1.07}
\expandafter\def\csname res@whisper_mlp_msp.subset.ccc.arousal\endcsname{0.64}
\expandafter\def\csname res@whisper_mlp_msp.subset.ccc.dominance\endcsname{0.51}
\expandafter\def\csname res@whisper_mlp_msp.subset.ccc.valence\endcsname{0.69}
\expandafter\def\csname res@whisper_mlp_msp.subset.delta\endcsname{-0.037}
\expandafter\def\csname res@whisper_mlp_msp.subset.deltaci\endcsname{[-0.051, -0.022]}
\expandafter\def\csname res@whisper_mlp_msp.subset.deltaoff\endcsname{-0.039}
\expandafter\def\csname res@whisper_mlp_msp.subset.deltaoffci\endcsname{[-0.055, -0.020]}
\expandafter\def\csname res@whisper_mlp_msp.subset.ece\endcsname{0.074}
\expandafter\def\csname res@whisper_mlp_msp.subset.ecev\endcsname{0.021}
\expandafter\def\csname res@whisper_mlp_msp.subset.ecevoracle\endcsname{0.015}
\expandafter\def\csname res@whisper_mlp_msp.subset.f1\endcsname{0.347}
\expandafter\def\csname res@whisper_mlp_msp.subset.f1ci\endcsname{[0.317, 0.372]}
\expandafter\def\csname res@whisper_mlp_msp.subset.f1off\endcsname{0.355}
\expandafter\def\csname res@whisper_mlp_msp.subset.f1offci\endcsname{[0.318, 0.388]}
\expandafter\def\csname res@whisper_mlp_msp.subset.gap\endcsname{0.037}
\expandafter\def\csname res@whisper_mlp_msp.subset.gapci\endcsname{[0.022, 0.051]}
\expandafter\def\csname res@whisper_mlp_msp.subset.ll\endcsname{1.507}
\expandafter\def\csname res@whisper_mlp_msp.subset.lloracle\endcsname{1.505}
\expandafter\def\csname res@whisper_mlp_msp.subset.toracle\endcsname{1.06}
\expandafter\def\csname res@zs.abl_base8_s43.calm\endcsname{0.164}
\expandafter\def\csname res@zs.abl_base8_s43.f1\endcsname{0.431}
\expandafter\def\csname res@zs.abl_base8_s43.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.abl_base8_s43.knownauc\endcsname{0.843}
\expandafter\def\csname res@zs.abl_base8_s43.novel\endcsname{0.033}
\expandafter\def\csname res@zs.abl_base8_s43.novelauc\endcsname{0.732}
\expandafter\def\csname res@zs.abl_base8_s44.calm\endcsname{0.201}
\expandafter\def\csname res@zs.abl_base8_s44.f1\endcsname{0.419}
\expandafter\def\csname res@zs.abl_base8_s44.f1pm\endcsname{0.549}
\expandafter\def\csname res@zs.abl_base8_s44.knownauc\endcsname{0.841}
\expandafter\def\csname res@zs.abl_base8_s44.novel\endcsname{0.040}
\expandafter\def\csname res@zs.abl_base8_s44.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.abl_base8_s45.calm\endcsname{0.037}
\expandafter\def\csname res@zs.abl_base8_s45.f1\endcsname{0.425}
\expandafter\def\csname res@zs.abl_base8_s45.f1pm\endcsname{0.550}
\expandafter\def\csname res@zs.abl_base8_s45.knownauc\endcsname{0.844}
\expandafter\def\csname res@zs.abl_base8_s45.novel\endcsname{0.011}
\expandafter\def\csname res@zs.abl_base8_s45.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.abl_last_s43.calm\endcsname{0.000}
\expandafter\def\csname res@zs.abl_last_s43.f1\endcsname{0.359}
\expandafter\def\csname res@zs.abl_last_s43.f1pm\endcsname{0.501}
\expandafter\def\csname res@zs.abl_last_s43.knownauc\endcsname{0.813}
\expandafter\def\csname res@zs.abl_last_s43.novel\endcsname{0.003}
\expandafter\def\csname res@zs.abl_last_s43.novelauc\endcsname{0.656}
\expandafter\def\csname res@zs.abl_last_s44.calm\endcsname{0.000}
\expandafter\def\csname res@zs.abl_last_s44.f1\endcsname{0.355}
\expandafter\def\csname res@zs.abl_last_s44.f1pm\endcsname{0.500}
\expandafter\def\csname res@zs.abl_last_s44.knownauc\endcsname{0.812}
\expandafter\def\csname res@zs.abl_last_s44.novel\endcsname{0.000}
\expandafter\def\csname res@zs.abl_last_s44.novelauc\endcsname{0.657}
\expandafter\def\csname res@zs.abl_mean_s43.calm\endcsname{0.427}
\expandafter\def\csname res@zs.abl_mean_s43.f1\endcsname{0.357}
\expandafter\def\csname res@zs.abl_mean_s43.f1pm\endcsname{0.506}
\expandafter\def\csname res@zs.abl_mean_s43.knownauc\endcsname{0.814}
\expandafter\def\csname res@zs.abl_mean_s43.novel\endcsname{0.096}
\expandafter\def\csname res@zs.abl_mean_s43.novelauc\endcsname{0.748}
\expandafter\def\csname res@zs.abl_mean_s44.calm\endcsname{0.434}
\expandafter\def\csname res@zs.abl_mean_s44.f1\endcsname{0.352}
\expandafter\def\csname res@zs.abl_mean_s44.f1pm\endcsname{0.507}
\expandafter\def\csname res@zs.abl_mean_s44.knownauc\endcsname{0.813}
\expandafter\def\csname res@zs.abl_mean_s44.novel\endcsname{0.096}
\expandafter\def\csname res@zs.abl_mean_s44.novelauc\endcsname{0.745}
\expandafter\def\csname res@zs.abl_nodistill.calm\endcsname{0.212}
\expandafter\def\csname res@zs.abl_nodistill.f1\endcsname{0.452}
\expandafter\def\csname res@zs.abl_nodistill.f1pm\endcsname{0.558}
\expandafter\def\csname res@zs.abl_nodistill.knownauc\endcsname{0.846}
\expandafter\def\csname res@zs.abl_nodistill.novel\endcsname{0.052}
\expandafter\def\csname res@zs.abl_nodistill.novelauc\endcsname{0.718}
\expandafter\def\csname res@zs.abl_nodiv.calm\endcsname{0.583}
\expandafter\def\csname res@zs.abl_nodiv.f1\endcsname{0.445}
\expandafter\def\csname res@zs.abl_nodiv.f1pm\endcsname{0.565}
\expandafter\def\csname res@zs.abl_nodiv.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.abl_nodiv.novel\endcsname{0.120}
\expandafter\def\csname res@zs.abl_nodiv.novelauc\endcsname{0.755}
\expandafter\def\csname res@zs.abl_noseg.calm\endcsname{0.343}
\expandafter\def\csname res@zs.abl_noseg.f1\endcsname{0.443}
\expandafter\def\csname res@zs.abl_noseg.f1pm\endcsname{0.565}
\expandafter\def\csname res@zs.abl_noseg.knownauc\endcsname{0.851}
\expandafter\def\csname res@zs.abl_noseg.novel\endcsname{0.069}
\expandafter\def\csname res@zs.abl_noseg.novelauc\endcsname{0.745}
\expandafter\def\csname res@zs.abl_seg64.calm\endcsname{0.105}
\expandafter\def\csname res@zs.abl_seg64.f1\endcsname{0.446}
\expandafter\def\csname res@zs.abl_seg64.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.abl_seg64.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.abl_seg64.novel\endcsname{0.021}
\expandafter\def\csname res@zs.abl_seg64.novelauc\endcsname{0.734}
\expandafter\def\csname res@zs.abl_v1_s43.calm\endcsname{0.196}
\expandafter\def\csname res@zs.abl_v1_s43.f1\endcsname{0.424}
\expandafter\def\csname res@zs.abl_v1_s43.f1pm\endcsname{0.550}
\expandafter\def\csname res@zs.abl_v1_s43.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.abl_v1_s43.novel\endcsname{0.039}
\expandafter\def\csname res@zs.abl_v1_s43.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.abl_v1_s44.calm\endcsname{0.082}
\expandafter\def\csname res@zs.abl_v1_s44.f1\endcsname{0.427}
\expandafter\def\csname res@zs.abl_v1_s44.f1pm\endcsname{0.550}
\expandafter\def\csname res@zs.abl_v1_s44.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.abl_v1_s44.novel\endcsname{0.016}
\expandafter\def\csname res@zs.abl_v1_s44.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.abl_w32only_s43.calm\endcsname{0.156}
\expandafter\def\csname res@zs.abl_w32only_s43.f1\endcsname{0.429}
\expandafter\def\csname res@zs.abl_w32only_s43.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.abl_w32only_s43.knownauc\endcsname{0.844}
\expandafter\def\csname res@zs.abl_w32only_s43.novel\endcsname{0.038}
\expandafter\def\csname res@zs.abl_w32only_s43.novelauc\endcsname{0.716}
\expandafter\def\csname res@zs.abl_w32only_s44.calm\endcsname{0.035}
\expandafter\def\csname res@zs.abl_w32only_s44.f1\endcsname{0.433}
\expandafter\def\csname res@zs.abl_w32only_s44.f1pm\endcsname{0.552}
\expandafter\def\csname res@zs.abl_w32only_s44.knownauc\endcsname{0.844}
\expandafter\def\csname res@zs.abl_w32only_s44.novel\endcsname{0.014}
\expandafter\def\csname res@zs.abl_w32only_s44.novelauc\endcsname{0.715}
\expandafter\def\csname res@zs.af3.asomclean\endcsname{0.456}
\expandafter\def\csname res@zs.af3.calm\endcsname{0.432}
\expandafter\def\csname res@zs.af3.cleancorpora\endcsname{18}
\expandafter\def\csname res@zs.af3.f1\endcsname{0.222}
\expandafter\def\csname res@zs.af3.f1ci\endcsname{[0.212, 0.230]}
\expandafter\def\csname res@zs.af3.f1clean\endcsname{0.220}
\expandafter\def\csname res@zs.af3.f1ctrl\endcsname{0.224}
\expandafter\def\csname res@zs.af3.f1ctrlci\endcsname{[0.213, 0.234]}
\expandafter\def\csname res@zs.af3.f1emobox\endcsname{0.234}
\expandafter\def\csname res@zs.af3.f1emoboxci\endcsname{[0.222, 0.244]}
\expandafter\def\csname res@zs.af3.f1en\endcsname{0.287}
\expandafter\def\csname res@zs.af3.f1enci\endcsname{[0.268, 0.306]}
\expandafter\def\csname res@zs.af3.f1lex\endcsname{0.212}
\expandafter\def\csname res@zs.af3.f1lexci\endcsname{[0.198, 0.226]}
\expandafter\def\csname res@zs.af3.f1nonen\endcsname{0.189}
\expandafter\def\csname res@zs.af3.f1nonenci\endcsname{[0.178, 0.198]}
\expandafter\def\csname res@zs.af3.f1other\endcsname{0.170}
\expandafter\def\csname res@zs.af3.f1otherci\endcsname{[0.159, 0.180]}
\expandafter\def\csname res@zs.af3.f1pm\endcsname{0.308}
\expandafter\def\csname res@zs.af3.f1pmctrl\endcsname{0.325}
\expandafter\def\csname res@zs.af3.f1pmen\endcsname{0.343}
\expandafter\def\csname res@zs.af3.f1pmlex\endcsname{0.233}
\expandafter\def\csname res@zs.af3.f1pmnonen\endcsname{0.290}
\expandafter\def\csname res@zs.af3.gap\endcsname{+0.211}
\expandafter\def\csname res@zs.af3.gapci\endcsname{[+0.196, +0.221]}
\expandafter\def\csname res@zs.af3.gapctrl\endcsname{+0.195}
\expandafter\def\csname res@zs.af3.gapctrlci\endcsname{[+0.178, +0.206]}
\expandafter\def\csname res@zs.af3.gapen\endcsname{+0.051}
\expandafter\def\csname res@zs.af3.gapenci\endcsname{[+0.027, +0.071]}
\expandafter\def\csname res@zs.af3.gaplex\endcsname{+0.281}
\expandafter\def\csname res@zs.af3.gaplexci\endcsname{[+0.254, +0.306]}
\expandafter\def\csname res@zs.af3.gapnonen\endcsname{+0.291}
\expandafter\def\csname res@zs.af3.gapnonenci\endcsname{[+0.273, +0.304]}
\expandafter\def\csname res@zs.af3.knownauc\endcsname{0.627}
\expandafter\def\csname res@zs.af3.novel\endcsname{0.325}
\expandafter\def\csname res@zs.af3.novelauc\endcsname{0.793}
\expandafter\def\csname res@zs.af3_cc.asomclean\endcsname{0.456}
\expandafter\def\csname res@zs.af3_cc.calm\endcsname{0.428}
\expandafter\def\csname res@zs.af3_cc.cleancorpora\endcsname{18}
\expandafter\def\csname res@zs.af3_cc.f1\endcsname{0.268}
\expandafter\def\csname res@zs.af3_cc.f1ci\endcsname{[0.259, 0.276]}
\expandafter\def\csname res@zs.af3_cc.f1clean\endcsname{0.272}
\expandafter\def\csname res@zs.af3_cc.f1ctrl\endcsname{0.276}
\expandafter\def\csname res@zs.af3_cc.f1ctrlci\endcsname{[0.265, 0.285]}
\expandafter\def\csname res@zs.af3_cc.f1emobox\endcsname{0.282}
\expandafter\def\csname res@zs.af3_cc.f1emoboxci\endcsname{[0.271, 0.290]}
\expandafter\def\csname res@zs.af3_cc.f1en\endcsname{0.327}
\expandafter\def\csname res@zs.af3_cc.f1enci\endcsname{[0.312, 0.341]}
\expandafter\def\csname res@zs.af3_cc.f1lex\endcsname{0.234}
\expandafter\def\csname res@zs.af3_cc.f1lexci\endcsname{[0.218, 0.248]}
\expandafter\def\csname res@zs.af3_cc.f1nonen\endcsname{0.239}
\expandafter\def\csname res@zs.af3_cc.f1nonenci\endcsname{[0.227, 0.248]}
\expandafter\def\csname res@zs.af3_cc.f1other\endcsname{0.211}
\expandafter\def\csname res@zs.af3_cc.f1otherci\endcsname{[0.200, 0.222]}
\expandafter\def\csname res@zs.af3_cc.f1pm\endcsname{0.311}
\expandafter\def\csname res@zs.af3_cc.f1pmctrl\endcsname{0.330}
\expandafter\def\csname res@zs.af3_cc.f1pmen\endcsname{0.344}
\expandafter\def\csname res@zs.af3_cc.f1pmlex\endcsname{0.233}
\expandafter\def\csname res@zs.af3_cc.f1pmnonen\endcsname{0.295}
\expandafter\def\csname res@zs.af3_cc.gap\endcsname{+0.165}
\expandafter\def\csname res@zs.af3_cc.gapci\endcsname{[+0.150, +0.175]}
\expandafter\def\csname res@zs.af3_cc.gapctrl\endcsname{+0.143}
\expandafter\def\csname res@zs.af3_cc.gapctrlci\endcsname{[+0.126, +0.154]}
\expandafter\def\csname res@zs.af3_cc.gapen\endcsname{+0.011}
\expandafter\def\csname res@zs.af3_cc.gapenci\endcsname{[-0.011, +0.029]}
\expandafter\def\csname res@zs.af3_cc.gaplex\endcsname{+0.260}
\expandafter\def\csname res@zs.af3_cc.gaplexci\endcsname{[+0.233, +0.285]}
\expandafter\def\csname res@zs.af3_cc.gapnonen\endcsname{+0.242}
\expandafter\def\csname res@zs.af3_cc.gapnonenci\endcsname{[+0.224, +0.255]}
\expandafter\def\csname res@zs.af3_cc.knownauc\endcsname{0.627}
\expandafter\def\csname res@zs.af3_cc.novel\endcsname{0.323}
\expandafter\def\csname res@zs.af3_cc.novelauc\endcsname{0.799}
\expandafter\def\csname res@zs.alms.novel.below\endcsname{0}
\expandafter\def\csname res@zs.alms.novel.n\endcsname{6}
\expandafter\def\csname res@zs.alms.novelauc.below\endcsname{5}
\expandafter\def\csname res@zs.alms.novelauc.n\endcsname{6}
\expandafter\def\csname res@zs.asom.calm\endcsname{0.092}
\expandafter\def\csname res@zs.asom.f1\endcsname{0.433}
\expandafter\def\csname res@zs.asom.f1ci\endcsname{[0.415, 0.443]}
\expandafter\def\csname res@zs.asom.f1ctrl\endcsname{0.419}
\expandafter\def\csname res@zs.asom.f1ctrlci\endcsname{[0.398, 0.430]}
\expandafter\def\csname res@zs.asom.f1emobox\endcsname{0.426}
\expandafter\def\csname res@zs.asom.f1emoboxci\endcsname{[0.405, 0.436]}
\expandafter\def\csname res@zs.asom.f1en\endcsname{0.338}
\expandafter\def\csname res@zs.asom.f1enci\endcsname{[0.319, 0.353]}
\expandafter\def\csname res@zs.asom.f1lex\endcsname{0.494}
\expandafter\def\csname res@zs.asom.f1lexci\endcsname{[0.473, 0.511]}
\expandafter\def\csname res@zs.asom.f1nonen\endcsname{0.481}
\expandafter\def\csname res@zs.asom.f1nonenci\endcsname{[0.457, 0.494]}
\expandafter\def\csname res@zs.asom.f1other\endcsname{0.466}
\expandafter\def\csname res@zs.asom.f1otherci\endcsname{[0.442, 0.486]}
\expandafter\def\csname res@zs.asom.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.asom.f1pmctrl\endcsname{0.556}
\expandafter\def\csname res@zs.asom.f1pmen\endcsname{0.462}
\expandafter\def\csname res@zs.asom.f1pmlex\endcsname{0.537}
\expandafter\def\csname res@zs.asom.f1pmnonen\endcsname{0.598}
\expandafter\def\csname res@zs.asom.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.asom.novel\endcsname{0.018}
\expandafter\def\csname res@zs.asom.novelauc\endcsname{0.721}
\expandafter\def\csname res@zs.asom.winsalm\endcsname{12}
\expandafter\def\csname res@zs.asom.winsctrl\endcsname{16}
\expandafter\def\csname res@zs.asom_30s.calm\endcsname{0.111}
\expandafter\def\csname res@zs.asom_30s.f1\endcsname{0.442}
\expandafter\def\csname res@zs.asom_30s.f1ci\endcsname{[0.423, 0.451]}
\expandafter\def\csname res@zs.asom_30s.f1ctrl\endcsname{0.428}
\expandafter\def\csname res@zs.asom_30s.f1ctrlci\endcsname{[0.406, 0.440]}
\expandafter\def\csname res@zs.asom_30s.f1emobox\endcsname{0.437}
\expandafter\def\csname res@zs.asom_30s.f1emoboxci\endcsname{[0.414, 0.448]}
\expandafter\def\csname res@zs.asom_30s.f1en\endcsname{0.338}
\expandafter\def\csname res@zs.asom_30s.f1enci\endcsname{[0.315, 0.354]}
\expandafter\def\csname res@zs.asom_30s.f1lex\endcsname{0.500}
\expandafter\def\csname res@zs.asom_30s.f1lexci\endcsname{[0.480, 0.515]}
\expandafter\def\csname res@zs.asom_30s.f1nonen\endcsname{0.494}
\expandafter\def\csname res@zs.asom_30s.f1nonenci\endcsname{[0.469, 0.506]}
\expandafter\def\csname res@zs.asom_30s.f1other\endcsname{0.464}
\expandafter\def\csname res@zs.asom_30s.f1otherci\endcsname{[0.442, 0.484]}
\expandafter\def\csname res@zs.asom_30s.f1pm\endcsname{0.562}
\expandafter\def\csname res@zs.asom_30s.f1pmctrl\endcsname{0.565}
\expandafter\def\csname res@zs.asom_30s.f1pmen\endcsname{0.464}
\expandafter\def\csname res@zs.asom_30s.f1pmlex\endcsname{0.545}
\expandafter\def\csname res@zs.asom_30s.f1pmnonen\endcsname{0.610}
\expandafter\def\csname res@zs.asom_30s.gap\endcsname{-0.009}
\expandafter\def\csname res@zs.asom_30s.gapci\endcsname{[-0.013, -0.003]}
\expandafter\def\csname res@zs.asom_30s.gapctrl\endcsname{-0.009}
\expandafter\def\csname res@zs.asom_30s.gapctrlci\endcsname{[-0.014, -0.003]}
\expandafter\def\csname res@zs.asom_30s.gapen\endcsname{+0.000}
\expandafter\def\csname res@zs.asom_30s.gapenci\endcsname{[-0.006, +0.009]}
\expandafter\def\csname res@zs.asom_30s.gaplex\endcsname{-0.006}
\expandafter\def\csname res@zs.asom_30s.gaplexci\endcsname{[-0.014, +0.002]}
\expandafter\def\csname res@zs.asom_30s.gapnonen\endcsname{-0.013}
\expandafter\def\csname res@zs.asom_30s.gapnonenci\endcsname{[-0.019, -0.007]}
\expandafter\def\csname res@zs.asom_30s.knownauc\endcsname{0.851}
\expandafter\def\csname res@zs.asom_30s.novel\endcsname{0.022}
\expandafter\def\csname res@zs.asom_30s.novelauc\endcsname{0.718}
\expandafter\def\csname res@zs.asom_cc.calm\endcsname{0.129}
\expandafter\def\csname res@zs.asom_cc.f1\endcsname{0.388}
\expandafter\def\csname res@zs.asom_cc.f1ci\endcsname{[0.374, 0.396]}
\expandafter\def\csname res@zs.asom_cc.f1ctrl\endcsname{0.389}
\expandafter\def\csname res@zs.asom_cc.f1ctrlci\endcsname{[0.372, 0.398]}
\expandafter\def\csname res@zs.asom_cc.f1emobox\endcsname{0.380}
\expandafter\def\csname res@zs.asom_cc.f1emoboxci\endcsname{[0.363, 0.390]}
\expandafter\def\csname res@zs.asom_cc.f1en\endcsname{0.338}
\expandafter\def\csname res@zs.asom_cc.f1enci\endcsname{[0.316, 0.352]}
\expandafter\def\csname res@zs.asom_cc.f1lex\endcsname{0.386}
\expandafter\def\csname res@zs.asom_cc.f1lexci\endcsname{[0.369, 0.401]}
\expandafter\def\csname res@zs.asom_cc.f1nonen\endcsname{0.414}
\expandafter\def\csname res@zs.asom_cc.f1nonenci\endcsname{[0.397, 0.425]}
\expandafter\def\csname res@zs.asom_cc.f1other\endcsname{0.424}
\expandafter\def\csname res@zs.asom_cc.f1otherci\endcsname{[0.409, 0.438]}
\expandafter\def\csname res@zs.asom_cc.f1pm\endcsname{0.543}
\expandafter\def\csname res@zs.asom_cc.f1pmctrl\endcsname{0.548}
\expandafter\def\csname res@zs.asom_cc.f1pmen\endcsname{0.459}
\expandafter\def\csname res@zs.asom_cc.f1pmlex\endcsname{0.521}
\expandafter\def\csname res@zs.asom_cc.f1pmnonen\endcsname{0.585}
\expandafter\def\csname res@zs.asom_cc.gap\endcsname{+0.045}
\expandafter\def\csname res@zs.asom_cc.gapci\endcsname{[+0.032, +0.055]}
\expandafter\def\csname res@zs.asom_cc.gapctrl\endcsname{+0.030}
\expandafter\def\csname res@zs.asom_cc.gapctrlci\endcsname{[+0.016, +0.042]}
\expandafter\def\csname res@zs.asom_cc.gapen\endcsname{+0.001}
\expandafter\def\csname res@zs.asom_cc.gapenci\endcsname{[-0.016, +0.017]}
\expandafter\def\csname res@zs.asom_cc.gaplex\endcsname{+0.107}
\expandafter\def\csname res@zs.asom_cc.gaplexci\endcsname{[+0.089, +0.126]}
\expandafter\def\csname res@zs.asom_cc.gapnonen\endcsname{+0.067}
\expandafter\def\csname res@zs.asom_cc.gapnonenci\endcsname{[+0.050, +0.080]}
\expandafter\def\csname res@zs.asom_cc.knownauc\endcsname{0.837}
\expandafter\def\csname res@zs.asom_cc.novel\endcsname{0.099}
\expandafter\def\csname res@zs.asom_cc.novelauc\endcsname{0.770}
\expandafter\def\csname res@zs.asom_clip.calm\endcsname{0.527}
\expandafter\def\csname res@zs.asom_clip.f1\endcsname{0.507}
\expandafter\def\csname res@zs.asom_clip.f1ci\endcsname{[0.487, 0.516]}
\expandafter\def\csname res@zs.asom_clip.f1ctrl\endcsname{0.511}
\expandafter\def\csname res@zs.asom_clip.f1ctrlci\endcsname{[0.487, 0.521]}
\expandafter\def\csname res@zs.asom_clip.f1emobox\endcsname{0.509}
\expandafter\def\csname res@zs.asom_clip.f1emoboxci\endcsname{[0.486, 0.519]}
\expandafter\def\csname res@zs.asom_clip.f1en\endcsname{0.454}
\expandafter\def\csname res@zs.asom_clip.f1enci\endcsname{[0.422, 0.478]}
\expandafter\def\csname res@zs.asom_clip.f1lex\endcsname{0.490}
\expandafter\def\csname res@zs.asom_clip.f1lexci\endcsname{[0.471, 0.505]}
\expandafter\def\csname res@zs.asom_clip.f1nonen\endcsname{0.533}
\expandafter\def\csname res@zs.asom_clip.f1nonenci\endcsname{[0.511, 0.544]}
\expandafter\def\csname res@zs.asom_clip.f1other\endcsname{0.497}
\expandafter\def\csname res@zs.asom_clip.f1otherci\endcsname{[0.477, 0.514]}
\expandafter\def\csname res@zs.asom_clip.f1pm\endcsname{0.566}
\expandafter\def\csname res@zs.asom_clip.f1pmctrl\endcsname{0.576}
\expandafter\def\csname res@zs.asom_clip.f1pmen\endcsname{0.487}
\expandafter\def\csname res@zs.asom_clip.f1pmlex\endcsname{0.524}
\expandafter\def\csname res@zs.asom_clip.f1pmnonen\endcsname{0.606}
\expandafter\def\csname res@zs.asom_clip.gap\endcsname{-0.073}
\expandafter\def\csname res@zs.asom_clip.gapci\endcsname{[-0.081, -0.064]}
\expandafter\def\csname res@zs.asom_clip.gapctrl\endcsname{-0.092}
\expandafter\def\csname res@zs.asom_clip.gapctrlci\endcsname{[-0.100, -0.081]}
\expandafter\def\csname res@zs.asom_clip.gapen\endcsname{-0.116}
\expandafter\def\csname res@zs.asom_clip.gapenci\endcsname{[-0.130, -0.097]}
\expandafter\def\csname res@zs.asom_clip.gaplex\endcsname{+0.004}
\expandafter\def\csname res@zs.asom_clip.gaplexci\endcsname{[-0.013, +0.022]}
\expandafter\def\csname res@zs.asom_clip.gapnonen\endcsname{-0.052}
\expandafter\def\csname res@zs.asom_clip.gapnonenci\endcsname{[-0.061, -0.042]}
\expandafter\def\csname res@zs.asom_clip.knownauc\endcsname{0.853}
\expandafter\def\csname res@zs.asom_clip.novel\endcsname{0.226}
\expandafter\def\csname res@zs.asom_clip.novelauc\endcsname{0.739}
\expandafter\def\csname res@zs.asom_em.calm\endcsname{0.000}
\expandafter\def\csname res@zs.asom_em.f1\endcsname{0.201}
\expandafter\def\csname res@zs.asom_em.f1ci\endcsname{[0.190, 0.207]}
\expandafter\def\csname res@zs.asom_em.f1ctrl\endcsname{0.192}
\expandafter\def\csname res@zs.asom_em.f1ctrlci\endcsname{[0.181, 0.199]}
\expandafter\def\csname res@zs.asom_em.f1emobox\endcsname{0.200}
\expandafter\def\csname res@zs.asom_em.f1emoboxci\endcsname{[0.188, 0.207]}
\expandafter\def\csname res@zs.asom_em.f1en\endcsname{0.135}
\expandafter\def\csname res@zs.asom_em.f1enci\endcsname{[0.124, 0.144]}
\expandafter\def\csname res@zs.asom_em.f1lex\endcsname{0.238}
\expandafter\def\csname res@zs.asom_em.f1lexci\endcsname{[0.220, 0.253]}
\expandafter\def\csname res@zs.asom_em.f1nonen\endcsname{0.234}
\expandafter\def\csname res@zs.asom_em.f1nonenci\endcsname{[0.220, 0.242]}
\expandafter\def\csname res@zs.asom_em.f1other\endcsname{0.204}
\expandafter\def\csname res@zs.asom_em.f1otherci\endcsname{[0.191, 0.216]}
\expandafter\def\csname res@zs.asom_em.f1pm\endcsname{0.394}
\expandafter\def\csname res@zs.asom_em.f1pmctrl\endcsname{0.380}
\expandafter\def\csname res@zs.asom_em.f1pmen\endcsname{0.293}
\expandafter\def\csname res@zs.asom_em.f1pmlex\endcsname{0.457}
\expandafter\def\csname res@zs.asom_em.f1pmnonen\endcsname{0.445}
\expandafter\def\csname res@zs.asom_em.gap\endcsname{+0.232}
\expandafter\def\csname res@zs.asom_em.gapci\endcsname{[+0.220, +0.241]}
\expandafter\def\csname res@zs.asom_em.gapctrl\endcsname{+0.227}
\expandafter\def\csname res@zs.asom_em.gapctrlci\endcsname{[+0.213, +0.236]}
\expandafter\def\csname res@zs.asom_em.gapen\endcsname{+0.204}
\expandafter\def\csname res@zs.asom_em.gapenci\endcsname{[+0.188, +0.216]}
\expandafter\def\csname res@zs.asom_em.gaplex\endcsname{+0.256}
\expandafter\def\csname res@zs.asom_em.gaplexci\endcsname{[+0.240, +0.271]}
\expandafter\def\csname res@zs.asom_em.gapnonen\endcsname{+0.247}
\expandafter\def\csname res@zs.asom_em.gapnonenci\endcsname{[+0.232, +0.257]}
\expandafter\def\csname res@zs.asom_em.knownauc\endcsname{0.856}
\expandafter\def\csname res@zs.asom_em.novel\endcsname{0.000}
\expandafter\def\csname res@zs.asom_s43.calm\endcsname{0.188}
\expandafter\def\csname res@zs.asom_s43.f1\endcsname{0.446}
\expandafter\def\csname res@zs.asom_s43.f1pm\endcsname{0.561}
\expandafter\def\csname res@zs.asom_s43.knownauc\endcsname{0.850}
\expandafter\def\csname res@zs.asom_s43.novel\endcsname{0.038}
\expandafter\def\csname res@zs.asom_s43.novelauc\endcsname{0.740}
\expandafter\def\csname res@zs.asom_s43_noprior.calm\endcsname{0.571}
\expandafter\def\csname res@zs.asom_s43_noprior.f1\endcsname{0.481}
\expandafter\def\csname res@zs.asom_s43_noprior.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_s43_noprior.knownauc\endcsname{0.852}
\expandafter\def\csname res@zs.asom_s43_noprior.novel\endcsname{0.155}
\expandafter\def\csname res@zs.asom_s43_noprior.novelauc\endcsname{0.752}
\expandafter\def\csname res@zs.asom_s44.calm\endcsname{0.116}
\expandafter\def\csname res@zs.asom_s44.f1\endcsname{0.439}
\expandafter\def\csname res@zs.asom_s44.f1pm\endcsname{0.561}
\expandafter\def\csname res@zs.asom_s44.knownauc\endcsname{0.848}
\expandafter\def\csname res@zs.asom_s44.novel\endcsname{0.023}
\expandafter\def\csname res@zs.asom_s44.novelauc\endcsname{0.730}
\expandafter\def\csname res@zs.asom_s44_noprior.calm\endcsname{0.473}
\expandafter\def\csname res@zs.asom_s44_noprior.f1\endcsname{0.476}
\expandafter\def\csname res@zs.asom_s44_noprior.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_s44_noprior.knownauc\endcsname{0.850}
\expandafter\def\csname res@zs.asom_s44_noprior.novel\endcsname{0.124}
\expandafter\def\csname res@zs.asom_s44_noprior.novelauc\endcsname{0.742}
\expandafter\def\csname res@zs.asom_s45.calm\endcsname{0.060}
\expandafter\def\csname res@zs.asom_s45.f1\endcsname{0.447}
\expandafter\def\csname res@zs.asom_s45.f1pm\endcsname{0.564}
\expandafter\def\csname res@zs.asom_s45.knownauc\endcsname{0.851}
\expandafter\def\csname res@zs.asom_s45.novel\endcsname{0.012}
\expandafter\def\csname res@zs.asom_s45.novelauc\endcsname{0.733}
\expandafter\def\csname res@zs.asom_s45_noprior.calm\endcsname{0.406}
\expandafter\def\csname res@zs.asom_s45_noprior.f1\endcsname{0.479}
\expandafter\def\csname res@zs.asom_s45_noprior.f1pm\endcsname{0.567}
\expandafter\def\csname res@zs.asom_s45_noprior.knownauc\endcsname{0.852}
\expandafter\def\csname res@zs.asom_s45_noprior.novel\endcsname{0.107}
\expandafter\def\csname res@zs.asom_s45_noprior.novelauc\endcsname{0.746}
\expandafter\def\csname res@zs.asom_u.calm\endcsname{0.395}
\expandafter\def\csname res@zs.asom_u.f1\endcsname{0.472}
\expandafter\def\csname res@zs.asom_u.f1ci\endcsname{[0.454, 0.482]}
\expandafter\def\csname res@zs.asom_u.f1ctrl\endcsname{0.462}
\expandafter\def\csname res@zs.asom_u.f1ctrlci\endcsname{[0.440, 0.474]}
\expandafter\def\csname res@zs.asom_u.f1emobox\endcsname{0.464}
\expandafter\def\csname res@zs.asom_u.f1emoboxci\endcsname{[0.443, 0.477]}
\expandafter\def\csname res@zs.asom_u.f1en\endcsname{0.387}
\expandafter\def\csname res@zs.asom_u.f1enci\endcsname{[0.360, 0.408]}
\expandafter\def\csname res@zs.asom_u.f1lex\endcsname{0.516}
\expandafter\def\csname res@zs.asom_u.f1lexci\endcsname{[0.497, 0.530]}
\expandafter\def\csname res@zs.asom_u.f1nonen\endcsname{0.515}
\expandafter\def\csname res@zs.asom_u.f1nonenci\endcsname{[0.493, 0.527]}
\expandafter\def\csname res@zs.asom_u.f1other\endcsname{0.504}
\expandafter\def\csname res@zs.asom_u.f1otherci\endcsname{[0.484, 0.522]}
\expandafter\def\csname res@zs.asom_u.f1pm\endcsname{0.554}
\expandafter\def\csname res@zs.asom_u.f1pmctrl\endcsname{0.558}
\expandafter\def\csname res@zs.asom_u.f1pmen\endcsname{0.465}
\expandafter\def\csname res@zs.asom_u.f1pmlex\endcsname{0.538}
\expandafter\def\csname res@zs.asom_u.f1pmnonen\endcsname{0.599}
\expandafter\def\csname res@zs.asom_u.gap\endcsname{-0.039}
\expandafter\def\csname res@zs.asom_u.gapci\endcsname{[-0.045, -0.032]}
\expandafter\def\csname res@zs.asom_u.gapctrl\endcsname{-0.043}
\expandafter\def\csname res@zs.asom_u.gapctrlci\endcsname{[-0.050, -0.036]}
\expandafter\def\csname res@zs.asom_u.gapen\endcsname{-0.049}
\expandafter\def\csname res@zs.asom_u.gapenci\endcsname{[-0.061, -0.035]}
\expandafter\def\csname res@zs.asom_u.gaplex\endcsname{-0.022}
\expandafter\def\csname res@zs.asom_u.gaplexci\endcsname{[-0.032, -0.011]}
\expandafter\def\csname res@zs.asom_u.gapnonen\endcsname{-0.034}
\expandafter\def\csname res@zs.asom_u.gapnonenci\endcsname{[-0.040, -0.028]}
\expandafter\def\csname res@zs.asom_u.knownauc\endcsname{0.848}
\expandafter\def\csname res@zs.asom_u.novel\endcsname{0.104}
\expandafter\def\csname res@zs.asom_u.novelauc\endcsname{0.736}
\expandafter\def\csname res@zs.asom_v2.calm\endcsname{0.176}
\expandafter\def\csname res@zs.asom_v2.f1\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2.f1ci\endcsname{[0.402, 0.441]}
\expandafter\def\csname res@zs.asom_v2.f1ctrl\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2.f1ctrlci\endcsname{[0.398, 0.443]}
\expandafter\def\csname res@zs.asom_v2.f1emobox\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2.f1emoboxci\endcsname{[0.398, 0.444]}
\expandafter\def\csname res@zs.asom_v2.f1en\endcsname{0.368}
\expandafter\def\csname res@zs.asom_v2.f1enci\endcsname{[0.325, 0.401]}
\expandafter\def\csname res@zs.asom_v2.f1lex\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2.f1lexci\endcsname{[0.405, 0.446]}
\expandafter\def\csname res@zs.asom_v2.f1nonen\endcsname{0.456}
\expandafter\def\csname res@zs.asom_v2.f1nonenci\endcsname{[0.432, 0.470]}
\expandafter\def\csname res@zs.asom_v2.f1other\endcsname{0.424}
\expandafter\def\csname res@zs.asom_v2.f1otherci\endcsname{[0.397, 0.447]}
\expandafter\def\csname res@zs.asom_v2.f1pm\endcsname{0.531}
\expandafter\def\csname res@zs.asom_v2.f1pmctrl\endcsname{0.541}
\expandafter\def\csname res@zs.asom_v2.f1pmen\endcsname{0.456}
\expandafter\def\csname res@zs.asom_v2.f1pmlex\endcsname{0.488}
\expandafter\def\csname res@zs.asom_v2.f1pmnonen\endcsname{0.568}
\expandafter\def\csname res@zs.asom_v2.gap\endcsname{+0.007}
\expandafter\def\csname res@zs.asom_v2.gapci\endcsname{[-0.005, +0.021]}
\expandafter\def\csname res@zs.asom_v2.gapctrl\endcsname{-0.008}
\expandafter\def\csname res@zs.asom_v2.gapctrlci\endcsname{[-0.021, +0.009]}
\expandafter\def\csname res@zs.asom_v2.gapen\endcsname{-0.030}
\expandafter\def\csname res@zs.asom_v2.gapenci\endcsname{[-0.056, +0.002]}
\expandafter\def\csname res@zs.asom_v2.gaplex\endcsname{+0.067}
\expandafter\def\csname res@zs.asom_v2.gaplexci\endcsname{[+0.051, +0.083]}
\expandafter\def\csname res@zs.asom_v2.gapnonen\endcsname{+0.025}
\expandafter\def\csname res@zs.asom_v2.gapnonenci\endcsname{[+0.015, +0.035]}
\expandafter\def\csname res@zs.asom_v2.knownauc\endcsname{0.822}
\expandafter\def\csname res@zs.asom_v2.novel\endcsname{0.035}
\expandafter\def\csname res@zs.asom_v2.novelauc\endcsname{0.735}
\expandafter\def\csname res@zs.asom_v2_s43.calm\endcsname{0.172}
\expandafter\def\csname res@zs.asom_v2_s43.f1\endcsname{0.434}
\expandafter\def\csname res@zs.asom_v2_s43.f1pm\endcsname{0.532}
\expandafter\def\csname res@zs.asom_v2_s43.knownauc\endcsname{0.820}
\expandafter\def\csname res@zs.asom_v2_s43.novel\endcsname{0.034}
\expandafter\def\csname res@zs.asom_v2_s43.novelauc\endcsname{0.740}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.calm\endcsname{0.646}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.f1\endcsname{0.460}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.f1pm\endcsname{0.537}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.knownauc\endcsname{0.824}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.novel\endcsname{0.154}
\expandafter\def\csname res@zs.asom_v2_s43_noprior.novelauc\endcsname{0.753}
\expandafter\def\csname res@zs.asom_v2_u.calm\endcsname{0.621}
\expandafter\def\csname res@zs.asom_v2_u.f1\endcsname{0.455}
\expandafter\def\csname res@zs.asom_v2_u.f1ci\endcsname{[0.430, 0.469]}
\expandafter\def\csname res@zs.asom_v2_u.f1ctrl\endcsname{0.456}
\expandafter\def\csname res@zs.asom_v2_u.f1ctrlci\endcsname{[0.426, 0.474]}
\expandafter\def\csname res@zs.asom_v2_u.f1emobox\endcsname{0.454}
\expandafter\def\csname res@zs.asom_v2_u.f1emoboxci\endcsname{[0.424, 0.472]}
\expandafter\def\csname res@zs.asom_v2_u.f1en\endcsname{0.407}
\expandafter\def\csname res@zs.asom_v2_u.f1enci\endcsname{[0.360, 0.441]}
\expandafter\def\csname res@zs.asom_v2_u.f1lex\endcsname{0.449}
\expandafter\def\csname res@zs.asom_v2_u.f1lexci\endcsname{[0.428, 0.467]}
\expandafter\def\csname res@zs.asom_v2_u.f1nonen\endcsname{0.479}
\expandafter\def\csname res@zs.asom_v2_u.f1nonenci\endcsname{[0.455, 0.492]}
\expandafter\def\csname res@zs.asom_v2_u.f1other\endcsname{0.456}
\expandafter\def\csname res@zs.asom_v2_u.f1otherci\endcsname{[0.432, 0.476]}
\expandafter\def\csname res@zs.asom_v2_u.f1pm\endcsname{0.536}
\expandafter\def\csname res@zs.asom_v2_u.f1pmctrl\endcsname{0.546}
\expandafter\def\csname res@zs.asom_v2_u.f1pmen\endcsname{0.458}
\expandafter\def\csname res@zs.asom_v2_u.f1pmlex\endcsname{0.492}
\expandafter\def\csname res@zs.asom_v2_u.f1pmnonen\endcsname{0.574}
\expandafter\def\csname res@zs.asom_v2_u.gap\endcsname{-0.021}
\expandafter\def\csname res@zs.asom_v2_u.gapci\endcsname{[-0.034, -0.007]}
\expandafter\def\csname res@zs.asom_v2_u.gapctrl\endcsname{-0.037}
\expandafter\def\csname res@zs.asom_v2_u.gapctrlci\endcsname{[-0.052, -0.019]}
\expandafter\def\csname res@zs.asom_v2_u.gapen\endcsname{-0.068}
\expandafter\def\csname res@zs.asom_v2_u.gapenci\endcsname{[-0.097, -0.032]}
\expandafter\def\csname res@zs.asom_v2_u.gaplex\endcsname{+0.045}
\expandafter\def\csname res@zs.asom_v2_u.gaplexci\endcsname{[+0.029, +0.061]}
\expandafter\def\csname res@zs.asom_v2_u.gapnonen\endcsname{+0.002}
\expandafter\def\csname res@zs.asom_v2_u.gapnonenci\endcsname{[-0.008, +0.012]}
\expandafter\def\csname res@zs.asom_v2_u.knownauc\endcsname{0.826}
\expandafter\def\csname res@zs.asom_v2_u.novel\endcsname{0.160}
\expandafter\def\csname res@zs.asom_v2_u.novelauc\endcsname{0.747}
\expandafter\def\csname res@zs.asom_v2_vg.calm\endcsname{0.172}
\expandafter\def\csname res@zs.asom_v2_vg.f1\endcsname{0.434}
\expandafter\def\csname res@zs.asom_v2_vg.f1ci\endcsname{[0.408, 0.448]}
\expandafter\def\csname res@zs.asom_v2_vg.f1ctrl\endcsname{0.435}
\expandafter\def\csname res@zs.asom_v2_vg.f1ctrlci\endcsname{[0.404, 0.451]}
\expandafter\def\csname res@zs.asom_v2_vg.f1emobox\endcsname{0.437}
\expandafter\def\csname res@zs.asom_v2_vg.f1emoboxci\endcsname{[0.406, 0.454]}
\expandafter\def\csname res@zs.asom_v2_vg.f1en\endcsname{0.371}
\expandafter\def\csname res@zs.asom_v2_vg.f1enci\endcsname{[0.324, 0.405]}
\expandafter\def\csname res@zs.asom_v2_vg.f1lex\endcsname{0.430}
\expandafter\def\csname res@zs.asom_v2_vg.f1lexci\endcsname{[0.407, 0.451]}
\expandafter\def\csname res@zs.asom_v2_vg.f1nonen\endcsname{0.465}
\expandafter\def\csname res@zs.asom_v2_vg.f1nonenci\endcsname{[0.440, 0.479]}
\expandafter\def\csname res@zs.asom_v2_vg.f1other\endcsname{0.419}
\expandafter\def\csname res@zs.asom_v2_vg.f1otherci\endcsname{[0.392, 0.442]}
\expandafter\def\csname res@zs.asom_v2_vg.f1pm\endcsname{0.532}
\expandafter\def\csname res@zs.asom_v2_vg.f1pmctrl\endcsname{0.541}
\expandafter\def\csname res@zs.asom_v2_vg.f1pmen\endcsname{0.459}
\expandafter\def\csname res@zs.asom_v2_vg.f1pmlex\endcsname{0.494}
\expandafter\def\csname res@zs.asom_v2_vg.f1pmnonen\endcsname{0.569}
\expandafter\def\csname res@zs.asom_v2_vg.gap\endcsname{-0.000}
\expandafter\def\csname res@zs.asom_v2_vg.gapci\endcsname{[-0.012, +0.015]}
\expandafter\def\csname res@zs.asom_v2_vg.gapctrl\endcsname{-0.015}
\expandafter\def\csname res@zs.asom_v2_vg.gapctrlci\endcsname{[-0.030, +0.003]}
\expandafter\def\csname res@zs.asom_v2_vg.gapen\endcsname{-0.033}
\expandafter\def\csname res@zs.asom_v2_vg.gapenci\endcsname{[-0.062, +0.002]}
\expandafter\def\csname res@zs.asom_v2_vg.gaplex\endcsname{+0.063}
\expandafter\def\csname res@zs.asom_v2_vg.gaplexci\endcsname{[+0.046, +0.080]}
\expandafter\def\csname res@zs.asom_v2_vg.gapnonen\endcsname{+0.016}
\expandafter\def\csname res@zs.asom_v2_vg.gapnonenci\endcsname{[+0.005, +0.027]}
\expandafter\def\csname res@zs.asom_v2_vg.knownauc\endcsname{0.820}
\expandafter\def\csname res@zs.asom_v2_vg.novel\endcsname{0.034}
\expandafter\def\csname res@zs.asom_v2_vg.novelauc\endcsname{0.740}
\expandafter\def\csname res@zs.asom_v2_vg_u.calm\endcsname{0.646}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1\endcsname{0.460}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1ci\endcsname{[0.435, 0.474]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1ctrl\endcsname{0.463}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1ctrlci\endcsname{[0.433, 0.480]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1emobox\endcsname{0.464}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1emoboxci\endcsname{[0.435, 0.482]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1en\endcsname{0.405}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1enci\endcsname{[0.360, 0.439]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1lex\endcsname{0.448}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1lexci\endcsname{[0.426, 0.466]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1nonen\endcsname{0.487}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1nonenci\endcsname{[0.463, 0.501]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1other\endcsname{0.440}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1otherci\endcsname{[0.416, 0.461]}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1pm\endcsname{0.537}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1pmctrl\endcsname{0.547}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1pmen\endcsname{0.460}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1pmlex\endcsname{0.495}
\expandafter\def\csname res@zs.asom_v2_vg_u.f1pmnonen\endcsname{0.576}
\expandafter\def\csname res@zs.asom_v2_vg_u.gap\endcsname{-0.027}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapci\endcsname{[-0.039, -0.012]}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapctrl\endcsname{-0.044}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapctrlci\endcsname{[-0.058, -0.027]}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapen\endcsname{-0.067}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapenci\endcsname{[-0.096, -0.033]}
\expandafter\def\csname res@zs.asom_v2_vg_u.gaplex\endcsname{+0.046}
\expandafter\def\csname res@zs.asom_v2_vg_u.gaplexci\endcsname{[+0.029, +0.062]}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapnonen\endcsname{-0.006}
\expandafter\def\csname res@zs.asom_v2_vg_u.gapnonenci\endcsname{[-0.017, +0.004]}
\expandafter\def\csname res@zs.asom_v2_vg_u.knownauc\endcsname{0.824}
\expandafter\def\csname res@zs.asom_v2_vg_u.novel\endcsname{0.154}
\expandafter\def\csname res@zs.asom_v2_vg_u.novelauc\endcsname{0.753}
\expandafter\def\csname res@zs.asom_v2g_s43.calm\endcsname{0.162}
\expandafter\def\csname res@zs.asom_v2g_s43.f1\endcsname{0.426}
\expandafter\def\csname res@zs.asom_v2g_s43.f1pm\endcsname{0.529}
\expandafter\def\csname res@zs.asom_v2g_s43.knownauc\endcsname{0.818}
\expandafter\def\csname res@zs.asom_v2g_s43.novel\endcsname{0.032}
\expandafter\def\csname res@zs.asom_v2g_s43.novelauc\endcsname{0.740}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.calm\endcsname{0.662}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.f1\endcsname{0.451}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.f1pm\endcsname{0.534}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.knownauc\endcsname{0.822}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.novel\endcsname{0.154}
\expandafter\def\csname res@zs.asom_v2g_s43_noprior.novelauc\endcsname{0.752}
\expandafter\def\csname res@zs.asom_v2g_s44.calm\endcsname{0.191}
\expandafter\def\csname res@zs.asom_v2g_s44.f1\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2g_s44.f1pm\endcsname{0.532}
\expandafter\def\csname res@zs.asom_v2g_s44.knownauc\endcsname{0.818}
\expandafter\def\csname res@zs.asom_v2g_s44.novel\endcsname{0.038}
\expandafter\def\csname res@zs.asom_v2g_s44.novelauc\endcsname{0.721}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.calm\endcsname{0.580}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.f1\endcsname{0.459}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.f1pm\endcsname{0.537}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.knownauc\endcsname{0.822}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.novel\endcsname{0.166}
\expandafter\def\csname res@zs.asom_v2g_s44_noprior.novelauc\endcsname{0.733}
\expandafter\def\csname res@zs.asom_v2na.calm\endcsname{0.410}
\expandafter\def\csname res@zs.asom_v2na.f1\endcsname{0.461}
\expandafter\def\csname res@zs.asom_v2na.f1ci\endcsname{[0.436, 0.475]}
\expandafter\def\csname res@zs.asom_v2na.f1ctrl\endcsname{0.452}
\expandafter\def\csname res@zs.asom_v2na.f1ctrlci\endcsname{[0.422, 0.470]}
\expandafter\def\csname res@zs.asom_v2na.f1emobox\endcsname{0.457}
\expandafter\def\csname res@zs.asom_v2na.f1emoboxci\endcsname{[0.426, 0.474]}
\expandafter\def\csname res@zs.asom_v2na.f1en\endcsname{0.383}
\expandafter\def\csname res@zs.asom_v2na.f1enci\endcsname{[0.337, 0.420]}
\expandafter\def\csname res@zs.asom_v2na.f1lex\endcsname{0.496}
\expandafter\def\csname res@zs.asom_v2na.f1lexci\endcsname{[0.476, 0.513]}
\expandafter\def\csname res@zs.asom_v2na.f1nonen\endcsname{0.500}
\expandafter\def\csname res@zs.asom_v2na.f1nonenci\endcsname{[0.474, 0.513]}
\expandafter\def\csname res@zs.asom_v2na.f1other\endcsname{0.478}
\expandafter\def\csname res@zs.asom_v2na.f1otherci\endcsname{[0.454, 0.498]}
\expandafter\def\csname res@zs.asom_v2na.f1pm\endcsname{0.558}
\expandafter\def\csname res@zs.asom_v2na.f1pmctrl\endcsname{0.563}
\expandafter\def\csname res@zs.asom_v2na.f1pmen\endcsname{0.465}
\expandafter\def\csname res@zs.asom_v2na.f1pmlex\endcsname{0.537}
\expandafter\def\csname res@zs.asom_v2na.f1pmnonen\endcsname{0.604}
\expandafter\def\csname res@zs.asom_v2na.gap\endcsname{-0.027}
\expandafter\def\csname res@zs.asom_v2na.gapci\endcsname{[-0.039, -0.014]}
\expandafter\def\csname res@zs.asom_v2na.gapctrl\endcsname{-0.033}
\expandafter\def\csname res@zs.asom_v2na.gapctrlci\endcsname{[-0.047, -0.017]}
\expandafter\def\csname res@zs.asom_v2na.gapen\endcsname{-0.045}
\expandafter\def\csname res@zs.asom_v2na.gapenci\endcsname{[-0.073, -0.012]}
\expandafter\def\csname res@zs.asom_v2na.gaplex\endcsname{-0.002}
\expandafter\def\csname res@zs.asom_v2na.gaplexci\endcsname{[-0.013, +0.009]}
\expandafter\def\csname res@zs.asom_v2na.gapnonen\endcsname{-0.019}
\expandafter\def\csname res@zs.asom_v2na.gapnonenci\endcsname{[-0.026, -0.010]}
\expandafter\def\csname res@zs.asom_v2na.knownauc\endcsname{0.846}
\expandafter\def\csname res@zs.asom_v2na.novel\endcsname{0.082}
\expandafter\def\csname res@zs.asom_v2na.novelauc\endcsname{0.746}
\expandafter\def\csname res@zs.asom_v2na_s43.calm\endcsname{0.364}
\expandafter\def\csname res@zs.asom_v2na_s43.f1\endcsname{0.460}
\expandafter\def\csname res@zs.asom_v2na_s43.f1pm\endcsname{0.556}
\expandafter\def\csname res@zs.asom_v2na_s43.knownauc\endcsname{0.840}
\expandafter\def\csname res@zs.asom_v2na_s43.novel\endcsname{0.073}
\expandafter\def\csname res@zs.asom_v2na_s43.novelauc\endcsname{0.751}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.calm\endcsname{0.557}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.f1\endcsname{0.488}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.f1pm\endcsname{0.556}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.novel\endcsname{0.154}
\expandafter\def\csname res@zs.asom_v2na_s43_noprior.novelauc\endcsname{0.763}
\expandafter\def\csname res@zs.asom_v2na_s44.calm\endcsname{0.502}
\expandafter\def\csname res@zs.asom_v2na_s44.f1\endcsname{0.465}
\expandafter\def\csname res@zs.asom_v2na_s44.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_v2na_s44.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.asom_v2na_s44.novel\endcsname{0.100}
\expandafter\def\csname res@zs.asom_v2na_s44.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.calm\endcsname{0.608}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.f1\endcsname{0.492}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.knownauc\endcsname{0.846}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.novel\endcsname{0.157}
\expandafter\def\csname res@zs.asom_v2na_s44_noprior.novelauc\endcsname{0.748}
\expandafter\def\csname res@zs.asom_v2na_s45.calm\endcsname{0.363}
\expandafter\def\csname res@zs.asom_v2na_s45.f1\endcsname{0.457}
\expandafter\def\csname res@zs.asom_v2na_s45.f1pm\endcsname{0.555}
\expandafter\def\csname res@zs.asom_v2na_s45.knownauc\endcsname{0.840}
\expandafter\def\csname res@zs.asom_v2na_s45.novel\endcsname{0.073}
\expandafter\def\csname res@zs.asom_v2na_s45.novelauc\endcsname{0.741}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.calm\endcsname{0.529}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.f1\endcsname{0.484}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.f1pm\endcsname{0.557}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.novel\endcsname{0.127}
\expandafter\def\csname res@zs.asom_v2na_s45_noprior.novelauc\endcsname{0.755}
\expandafter\def\csname res@zs.asom_v2na_u.calm\endcsname{0.565}
\expandafter\def\csname res@zs.asom_v2na_u.f1\endcsname{0.488}
\expandafter\def\csname res@zs.asom_v2na_u.f1ci\endcsname{[0.464, 0.502]}
\expandafter\def\csname res@zs.asom_v2na_u.f1ctrl\endcsname{0.481}
\expandafter\def\csname res@zs.asom_v2na_u.f1ctrlci\endcsname{[0.452, 0.498]}
\expandafter\def\csname res@zs.asom_v2na_u.f1emobox\endcsname{0.479}
\expandafter\def\csname res@zs.asom_v2na_u.f1emoboxci\endcsname{[0.449, 0.496]}
\expandafter\def\csname res@zs.asom_v2na_u.f1en\endcsname{0.407}
\expandafter\def\csname res@zs.asom_v2na_u.f1enci\endcsname{[0.360, 0.443]}
\expandafter\def\csname res@zs.asom_v2na_u.f1lex\endcsname{0.518}
\expandafter\def\csname res@zs.asom_v2na_u.f1lexci\endcsname{[0.499, 0.533]}
\expandafter\def\csname res@zs.asom_v2na_u.f1nonen\endcsname{0.529}
\expandafter\def\csname res@zs.asom_v2na_u.f1nonenci\endcsname{[0.505, 0.541]}
\expandafter\def\csname res@zs.asom_v2na_u.f1other\endcsname{0.527}
\expandafter\def\csname res@zs.asom_v2na_u.f1otherci\endcsname{[0.505, 0.546]}
\expandafter\def\csname res@zs.asom_v2na_u.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.asom_v2na_u.f1pmctrl\endcsname{0.564}
\expandafter\def\csname res@zs.asom_v2na_u.f1pmen\endcsname{0.465}
\expandafter\def\csname res@zs.asom_v2na_u.f1pmlex\endcsname{0.536}
\expandafter\def\csname res@zs.asom_v2na_u.f1pmnonen\endcsname{0.606}
\expandafter\def\csname res@zs.asom_v2na_u.gap\endcsname{-0.055}
\expandafter\def\csname res@zs.asom_v2na_u.gapci\endcsname{[-0.066, -0.041]}
\expandafter\def\csname res@zs.asom_v2na_u.gapctrl\endcsname{-0.062}
\expandafter\def\csname res@zs.asom_v2na_u.gapctrlci\endcsname{[-0.076, -0.046]}
\expandafter\def\csname res@zs.asom_v2na_u.gapen\endcsname{-0.069}
\expandafter\def\csname res@zs.asom_v2na_u.gapenci\endcsname{[-0.098, -0.034]}
\expandafter\def\csname res@zs.asom_v2na_u.gaplex\endcsname{-0.024}
\expandafter\def\csname res@zs.asom_v2na_u.gaplexci\endcsname{[-0.037, -0.011]}
\expandafter\def\csname res@zs.asom_v2na_u.gapnonen\endcsname{-0.048}
\expandafter\def\csname res@zs.asom_v2na_u.gapnonenci\endcsname{[-0.055, -0.040]}
\expandafter\def\csname res@zs.asom_v2na_u.knownauc\endcsname{0.848}
\expandafter\def\csname res@zs.asom_v2na_u.novel\endcsname{0.146}
\expandafter\def\csname res@zs.asom_v2na_u.novelauc\endcsname{0.758}
\expandafter\def\csname res@zs.asom_v2ne_s43.calm\endcsname{0.415}
\expandafter\def\csname res@zs.asom_v2ne_s43.f1\endcsname{0.432}
\expandafter\def\csname res@zs.asom_v2ne_s43.f1pm\endcsname{0.532}
\expandafter\def\csname res@zs.asom_v2ne_s43.knownauc\endcsname{0.817}
\expandafter\def\csname res@zs.asom_v2ne_s43.novel\endcsname{0.083}
\expandafter\def\csname res@zs.asom_v2ne_s43.novelauc\endcsname{0.723}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.calm\endcsname{0.615}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.f1\endcsname{0.452}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.f1pm\endcsname{0.538}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.knownauc\endcsname{0.822}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.novel\endcsname{0.158}
\expandafter\def\csname res@zs.asom_v2ne_s43_noprior.novelauc\endcsname{0.739}
\expandafter\def\csname res@zs.asom_v2r1_s43.calm\endcsname{0.061}
\expandafter\def\csname res@zs.asom_v2r1_s43.f1\endcsname{0.427}
\expandafter\def\csname res@zs.asom_v2r1_s43.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.asom_v2r1_s43.knownauc\endcsname{0.838}
\expandafter\def\csname res@zs.asom_v2r1_s43.novel\endcsname{0.012}
\expandafter\def\csname res@zs.asom_v2r1_s43.novelauc\endcsname{0.742}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.calm\endcsname{0.473}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.f1\endcsname{0.456}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.f1pm\endcsname{0.558}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.knownauc\endcsname{0.843}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.novel\endcsname{0.124}
\expandafter\def\csname res@zs.asom_v2r1_s43_noprior.novelauc\endcsname{0.753}
\expandafter\def\csname res@zs.asom_v2sp.calm\endcsname{0.482}
\expandafter\def\csname res@zs.asom_v2sp.f1\endcsname{0.472}
\expandafter\def\csname res@zs.asom_v2sp.f1ci\endcsname{[0.446, 0.487]}
\expandafter\def\csname res@zs.asom_v2sp.f1ctrl\endcsname{0.468}
\expandafter\def\csname res@zs.asom_v2sp.f1ctrlci\endcsname{[0.437, 0.487]}
\expandafter\def\csname res@zs.asom_v2sp.f1emobox\endcsname{0.463}
\expandafter\def\csname res@zs.asom_v2sp.f1emoboxci\endcsname{[0.430, 0.481]}
\expandafter\def\csname res@zs.asom_v2sp.f1en\endcsname{0.393}
\expandafter\def\csname res@zs.asom_v2sp.f1enci\endcsname{[0.343, 0.433]}
\expandafter\def\csname res@zs.asom_v2sp.f1lex\endcsname{0.488}
\expandafter\def\csname res@zs.asom_v2sp.f1lexci\endcsname{[0.468, 0.505]}
\expandafter\def\csname res@zs.asom_v2sp.f1nonen\endcsname{0.511}
\expandafter\def\csname res@zs.asom_v2sp.f1nonenci\endcsname{[0.486, 0.524]}
\expandafter\def\csname res@zs.asom_v2sp.f1other\endcsname{0.512}
\expandafter\def\csname res@zs.asom_v2sp.f1otherci\endcsname{[0.490, 0.532]}
\expandafter\def\csname res@zs.asom_v2sp.f1pm\endcsname{0.561}
\expandafter\def\csname res@zs.asom_v2sp.f1pmctrl\endcsname{0.568}
\expandafter\def\csname res@zs.asom_v2sp.f1pmen\endcsname{0.470}
\expandafter\def\csname res@zs.asom_v2sp.f1pmlex\endcsname{0.530}
\expandafter\def\csname res@zs.asom_v2sp.f1pmnonen\endcsname{0.606}
\expandafter\def\csname res@zs.asom_v2sp.gap\endcsname{-0.039}
\expandafter\def\csname res@zs.asom_v2sp.gapci\endcsname{[-0.051, -0.024]}
\expandafter\def\csname res@zs.asom_v2sp.gapctrl\endcsname{-0.049}
\expandafter\def\csname res@zs.asom_v2sp.gapctrlci\endcsname{[-0.064, -0.031]}
\expandafter\def\csname res@zs.asom_v2sp.gapen\endcsname{-0.055}
\expandafter\def\csname res@zs.asom_v2sp.gapenci\endcsname{[-0.085, -0.019]}
\expandafter\def\csname res@zs.asom_v2sp.gaplex\endcsname{+0.006}
\expandafter\def\csname res@zs.asom_v2sp.gaplexci\endcsname{[-0.004, +0.016]}
\expandafter\def\csname res@zs.asom_v2sp.gapnonen\endcsname{-0.031}
\expandafter\def\csname res@zs.asom_v2sp.gapnonenci\endcsname{[-0.039, -0.022]}
\expandafter\def\csname res@zs.asom_v2sp.knownauc\endcsname{0.848}
\expandafter\def\csname res@zs.asom_v2sp.novel\endcsname{0.107}
\expandafter\def\csname res@zs.asom_v2sp.novelauc\endcsname{0.740}
\expandafter\def\csname res@zs.asom_v2sp_em.calm\endcsname{0.145}
\expandafter\def\csname res@zs.asom_v2sp_em.f1\endcsname{0.262}
\expandafter\def\csname res@zs.asom_v2sp_em.f1ci\endcsname{[0.245, 0.272]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1ctrl\endcsname{0.264}
\expandafter\def\csname res@zs.asom_v2sp_em.f1ctrlci\endcsname{[0.244, 0.276]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1emobox\endcsname{0.265}
\expandafter\def\csname res@zs.asom_v2sp_em.f1emoboxci\endcsname{[0.244, 0.277]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1en\endcsname{0.208}
\expandafter\def\csname res@zs.asom_v2sp_em.f1enci\endcsname{[0.174, 0.232]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1lex\endcsname{0.254}
\expandafter\def\csname res@zs.asom_v2sp_em.f1lexci\endcsname{[0.234, 0.270]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1nonen\endcsname{0.289}
\expandafter\def\csname res@zs.asom_v2sp_em.f1nonenci\endcsname{[0.273, 0.298]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1other\endcsname{0.248}
\expandafter\def\csname res@zs.asom_v2sp_em.f1otherci\endcsname{[0.233, 0.262]}
\expandafter\def\csname res@zs.asom_v2sp_em.f1pm\endcsname{0.436}
\expandafter\def\csname res@zs.asom_v2sp_em.f1pmctrl\endcsname{0.436}
\expandafter\def\csname res@zs.asom_v2sp_em.f1pmen\endcsname{0.359}
\expandafter\def\csname res@zs.asom_v2sp_em.f1pmlex\endcsname{0.437}
\expandafter\def\csname res@zs.asom_v2sp_em.f1pmnonen\endcsname{0.475}
\expandafter\def\csname res@zs.asom_v2sp_em.gap\endcsname{+0.171}
\expandafter\def\csname res@zs.asom_v2sp_em.gapci\endcsname{[+0.160, +0.182]}
\expandafter\def\csname res@zs.asom_v2sp_em.gapctrl\endcsname{+0.155}
\expandafter\def\csname res@zs.asom_v2sp_em.gapctrlci\endcsname{[+0.141, +0.168]}
\expandafter\def\csname res@zs.asom_v2sp_em.gapen\endcsname{+0.130}
\expandafter\def\csname res@zs.asom_v2sp_em.gapenci\endcsname{[+0.108, +0.156]}
\expandafter\def\csname res@zs.asom_v2sp_em.gaplex\endcsname{+0.239}
\expandafter\def\csname res@zs.asom_v2sp_em.gaplexci\endcsname{[+0.223, +0.254]}
\expandafter\def\csname res@zs.asom_v2sp_em.gapnonen\endcsname{+0.192}
\expandafter\def\csname res@zs.asom_v2sp_em.gapnonenci\endcsname{[+0.178, +0.202]}
\expandafter\def\csname res@zs.asom_v2sp_em.knownauc\endcsname{0.855}
\expandafter\def\csname res@zs.asom_v2sp_em.novel\endcsname{0.029}
\expandafter\def\csname res@zs.asom_v2sp_em.novelauc\endcsname{0.919}
\expandafter\def\csname res@zs.asom_v2sp_s43.calm\endcsname{0.448}
\expandafter\def\csname res@zs.asom_v2sp_s43.f1\endcsname{0.478}
\expandafter\def\csname res@zs.asom_v2sp_s43.f1pm\endcsname{0.561}
\expandafter\def\csname res@zs.asom_v2sp_s43.knownauc\endcsname{0.847}
\expandafter\def\csname res@zs.asom_v2sp_s43.novel\endcsname{0.111}
\expandafter\def\csname res@zs.asom_v2sp_s43.novelauc\endcsname{0.735}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.calm\endcsname{0.530}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.f1\endcsname{0.499}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.f1pm\endcsname{0.565}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.novel\endcsname{0.148}
\expandafter\def\csname res@zs.asom_v2sp_s43_noprior.novelauc\endcsname{0.751}
\expandafter\def\csname res@zs.asom_v2sp_s44.calm\endcsname{0.523}
\expandafter\def\csname res@zs.asom_v2sp_s44.f1\endcsname{0.469}
\expandafter\def\csname res@zs.asom_v2sp_s44.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_v2sp_s44.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.asom_v2sp_s44.novel\endcsname{0.111}
\expandafter\def\csname res@zs.asom_v2sp_s44.novelauc\endcsname{0.736}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.calm\endcsname{0.621}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.f1\endcsname{0.492}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.f1pm\endcsname{0.564}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.knownauc\endcsname{0.847}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.novel\endcsname{0.152}
\expandafter\def\csname res@zs.asom_v2sp_s44_noprior.novelauc\endcsname{0.752}
\expandafter\def\csname res@zs.asom_v2sp_s45.calm\endcsname{0.474}
\expandafter\def\csname res@zs.asom_v2sp_s45.f1\endcsname{0.469}
\expandafter\def\csname res@zs.asom_v2sp_s45.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.asom_v2sp_s45.knownauc\endcsname{0.843}
\expandafter\def\csname res@zs.asom_v2sp_s45.novel\endcsname{0.098}
\expandafter\def\csname res@zs.asom_v2sp_s45.novelauc\endcsname{0.743}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.calm\endcsname{0.598}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.f1\endcsname{0.489}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.f1pm\endcsname{0.560}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.knownauc\endcsname{0.846}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.novel\endcsname{0.149}
\expandafter\def\csname res@zs.asom_v2sp_s45_noprior.novelauc\endcsname{0.758}
\expandafter\def\csname res@zs.asom_v2sp_u.calm\endcsname{0.583}
\expandafter\def\csname res@zs.asom_v2sp_u.f1\endcsname{0.494}
\expandafter\def\csname res@zs.asom_v2sp_u.f1ci\endcsname{[0.467, 0.508]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1ctrl\endcsname{0.490}
\expandafter\def\csname res@zs.asom_v2sp_u.f1ctrlci\endcsname{[0.459, 0.508]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1emobox\endcsname{0.482}
\expandafter\def\csname res@zs.asom_v2sp_u.f1emoboxci\endcsname{[0.451, 0.500]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1en\endcsname{0.418}
\expandafter\def\csname res@zs.asom_v2sp_u.f1enci\endcsname{[0.364, 0.458]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1lex\endcsname{0.508}
\expandafter\def\csname res@zs.asom_v2sp_u.f1lexci\endcsname{[0.489, 0.523]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1nonen\endcsname{0.531}
\expandafter\def\csname res@zs.asom_v2sp_u.f1nonenci\endcsname{[0.508, 0.543]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1other\endcsname{0.542}
\expandafter\def\csname res@zs.asom_v2sp_u.f1otherci\endcsname{[0.520, 0.561]}
\expandafter\def\csname res@zs.asom_v2sp_u.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.asom_v2sp_u.f1pmctrl\endcsname{0.570}
\expandafter\def\csname res@zs.asom_v2sp_u.f1pmen\endcsname{0.472}
\expandafter\def\csname res@zs.asom_v2sp_u.f1pmlex\endcsname{0.533}
\expandafter\def\csname res@zs.asom_v2sp_u.f1pmnonen\endcsname{0.609}
\expandafter\def\csname res@zs.asom_v2sp_u.gap\endcsname{-0.060}
\expandafter\def\csname res@zs.asom_v2sp_u.gapci\endcsname{[-0.073, -0.045]}
\expandafter\def\csname res@zs.asom_v2sp_u.gapctrl\endcsname{-0.071}
\expandafter\def\csname res@zs.asom_v2sp_u.gapctrlci\endcsname{[-0.086, -0.052]}
\expandafter\def\csname res@zs.asom_v2sp_u.gapen\endcsname{-0.080}
\expandafter\def\csname res@zs.asom_v2sp_u.gapenci\endcsname{[-0.112, -0.041]}
\expandafter\def\csname res@zs.asom_v2sp_u.gaplex\endcsname{-0.014}
\expandafter\def\csname res@zs.asom_v2sp_u.gaplexci\endcsname{[-0.028, -0.001]}
\expandafter\def\csname res@zs.asom_v2sp_u.gapnonen\endcsname{-0.051}
\expandafter\def\csname res@zs.asom_v2sp_u.gapnonenci\endcsname{[-0.059, -0.041]}
\expandafter\def\csname res@zs.asom_v2sp_u.knownauc\endcsname{0.851}
\expandafter\def\csname res@zs.asom_v2sp_u.novel\endcsname{0.150}
\expandafter\def\csname res@zs.asom_v2sp_u.novelauc\endcsname{0.756}
\expandafter\def\csname res@zs.bestalm.ctrl.f1\endcsname{0.281}
\expandafter\def\csname res@zs.bestalm.ctrl.f1pm\endcsname{0.385}
\expandafter\def\csname res@zs.bestalm.ctrl.gap\endcsname{+0.138}
\expandafter\def\csname res@zs.bestalm.ctrl.gapabs\endcsname{0.138}
\expandafter\def\csname res@zs.bestalm.ctrl.gapci\endcsname{[+0.119, +0.152]}
\expandafter\def\csname res@zs.bestalm.ctrl.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@zs.bestalm.en.f1\endcsname{0.382}
\expandafter\def\csname res@zs.bestalm.en.f1pm\endcsname{0.468}
\expandafter\def\csname res@zs.bestalm.en.gap\endcsname{-0.044}
\expandafter\def\csname res@zs.bestalm.en.gapabs\endcsname{0.044}
\expandafter\def\csname res@zs.bestalm.en.gapci\endcsname{[-0.059, -0.027]}
\expandafter\def\csname res@zs.bestalm.en.name\endcsname{Qwen2-Audio-7B-Instruct}
\expandafter\def\csname res@zs.bestalm.f1\endcsname{0.313}
\expandafter\def\csname res@zs.bestalm.gap\endcsname{+0.120}
\expandafter\def\csname res@zs.bestalm.gapci\endcsname{[+0.104, +0.132]}
\expandafter\def\csname res@zs.bestalm.lex.f1\endcsname{0.550}
\expandafter\def\csname res@zs.bestalm.lex.f1pm\endcsname{0.551}
\expandafter\def\csname res@zs.bestalm.lex.gap\endcsname{-0.056}
\expandafter\def\csname res@zs.bestalm.lex.gapabs\endcsname{0.056}
\expandafter\def\csname res@zs.bestalm.lex.gapci\endcsname{[-0.076, -0.037]}
\expandafter\def\csname res@zs.bestalm.lex.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@zs.bestalm.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@zs.bestalm.nonen.f1\endcsname{0.312}
\expandafter\def\csname res@zs.bestalm.nonen.f1pm\endcsname{0.398}
\expandafter\def\csname res@zs.bestalm.nonen.gap\endcsname{+0.169}
\expandafter\def\csname res@zs.bestalm.nonen.gapabs\endcsname{0.169}
\expandafter\def\csname res@zs.bestalm.nonen.gapci\endcsname{[+0.151, +0.181]}
\expandafter\def\csname res@zs.bestalm.nonen.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@zs.bestalm.novel\endcsname{0.325}
\expandafter\def\csname res@zs.bestalm.novel.name\endcsname{Audio Flamingo 3}
\expandafter\def\csname res@zs.bestalm.novelauc\endcsname{0.799}
\expandafter\def\csname res@zs.bestalm.novelauc.name\endcsname{Audio Flamingo 3 + CC}
\expandafter\def\csname res@zs.bestalmcc.ctrl.f1\endcsname{0.302}
\expandafter\def\csname res@zs.bestalmcc.ctrl.f1pm\endcsname{0.389}
\expandafter\def\csname res@zs.bestalmcc.ctrl.gap\endcsname{+0.117}
\expandafter\def\csname res@zs.bestalmcc.ctrl.gapabs\endcsname{0.117}
\expandafter\def\csname res@zs.bestalmcc.ctrl.gapci\endcsname{[+0.100, +0.129]}
\expandafter\def\csname res@zs.bestalmcc.ctrl.name\endcsname{Qwen2-Audio-7B-Instruct + CC}
\expandafter\def\csname res@zs.bestalmcc.en.f1\endcsname{0.413}
\expandafter\def\csname res@zs.bestalmcc.en.f1pm\endcsname{0.474}
\expandafter\def\csname res@zs.bestalmcc.en.gap\endcsname{-0.075}
\expandafter\def\csname res@zs.bestalmcc.en.gapabs\endcsname{0.075}
\expandafter\def\csname res@zs.bestalmcc.en.gapci\endcsname{[-0.091, -0.059]}
\expandafter\def\csname res@zs.bestalmcc.en.name\endcsname{Qwen2-Audio-7B-Instruct + CC}
\expandafter\def\csname res@zs.bestalmcc.f1\endcsname{0.329}
\expandafter\def\csname res@zs.bestalmcc.gap\endcsname{+0.104}
\expandafter\def\csname res@zs.bestalmcc.gapci\endcsname{[+0.089, +0.115]}
\expandafter\def\csname res@zs.bestalmcc.lex.f1\endcsname{0.527}
\expandafter\def\csname res@zs.bestalmcc.lex.f1pm\endcsname{0.540}
\expandafter\def\csname res@zs.bestalmcc.lex.gap\endcsname{-0.033}
\expandafter\def\csname res@zs.bestalmcc.lex.gapabs\endcsname{0.033}
\expandafter\def\csname res@zs.bestalmcc.lex.gapci\endcsname{[-0.055, -0.010]}
\expandafter\def\csname res@zs.bestalmcc.lex.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@zs.bestalmcc.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@zs.bestalmcc.nonen.f1\endcsname{0.320}
\expandafter\def\csname res@zs.bestalmcc.nonen.f1pm\endcsname{0.403}
\expandafter\def\csname res@zs.bestalmcc.nonen.gap\endcsname{+0.161}
\expandafter\def\csname res@zs.bestalmcc.nonen.gapabs\endcsname{0.161}
\expandafter\def\csname res@zs.bestalmcc.nonen.gapci\endcsname{[+0.142, +0.173]}
\expandafter\def\csname res@zs.bestalmcc.nonen.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@zs.bestalmpm.f1\endcsname{0.404}
\expandafter\def\csname res@zs.bestalmpm.name\endcsname{Qwen2-Audio-7B-Instruct + CC}
\expandafter\def\csname res@zs.chance.ctrl\endcsname{0.173}
\expandafter\def\csname res@zs.chance.f1\endcsname{0.172}
\expandafter\def\csname res@zs.chance.lex\endcsname{0.171}
\expandafter\def\csname res@zs.clap_laion.calm\endcsname{0.255}
\expandafter\def\csname res@zs.clap_laion.f1\endcsname{0.132}
\expandafter\def\csname res@zs.clap_laion.f1ci\endcsname{[0.121, 0.138]}
\expandafter\def\csname res@zs.clap_laion.f1ctrl\endcsname{0.140}
\expandafter\def\csname res@zs.clap_laion.f1ctrlci\endcsname{[0.126, 0.147]}
\expandafter\def\csname res@zs.clap_laion.f1emobox\endcsname{0.132}
\expandafter\def\csname res@zs.clap_laion.f1emoboxci\endcsname{[0.119, 0.139]}
\expandafter\def\csname res@zs.clap_laion.f1en\endcsname{0.093}
\expandafter\def\csname res@zs.clap_laion.f1enci\endcsname{[0.084, 0.099]}
\expandafter\def\csname res@zs.clap_laion.f1lex\endcsname{0.098}
\expandafter\def\csname res@zs.clap_laion.f1lexci\endcsname{[0.088, 0.107]}
\expandafter\def\csname res@zs.clap_laion.f1nonen\endcsname{0.152}
\expandafter\def\csname res@zs.clap_laion.f1nonenci\endcsname{[0.136, 0.161]}
\expandafter\def\csname res@zs.clap_laion.f1other\endcsname{0.130}
\expandafter\def\csname res@zs.clap_laion.f1otherci\endcsname{[0.119, 0.140]}
\expandafter\def\csname res@zs.clap_laion.f1pm\endcsname{0.237}
\expandafter\def\csname res@zs.clap_laion.f1pmctrl\endcsname{0.246}
\expandafter\def\csname res@zs.clap_laion.f1pmen\endcsname{0.182}
\expandafter\def\csname res@zs.clap_laion.f1pmlex\endcsname{0.197}
\expandafter\def\csname res@zs.clap_laion.f1pmnonen\endcsname{0.264}
\expandafter\def\csname res@zs.clap_laion.gap\endcsname{+0.301}
\expandafter\def\csname res@zs.clap_laion.gapci\endcsname{[+0.286, +0.313]}
\expandafter\def\csname res@zs.clap_laion.gapctrl\endcsname{+0.279}
\expandafter\def\csname res@zs.clap_laion.gapctrlci\endcsname{[+0.261, +0.293]}
\expandafter\def\csname res@zs.clap_laion.gapen\endcsname{+0.246}
\expandafter\def\csname res@zs.clap_laion.gapenci\endcsname{[+0.223, +0.266]}
\expandafter\def\csname res@zs.clap_laion.gaplex\endcsname{+0.396}
\expandafter\def\csname res@zs.clap_laion.gaplexci\endcsname{[+0.373, +0.415]}
\expandafter\def\csname res@zs.clap_laion.gapnonen\endcsname{+0.329}
\expandafter\def\csname res@zs.clap_laion.gapnonenci\endcsname{[+0.310, +0.345]}
\expandafter\def\csname res@zs.clap_laion.knownauc\endcsname{0.596}
\expandafter\def\csname res@zs.clap_laion.novel\endcsname{0.094}
\expandafter\def\csname res@zs.clap_laion.novelauc\endcsname{0.461}
\expandafter\def\csname res@zs.clap_laion_desc.calm\endcsname{0.254}
\expandafter\def\csname res@zs.clap_laion_desc.f1\endcsname{0.103}
\expandafter\def\csname res@zs.clap_laion_desc.f1ci\endcsname{[0.096, 0.108]}
\expandafter\def\csname res@zs.clap_laion_desc.f1ctrl\endcsname{0.108}
\expandafter\def\csname res@zs.clap_laion_desc.f1ctrlci\endcsname{[0.099, 0.114]}
\expandafter\def\csname res@zs.clap_laion_desc.f1emobox\endcsname{0.099}
\expandafter\def\csname res@zs.clap_laion_desc.f1emoboxci\endcsname{[0.091, 0.105]}
\expandafter\def\csname res@zs.clap_laion_desc.f1en\endcsname{0.076}
\expandafter\def\csname res@zs.clap_laion_desc.f1enci\endcsname{[0.072, 0.081]}
\expandafter\def\csname res@zs.clap_laion_desc.f1lex\endcsname{0.081}
\expandafter\def\csname res@zs.clap_laion_desc.f1lexci\endcsname{[0.073, 0.091]}
\expandafter\def\csname res@zs.clap_laion_desc.f1nonen\endcsname{0.116}
\expandafter\def\csname res@zs.clap_laion_desc.f1nonenci\endcsname{[0.105, 0.123]}
\expandafter\def\csname res@zs.clap_laion_desc.f1other\endcsname{0.118}
\expandafter\def\csname res@zs.clap_laion_desc.f1otherci\endcsname{[0.108, 0.128]}
\expandafter\def\csname res@zs.clap_laion_desc.f1pm\endcsname{0.205}
\expandafter\def\csname res@zs.clap_laion_desc.f1pmctrl\endcsname{0.209}
\expandafter\def\csname res@zs.clap_laion_desc.f1pmen\endcsname{0.162}
\expandafter\def\csname res@zs.clap_laion_desc.f1pmlex\endcsname{0.190}
\expandafter\def\csname res@zs.clap_laion_desc.f1pmnonen\endcsname{0.227}
\expandafter\def\csname res@zs.clap_laion_desc.gap\endcsname{+0.330}
\expandafter\def\csname res@zs.clap_laion_desc.gapci\endcsname{[+0.314, +0.341]}
\expandafter\def\csname res@zs.clap_laion_desc.gapctrl\endcsname{+0.311}
\expandafter\def\csname res@zs.clap_laion_desc.gapctrlci\endcsname{[+0.292, +0.323]}
\expandafter\def\csname res@zs.clap_laion_desc.gapen\endcsname{+0.262}
\expandafter\def\csname res@zs.clap_laion_desc.gapenci\endcsname{[+0.243, +0.277]}
\expandafter\def\csname res@zs.clap_laion_desc.gaplex\endcsname{+0.412}
\expandafter\def\csname res@zs.clap_laion_desc.gaplexci\endcsname{[+0.391, +0.429]}
\expandafter\def\csname res@zs.clap_laion_desc.gapnonen\endcsname{+0.365}
\expandafter\def\csname res@zs.clap_laion_desc.gapnonenci\endcsname{[+0.343, +0.379]}
\expandafter\def\csname res@zs.clap_laion_desc.knownauc\endcsname{0.562}
\expandafter\def\csname res@zs.clap_laion_desc.novel\endcsname{0.098}
\expandafter\def\csname res@zs.clap_laion_desc.novelauc\endcsname{0.513}
\expandafter\def\csname res@zs.clap_ms.calm\endcsname{0.000}
\expandafter\def\csname res@zs.clap_ms.f1\endcsname{0.249}
\expandafter\def\csname res@zs.clap_ms.f1ci\endcsname{[0.235, 0.256]}
\expandafter\def\csname res@zs.clap_ms.f1ctrl\endcsname{0.249}
\expandafter\def\csname res@zs.clap_ms.f1ctrlci\endcsname{[0.232, 0.257]}
\expandafter\def\csname res@zs.clap_ms.f1emobox\endcsname{0.249}
\expandafter\def\csname res@zs.clap_ms.f1emoboxci\endcsname{[0.233, 0.258]}
\expandafter\def\csname res@zs.clap_ms.f1en\endcsname{0.204}
\expandafter\def\csname res@zs.clap_ms.f1enci\endcsname{[0.185, 0.216]}
\expandafter\def\csname res@zs.clap_ms.f1lex\endcsname{0.249}
\expandafter\def\csname res@zs.clap_ms.f1lexci\endcsname{[0.232, 0.264]}
\expandafter\def\csname res@zs.clap_ms.f1nonen\endcsname{0.271}
\expandafter\def\csname res@zs.clap_ms.f1nonenci\endcsname{[0.252, 0.281]}
\expandafter\def\csname res@zs.clap_ms.f1other\endcsname{0.247}
\expandafter\def\csname res@zs.clap_ms.f1otherci\endcsname{[0.229, 0.262]}
\expandafter\def\csname res@zs.clap_ms.f1pm\endcsname{0.356}
\expandafter\def\csname res@zs.clap_ms.f1pmctrl\endcsname{0.359}
\expandafter\def\csname res@zs.clap_ms.f1pmen\endcsname{0.323}
\expandafter\def\csname res@zs.clap_ms.f1pmlex\endcsname{0.343}
\expandafter\def\csname res@zs.clap_ms.f1pmnonen\endcsname{0.372}
\expandafter\def\csname res@zs.clap_ms.gap\endcsname{+0.185}
\expandafter\def\csname res@zs.clap_ms.gapci\endcsname{[+0.172, +0.197]}
\expandafter\def\csname res@zs.clap_ms.gapctrl\endcsname{+0.170}
\expandafter\def\csname res@zs.clap_ms.gapctrlci\endcsname{[+0.156, +0.184]}
\expandafter\def\csname res@zs.clap_ms.gapen\endcsname{+0.134}
\expandafter\def\csname res@zs.clap_ms.gapenci\endcsname{[+0.114, +0.156]}
\expandafter\def\csname res@zs.clap_ms.gaplex\endcsname{+0.245}
\expandafter\def\csname res@zs.clap_ms.gaplexci\endcsname{[+0.222, +0.267]}
\expandafter\def\csname res@zs.clap_ms.gapnonen\endcsname{+0.210}
\expandafter\def\csname res@zs.clap_ms.gapnonenci\endcsname{[+0.194, +0.224]}
\expandafter\def\csname res@zs.clap_ms.knownauc\endcsname{0.696}
\expandafter\def\csname res@zs.clap_ms.novel\endcsname{0.122}
\expandafter\def\csname res@zs.clap_ms.novelauc\endcsname{0.664}
\expandafter\def\csname res@zs.clap_ms_desc.calm\endcsname{0.429}
\expandafter\def\csname res@zs.clap_ms_desc.f1\endcsname{0.157}
\expandafter\def\csname res@zs.clap_ms_desc.f1ci\endcsname{[0.147, 0.164]}
\expandafter\def\csname res@zs.clap_ms_desc.f1ctrl\endcsname{0.147}
\expandafter\def\csname res@zs.clap_ms_desc.f1ctrlci\endcsname{[0.136, 0.155]}
\expandafter\def\csname res@zs.clap_ms_desc.f1emobox\endcsname{0.162}
\expandafter\def\csname res@zs.clap_ms_desc.f1emoboxci\endcsname{[0.151, 0.170]}
\expandafter\def\csname res@zs.clap_ms_desc.f1en\endcsname{0.134}
\expandafter\def\csname res@zs.clap_ms_desc.f1enci\endcsname{[0.125, 0.142]}
\expandafter\def\csname res@zs.clap_ms_desc.f1lex\endcsname{0.198}
\expandafter\def\csname res@zs.clap_ms_desc.f1lexci\endcsname{[0.183, 0.211]}
\expandafter\def\csname res@zs.clap_ms_desc.f1nonen\endcsname{0.169}
\expandafter\def\csname res@zs.clap_ms_desc.f1nonenci\endcsname{[0.155, 0.177]}
\expandafter\def\csname res@zs.clap_ms_desc.f1other\endcsname{0.134}
\expandafter\def\csname res@zs.clap_ms_desc.f1otherci\endcsname{[0.120, 0.148]}
\expandafter\def\csname res@zs.clap_ms_desc.f1pm\endcsname{0.293}
\expandafter\def\csname res@zs.clap_ms_desc.f1pmctrl\endcsname{0.293}
\expandafter\def\csname res@zs.clap_ms_desc.f1pmen\endcsname{0.273}
\expandafter\def\csname res@zs.clap_ms_desc.f1pmlex\endcsname{0.295}
\expandafter\def\csname res@zs.clap_ms_desc.f1pmnonen\endcsname{0.303}
\expandafter\def\csname res@zs.clap_ms_desc.gap\endcsname{+0.276}
\expandafter\def\csname res@zs.clap_ms_desc.gapci\endcsname{[+0.261, +0.287]}
\expandafter\def\csname res@zs.clap_ms_desc.gapctrl\endcsname{+0.272}
\expandafter\def\csname res@zs.clap_ms_desc.gapctrlci\endcsname{[+0.254, +0.284]}
\expandafter\def\csname res@zs.clap_ms_desc.gapen\endcsname{+0.205}
\expandafter\def\csname res@zs.clap_ms_desc.gapenci\endcsname{[+0.187, +0.218]}
\expandafter\def\csname res@zs.clap_ms_desc.gaplex\endcsname{+0.296}
\expandafter\def\csname res@zs.clap_ms_desc.gaplexci\endcsname{[+0.273, +0.317]}
\expandafter\def\csname res@zs.clap_ms_desc.gapnonen\endcsname{+0.312}
\expandafter\def\csname res@zs.clap_ms_desc.gapnonenci\endcsname{[+0.292, +0.328]}
\expandafter\def\csname res@zs.clap_ms_desc.knownauc\endcsname{0.646}
\expandafter\def\csname res@zs.clap_ms_desc.novel\endcsname{0.153}
\expandafter\def\csname res@zs.clap_ms_desc.novelauc\endcsname{0.618}
\expandafter\def\csname res@zs.clap_para.calm\endcsname{0.152}
\expandafter\def\csname res@zs.clap_para.f1\endcsname{0.312}
\expandafter\def\csname res@zs.clap_para.f1ci\endcsname{[0.299, 0.320]}
\expandafter\def\csname res@zs.clap_para.f1ctrl\endcsname{0.314}
\expandafter\def\csname res@zs.clap_para.f1ctrlci\endcsname{[0.299, 0.324]}
\expandafter\def\csname res@zs.clap_para.f1emobox\endcsname{0.305}
\expandafter\def\csname res@zs.clap_para.f1emoboxci\endcsname{[0.289, 0.315]}
\expandafter\def\csname res@zs.clap_para.f1en\endcsname{0.253}
\expandafter\def\csname res@zs.clap_para.f1enci\endcsname{[0.237, 0.263]}
\expandafter\def\csname res@zs.clap_para.f1lex\endcsname{0.301}
\expandafter\def\csname res@zs.clap_para.f1lexci\endcsname{[0.283, 0.316]}
\expandafter\def\csname res@zs.clap_para.f1nonen\endcsname{0.341}
\expandafter\def\csname res@zs.clap_para.f1nonenci\endcsname{[0.324, 0.353]}
\expandafter\def\csname res@zs.clap_para.f1other\endcsname{0.343}
\expandafter\def\csname res@zs.clap_para.f1otherci\endcsname{[0.328, 0.357]}
\expandafter\def\csname res@zs.clap_para.f1pm\endcsname{0.326}
\expandafter\def\csname res@zs.clap_para.f1pmctrl\endcsname{0.327}
\expandafter\def\csname res@zs.clap_para.f1pmen\endcsname{0.269}
\expandafter\def\csname res@zs.clap_para.f1pmlex\endcsname{0.326}
\expandafter\def\csname res@zs.clap_para.f1pmnonen\endcsname{0.355}
\expandafter\def\csname res@zs.clap_para.gap\endcsname{+0.121}
\expandafter\def\csname res@zs.clap_para.gapci\endcsname{[+0.107, +0.133]}
\expandafter\def\csname res@zs.clap_para.gapctrl\endcsname{+0.105}
\expandafter\def\csname res@zs.clap_para.gapctrlci\endcsname{[+0.089, +0.119]}
\expandafter\def\csname res@zs.clap_para.gapen\endcsname{+0.085}
\expandafter\def\csname res@zs.clap_para.gapenci\endcsname{[+0.071, +0.104]}
\expandafter\def\csname res@zs.clap_para.gaplex\endcsname{+0.193}
\expandafter\def\csname res@zs.clap_para.gaplexci\endcsname{[+0.169, +0.217]}
\expandafter\def\csname res@zs.clap_para.gapnonen\endcsname{+0.139}
\expandafter\def\csname res@zs.clap_para.gapnonenci\endcsname{[+0.120, +0.154]}
\expandafter\def\csname res@zs.clap_para.knownauc\endcsname{0.699}
\expandafter\def\csname res@zs.clap_para.novel\endcsname{0.070}
\expandafter\def\csname res@zs.clap_para.novelauc\endcsname{0.617}
\expandafter\def\csname res@zs.clap_para_desc.calm\endcsname{0.214}
\expandafter\def\csname res@zs.clap_para_desc.f1\endcsname{0.267}
\expandafter\def\csname res@zs.clap_para_desc.f1ci\endcsname{[0.253, 0.273]}
\expandafter\def\csname res@zs.clap_para_desc.f1ctrl\endcsname{0.266}
\expandafter\def\csname res@zs.clap_para_desc.f1ctrlci\endcsname{[0.251, 0.274]}
\expandafter\def\csname res@zs.clap_para_desc.f1emobox\endcsname{0.255}
\expandafter\def\csname res@zs.clap_para_desc.f1emoboxci\endcsname{[0.239, 0.263]}
\expandafter\def\csname res@zs.clap_para_desc.f1en\endcsname{0.220}
\expandafter\def\csname res@zs.clap_para_desc.f1enci\endcsname{[0.200, 0.229]}
\expandafter\def\csname res@zs.clap_para_desc.f1lex\endcsname{0.267}
\expandafter\def\csname res@zs.clap_para_desc.f1lexci\endcsname{[0.251, 0.281]}
\expandafter\def\csname res@zs.clap_para_desc.f1nonen\endcsname{0.290}
\expandafter\def\csname res@zs.clap_para_desc.f1nonenci\endcsname{[0.273, 0.300]}
\expandafter\def\csname res@zs.clap_para_desc.f1other\endcsname{0.316}
\expandafter\def\csname res@zs.clap_para_desc.f1otherci\endcsname{[0.302, 0.329]}
\expandafter\def\csname res@zs.clap_para_desc.f1pm\endcsname{0.287}
\expandafter\def\csname res@zs.clap_para_desc.f1pmctrl\endcsname{0.290}
\expandafter\def\csname res@zs.clap_para_desc.f1pmen\endcsname{0.250}
\expandafter\def\csname res@zs.clap_para_desc.f1pmlex\endcsname{0.276}
\expandafter\def\csname res@zs.clap_para_desc.f1pmnonen\endcsname{0.306}
\expandafter\def\csname res@zs.clap_para_desc.gap\endcsname{+0.167}
\expandafter\def\csname res@zs.clap_para_desc.gapci\endcsname{[+0.152, +0.181]}
\expandafter\def\csname res@zs.clap_para_desc.gapctrl\endcsname{+0.153}
\expandafter\def\csname res@zs.clap_para_desc.gapctrlci\endcsname{[+0.136, +0.168]}
\expandafter\def\csname res@zs.clap_para_desc.gapen\endcsname{+0.118}
\expandafter\def\csname res@zs.clap_para_desc.gapenci\endcsname{[+0.101, +0.142]}
\expandafter\def\csname res@zs.clap_para_desc.gaplex\endcsname{+0.226}
\expandafter\def\csname res@zs.clap_para_desc.gaplexci\endcsname{[+0.204, +0.250]}
\expandafter\def\csname res@zs.clap_para_desc.gapnonen\endcsname{+0.191}
\expandafter\def\csname res@zs.clap_para_desc.gapnonenci\endcsname{[+0.171, +0.208]}
\expandafter\def\csname res@zs.clap_para_desc.knownauc\endcsname{0.669}
\expandafter\def\csname res@zs.clap_para_desc.novel\endcsname{0.113}
\expandafter\def\csname res@zs.clap_para_desc.novelauc\endcsname{0.574}
\expandafter\def\csname res@zs.clips\endcsname{20,585}
\expandafter\def\csname res@zs.corpora\endcsname{21}
\expandafter\def\csname res@zs.ctrl.n\endcsname{17}
\expandafter\def\csname res@zs.e2v.asomclean\endcsname{0.466}
\expandafter\def\csname res@zs.e2v.calm\endcsname{0.000}
\expandafter\def\csname res@zs.e2v.cleancorpora\endcsname{4}
\expandafter\def\csname res@zs.e2v.f1\endcsname{0.667}
\expandafter\def\csname res@zs.e2v.f1ci\endcsname{[0.652, 0.677]}
\expandafter\def\csname res@zs.e2v.f1clean\endcsname{0.492}
\expandafter\def\csname res@zs.e2v.f1ctrl\endcsname{0.699}
\expandafter\def\csname res@zs.e2v.f1ctrlci\endcsname{[0.682, 0.710]}
\expandafter\def\csname res@zs.e2v.f1emobox\endcsname{0.708}
\expandafter\def\csname res@zs.e2v.f1emoboxci\endcsname{[0.691, 0.719]}
\expandafter\def\csname res@zs.e2v.f1en\endcsname{0.657}
\expandafter\def\csname res@zs.e2v.f1enci\endcsname{[0.644, 0.670]}
\expandafter\def\csname res@zs.e2v.f1lex\endcsname{0.533}
\expandafter\def\csname res@zs.e2v.f1lexci\endcsname{[0.511, 0.553]}
\expandafter\def\csname res@zs.e2v.f1nonen\endcsname{0.672}
\expandafter\def\csname res@zs.e2v.f1nonenci\endcsname{[0.652, 0.685]}
\expandafter\def\csname res@zs.e2v.f1other\endcsname{0.492}
\expandafter\def\csname res@zs.e2v.f1otherci\endcsname{[0.472, 0.512]}
\expandafter\def\csname res@zs.e2v.f1pm\endcsname{0.685}
\expandafter\def\csname res@zs.e2v.f1pmctrl\endcsname{0.719}
\expandafter\def\csname res@zs.e2v.f1pmen\endcsname{0.680}
\expandafter\def\csname res@zs.e2v.f1pmlex\endcsname{0.540}
\expandafter\def\csname res@zs.e2v.f1pmnonen\endcsname{0.688}
\expandafter\def\csname res@zs.e2v.gap\endcsname{-0.234}
\expandafter\def\csname res@zs.e2v.gapci\endcsname{[-0.249, -0.221]}
\expandafter\def\csname res@zs.e2v.gapctrl\endcsname{-0.279}
\expandafter\def\csname res@zs.e2v.gapctrlci\endcsname{[-0.297, -0.266]}
\expandafter\def\csname res@zs.e2v.gapen\endcsname{-0.319}
\expandafter\def\csname res@zs.e2v.gapenci\endcsname{[-0.341, -0.301]}
\expandafter\def\csname res@zs.e2v.gaplex\endcsname{-0.039}
\expandafter\def\csname res@zs.e2v.gaplexci\endcsname{[-0.064, -0.015]}
\expandafter\def\csname res@zs.e2v.gapnonen\endcsname{-0.191}
\expandafter\def\csname res@zs.e2v.gapnonenci\endcsname{[-0.211, -0.175]}
\expandafter\def\csname res@zs.e2v.knownauc\endcsname{0.896}
\expandafter\def\csname res@zs.e2v.novel\endcsname{0.000}
\expandafter\def\csname res@zs.eff_t14.calm\endcsname{0.000}
\expandafter\def\csname res@zs.eff_t14.f1\endcsname{0.426}
\expandafter\def\csname res@zs.eff_t14.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.eff_t14.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.eff_t14.novel\endcsname{0.006}
\expandafter\def\csname res@zs.eff_t14.novelauc\endcsname{0.724}
\expandafter\def\csname res@zs.eff_t7.calm\endcsname{0.000}
\expandafter\def\csname res@zs.eff_t7.f1\endcsname{0.418}
\expandafter\def\csname res@zs.eff_t7.f1pm\endcsname{0.549}
\expandafter\def\csname res@zs.eff_t7.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.eff_t7.novel\endcsname{0.003}
\expandafter\def\csname res@zs.eff_t7.novelauc\endcsname{0.681}
\expandafter\def\csname res@zs.eff_w24.calm\endcsname{0.355}
\expandafter\def\csname res@zs.eff_w24.f1\endcsname{0.421}
\expandafter\def\csname res@zs.eff_w24.f1pm\endcsname{0.548}
\expandafter\def\csname res@zs.eff_w24.knownauc\endcsname{0.837}
\expandafter\def\csname res@zs.eff_w24.novel\endcsname{0.071}
\expandafter\def\csname res@zs.eff_w24.novelauc\endcsname{0.760}
\expandafter\def\csname res@zs.indomain.af3.f1\endcsname{0.195}
\expandafter\def\csname res@zs.indomain.af3.f1ci\endcsname{[0.182, 0.204]}
\expandafter\def\csname res@zs.indomain.af3.f1emobox\endcsname{0.211}
\expandafter\def\csname res@zs.indomain.af3.f1other\endcsname{0.137}
\expandafter\def\csname res@zs.indomain.af3.f1si\endcsname{0.202}
\expandafter\def\csname res@zs.indomain.af3.share\endcsname{3}
\expandafter\def\csname res@zs.indomain.af3.shareemobox\endcsname{6}
\expandafter\def\csname res@zs.indomain.af3.shareother\endcsname{-7}
\expandafter\def\csname res@zs.indomain.af3.sharesi\endcsname{3}
\expandafter\def\csname res@zs.indomain.af3_cc.f1\endcsname{0.251}
\expandafter\def\csname res@zs.indomain.af3_cc.f1ci\endcsname{[0.234, 0.262]}
\expandafter\def\csname res@zs.indomain.af3_cc.f1emobox\endcsname{0.270}
\expandafter\def\csname res@zs.indomain.af3_cc.f1other\endcsname{0.177}
\expandafter\def\csname res@zs.indomain.af3_cc.f1si\endcsname{0.264}
\expandafter\def\csname res@zs.indomain.af3_cc.share\endcsname{13}
\expandafter\def\csname res@zs.indomain.af3_cc.shareemobox\endcsname{18}
\expandafter\def\csname res@zs.indomain.af3_cc.shareother\endcsname{0}
\expandafter\def\csname res@zs.indomain.af3_cc.sharesi\endcsname{15}
\expandafter\def\csname res@zs.indomain.asom.f1\endcsname{0.432}
\expandafter\def\csname res@zs.indomain.asom.f1ci\endcsname{[0.401, 0.448]}
\expandafter\def\csname res@zs.indomain.asom.f1emobox\endcsname{0.422}
\expandafter\def\csname res@zs.indomain.asom.f1other\endcsname{0.472}
\expandafter\def\csname res@zs.indomain.asom.f1si\endcsname{0.446}
\expandafter\def\csname res@zs.indomain.asom.share\endcsname{48}
\expandafter\def\csname res@zs.indomain.asom.shareemobox\endcsname{47}
\expandafter\def\csname res@zs.indomain.asom.shareother\endcsname{51}
\expandafter\def\csname res@zs.indomain.asom.sharesi\endcsname{51}
\expandafter\def\csname res@zs.indomain.asom_u.f1\endcsname{0.476}
\expandafter\def\csname res@zs.indomain.asom_u.f1ci\endcsname{[0.447, 0.488]}
\expandafter\def\csname res@zs.indomain.asom_u.f1emobox\endcsname{0.469}
\expandafter\def\csname res@zs.indomain.asom_u.f1other\endcsname{0.502}
\expandafter\def\csname res@zs.indomain.asom_u.f1si\endcsname{0.492}
\expandafter\def\csname res@zs.indomain.asom_u.share\endcsname{56}
\expandafter\def\csname res@zs.indomain.asom_u.shareemobox\endcsname{57}
\expandafter\def\csname res@zs.indomain.asom_u.shareother\endcsname{56}
\expandafter\def\csname res@zs.indomain.asom_u.sharesi\endcsname{60}
\expandafter\def\csname res@zs.indomain.bestalm.f1\endcsname{0.328}
\expandafter\def\csname res@zs.indomain.bestalm.name\endcsname{Qwen2.5-Omni-7B}
\expandafter\def\csname res@zs.indomain.bestalm.share\endcsname{28}
\expandafter\def\csname res@zs.indomain.bestalmcc.f1\endcsname{0.354}
\expandafter\def\csname res@zs.indomain.bestalmcc.name\endcsname{Qwen2.5-Omni-7B + CC}
\expandafter\def\csname res@zs.indomain.bestalmcc.share\endcsname{33}
\expandafter\def\csname res@zs.indomain.chance\endcsname{0.180}
\expandafter\def\csname res@zs.indomain.clap_laion.f1\endcsname{0.103}
\expandafter\def\csname res@zs.indomain.clap_laion.f1ci\endcsname{[0.094, 0.112]}
\expandafter\def\csname res@zs.indomain.clap_laion.f1emobox\endcsname{0.094}
\expandafter\def\csname res@zs.indomain.clap_laion.f1other\endcsname{0.140}
\expandafter\def\csname res@zs.indomain.clap_laion.f1si\endcsname{0.101}
\expandafter\def\csname res@zs.indomain.clap_laion.share\endcsname{-15}
\expandafter\def\csname res@zs.indomain.clap_laion.shareemobox\endcsname{-17}
\expandafter\def\csname res@zs.indomain.clap_laion.shareother\endcsname{-6}
\expandafter\def\csname res@zs.indomain.clap_laion.sharesi\endcsname{-16}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.f1\endcsname{0.089}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.f1ci\endcsname{[0.082, 0.096]}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.f1emobox\endcsname{0.090}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.f1other\endcsname{0.085}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.f1si\endcsname{0.087}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.share\endcsname{-17}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.shareemobox\endcsname{-18}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.shareother\endcsname{-16}
\expandafter\def\csname res@zs.indomain.clap_laion_desc.sharesi\endcsname{-19}
\expandafter\def\csname res@zs.indomain.clap_ms.f1\endcsname{0.240}
\expandafter\def\csname res@zs.indomain.clap_ms.f1ci\endcsname{[0.218, 0.249]}
\expandafter\def\csname res@zs.indomain.clap_ms.f1emobox\endcsname{0.239}
\expandafter\def\csname res@zs.indomain.clap_ms.f1other\endcsname{0.244}
\expandafter\def\csname res@zs.indomain.clap_ms.f1si\endcsname{0.242}
\expandafter\def\csname res@zs.indomain.clap_ms.share\endcsname{11}
\expandafter\def\csname res@zs.indomain.clap_ms.shareemobox\endcsname{11}
\expandafter\def\csname res@zs.indomain.clap_ms.shareother\endcsname{12}
\expandafter\def\csname res@zs.indomain.clap_ms.sharesi\endcsname{11}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.f1\endcsname{0.157}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.f1ci\endcsname{[0.142, 0.164]}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.f1emobox\endcsname{0.158}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.f1other\endcsname{0.151}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.f1si\endcsname{0.162}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.share\endcsname{-4}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.shareemobox\endcsname{-5}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.shareother\endcsname{-4}
\expandafter\def\csname res@zs.indomain.clap_ms_desc.sharesi\endcsname{-4}
\expandafter\def\csname res@zs.indomain.clap_para.f1\endcsname{0.312}
\expandafter\def\csname res@zs.indomain.clap_para.f1ci\endcsname{[0.290, 0.326]}
\expandafter\def\csname res@zs.indomain.clap_para.f1emobox\endcsname{0.303}
\expandafter\def\csname res@zs.indomain.clap_para.f1other\endcsname{0.346}
\expandafter\def\csname res@zs.indomain.clap_para.f1si\endcsname{0.320}
\expandafter\def\csname res@zs.indomain.clap_para.share\endcsname{25}
\expandafter\def\csname res@zs.indomain.clap_para.shareemobox\endcsname{24}
\expandafter\def\csname res@zs.indomain.clap_para.shareother\endcsname{29}
\expandafter\def\csname res@zs.indomain.clap_para.sharesi\endcsname{26}
\expandafter\def\csname res@zs.indomain.clap_para_desc.f1\endcsname{0.265}
\expandafter\def\csname res@zs.indomain.clap_para_desc.f1ci\endcsname{[0.246, 0.275]}
\expandafter\def\csname res@zs.indomain.clap_para_desc.f1emobox\endcsname{0.246}
\expandafter\def\csname res@zs.indomain.clap_para_desc.f1other\endcsname{0.336}
\expandafter\def\csname res@zs.indomain.clap_para_desc.f1si\endcsname{0.263}
\expandafter\def\csname res@zs.indomain.clap_para_desc.share\endcsname{16}
\expandafter\def\csname res@zs.indomain.clap_para_desc.shareemobox\endcsname{13}
\expandafter\def\csname res@zs.indomain.clap_para_desc.shareother\endcsname{28}
\expandafter\def\csname res@zs.indomain.clap_para_desc.sharesi\endcsname{15}
\expandafter\def\csname res@zs.indomain.clips\endcsname{3,209}
\expandafter\def\csname res@zs.indomain.corpora\endcsname{19}
\expandafter\def\csname res@zs.indomain.corporaemobox\endcsname{15}
\expandafter\def\csname res@zs.indomain.corporaother\endcsname{4}
\expandafter\def\csname res@zs.indomain.corporasi\endcsname{14}
\expandafter\def\csname res@zs.indomain.deepser.f1\endcsname{0.703}
\expandafter\def\csname res@zs.indomain.deepser.f1ci\endcsname{[0.680, 0.717]}
\expandafter\def\csname res@zs.indomain.deepser.f1emobox\endcsname{0.688}
\expandafter\def\csname res@zs.indomain.deepser.f1other\endcsname{0.758}
\expandafter\def\csname res@zs.indomain.deepser.f1si\endcsname{0.700}
\expandafter\def\csname res@zs.indomain.deepser.share\endcsname{100}
\expandafter\def\csname res@zs.indomain.deepser.shareemobox\endcsname{100}
\expandafter\def\csname res@zs.indomain.deepser.shareother\endcsname{100}
\expandafter\def\csname res@zs.indomain.deepser.sharesi\endcsname{100}
\expandafter\def\csname res@zs.indomain.e2v.f1\endcsname{0.646}
\expandafter\def\csname res@zs.indomain.e2v.f1ci\endcsname{[0.611, 0.658]}
\expandafter\def\csname res@zs.indomain.e2v.f1emobox\endcsname{0.705}
\expandafter\def\csname res@zs.indomain.e2v.f1other\endcsname{0.425}
\expandafter\def\csname res@zs.indomain.e2v.f1si\endcsname{0.729}
\expandafter\def\csname res@zs.indomain.e2v.share\endcsname{89}
\expandafter\def\csname res@zs.indomain.e2v.shareemobox\endcsname{103}
\expandafter\def\csname res@zs.indomain.e2v.shareother\endcsname{43}
\expandafter\def\csname res@zs.indomain.e2v.sharesi\endcsname{106}
\expandafter\def\csname res@zs.indomain.omni3b.f1\endcsname{0.218}
\expandafter\def\csname res@zs.indomain.omni3b.f1ci\endcsname{[0.200, 0.230]}
\expandafter\def\csname res@zs.indomain.omni3b.f1emobox\endcsname{0.233}
\expandafter\def\csname res@zs.indomain.omni3b.f1other\endcsname{0.160}
\expandafter\def\csname res@zs.indomain.omni3b.f1si\endcsname{0.213}
\expandafter\def\csname res@zs.indomain.omni3b.share\endcsname{7}
\expandafter\def\csname res@zs.indomain.omni3b.shareemobox\endcsname{10}
\expandafter\def\csname res@zs.indomain.omni3b.shareother\endcsname{-3}
\expandafter\def\csname res@zs.indomain.omni3b.sharesi\endcsname{5}
\expandafter\def\csname res@zs.indomain.omni3b_cc.f1\endcsname{0.285}
\expandafter\def\csname res@zs.indomain.omni3b_cc.f1ci\endcsname{[0.267, 0.297]}
\expandafter\def\csname res@zs.indomain.omni3b_cc.f1emobox\endcsname{0.306}
\expandafter\def\csname res@zs.indomain.omni3b_cc.f1other\endcsname{0.207}
\expandafter\def\csname res@zs.indomain.omni3b_cc.f1si\endcsname{0.284}
\expandafter\def\csname res@zs.indomain.omni3b_cc.share\endcsname{20}
\expandafter\def\csname res@zs.indomain.omni3b_cc.shareemobox\endcsname{25}
\expandafter\def\csname res@zs.indomain.omni3b_cc.shareother\endcsname{5}
\expandafter\def\csname res@zs.indomain.omni3b_cc.sharesi\endcsname{19}
\expandafter\def\csname res@zs.indomain.omni3b_ft.f1\endcsname{0.363}
\expandafter\def\csname res@zs.indomain.omni3b_ft.f1ci\endcsname{[0.340, 0.378]}
\expandafter\def\csname res@zs.indomain.omni3b_ft.f1emobox\endcsname{0.381}
\expandafter\def\csname res@zs.indomain.omni3b_ft.f1other\endcsname{0.296}
\expandafter\def\csname res@zs.indomain.omni3b_ft.f1si\endcsname{0.352}
\expandafter\def\csname res@zs.indomain.omni3b_ft.share\endcsname{35}
\expandafter\def\csname res@zs.indomain.omni3b_ft.shareemobox\endcsname{39}
\expandafter\def\csname res@zs.indomain.omni3b_ft.shareother\endcsname{21}
\expandafter\def\csname res@zs.indomain.omni3b_ft.sharesi\endcsname{33}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.f1\endcsname{0.400}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.f1ci\endcsname{[0.378, 0.414]}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.f1emobox\endcsname{0.416}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.f1other\endcsname{0.340}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.f1si\endcsname{0.391}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.share\endcsname{42}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.shareemobox\endcsname{46}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.shareother\endcsname{28}
\expandafter\def\csname res@zs.indomain.omni3b_ftfull.sharesi\endcsname{40}
\expandafter\def\csname res@zs.indomain.omni7b.f1\endcsname{0.328}
\expandafter\def\csname res@zs.indomain.omni7b.f1ci\endcsname{[0.307, 0.341]}
\expandafter\def\csname res@zs.indomain.omni7b.f1emobox\endcsname{0.353}
\expandafter\def\csname res@zs.indomain.omni7b.f1other\endcsname{0.235}
\expandafter\def\csname res@zs.indomain.omni7b.f1si\endcsname{0.307}
\expandafter\def\csname res@zs.indomain.omni7b.share\endcsname{28}
\expandafter\def\csname res@zs.indomain.omni7b.shareemobox\endcsname{34}
\expandafter\def\csname res@zs.indomain.omni7b.shareother\endcsname{10}
\expandafter\def\csname res@zs.indomain.omni7b.sharesi\endcsname{24}
\expandafter\def\csname res@zs.indomain.omni7b_cc.f1\endcsname{0.354}
\expandafter\def\csname res@zs.indomain.omni7b_cc.f1ci\endcsname{[0.333, 0.365]}
\expandafter\def\csname res@zs.indomain.omni7b_cc.f1emobox\endcsname{0.382}
\expandafter\def\csname res@zs.indomain.omni7b_cc.f1other\endcsname{0.251}
\expandafter\def\csname res@zs.indomain.omni7b_cc.f1si\endcsname{0.337}
\expandafter\def\csname res@zs.indomain.omni7b_cc.share\endcsname{33}
\expandafter\def\csname res@zs.indomain.omni7b_cc.shareemobox\endcsname{39}
\expandafter\def\csname res@zs.indomain.omni7b_cc.shareother\endcsname{13}
\expandafter\def\csname res@zs.indomain.omni7b_cc.sharesi\endcsname{30}
\expandafter\def\csname res@zs.indomain.phi4mm.f1\endcsname{0.223}
\expandafter\def\csname res@zs.indomain.phi4mm.f1ci\endcsname{[0.208, 0.232]}
\expandafter\def\csname res@zs.indomain.phi4mm.f1emobox\endcsname{0.228}
\expandafter\def\csname res@zs.indomain.phi4mm.f1other\endcsname{0.204}
\expandafter\def\csname res@zs.indomain.phi4mm.f1si\endcsname{0.225}
\expandafter\def\csname res@zs.indomain.phi4mm.share\endcsname{8}
\expandafter\def\csname res@zs.indomain.phi4mm.shareemobox\endcsname{9}
\expandafter\def\csname res@zs.indomain.phi4mm.shareother\endcsname{5}
\expandafter\def\csname res@zs.indomain.phi4mm.sharesi\endcsname{8}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.f1\endcsname{0.214}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.f1ci\endcsname{[0.201, 0.223]}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.f1emobox\endcsname{0.216}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.f1other\endcsname{0.205}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.f1si\endcsname{0.213}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.share\endcsname{6}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.shareemobox\endcsname{7}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.shareother\endcsname{5}
\expandafter\def\csname res@zs.indomain.phi4mm_cc.sharesi\endcsname{6}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.f1\endcsname{0.292}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.f1ci\endcsname{[0.277, 0.301]}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.f1emobox\endcsname{0.322}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.f1other\endcsname{0.182}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.f1si\endcsname{0.294}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.share\endcsname{21}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.shareemobox\endcsname{28}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.shareother\endcsname{1}
\expandafter\def\csname res@zs.indomain.qwen2audio7b.sharesi\endcsname{21}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.f1\endcsname{0.313}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.f1ci\endcsname{[0.295, 0.323]}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.f1emobox\endcsname{0.335}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.f1other\endcsname{0.228}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.f1si\endcsname{0.296}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.share\endcsname{25}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.shareemobox\endcsname{30}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.shareother\endcsname{9}
\expandafter\def\csname res@zs.indomain.qwen2audio7b_cc.sharesi\endcsname{22}
\expandafter\def\csname res@zs.indomain.voxtral3b.f1\endcsname{0.222}
\expandafter\def\csname res@zs.indomain.voxtral3b.f1ci\endcsname{[0.206, 0.232]}
\expandafter\def\csname res@zs.indomain.voxtral3b.f1emobox\endcsname{0.224}
\expandafter\def\csname res@zs.indomain.voxtral3b.f1other\endcsname{0.215}
\expandafter\def\csname res@zs.indomain.voxtral3b.f1si\endcsname{0.212}
\expandafter\def\csname res@zs.indomain.voxtral3b.share\endcsname{8}
\expandafter\def\csname res@zs.indomain.voxtral3b.shareemobox\endcsname{8}
\expandafter\def\csname res@zs.indomain.voxtral3b.shareother\endcsname{7}
\expandafter\def\csname res@zs.indomain.voxtral3b.sharesi\endcsname{5}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.f1\endcsname{0.240}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.f1ci\endcsname{[0.223, 0.251]}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.f1emobox\endcsname{0.240}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.f1other\endcsname{0.243}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.f1si\endcsname{0.230}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.share\endcsname{11}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.shareemobox\endcsname{11}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.shareother\endcsname{12}
\expandafter\def\csname res@zs.indomain.voxtral3b_cc.sharesi\endcsname{9}
\expandafter\def\csname res@zs.indomain.whisper_mlp.f1\endcsname{0.404}
\expandafter\def\csname res@zs.indomain.whisper_mlp.f1ci\endcsname{[0.374, 0.423]}
\expandafter\def\csname res@zs.indomain.whisper_mlp.f1emobox\endcsname{0.391}
\expandafter\def\csname res@zs.indomain.whisper_mlp.f1other\endcsname{0.454}
\expandafter\def\csname res@zs.indomain.whisper_mlp.f1si\endcsname{0.421}
\expandafter\def\csname res@zs.indomain.whisper_mlp.share\endcsname{43}
\expandafter\def\csname res@zs.indomain.whisper_mlp.shareemobox\endcsname{41}
\expandafter\def\csname res@zs.indomain.whisper_mlp.shareother\endcsname{48}
\expandafter\def\csname res@zs.indomain.whisper_mlp.sharesi\endcsname{46}
\expandafter\def\csname res@zs.langs\endcsname{13}
\expandafter\def\csname res@zs.lex.n\endcsname{4}
\expandafter\def\csname res@zs.lex.names\endcsname{IEMOCAP, MEACorpus, MELD, Oréau}
\expandafter\def\csname res@zs.omni3b.calm\endcsname{0.109}
\expandafter\def\csname res@zs.omni3b.f1\endcsname{0.205}
\expandafter\def\csname res@zs.omni3b.f1ci\endcsname{[0.196, 0.212]}
\expandafter\def\csname res@zs.omni3b.f1ctrl\endcsname{0.156}
\expandafter\def\csname res@zs.omni3b.f1ctrlci\endcsname{[0.146, 0.163]}
\expandafter\def\csname res@zs.omni3b.f1emobox\endcsname{0.215}
\expandafter\def\csname res@zs.omni3b.f1emoboxci\endcsname{[0.204, 0.224]}
\expandafter\def\csname res@zs.omni3b.f1en\endcsname{0.209}
\expandafter\def\csname res@zs.omni3b.f1enci\endcsname{[0.193, 0.221]}
\expandafter\def\csname res@zs.omni3b.f1lex\endcsname{0.415}
\expandafter\def\csname res@zs.omni3b.f1lexci\endcsname{[0.395, 0.433]}
\expandafter\def\csname res@zs.omni3b.f1nonen\endcsname{0.204}
\expandafter\def\csname res@zs.omni3b.f1nonenci\endcsname{[0.193, 0.212]}
\expandafter\def\csname res@zs.omni3b.f1other\endcsname{0.162}
\expandafter\def\csname res@zs.omni3b.f1otherci\endcsname{[0.153, 0.171]}
\expandafter\def\csname res@zs.omni3b.f1pm\endcsname{0.312}
\expandafter\def\csname res@zs.omni3b.f1pmctrl\endcsname{0.275}
\expandafter\def\csname res@zs.omni3b.f1pmen\endcsname{0.297}
\expandafter\def\csname res@zs.omni3b.f1pmlex\endcsname{0.466}
\expandafter\def\csname res@zs.omni3b.f1pmnonen\endcsname{0.319}
\expandafter\def\csname res@zs.omni3b.gap\endcsname{+0.228}
\expandafter\def\csname res@zs.omni3b.gapci\endcsname{[+0.212, +0.240]}
\expandafter\def\csname res@zs.omni3b.gapctrl\endcsname{+0.263}
\expandafter\def\csname res@zs.omni3b.gapctrlci\endcsname{[+0.243, +0.277]}
\expandafter\def\csname res@zs.omni3b.gapen\endcsname{+0.130}
\expandafter\def\csname res@zs.omni3b.gapenci\endcsname{[+0.106, +0.152]}
\expandafter\def\csname res@zs.omni3b.gaplex\endcsname{+0.079}
\expandafter\def\csname res@zs.omni3b.gaplexci\endcsname{[+0.058, +0.098]}
\expandafter\def\csname res@zs.omni3b.gapnonen\endcsname{+0.277}
\expandafter\def\csname res@zs.omni3b.gapnonenci\endcsname{[+0.256, +0.292]}
\expandafter\def\csname res@zs.omni3b.knownauc\endcsname{0.649}
\expandafter\def\csname res@zs.omni3b.novel\endcsname{0.126}
\expandafter\def\csname res@zs.omni3b.novelauc\endcsname{0.580}
\expandafter\def\csname res@zs.omni3b_cc.calm\endcsname{0.037}
\expandafter\def\csname res@zs.omni3b_cc.f1\endcsname{0.270}
\expandafter\def\csname res@zs.omni3b_cc.f1ci\endcsname{[0.258, 0.278]}
\expandafter\def\csname res@zs.omni3b_cc.f1ctrl\endcsname{0.220}
\expandafter\def\csname res@zs.omni3b_cc.f1ctrlci\endcsname{[0.207, 0.230]}
\expandafter\def\csname res@zs.omni3b_cc.f1emobox\endcsname{0.283}
\expandafter\def\csname res@zs.omni3b_cc.f1emoboxci\endcsname{[0.269, 0.293]}
\expandafter\def\csname res@zs.omni3b_cc.f1en\endcsname{0.264}
\expandafter\def\csname res@zs.omni3b_cc.f1enci\endcsname{[0.244, 0.279]}
\expandafter\def\csname res@zs.omni3b_cc.f1lex\endcsname{0.482}
\expandafter\def\csname res@zs.omni3b_cc.f1lexci\endcsname{[0.464, 0.498]}
\expandafter\def\csname res@zs.omni3b_cc.f1nonen\endcsname{0.273}
\expandafter\def\csname res@zs.omni3b_cc.f1nonenci\endcsname{[0.260, 0.283]}
\expandafter\def\csname res@zs.omni3b_cc.f1other\endcsname{0.214}
\expandafter\def\csname res@zs.omni3b_cc.f1otherci\endcsname{[0.203, 0.223]}
\expandafter\def\csname res@zs.omni3b_cc.f1pm\endcsname{0.329}
\expandafter\def\csname res@zs.omni3b_cc.f1pmctrl\endcsname{0.291}
\expandafter\def\csname res@zs.omni3b_cc.f1pmen\endcsname{0.310}
\expandafter\def\csname res@zs.omni3b_cc.f1pmlex\endcsname{0.490}
\expandafter\def\csname res@zs.omni3b_cc.f1pmnonen\endcsname{0.338}
\expandafter\def\csname res@zs.omni3b_cc.gap\endcsname{+0.163}
\expandafter\def\csname res@zs.omni3b_cc.gapci\endcsname{[+0.146, +0.177]}
\expandafter\def\csname res@zs.omni3b_cc.gapctrl\endcsname{+0.199}
\expandafter\def\csname res@zs.omni3b_cc.gapctrlci\endcsname{[+0.178, +0.215]}
\expandafter\def\csname res@zs.omni3b_cc.gapen\endcsname{+0.074}
\expandafter\def\csname res@zs.omni3b_cc.gapenci\endcsname{[+0.050, +0.099]}
\expandafter\def\csname res@zs.omni3b_cc.gaplex\endcsname{+0.012}
\expandafter\def\csname res@zs.omni3b_cc.gaplexci\endcsname{[-0.009, +0.032]}
\expandafter\def\csname res@zs.omni3b_cc.gapnonen\endcsname{+0.208}
\expandafter\def\csname res@zs.omni3b_cc.gapnonenci\endcsname{[+0.185, +0.224]}
\expandafter\def\csname res@zs.omni3b_cc.knownauc\endcsname{0.656}
\expandafter\def\csname res@zs.omni3b_cc.novel\endcsname{0.135}
\expandafter\def\csname res@zs.omni3b_cc.novelauc\endcsname{0.598}
\expandafter\def\csname res@zs.omni3b_ft.calm\endcsname{0.470}
\expandafter\def\csname res@zs.omni3b_ft.f1\endcsname{0.384}
\expandafter\def\csname res@zs.omni3b_ft.f1ci\endcsname{[0.370, 0.393]}
\expandafter\def\csname res@zs.omni3b_ft.f1ctrl\endcsname{0.351}
\expandafter\def\csname res@zs.omni3b_ft.f1ctrlci\endcsname{[0.335, 0.361]}
\expandafter\def\csname res@zs.omni3b_ft.f1emobox\endcsname{0.395}
\expandafter\def\csname res@zs.omni3b_ft.f1emoboxci\endcsname{[0.378, 0.405]}
\expandafter\def\csname res@zs.omni3b_ft.f1en\endcsname{0.380}
\expandafter\def\csname res@zs.omni3b_ft.f1enci\endcsname{[0.365, 0.394]}
\expandafter\def\csname res@zs.omni3b_ft.f1lex\endcsname{0.524}
\expandafter\def\csname res@zs.omni3b_ft.f1lexci\endcsname{[0.503, 0.542]}
\expandafter\def\csname res@zs.omni3b_ft.f1nonen\endcsname{0.386}
\expandafter\def\csname res@zs.omni3b_ft.f1nonenci\endcsname{[0.367, 0.398]}
\expandafter\def\csname res@zs.omni3b_ft.f1other\endcsname{0.336}
\expandafter\def\csname res@zs.omni3b_ft.f1otherci\endcsname{[0.320, 0.350]}
\expandafter\def\csname res@zs.omni3b_ft.f1pm\endcsname{0.502}
\expandafter\def\csname res@zs.omni3b_ft.f1pmctrl\endcsname{0.486}
\expandafter\def\csname res@zs.omni3b_ft.f1pmen\endcsname{0.482}
\expandafter\def\csname res@zs.omni3b_ft.f1pmlex\endcsname{0.571}
\expandafter\def\csname res@zs.omni3b_ft.f1pmnonen\endcsname{0.512}
\expandafter\def\csname res@zs.omni3b_ft.gap\endcsname{+0.049}
\expandafter\def\csname res@zs.omni3b_ft.gapci\endcsname{[+0.037, +0.060]}
\expandafter\def\csname res@zs.omni3b_ft.gapctrl\endcsname{+0.068}
\expandafter\def\csname res@zs.omni3b_ft.gapctrlci\endcsname{[+0.053, +0.080]}
\expandafter\def\csname res@zs.omni3b_ft.gapen\endcsname{-0.042}
\expandafter\def\csname res@zs.omni3b_ft.gapenci\endcsname{[-0.063, -0.023]}
\expandafter\def\csname res@zs.omni3b_ft.gaplex\endcsname{-0.030}
\expandafter\def\csname res@zs.omni3b_ft.gaplexci\endcsname{[-0.050, -0.009]}
\expandafter\def\csname res@zs.omni3b_ft.gapnonen\endcsname{+0.095}
\expandafter\def\csname res@zs.omni3b_ft.gapnonenci\endcsname{[+0.080, +0.108]}
\expandafter\def\csname res@zs.omni3b_ft.knownauc\endcsname{0.815}
\expandafter\def\csname res@zs.omni3b_ft.novel\endcsname{0.196}
\expandafter\def\csname res@zs.omni3b_ft.novelauc\endcsname{0.691}
\expandafter\def\csname res@zs.omni3b_ftfull.calm\endcsname{0.600}
\expandafter\def\csname res@zs.omni3b_ftfull.f1\endcsname{0.402}
\expandafter\def\csname res@zs.omni3b_ftfull.f1ci\endcsname{[0.389, 0.410]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1ctrl\endcsname{0.374}
\expandafter\def\csname res@zs.omni3b_ftfull.f1ctrlci\endcsname{[0.359, 0.384]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1emobox\endcsname{0.413}
\expandafter\def\csname res@zs.omni3b_ftfull.f1emoboxci\endcsname{[0.397, 0.423]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1en\endcsname{0.388}
\expandafter\def\csname res@zs.omni3b_ftfull.f1enci\endcsname{[0.376, 0.399]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1lex\endcsname{0.521}
\expandafter\def\csname res@zs.omni3b_ftfull.f1lexci\endcsname{[0.502, 0.537]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1nonen\endcsname{0.409}
\expandafter\def\csname res@zs.omni3b_ftfull.f1nonenci\endcsname{[0.391, 0.421]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1other\endcsname{0.356}
\expandafter\def\csname res@zs.omni3b_ftfull.f1otherci\endcsname{[0.340, 0.370]}
\expandafter\def\csname res@zs.omni3b_ftfull.f1pm\endcsname{0.504}
\expandafter\def\csname res@zs.omni3b_ftfull.f1pmctrl\endcsname{0.483}
\expandafter\def\csname res@zs.omni3b_ftfull.f1pmen\endcsname{0.483}
\expandafter\def\csname res@zs.omni3b_ftfull.f1pmlex\endcsname{0.589}
\expandafter\def\csname res@zs.omni3b_ftfull.f1pmnonen\endcsname{0.514}
\expandafter\def\csname res@zs.omni3b_ftfull.gap\endcsname{+0.031}
\expandafter\def\csname res@zs.omni3b_ftfull.gapci\endcsname{[+0.019, +0.040]}
\expandafter\def\csname res@zs.omni3b_ftfull.gapctrl\endcsname{+0.045}
\expandafter\def\csname res@zs.omni3b_ftfull.gapctrlci\endcsname{[+0.032, +0.055]}
\expandafter\def\csname res@zs.omni3b_ftfull.gapen\endcsname{-0.050}
\expandafter\def\csname res@zs.omni3b_ftfull.gapenci\endcsname{[-0.066, -0.036]}
\expandafter\def\csname res@zs.omni3b_ftfull.gaplex\endcsname{-0.027}
\expandafter\def\csname res@zs.omni3b_ftfull.gaplexci\endcsname{[-0.047, -0.006]}
\expandafter\def\csname res@zs.omni3b_ftfull.gapnonen\endcsname{+0.072}
\expandafter\def\csname res@zs.omni3b_ftfull.gapnonenci\endcsname{[+0.057, +0.084]}
\expandafter\def\csname res@zs.omni3b_ftfull.knownauc\endcsname{0.818}
\expandafter\def\csname res@zs.omni3b_ftfull.novel\endcsname{0.216}
\expandafter\def\csname res@zs.omni3b_ftfull.novelauc\endcsname{0.668}
\expandafter\def\csname res@zs.omni7b.calm\endcsname{0.000}
\expandafter\def\csname res@zs.omni7b.f1\endcsname{0.313}
\expandafter\def\csname res@zs.omni7b.f1ci\endcsname{[0.300, 0.322]}
\expandafter\def\csname res@zs.omni7b.f1ctrl\endcsname{0.257}
\expandafter\def\csname res@zs.omni7b.f1ctrlci\endcsname{[0.242, 0.268]}
\expandafter\def\csname res@zs.omni7b.f1emobox\endcsname{0.328}
\expandafter\def\csname res@zs.omni7b.f1emoboxci\endcsname{[0.313, 0.339]}
\expandafter\def\csname res@zs.omni7b.f1en\endcsname{0.315}
\expandafter\def\csname res@zs.omni7b.f1enci\endcsname{[0.292, 0.331]}
\expandafter\def\csname res@zs.omni7b.f1lex\endcsname{0.550}
\expandafter\def\csname res@zs.omni7b.f1lexci\endcsname{[0.531, 0.566]}
\expandafter\def\csname res@zs.omni7b.f1nonen\endcsname{0.312}
\expandafter\def\csname res@zs.omni7b.f1nonenci\endcsname{[0.298, 0.323]}
\expandafter\def\csname res@zs.omni7b.f1other\endcsname{0.249}
\expandafter\def\csname res@zs.omni7b.f1otherci\endcsname{[0.238, 0.260]}
\expandafter\def\csname res@zs.omni7b.f1pm\endcsname{0.393}
\expandafter\def\csname res@zs.omni7b.f1pmctrl\endcsname{0.356}
\expandafter\def\csname res@zs.omni7b.f1pmen\endcsname{0.384}
\expandafter\def\csname res@zs.omni7b.f1pmlex\endcsname{0.551}
\expandafter\def\csname res@zs.omni7b.f1pmnonen\endcsname{0.398}
\expandafter\def\csname res@zs.omni7b.gap\endcsname{+0.120}
\expandafter\def\csname res@zs.omni7b.gapci\endcsname{[+0.104, +0.132]}
\expandafter\def\csname res@zs.omni7b.gapctrl\endcsname{+0.162}
\expandafter\def\csname res@zs.omni7b.gapctrlci\endcsname{[+0.143, +0.177]}
\expandafter\def\csname res@zs.omni7b.gapen\endcsname{+0.024}
\expandafter\def\csname res@zs.omni7b.gapenci\endcsname{[-0.003, +0.052]}
\expandafter\def\csname res@zs.omni7b.gaplex\endcsname{-0.056}
\expandafter\def\csname res@zs.omni7b.gaplexci\endcsname{[-0.076, -0.037]}
\expandafter\def\csname res@zs.omni7b.gapnonen\endcsname{+0.169}
\expandafter\def\csname res@zs.omni7b.gapnonenci\endcsname{[+0.151, +0.181]}
\expandafter\def\csname res@zs.omni7b.knownauc\endcsname{0.708}
\expandafter\def\csname res@zs.omni7b.novel\endcsname{0.073}
\expandafter\def\csname res@zs.omni7b.novelauc\endcsname{0.559}
\expandafter\def\csname res@zs.omni7b_cc.calm\endcsname{0.000}
\expandafter\def\csname res@zs.omni7b_cc.f1\endcsname{0.329}
\expandafter\def\csname res@zs.omni7b_cc.f1ci\endcsname{[0.317, 0.338]}
\expandafter\def\csname res@zs.omni7b_cc.f1ctrl\endcsname{0.282}
\expandafter\def\csname res@zs.omni7b_cc.f1ctrlci\endcsname{[0.269, 0.293]}
\expandafter\def\csname res@zs.omni7b_cc.f1emobox\endcsname{0.345}
\expandafter\def\csname res@zs.omni7b_cc.f1emoboxci\endcsname{[0.331, 0.356]}
\expandafter\def\csname res@zs.omni7b_cc.f1en\endcsname{0.348}
\expandafter\def\csname res@zs.omni7b_cc.f1enci\endcsname{[0.328, 0.361]}
\expandafter\def\csname res@zs.omni7b_cc.f1lex\endcsname{0.527}
\expandafter\def\csname res@zs.omni7b_cc.f1lexci\endcsname{[0.508, 0.542]}
\expandafter\def\csname res@zs.omni7b_cc.f1nonen\endcsname{0.320}
\expandafter\def\csname res@zs.omni7b_cc.f1nonenci\endcsname{[0.306, 0.332]}
\expandafter\def\csname res@zs.omni7b_cc.f1other\endcsname{0.259}
\expandafter\def\csname res@zs.omni7b_cc.f1otherci\endcsname{[0.247, 0.270]}
\expandafter\def\csname res@zs.omni7b_cc.f1pm\endcsname{0.398}
\expandafter\def\csname res@zs.omni7b_cc.f1pmctrl\endcsname{0.364}
\expandafter\def\csname res@zs.omni7b_cc.f1pmen\endcsname{0.387}
\expandafter\def\csname res@zs.omni7b_cc.f1pmlex\endcsname{0.540}
\expandafter\def\csname res@zs.omni7b_cc.f1pmnonen\endcsname{0.403}
\expandafter\def\csname res@zs.omni7b_cc.gap\endcsname{+0.104}
\expandafter\def\csname res@zs.omni7b_cc.gapci\endcsname{[+0.089, +0.115]}
\expandafter\def\csname res@zs.omni7b_cc.gapctrl\endcsname{+0.137}
\expandafter\def\csname res@zs.omni7b_cc.gapctrlci\endcsname{[+0.118, +0.149]}
\expandafter\def\csname res@zs.omni7b_cc.gapen\endcsname{-0.009}
\expandafter\def\csname res@zs.omni7b_cc.gapenci\endcsname{[-0.032, +0.016]}
\expandafter\def\csname res@zs.omni7b_cc.gaplex\endcsname{-0.033}
\expandafter\def\csname res@zs.omni7b_cc.gaplexci\endcsname{[-0.055, -0.010]}
\expandafter\def\csname res@zs.omni7b_cc.gapnonen\endcsname{+0.161}
\expandafter\def\csname res@zs.omni7b_cc.gapnonenci\endcsname{[+0.142, +0.173]}
\expandafter\def\csname res@zs.omni7b_cc.knownauc\endcsname{0.713}
\expandafter\def\csname res@zs.omni7b_cc.novel\endcsname{0.075}
\expandafter\def\csname res@zs.omni7b_cc.novelauc\endcsname{0.582}
\expandafter\def\csname res@zs.omni7b_text.calm\endcsname{0.000}
\expandafter\def\csname res@zs.omni7b_text.f1\endcsname{0.211}
\expandafter\def\csname res@zs.omni7b_text.f1ci\endcsname{[0.202, 0.218]}
\expandafter\def\csname res@zs.omni7b_text.f1ctrl\endcsname{0.146}
\expandafter\def\csname res@zs.omni7b_text.f1ctrlci\endcsname{[0.136, 0.153]}
\expandafter\def\csname res@zs.omni7b_text.f1emobox\endcsname{0.216}
\expandafter\def\csname res@zs.omni7b_text.f1emoboxci\endcsname{[0.206, 0.224]}
\expandafter\def\csname res@zs.omni7b_text.f1en\endcsname{0.190}
\expandafter\def\csname res@zs.omni7b_text.f1enci\endcsname{[0.182, 0.198]}
\expandafter\def\csname res@zs.omni7b_text.f1lex\endcsname{0.487}
\expandafter\def\csname res@zs.omni7b_text.f1lexci\endcsname{[0.468, 0.503]}
\expandafter\def\csname res@zs.omni7b_text.f1nonen\endcsname{0.222}
\expandafter\def\csname res@zs.omni7b_text.f1nonenci\endcsname{[0.209, 0.231]}
\expandafter\def\csname res@zs.omni7b_text.f1other\endcsname{0.189}
\expandafter\def\csname res@zs.omni7b_text.f1otherci\endcsname{[0.180, 0.198]}
\expandafter\def\csname res@zs.omni7b_text.f1pm\endcsname{0.257}
\expandafter\def\csname res@zs.omni7b_text.f1pmctrl\endcsname{0.200}
\expandafter\def\csname res@zs.omni7b_text.f1pmen\endcsname{0.231}
\expandafter\def\csname res@zs.omni7b_text.f1pmlex\endcsname{0.498}
\expandafter\def\csname res@zs.omni7b_text.f1pmnonen\endcsname{0.270}
\expandafter\def\csname res@zs.omni7b_text.gap\endcsname{+0.222}
\expandafter\def\csname res@zs.omni7b_text.gapci\endcsname{[+0.207, +0.232]}
\expandafter\def\csname res@zs.omni7b_text.gapctrl\endcsname{+0.273}
\expandafter\def\csname res@zs.omni7b_text.gapctrlci\endcsname{[+0.254, +0.285]}
\expandafter\def\csname res@zs.omni7b_text.gapen\endcsname{+0.148}
\expandafter\def\csname res@zs.omni7b_text.gapenci\endcsname{[+0.129, +0.163]}
\expandafter\def\csname res@zs.omni7b_text.gaplex\endcsname{+0.007}
\expandafter\def\csname res@zs.omni7b_text.gaplexci\endcsname{[-0.016, +0.028]}
\expandafter\def\csname res@zs.omni7b_text.gapnonen\endcsname{+0.259}
\expandafter\def\csname res@zs.omni7b_text.gapnonenci\endcsname{[+0.239, +0.273]}
\expandafter\def\csname res@zs.omni7b_text.knownauc\endcsname{0.595}
\expandafter\def\csname res@zs.omni7b_text.novel\endcsname{0.082}
\expandafter\def\csname res@zs.omni7b_text.novelauc\endcsname{0.513}
\expandafter\def\csname res@zs.phi4mm.calm\endcsname{0.254}
\expandafter\def\csname res@zs.phi4mm.f1\endcsname{0.219}
\expandafter\def\csname res@zs.phi4mm.f1ci\endcsname{[0.209, 0.225]}
\expandafter\def\csname res@zs.phi4mm.f1ctrl\endcsname{0.184}
\expandafter\def\csname res@zs.phi4mm.f1ctrlci\endcsname{[0.173, 0.191]}
\expandafter\def\csname res@zs.phi4mm.f1emobox\endcsname{0.218}
\expandafter\def\csname res@zs.phi4mm.f1emoboxci\endcsname{[0.206, 0.225]}
\expandafter\def\csname res@zs.phi4mm.f1en\endcsname{0.182}
\expandafter\def\csname res@zs.phi4mm.f1enci\endcsname{[0.172, 0.191]}
\expandafter\def\csname res@zs.phi4mm.f1lex\endcsname{0.365}
\expandafter\def\csname res@zs.phi4mm.f1lexci\endcsname{[0.345, 0.381]}
\expandafter\def\csname res@zs.phi4mm.f1nonen\endcsname{0.237}
\expandafter\def\csname res@zs.phi4mm.f1nonenci\endcsname{[0.223, 0.245]}
\expandafter\def\csname res@zs.phi4mm.f1other\endcsname{0.222}
\expandafter\def\csname res@zs.phi4mm.f1otherci\endcsname{[0.211, 0.233]}
\expandafter\def\csname res@zs.phi4mm.f1pm\endcsname{0.266}
\expandafter\def\csname res@zs.phi4mm.f1pmctrl\endcsname{0.230}
\expandafter\def\csname res@zs.phi4mm.f1pmen\endcsname{0.231}
\expandafter\def\csname res@zs.phi4mm.f1pmlex\endcsname{0.421}
\expandafter\def\csname res@zs.phi4mm.f1pmnonen\endcsname{0.284}
\expandafter\def\csname res@zs.phi4mm.gap\endcsname{+0.215}
\expandafter\def\csname res@zs.phi4mm.gapci\endcsname{[+0.199, +0.227]}
\expandafter\def\csname res@zs.phi4mm.gapctrl\endcsname{+0.235}
\expandafter\def\csname res@zs.phi4mm.gapctrlci\endcsname{[+0.216, +0.248]}
\expandafter\def\csname res@zs.phi4mm.gapen\endcsname{+0.157}
\expandafter\def\csname res@zs.phi4mm.gapenci\endcsname{[+0.137, +0.174]}
\expandafter\def\csname res@zs.phi4mm.gaplex\endcsname{+0.129}
\expandafter\def\csname res@zs.phi4mm.gaplexci\endcsname{[+0.108, +0.151]}
\expandafter\def\csname res@zs.phi4mm.gapnonen\endcsname{+0.244}
\expandafter\def\csname res@zs.phi4mm.gapnonenci\endcsname{[+0.223, +0.259]}
\expandafter\def\csname res@zs.phi4mm.knownauc\endcsname{0.606}
\expandafter\def\csname res@zs.phi4mm.novel\endcsname{0.125}
\expandafter\def\csname res@zs.phi4mm.novelauc\endcsname{0.546}
\expandafter\def\csname res@zs.phi4mm_cc.calm\endcsname{0.292}
\expandafter\def\csname res@zs.phi4mm_cc.f1\endcsname{0.208}
\expandafter\def\csname res@zs.phi4mm_cc.f1ci\endcsname{[0.200, 0.214]}
\expandafter\def\csname res@zs.phi4mm_cc.f1ctrl\endcsname{0.176}
\expandafter\def\csname res@zs.phi4mm_cc.f1ctrlci\endcsname{[0.166, 0.182]}
\expandafter\def\csname res@zs.phi4mm_cc.f1emobox\endcsname{0.209}
\expandafter\def\csname res@zs.phi4mm_cc.f1emoboxci\endcsname{[0.198, 0.216]}
\expandafter\def\csname res@zs.phi4mm_cc.f1en\endcsname{0.184}
\expandafter\def\csname res@zs.phi4mm_cc.f1enci\endcsname{[0.174, 0.192]}
\expandafter\def\csname res@zs.phi4mm_cc.f1lex\endcsname{0.347}
\expandafter\def\csname res@zs.phi4mm_cc.f1lexci\endcsname{[0.327, 0.364]}
\expandafter\def\csname res@zs.phi4mm_cc.f1nonen\endcsname{0.221}
\expandafter\def\csname res@zs.phi4mm_cc.f1nonenci\endcsname{[0.208, 0.229]}
\expandafter\def\csname res@zs.phi4mm_cc.f1other\endcsname{0.206}
\expandafter\def\csname res@zs.phi4mm_cc.f1otherci\endcsname{[0.196, 0.216]}
\expandafter\def\csname res@zs.phi4mm_cc.f1pm\endcsname{0.267}
\expandafter\def\csname res@zs.phi4mm_cc.f1pmctrl\endcsname{0.232}
\expandafter\def\csname res@zs.phi4mm_cc.f1pmen\endcsname{0.234}
\expandafter\def\csname res@zs.phi4mm_cc.f1pmlex\endcsname{0.418}
\expandafter\def\csname res@zs.phi4mm_cc.f1pmnonen\endcsname{0.284}
\expandafter\def\csname res@zs.phi4mm_cc.gap\endcsname{+0.225}
\expandafter\def\csname res@zs.phi4mm_cc.gapci\endcsname{[+0.208, +0.236]}
\expandafter\def\csname res@zs.phi4mm_cc.gapctrl\endcsname{+0.243}
\expandafter\def\csname res@zs.phi4mm_cc.gapctrlci\endcsname{[+0.224, +0.256]}
\expandafter\def\csname res@zs.phi4mm_cc.gapen\endcsname{+0.154}
\expandafter\def\csname res@zs.phi4mm_cc.gapenci\endcsname{[+0.134, +0.171]}
\expandafter\def\csname res@zs.phi4mm_cc.gaplex\endcsname{+0.147}
\expandafter\def\csname res@zs.phi4mm_cc.gaplexci\endcsname{[+0.125, +0.170]}
\expandafter\def\csname res@zs.phi4mm_cc.gapnonen\endcsname{+0.260}
\expandafter\def\csname res@zs.phi4mm_cc.gapnonenci\endcsname{[+0.239, +0.276]}
\expandafter\def\csname res@zs.phi4mm_cc.knownauc\endcsname{0.603}
\expandafter\def\csname res@zs.phi4mm_cc.novel\endcsname{0.161}
\expandafter\def\csname res@zs.phi4mm_cc.novelauc\endcsname{0.577}
\expandafter\def\csname res@zs.qwen2audio7b.calm\endcsname{0.581}
\expandafter\def\csname res@zs.qwen2audio7b.f1\endcsname{0.303}
\expandafter\def\csname res@zs.qwen2audio7b.f1ci\endcsname{[0.291, 0.309]}
\expandafter\def\csname res@zs.qwen2audio7b.f1ctrl\endcsname{0.281}
\expandafter\def\csname res@zs.qwen2audio7b.f1ctrlci\endcsname{[0.268, 0.289]}
\expandafter\def\csname res@zs.qwen2audio7b.f1emobox\endcsname{0.329}
\expandafter\def\csname res@zs.qwen2audio7b.f1emoboxci\endcsname{[0.316, 0.337]}
\expandafter\def\csname res@zs.qwen2audio7b.f1en\endcsname{0.382}
\expandafter\def\csname res@zs.qwen2audio7b.f1enci\endcsname{[0.367, 0.394]}
\expandafter\def\csname res@zs.qwen2audio7b.f1lex\endcsname{0.394}
\expandafter\def\csname res@zs.qwen2audio7b.f1lexci\endcsname{[0.375, 0.410]}
\expandafter\def\csname res@zs.qwen2audio7b.f1nonen\endcsname{0.263}
\expandafter\def\csname res@zs.qwen2audio7b.f1nonenci\endcsname{[0.247, 0.272]}
\expandafter\def\csname res@zs.qwen2audio7b.f1other\endcsname{0.189}
\expandafter\def\csname res@zs.qwen2audio7b.f1otherci\endcsname{[0.179, 0.199]}
\expandafter\def\csname res@zs.qwen2audio7b.f1pm\endcsname{0.399}
\expandafter\def\csname res@zs.qwen2audio7b.f1pmctrl\endcsname{0.385}
\expandafter\def\csname res@zs.qwen2audio7b.f1pmen\endcsname{0.468}
\expandafter\def\csname res@zs.qwen2audio7b.f1pmlex\endcsname{0.459}
\expandafter\def\csname res@zs.qwen2audio7b.f1pmnonen\endcsname{0.365}
\expandafter\def\csname res@zs.qwen2audio7b.gap\endcsname{+0.131}
\expandafter\def\csname res@zs.qwen2audio7b.gapci\endcsname{[+0.115, +0.143]}
\expandafter\def\csname res@zs.qwen2audio7b.gapctrl\endcsname{+0.138}
\expandafter\def\csname res@zs.qwen2audio7b.gapctrlci\endcsname{[+0.119, +0.152]}
\expandafter\def\csname res@zs.qwen2audio7b.gapen\endcsname{-0.044}
\expandafter\def\csname res@zs.qwen2audio7b.gapenci\endcsname{[-0.059, -0.027]}
\expandafter\def\csname res@zs.qwen2audio7b.gaplex\endcsname{+0.099}
\expandafter\def\csname res@zs.qwen2audio7b.gaplexci\endcsname{[+0.079, +0.121]}
\expandafter\def\csname res@zs.qwen2audio7b.gapnonen\endcsname{+0.218}
\expandafter\def\csname res@zs.qwen2audio7b.gapnonenci\endcsname{[+0.196, +0.235]}
\expandafter\def\csname res@zs.qwen2audio7b.knownauc\endcsname{0.715}
\expandafter\def\csname res@zs.qwen2audio7b.novel\endcsname{0.194}
\expandafter\def\csname res@zs.qwen2audio7b.novelauc\endcsname{0.630}
\expandafter\def\csname res@zs.qwen2audio7b_cc.calm\endcsname{0.603}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1\endcsname{0.322}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1ci\endcsname{[0.312, 0.329]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1ctrl\endcsname{0.302}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1ctrlci\endcsname{[0.291, 0.310]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1emobox\endcsname{0.337}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1emoboxci\endcsname{[0.326, 0.346]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1en\endcsname{0.413}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1enci\endcsname{[0.398, 0.428]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1lex\endcsname{0.407}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1lexci\endcsname{[0.385, 0.425]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1nonen\endcsname{0.276}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1nonenci\endcsname{[0.263, 0.285]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1other\endcsname{0.255}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1otherci\endcsname{[0.243, 0.267]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1pm\endcsname{0.404}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1pmctrl\endcsname{0.389}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1pmen\endcsname{0.474}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1pmlex\endcsname{0.470}
\expandafter\def\csname res@zs.qwen2audio7b_cc.f1pmnonen\endcsname{0.369}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gap\endcsname{+0.112}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapci\endcsname{[+0.097, +0.121]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapctrl\endcsname{+0.117}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapctrlci\endcsname{[+0.100, +0.129]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapen\endcsname{-0.075}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapenci\endcsname{[-0.091, -0.059]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gaplex\endcsname{+0.087}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gaplexci\endcsname{[+0.066, +0.107]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapnonen\endcsname{+0.205}
\expandafter\def\csname res@zs.qwen2audio7b_cc.gapnonenci\endcsname{[+0.185, +0.217]}
\expandafter\def\csname res@zs.qwen2audio7b_cc.knownauc\endcsname{0.723}
\expandafter\def\csname res@zs.qwen2audio7b_cc.novel\endcsname{0.228}
\expandafter\def\csname res@zs.qwen2audio7b_cc.novelauc\endcsname{0.642}
\expandafter\def\csname res@zs.r1_bkt_s43.calm\endcsname{0.160}
\expandafter\def\csname res@zs.r1_bkt_s43.f1\endcsname{0.430}
\expandafter\def\csname res@zs.r1_bkt_s43.f1pm\endcsname{0.553}
\expandafter\def\csname res@zs.r1_bkt_s43.knownauc\endcsname{0.843}
\expandafter\def\csname res@zs.r1_bkt_s43.novel\endcsname{0.032}
\expandafter\def\csname res@zs.r1_bkt_s43.novelauc\endcsname{0.728}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.calm\endcsname{0.466}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.f1\endcsname{0.468}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.f1pm\endcsname{0.555}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.novel\endcsname{0.108}
\expandafter\def\csname res@zs.r1_bkt_s43_noprior.novelauc\endcsname{0.742}
\expandafter\def\csname res@zs.r1_bkt_s44.calm\endcsname{0.069}
\expandafter\def\csname res@zs.r1_bkt_s44.f1\endcsname{0.437}
\expandafter\def\csname res@zs.r1_bkt_s44.f1pm\endcsname{0.554}
\expandafter\def\csname res@zs.r1_bkt_s44.knownauc\endcsname{0.843}
\expandafter\def\csname res@zs.r1_bkt_s44.novel\endcsname{0.014}
\expandafter\def\csname res@zs.r1_bkt_s44.novelauc\endcsname{0.720}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.calm\endcsname{0.392}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.f1\endcsname{0.479}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.f1pm\endcsname{0.555}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.novel\endcsname{0.110}
\expandafter\def\csname res@zs.r1_bkt_s44_noprior.novelauc\endcsname{0.736}
\expandafter\def\csname res@zs.r1_bkt_s45.calm\endcsname{0.048}
\expandafter\def\csname res@zs.r1_bkt_s45.f1\endcsname{0.432}
\expandafter\def\csname res@zs.r1_bkt_s45.f1pm\endcsname{0.550}
\expandafter\def\csname res@zs.r1_bkt_s45.knownauc\endcsname{0.841}
\expandafter\def\csname res@zs.r1_bkt_s45.novel\endcsname{0.010}
\expandafter\def\csname res@zs.r1_bkt_s45.novelauc\endcsname{0.710}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.calm\endcsname{0.327}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.f1\endcsname{0.469}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.f1pm\endcsname{0.552}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.knownauc\endcsname{0.844}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.novel\endcsname{0.093}
\expandafter\def\csname res@zs.r1_bkt_s45_noprior.novelauc\endcsname{0.723}
\expandafter\def\csname res@zs.r1_clapobj_s43.calm\endcsname{0.527}
\expandafter\def\csname res@zs.r1_clapobj_s43.f1\endcsname{0.507}
\expandafter\def\csname res@zs.r1_clapobj_s43.f1pm\endcsname{0.566}
\expandafter\def\csname res@zs.r1_clapobj_s43.knownauc\endcsname{0.853}
\expandafter\def\csname res@zs.r1_clapobj_s43.novel\endcsname{0.226}
\expandafter\def\csname res@zs.r1_clapobj_s43.novelauc\endcsname{0.739}
\expandafter\def\csname res@zs.r1_drop16_s43.calm\endcsname{0.162}
\expandafter\def\csname res@zs.r1_drop16_s43.f1\endcsname{0.449}
\expandafter\def\csname res@zs.r1_drop16_s43.f1pm\endcsname{0.562}
\expandafter\def\csname res@zs.r1_drop16_s43.knownauc\endcsname{0.850}
\expandafter\def\csname res@zs.r1_drop16_s43.novel\endcsname{0.032}
\expandafter\def\csname res@zs.r1_drop16_s43.novelauc\endcsname{0.712}
\expandafter\def\csname res@zs.r1_drop24_s43.calm\endcsname{0.221}
\expandafter\def\csname res@zs.r1_drop24_s43.f1\endcsname{0.444}
\expandafter\def\csname res@zs.r1_drop24_s43.f1pm\endcsname{0.554}
\expandafter\def\csname res@zs.r1_drop24_s43.knownauc\endcsname{0.846}
\expandafter\def\csname res@zs.r1_drop24_s43.novel\endcsname{0.044}
\expandafter\def\csname res@zs.r1_drop24_s43.novelauc\endcsname{0.715}
\expandafter\def\csname res@zs.r1_drop8_s43.calm\endcsname{0.261}
\expandafter\def\csname res@zs.r1_drop8_s43.f1\endcsname{0.445}
\expandafter\def\csname res@zs.r1_drop8_s43.f1pm\endcsname{0.564}
\expandafter\def\csname res@zs.r1_drop8_s43.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.r1_drop8_s43.novel\endcsname{0.052}
\expandafter\def\csname res@zs.r1_drop8_s43.novelauc\endcsname{0.714}
\expandafter\def\csname res@zs.r1_dyn_s43.calm\endcsname{0.106}
\expandafter\def\csname res@zs.r1_dyn_s43.f1\endcsname{0.394}
\expandafter\def\csname res@zs.r1_dyn_s43.f1pm\endcsname{0.519}
\expandafter\def\csname res@zs.r1_dyn_s43.knownauc\endcsname{0.820}
\expandafter\def\csname res@zs.r1_dyn_s43.novel\endcsname{0.021}
\expandafter\def\csname res@zs.r1_dyn_s43.novelauc\endcsname{0.712}
\expandafter\def\csname res@zs.r1_nodistill_s43.calm\endcsname{0.210}
\expandafter\def\csname res@zs.r1_nodistill_s43.f1\endcsname{0.459}
\expandafter\def\csname res@zs.r1_nodistill_s43.f1pm\endcsname{0.560}
\expandafter\def\csname res@zs.r1_nodistill_s43.knownauc\endcsname{0.847}
\expandafter\def\csname res@zs.r1_nodistill_s43.novel\endcsname{0.045}
\expandafter\def\csname res@zs.r1_nodistill_s43.novelauc\endcsname{0.720}
\expandafter\def\csname res@zs.r1_nodiv_s43.calm\endcsname{0.612}
\expandafter\def\csname res@zs.r1_nodiv_s43.f1\endcsname{0.451}
\expandafter\def\csname res@zs.r1_nodiv_s43.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.r1_nodiv_s43.knownauc\endcsname{0.850}
\expandafter\def\csname res@zs.r1_nodiv_s43.novel\endcsname{0.122}
\expandafter\def\csname res@zs.r1_nodiv_s43.novelauc\endcsname{0.742}
\expandafter\def\csname res@zs.r1_q1_s43.calm\endcsname{0.105}
\expandafter\def\csname res@zs.r1_q1_s43.f1\endcsname{0.444}
\expandafter\def\csname res@zs.r1_q1_s43.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.r1_q1_s43.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.r1_q1_s43.novel\endcsname{0.021}
\expandafter\def\csname res@zs.r1_q1_s43.novelauc\endcsname{0.722}
\expandafter\def\csname res@zs.r1_s43.calm\endcsname{0.167}
\expandafter\def\csname res@zs.r1_s43.f1\endcsname{0.440}
\expandafter\def\csname res@zs.r1_s43.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.r1_s43.knownauc\endcsname{0.847}
\expandafter\def\csname res@zs.r1_s43.novel\endcsname{0.033}
\expandafter\def\csname res@zs.r1_s43.novelauc\endcsname{0.721}
\expandafter\def\csname res@zs.r1_s43_noprior.calm\endcsname{0.545}
\expandafter\def\csname res@zs.r1_s43_noprior.f1\endcsname{0.475}
\expandafter\def\csname res@zs.r1_s43_noprior.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.r1_s43_noprior.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.r1_s43_noprior.novel\endcsname{0.115}
\expandafter\def\csname res@zs.r1_s43_noprior.novelauc\endcsname{0.737}
\expandafter\def\csname res@zs.r1_s44.calm\endcsname{0.083}
\expandafter\def\csname res@zs.r1_s44.f1\endcsname{0.441}
\expandafter\def\csname res@zs.r1_s44.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.r1_s44.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.r1_s44.novel\endcsname{0.017}
\expandafter\def\csname res@zs.r1_s44.novelauc\endcsname{0.718}
\expandafter\def\csname res@zs.r1_s44_noprior.calm\endcsname{0.391}
\expandafter\def\csname res@zs.r1_s44_noprior.f1\endcsname{0.475}
\expandafter\def\csname res@zs.r1_s44_noprior.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.r1_s44_noprior.knownauc\endcsname{0.851}
\expandafter\def\csname res@zs.r1_s44_noprior.novel\endcsname{0.098}
\expandafter\def\csname res@zs.r1_s44_noprior.novelauc\endcsname{0.738}
\expandafter\def\csname res@zs.r1_s45.calm\endcsname{0.081}
\expandafter\def\csname res@zs.r1_s45.f1\endcsname{0.444}
\expandafter\def\csname res@zs.r1_s45.f1pm\endcsname{0.563}
\expandafter\def\csname res@zs.r1_s45.knownauc\endcsname{0.850}
\expandafter\def\csname res@zs.r1_s45.novel\endcsname{0.016}
\expandafter\def\csname res@zs.r1_s45.novelauc\endcsname{0.707}
\expandafter\def\csname res@zs.r1_s45_noprior.calm\endcsname{0.473}
\expandafter\def\csname res@zs.r1_s45_noprior.f1\endcsname{0.480}
\expandafter\def\csname res@zs.r1_s45_noprior.f1pm\endcsname{0.565}
\expandafter\def\csname res@zs.r1_s45_noprior.knownauc\endcsname{0.852}
\expandafter\def\csname res@zs.r1_s45_noprior.novel\endcsname{0.107}
\expandafter\def\csname res@zs.r1_s45_noprior.novelauc\endcsname{0.723}
\expandafter\def\csname res@zs.r1_seg0_s43.calm\endcsname{0.260}
\expandafter\def\csname res@zs.r1_seg0_s43.f1\endcsname{0.442}
\expandafter\def\csname res@zs.r1_seg0_s43.f1pm\endcsname{0.564}
\expandafter\def\csname res@zs.r1_seg0_s43.knownauc\endcsname{0.852}
\expandafter\def\csname res@zs.r1_seg0_s43.novel\endcsname{0.052}
\expandafter\def\csname res@zs.r1_seg0_s43.novelauc\endcsname{0.725}
\expandafter\def\csname res@zs.r1_seg128_s43.calm\endcsname{0.116}
\expandafter\def\csname res@zs.r1_seg128_s43.f1\endcsname{0.441}
\expandafter\def\csname res@zs.r1_seg128_s43.f1pm\endcsname{0.559}
\expandafter\def\csname res@zs.r1_seg128_s43.knownauc\endcsname{0.848}
\expandafter\def\csname res@zs.r1_seg128_s43.novel\endcsname{0.023}
\expandafter\def\csname res@zs.r1_seg128_s43.novelauc\endcsname{0.730}
\expandafter\def\csname res@zs.r1_seg16_s43.calm\endcsname{0.162}
\expandafter\def\csname res@zs.r1_seg16_s43.f1\endcsname{0.433}
\expandafter\def\csname res@zs.r1_seg16_s43.f1pm\endcsname{0.550}
\expandafter\def\csname res@zs.r1_seg16_s43.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_seg16_s43.novel\endcsname{0.032}
\expandafter\def\csname res@zs.r1_seg16_s43.novelauc\endcsname{0.726}
\expandafter\def\csname res@zs.r1_seg32_s43.calm\endcsname{0.271}
\expandafter\def\csname res@zs.r1_seg32_s43.f1\endcsname{0.441}
\expandafter\def\csname res@zs.r1_seg32_s43.f1pm\endcsname{0.558}
\expandafter\def\csname res@zs.r1_seg32_s43.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_seg32_s43.novel\endcsname{0.054}
\expandafter\def\csname res@zs.r1_seg32_s43.novelauc\endcsname{0.715}
\expandafter\def\csname res@zs.r1_seg8_s43.calm\endcsname{0.173}
\expandafter\def\csname res@zs.r1_seg8_s43.f1\endcsname{0.421}
\expandafter\def\csname res@zs.r1_seg8_s43.f1pm\endcsname{0.546}
\expandafter\def\csname res@zs.r1_seg8_s43.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.r1_seg8_s43.novel\endcsname{0.035}
\expandafter\def\csname res@zs.r1_seg8_s43.novelauc\endcsname{0.722}
\expandafter\def\csname res@zs.r1_v1only_s43.calm\endcsname{0.037}
\expandafter\def\csname res@zs.r1_v1only_s43.f1\endcsname{0.362}
\expandafter\def\csname res@zs.r1_v1only_s43.f1pm\endcsname{0.516}
\expandafter\def\csname res@zs.r1_v1only_s43.knownauc\endcsname{0.819}
\expandafter\def\csname res@zs.r1_v1only_s43.novel\endcsname{0.007}
\expandafter\def\csname res@zs.r1_v1only_s43.novelauc\endcsname{0.707}
\expandafter\def\csname res@zs.r1_v2acted_s43.calm\endcsname{0.532}
\expandafter\def\csname res@zs.r1_v2acted_s43.f1\endcsname{0.469}
\expandafter\def\csname res@zs.r1_v2acted_s43.f1pm\endcsname{0.560}
\expandafter\def\csname res@zs.r1_v2acted_s43.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_v2acted_s43.novel\endcsname{0.106}
\expandafter\def\csname res@zs.r1_v2acted_s43.novelauc\endcsname{0.734}
\expandafter\def\csname res@zs.r1_v2all_s43.calm\endcsname{0.085}
\expandafter\def\csname res@zs.r1_v2all_s43.f1\endcsname{0.422}
\expandafter\def\csname res@zs.r1_v2all_s43.f1pm\endcsname{0.532}
\expandafter\def\csname res@zs.r1_v2all_s43.knownauc\endcsname{0.817}
\expandafter\def\csname res@zs.r1_v2all_s43.novel\endcsname{0.017}
\expandafter\def\csname res@zs.r1_v2all_s43.novelauc\endcsname{0.713}
\expandafter\def\csname res@zs.r1_w2432_s43.calm\endcsname{0.180}
\expandafter\def\csname res@zs.r1_w2432_s43.f1\endcsname{0.436}
\expandafter\def\csname res@zs.r1_w2432_s43.f1pm\endcsname{0.562}
\expandafter\def\csname res@zs.r1_w2432_s43.knownauc\endcsname{0.849}
\expandafter\def\csname res@zs.r1_w2432_s43.novel\endcsname{0.036}
\expandafter\def\csname res@zs.r1_w2432_s43.novelauc\endcsname{0.713}
\expandafter\def\csname res@zs.r1_w24_s43.calm\endcsname{0.227}
\expandafter\def\csname res@zs.r1_w24_s43.f1\endcsname{0.429}
\expandafter\def\csname res@zs.r1_w24_s43.f1pm\endcsname{0.566}
\expandafter\def\csname res@zs.r1_w24_s43.knownauc\endcsname{0.844}
\expandafter\def\csname res@zs.r1_w24_s43.novel\endcsname{0.045}
\expandafter\def\csname res@zs.r1_w24_s43.novelauc\endcsname{0.749}
\expandafter\def\csname res@zs.r1_w32_s43.calm\endcsname{0.127}
\expandafter\def\csname res@zs.r1_w32_s43.f1\endcsname{0.428}
\expandafter\def\csname res@zs.r1_w32_s43.f1pm\endcsname{0.552}
\expandafter\def\csname res@zs.r1_w32_s43.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.r1_w32_s43.novel\endcsname{0.025}
\expandafter\def\csname res@zs.r1_w32_s43.novelauc\endcsname{0.703}
\expandafter\def\csname res@zs.tbkt_s43.calm\endcsname{0.000}
\expandafter\def\csname res@zs.tbkt_s43.f1\endcsname{0.410}
\expandafter\def\csname res@zs.tbkt_s43.f1pm\endcsname{0.536}
\expandafter\def\csname res@zs.tbkt_s43.knownauc\endcsname{0.842}
\expandafter\def\csname res@zs.tbkt_s43.novel\endcsname{0.000}
\expandafter\def\csname res@zs.tbkt_s44.calm\endcsname{0.000}
\expandafter\def\csname res@zs.tbkt_s44.f1\endcsname{0.419}
\expandafter\def\csname res@zs.tbkt_s44.f1pm\endcsname{0.537}
\expandafter\def\csname res@zs.tbkt_s44.knownauc\endcsname{0.841}
\expandafter\def\csname res@zs.tbkt_s44.novel\endcsname{0.000}
\expandafter\def\csname res@zs.tbkt_s45.calm\endcsname{0.000}
\expandafter\def\csname res@zs.tbkt_s45.f1\endcsname{0.421}
\expandafter\def\csname res@zs.tbkt_s45.f1pm\endcsname{0.545}
\expandafter\def\csname res@zs.tbkt_s45.knownauc\endcsname{0.845}
\expandafter\def\csname res@zs.tbkt_s45.novel\endcsname{0.000}
\expandafter\def\csname res@zs.voxtral3b.calm\endcsname{0.144}
\expandafter\def\csname res@zs.voxtral3b.f1\endcsname{0.209}
\expandafter\def\csname res@zs.voxtral3b.f1ci\endcsname{[0.200, 0.214]}
\expandafter\def\csname res@zs.voxtral3b.f1ctrl\endcsname{0.152}
\expandafter\def\csname res@zs.voxtral3b.f1ctrlci\endcsname{[0.143, 0.158]}
\expandafter\def\csname res@zs.voxtral3b.f1emobox\endcsname{0.210}
\expandafter\def\csname res@zs.voxtral3b.f1emoboxci\endcsname{[0.199, 0.216]}
\expandafter\def\csname res@zs.voxtral3b.f1en\endcsname{0.202}
\expandafter\def\csname res@zs.voxtral3b.f1enci\endcsname{[0.192, 0.211]}
\expandafter\def\csname res@zs.voxtral3b.f1lex\endcsname{0.448}
\expandafter\def\csname res@zs.voxtral3b.f1lexci\endcsname{[0.426, 0.467]}
\expandafter\def\csname res@zs.voxtral3b.f1nonen\endcsname{0.212}
\expandafter\def\csname res@zs.voxtral3b.f1nonenci\endcsname{[0.200, 0.219]}
\expandafter\def\csname res@zs.voxtral3b.f1other\endcsname{0.205}
\expandafter\def\csname res@zs.voxtral3b.f1otherci\endcsname{[0.195, 0.215]}
\expandafter\def\csname res@zs.voxtral3b.f1pm\endcsname{0.265}
\expandafter\def\csname res@zs.voxtral3b.f1pmctrl\endcsname{0.218}
\expandafter\def\csname res@zs.voxtral3b.f1pmen\endcsname{0.249}
\expandafter\def\csname res@zs.voxtral3b.f1pmlex\endcsname{0.467}
\expandafter\def\csname res@zs.voxtral3b.f1pmnonen\endcsname{0.273}
\expandafter\def\csname res@zs.voxtral3b.gap\endcsname{+0.225}
\expandafter\def\csname res@zs.voxtral3b.gapci\endcsname{[+0.208, +0.236]}
\expandafter\def\csname res@zs.voxtral3b.gapctrl\endcsname{+0.267}
\expandafter\def\csname res@zs.voxtral3b.gapctrlci\endcsname{[+0.247, +0.280]}
\expandafter\def\csname res@zs.voxtral3b.gapen\endcsname{+0.136}
\expandafter\def\csname res@zs.voxtral3b.gapenci\endcsname{[+0.116, +0.154]}
\expandafter\def\csname res@zs.voxtral3b.gaplex\endcsname{+0.046}
\expandafter\def\csname res@zs.voxtral3b.gaplexci\endcsname{[+0.023, +0.068]}
\expandafter\def\csname res@zs.voxtral3b.gapnonen\endcsname{+0.269}
\expandafter\def\csname res@zs.voxtral3b.gapnonenci\endcsname{[+0.248, +0.284]}
\expandafter\def\csname res@zs.voxtral3b.knownauc\endcsname{0.595}
\expandafter\def\csname res@zs.voxtral3b.novel\endcsname{0.111}
\expandafter\def\csname res@zs.voxtral3b.novelauc\endcsname{0.518}
\expandafter\def\csname res@zs.voxtral3b_cc.calm\endcsname{0.244}
\expandafter\def\csname res@zs.voxtral3b_cc.f1\endcsname{0.226}
\expandafter\def\csname res@zs.voxtral3b_cc.f1ci\endcsname{[0.217, 0.232]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1ctrl\endcsname{0.173}
\expandafter\def\csname res@zs.voxtral3b_cc.f1ctrlci\endcsname{[0.163, 0.180]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1emobox\endcsname{0.227}
\expandafter\def\csname res@zs.voxtral3b_cc.f1emoboxci\endcsname{[0.216, 0.234]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1en\endcsname{0.212}
\expandafter\def\csname res@zs.voxtral3b_cc.f1enci\endcsname{[0.202, 0.221]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1lex\endcsname{0.450}
\expandafter\def\csname res@zs.voxtral3b_cc.f1lexci\endcsname{[0.429, 0.467]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1nonen\endcsname{0.233}
\expandafter\def\csname res@zs.voxtral3b_cc.f1nonenci\endcsname{[0.220, 0.241]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1other\endcsname{0.220}
\expandafter\def\csname res@zs.voxtral3b_cc.f1otherci\endcsname{[0.210, 0.230]}
\expandafter\def\csname res@zs.voxtral3b_cc.f1pm\endcsname{0.269}
\expandafter\def\csname res@zs.voxtral3b_cc.f1pmctrl\endcsname{0.225}
\expandafter\def\csname res@zs.voxtral3b_cc.f1pmen\endcsname{0.248}
\expandafter\def\csname res@zs.voxtral3b_cc.f1pmlex\endcsname{0.458}
\expandafter\def\csname res@zs.voxtral3b_cc.f1pmnonen\endcsname{0.280}
\expandafter\def\csname res@zs.voxtral3b_cc.gap\endcsname{+0.207}
\expandafter\def\csname res@zs.voxtral3b_cc.gapci\endcsname{[+0.191, +0.219]}
\expandafter\def\csname res@zs.voxtral3b_cc.gapctrl\endcsname{+0.246}
\expandafter\def\csname res@zs.voxtral3b_cc.gapctrlci\endcsname{[+0.228, +0.259]}
\expandafter\def\csname res@zs.voxtral3b_cc.gapen\endcsname{+0.126}
\expandafter\def\csname res@zs.voxtral3b_cc.gapenci\endcsname{[+0.106, +0.143]}
\expandafter\def\csname res@zs.voxtral3b_cc.gaplex\endcsname{+0.044}
\expandafter\def\csname res@zs.voxtral3b_cc.gaplexci\endcsname{[+0.023, +0.065]}
\expandafter\def\csname res@zs.voxtral3b_cc.gapnonen\endcsname{+0.248}
\expandafter\def\csname res@zs.voxtral3b_cc.gapnonenci\endcsname{[+0.227, +0.264]}
\expandafter\def\csname res@zs.voxtral3b_cc.knownauc\endcsname{0.595}
\expandafter\def\csname res@zs.voxtral3b_cc.novel\endcsname{0.143}
\expandafter\def\csname res@zs.voxtral3b_cc.novelauc\endcsname{0.531}
\expandafter\def\csname res@zs.whisper_mlp.calm\endcsname{0.000}
\expandafter\def\csname res@zs.whisper_mlp.f1\endcsname{0.417}
\expandafter\def\csname res@zs.whisper_mlp.f1ci\endcsname{[0.399, 0.426]}
\expandafter\def\csname res@zs.whisper_mlp.f1ctrl\endcsname{0.402}
\expandafter\def\csname res@zs.whisper_mlp.f1ctrlci\endcsname{[0.381, 0.413]}
\expandafter\def\csname res@zs.whisper_mlp.f1emobox\endcsname{0.408}
\expandafter\def\csname res@zs.whisper_mlp.f1emoboxci\endcsname{[0.387, 0.419]}
\expandafter\def\csname res@zs.whisper_mlp.f1en\endcsname{0.314}
\expandafter\def\csname res@zs.whisper_mlp.f1enci\endcsname{[0.297, 0.327]}
\expandafter\def\csname res@zs.whisper_mlp.f1lex\endcsname{0.479}
\expandafter\def\csname res@zs.whisper_mlp.f1lexci\endcsname{[0.459, 0.497]}
\expandafter\def\csname res@zs.whisper_mlp.f1nonen\endcsname{0.468}
\expandafter\def\csname res@zs.whisper_mlp.f1nonenci\endcsname{[0.444, 0.481]}
\expandafter\def\csname res@zs.whisper_mlp.f1other\endcsname{0.455}
\expandafter\def\csname res@zs.whisper_mlp.f1otherci\endcsname{[0.432, 0.474]}
\expandafter\def\csname res@zs.whisper_mlp.f1pm\endcsname{0.539}
\expandafter\def\csname res@zs.whisper_mlp.f1pmctrl\endcsname{0.540}
\expandafter\def\csname res@zs.whisper_mlp.f1pmen\endcsname{0.429}
\expandafter\def\csname res@zs.whisper_mlp.f1pmlex\endcsname{0.538}
\expandafter\def\csname res@zs.whisper_mlp.f1pmnonen\endcsname{0.595}
\expandafter\def\csname res@zs.whisper_mlp.gap\endcsname{+0.017}
\expandafter\def\csname res@zs.whisper_mlp.gapci\endcsname{[+0.013, +0.021]}
\expandafter\def\csname res@zs.whisper_mlp.gapctrl\endcsname{+0.017}
\expandafter\def\csname res@zs.whisper_mlp.gapctrlci\endcsname{[+0.013, +0.022]}
\expandafter\def\csname res@zs.whisper_mlp.gapen\endcsname{+0.024}
\expandafter\def\csname res@zs.whisper_mlp.gapenci\endcsname{[+0.018, +0.029]}
\expandafter\def\csname res@zs.whisper_mlp.gaplex\endcsname{+0.014}
\expandafter\def\csname res@zs.whisper_mlp.gaplexci\endcsname{[+0.004, +0.025]}
\expandafter\def\csname res@zs.whisper_mlp.gapnonen\endcsname{+0.013}
\expandafter\def\csname res@zs.whisper_mlp.gapnonenci\endcsname{[+0.008, +0.019]}
\expandafter\def\csname res@zs.whisper_mlp.knownauc\endcsname{0.847}
\expandafter\def\csname res@zs.whisper_mlp.novel\endcsname{0.000}
\expandafter\def\csname res@zs.whisper_mlp_msp.calm\endcsname{0.000}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1\endcsname{0.330}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1ci\endcsname{[0.315, 0.338]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1ctrl\endcsname{0.310}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1ctrlci\endcsname{[0.292, 0.319]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1emobox\endcsname{0.333}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1emoboxci\endcsname{[0.315, 0.343]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1en\endcsname{0.265}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1enci\endcsname{[0.245, 0.280]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1lex\endcsname{0.415}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1lexci\endcsname{[0.396, 0.432]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1nonen\endcsname{0.362}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1nonenci\endcsname{[0.343, 0.373]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1other\endcsname{0.316}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1otherci\endcsname{[0.298, 0.333]}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1pm\endcsname{0.458}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1pmctrl\endcsname{0.449}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1pmen\endcsname{0.412}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1pmlex\endcsname{0.493}
\expandafter\def\csname res@zs.whisper_mlp_msp.f1pmnonen\endcsname{0.480}
\expandafter\def\csname res@zs.whisper_mlp_msp.gap\endcsname{+0.103}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapci\endcsname{[+0.092, +0.114]}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapctrl\endcsname{+0.109}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapctrlci\endcsname{[+0.095, +0.122]}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapen\endcsname{+0.073}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapenci\endcsname{[+0.059, +0.090]}
\expandafter\def\csname res@zs.whisper_mlp_msp.gaplex\endcsname{+0.078}
\expandafter\def\csname res@zs.whisper_mlp_msp.gaplexci\endcsname{[+0.062, +0.094]}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapnonen\endcsname{+0.118}
\expandafter\def\csname res@zs.whisper_mlp_msp.gapnonenci\endcsname{[+0.102, +0.132]}
\expandafter\def\csname res@zs.whisper_mlp_msp.knownauc\endcsname{0.783}
\expandafter\def\csname res@zs.whisper_mlp_msp.novel\endcsname{0.000}
\makeatother

